Optimal Single-History Tokenization Disambiguation for Provably Secure Linguistic Steganography

Provably secure linguistic steganography assumes the receiver recovers the sender's tokens, but the channel carries only text, which can have several tokenizations. Existing fixes bias sampling, lose most capacity at large vocabularies, run the model on several tokenizations per step, or repair bit errors over a second text. We prove that for any universal scheme whose sender queries the language model only along the emitted token history, exactness and zero error across models force each key's candidate strings to be prefix-free at every step, however far ahead the receiver reads. Each step therefore loses at least the stop entropy, the graph entropy of deciding whether a token ends at a string that other candidates extend. Our scheme, coin projection, makes these stop decisions with shared randomness at one model call per token; it is exact and attains the bound. On English, Chinese and Japanese, at most 8 in 1,000 sampled tokens are tokenized non-canonically, yet the stop entropy takes 7.0-9.0% of the string entropy. Coin projection turns 2.18-6.83 times as much entropy into message bits as SyncPool at the full vocabulary, and carries 1.29-2.18 times its bits per token at each method's best vocabulary size. It decoded all 1,800 texts of the main comparison and, at the full vocabulary, came within 6.0-7.0 utilization points of a multi-history scheme making 4.13-4.74 calls per token.

==> gen/numbers.tex <==
% generated by plots/make_figs.py -- do not edit
\makeatletter
\expandafter\def\csname res@llama@e0@16@root\endcsname{80.5}
\expandafter\def\csname res@llama@e0@16@branch\endcsname{11.6}
\expandafter\def\csname res@llama@e0@16@stop\endcsname{8.0}
\expandafter\def\csname res@llama@e0@16@coin\endcsname{92.0}
\expandafter\def\csname res@llama@e0@16@noncanon\endcsname{0.0}
\expandafter\def\csname res@llama@e0@16@Hstr\endcsname{2.09}
\expandafter\def\csname res@llama@e0@16@hubdrop\endcsname{87.6}
\expandafter\def\csname res@llama@e0@16@largest\endcsname{63}
\expandafter\def\csname res@llama@e0@16@spacebranch\endcsname{86}
\expandafter\def\csname res@llama@e0@64@root\endcsname{54.8}
\expandafter\def\csname res@llama@e0@64@branch\endcsname{37.2}
\expandafter\def\csname res@llama@e0@64@stop\endcsname{8.0}
\expandafter\def\csname res@llama@e0@64@coin\endcsname{92.0}
\expandafter\def\csname res@llama@e0@64@noncanon\endcsname{1.9}
\expandafter\def\csname res@llama@e0@64@Hstr\endcsname{2.74}
\expandafter\def\csname res@llama@e0@64@hubdrop\endcsname{86.6}
\expandafter\def\csname res@llama@e0@64@largest\endcsname{71}
\expandafter\def\csname res@llama@e0@64@spacebranch\endcsname{87}
\expandafter\def\csname res@llama@e0@256@root\endcsname{29.0}
\expandafter\def\csname res@llama@e0@256@branch\endcsname{62.7}
\expandafter\def\csname res@llama@e0@256@stop\endcsname{8.3}
\expandafter\def\csname res@llama@e0@256@coin\endcsname{91.7}
\expandafter\def\csname res@llama@e0@256@noncanon\endcsname{0.0}
\expandafter\def\csname res@llama@e0@256@Hstr\endcsname{3.20}
\expandafter\def\csname res@llama@e0@256@hubdrop\endcsname{84.9}
\expandafter\def\csname res@llama@e0@256@largest\endcsname{82}
\expandafter\def\csname res@llama@e0@256@spacebranch\endcsname{85}
\expandafter\def\csname res@llama@e0@1k@root\endcsname{14.2}
\expandafter\def\csname res@llama@e0@1k@branch\endcsname{77.2}
\expandafter\def\csname res@llama@e0@1k@stop\endcsname{8.6}
\expandafter\def\csname res@llama@e0@1k@coin\endcsname{91.4}
\expandafter\def\csname res@llama@e0@1k@noncanon\endcsname{0.0}
\expandafter\def\csname res@llama@e0@1k@Hstr\endcsname{3.46}
\expandafter\def\csname res@llama@e0@1k@hubdrop\endcsname{84.3}
\expandafter\def\csname res@llama@e0@1k@largest\endcsname{89}
\expandafter\def\csname res@llama@e0@1k@spacebranch\endcsname{73}
\expandafter\def\csname res@llama@e0@4k@root\endcsname{14.7}
\expandafter\def\csname res@llama@e0@4k@branch\endcsname{76.6}
\expandafter\def\csname res@llama@e0@4k@stop\endcsname{8.7}
\expandafter\def\csname res@llama@e0@4k@coin\endcsname{91.3}
\expandafter\def\csname res@llama@e0@4k@noncanon\endcsname{0.0}
\expandafter\def\csname res@llama@e0@4k@Hstr\endcsname{3.78}
\expandafter\def\csname res@llama@e0@4k@hubdrop\endcsname{83.3}
\expandafter\def\csname res@llama@e0@4k@largest\endcsname{88}
\expandafter\def\csname res@llama@e0@4k@spacebranch\endcsname{65}
\expandafter\def\csname res@llama@e0@Full@root\endcsname{14.2}
\expandafter\def\csname res@llama@e0@Full@branch\endcsname{77.0}
\expandafter\def\csname res@llama@e0@Full@stop\endcsname{8.7}
\expandafter\def\csname res@llama@e0@Full@coin\endcsname{91.3}
\expandafter\def\csname res@llama@e0@Full@noncanon\endcsname{0.9}
\expandafter\def\csname res@llama@e0@Full@Hstr\endcsname{3.77}
\expandafter\def\csname res@llama@e0@Full@hubdrop\endcsname{82.4}
\expandafter\def\csname res@llama@e0@Full@largest\endcsname{88}
\expandafter\def\csname res@llama@e0@Full@spacebranch\endcsname{64}
\expandafter\def\csname res@llama@e0@Full@leadbranch\endcsname{0}
\expandafter\def\csname res@llama@e0@Full@hubbranch\endcsname{64}
\expandafter\def\csname res@llama@e0@Full@topstopone\endcsname{9}
\expandafter\def\csname res@llama@e0@Full@topbranchone\endcsname{64}
\expandafter\def\csname res@llama@e0@Full@polar\endcsname{93}
\expandafter\def\csname res@llama@e0@Full@spacemass\endcsname{0.75}
\expandafter\def\csname res@qwen@e0@16@root\endcsname{87.0}
\expandafter\def\csname res@qwen@e0@16@branch\endcsname{3.9}
\expandafter\def\csname res@qwen@e0@16@stop\endcsname{9.0}
\expandafter\def\csname res@qwen@e0@16@coin\endcsname{91.0}
\expandafter\def\csname res@qwen@e0@16@noncanon\endcsname{0.9}
\expandafter\def\csname res@qwen@e0@16@Hstr\endcsname{1.74}
\expandafter\def\csname res@qwen@e0@16@hubdrop\endcsname{87.8}
\expandafter\def\csname res@qwen@e0@16@largest\endcsname{67}
\expandafter\def\csname res@qwen@e0@16@spacebranch\endcsname{52}
\expandafter\def\csname res@qwen@e0@64@root\endcsname{85.4}
\expandafter\def\csname res@qwen@e0@64@branch\endcsname{6.1}
\expandafter\def\csname res@qwen@e0@64@stop\endcsname{8.5}
\expandafter\def\csname res@qwen@e0@64@coin\endcsname{91.5}
\expandafter\def\csname res@qwen@e0@64@noncanon\endcsname{2.5}
\expandafter\def\csname res@qwen@e0@64@Hstr\endcsname{2.50}
\expandafter\def\csname res@qwen@e0@64@hubdrop\endcsname{86.4}
\expandafter\def\csname res@qwen@e0@64@largest\endcsname{60}
\expandafter\def\csname res@qwen@e0@64@spacebranch\endcsname{42}
\expandafter\def\csname res@qwen@e0@256@root\endcsname{85.1}
\expandafter\def\csname res@qwen@e0@256@branch\endcsname{6.7}
\expandafter\def\csname res@qwen@e0@256@stop\endcsname{8.3}
\expandafter\def\csname res@qwen@e0@256@coin\endcsname{91.7}
\expandafter\def\csname res@qwen@e0@256@noncanon\endcsname{0.0}
\expandafter\def\csname res@qwen@e0@256@Hstr\endcsname{3.10}
\expandafter\def\csname res@qwen@e0@256@hubdrop\endcsname{87.0}
\expandafter\def\csname res@qwen@e0@256@largest\endcsname{56}
\expandafter\def\csname res@qwen@e0@256@spacebranch\endcsname{29}
\expandafter\def\csname res@qwen@e0@1k@root\endcsname{82.8}
\expandafter\def\csname res@qwen@e0@1k@branch\endcsname{9.3}
\expandafter\def\csname res@qwen@e0@1k@stop\endcsname{7.8}
\expandafter\def\csname res@qwen@e0@1k@coin\endcsname{92.2}
\expandafter\def\csname res@qwen@e0@1k@noncanon\endcsname{3.1}
\expandafter\def\csname res@qwen@e0@1k@Hstr\endcsname{3.67}
\expandafter\def\csname res@qwen@e0@1k@hubdrop\endcsname{86.5}
\expandafter\def\csname res@qwen@e0@1k@largest\endcsname{52}
\expandafter\def\csname res@qwen@e0@1k@spacebranch\endcsname{28}
\expandafter\def\csname res@qwen@e0@4k@root\endcsname{79.0}
\expandafter\def\csname res@qwen@e0@4k@branch\endcsname{13.0}
\expandafter\def\csname res@qwen@e0@4k@stop\endcsname{8.0}
\expandafter\def\csname res@qwen@e0@4k@coin\endcsname{92.0}
\expandafter\def\csname res@qwen@e0@4k@noncanon\endcsname{0.9}
\expandafter\def\csname res@qwen@e0@4k@Hstr\endcsname{4.08}
\expandafter\def\csname res@qwen@e0@4k@hubdrop\endcsname{85.9}
\expandafter\def\csname res@qwen@e0@4k@largest\endcsname{50}
\expandafter\def\csname res@qwen@e0@4k@spacebranch\endcsname{14}
\expandafter\def\csname res@qwen@e0@Full@root\endcsname{43.0}
\expandafter\def\csname res@qwen@e0@Full@branch\endcsname{49.1}
\expandafter\def\csname res@qwen@e0@Full@stop\endcsname{7.9}
\expandafter\def\csname res@qwen@e0@Full@coin\endcsname{92.1}
\expandafter\def\csname res@qwen@e0@Full@noncanon\endcsname{0.9}
\expandafter\def\csname res@qwen@e0@Full@Hstr\endcsname{4.04}
\expandafter\def\csname res@qwen@e0@Full@hubdrop\endcsname{85.2}
\expandafter\def\csname res@qwen@e0@Full@largest\endcsname{59}
\expandafter\def\csname res@qwen@e0@Full@spacebranch\endcsname{4}
\expandafter\def\csname res@qwen@e0@Full@leadbranch\endcsname{61}
\expandafter\def\csname res@qwen@e0@Full@hubbranch\endcsname{66}
\expandafter\def\csname res@qwen@e0@Full@topstopone\endcsname{6}
\expandafter\def\csname res@qwen@e0@Full@topbranchone\endcsname{22}
\expandafter\def\csname res@qwen@e0@Full@polar\endcsname{89}
\expandafter\def\csname res@qwen@e0@Full@spacemass\endcsname{0.05}
\expandafter\def\csname res@llmjp@e0@16@root\endcsname{87.7}
\expandafter\def\csname res@llmjp@e0@16@branch\endcsname{5.3}
\expandafter\def\csname res@llmjp@e0@16@stop\endcsname{7.0}
\expandafter\def\csname res@llmjp@e0@16@coin\endcsname{93.0}
\expandafter\def\csname res@llmjp@e0@16@noncanon\endcsname{0.0}
\expandafter\def\csname res@llmjp@e0@16@Hstr\endcsname{1.76}
\expandafter\def\csname res@llmjp@e0@16@hubdrop\endcsname{89.9}
\expandafter\def\csname res@llmjp@e0@16@largest\endcsname{66}
\expandafter\def\csname res@llmjp@e0@16@spacebranch\endcsname{50}
\expandafter\def\csname res@llmjp@e0@64@root\endcsname{81.2}
\expandafter\def\csname res@llmjp@e0@64@branch\endcsname{11.3}
\expandafter\def\csname res@llmjp@e0@64@stop\endcsname{7.5}
\expandafter\def\csname res@llmjp@e0@64@coin\endcsname{92.5}
\expandafter\def\csname res@llmjp@e0@64@noncanon\endcsname{7.2}
\expandafter\def\csname res@llmjp@e0@64@Hstr\endcsname{2.34}
\expandafter\def\csname res@llmjp@e0@64@hubdrop\endcsname{87.7}
\expandafter\def\csname res@llmjp@e0@64@largest\endcsname{64}
\expandafter\def\csname res@llmjp@e0@64@spacebranch\endcsname{47}
\expandafter\def\csname res@llmjp@e0@256@root\endcsname{74.0}
\expandafter\def\csname res@llmjp@e0@256@branch\endcsname{17.9}
\expandafter\def\csname res@llmjp@e0@256@stop\endcsname{8.1}
\expandafter\def\csname res@llmjp@e0@256@coin\endcsname{91.9}
\expandafter\def\csname res@llmjp@e0@256@noncanon\endcsname{8.1}
\expandafter\def\csname res@llmjp@e0@256@Hstr\endcsname{3.07}
\expandafter\def\csname res@llmjp@e0@256@hubdrop\endcsname{86.2}
\expandafter\def\csname res@llmjp@e0@256@largest\endcsname{61}
\expandafter\def\csname res@llmjp@e0@256@spacebranch\endcsname{50}
\expandafter\def\csname res@llmjp@e0@1k@root\endcsname{70.7}
\expandafter\def\csname res@llmjp@e0@1k@branch\endcsname{21.9}
\expandafter\def\csname res@llmjp@e0@1k@stop\endcsname{7.4}
\expandafter\def\csname res@llmjp@e0@1k@coin\endcsname{92.6}
\expandafter\def\csname res@llmjp@e0@1k@noncanon\endcsname{2.8}
\expandafter\def\csname res@llmjp@e0@1k@Hstr\endcsname{3.67}
\expandafter\def\csname res@llmjp@e0@1k@hubdrop\endcsname{85.7}
\expandafter\def\csname res@llmjp@e0@1k@largest\endcsname{58}
\expandafter\def\csname res@llmjp@e0@1k@spacebranch\endcsname{38}
\expandafter\def\csname res@llmjp@e0@4k@root\endcsname{57.7}
\expandafter\def\csname res@llmjp@e0@4k@branch\endcsname{34.5}
\expandafter\def\csname res@llmjp@e0@4k@stop\endcsname{7.8}
\expandafter\def\csname res@llmjp@e0@4k@coin\endcsname{92.2}
\expandafter\def\csname res@llmjp@e0@4k@noncanon\endcsname{5.0}
\expandafter\def\csname res@llmjp@e0@4k@Hstr\endcsname{3.84}
\expandafter\def\csname res@llmjp@e0@4k@hubdrop\endcsname{83.9}
\expandafter\def\csname res@llmjp@e0@4k@largest\endcsname{63}
\expandafter\def\csname res@llmjp@e0@4k@spacebranch\endcsname{22}
\expandafter\def\csname res@llmjp@e0@Full@root\endcsname{36.4}
\expandafter\def\csname res@llmjp@e0@Full@branch\endcsname{55.8}
\expandafter\def\csname res@llmjp@e0@Full@stop\endcsname{7.8}
\expandafter\def\csname res@llmjp@e0@Full@coin\endcsname{92.2}
\expandafter\def\csname res@llmjp@e0@Full@noncanon\endcsname{10.3}
\expandafter\def\csname res@llmjp@e0@Full@Hstr\endcsname{3.95}
\expandafter\def\csname res@llmjp@e0@Full@hubdrop\endcsname{83.8}
\expandafter\def\csname res@llmjp@e0@Full@largest\endcsname{70}
\expandafter\def\csname res@llmjp@e0@Full@spacebranch\endcsname{15}
\expandafter\def\csname res@llmjp@e0@Full@leadbranch\endcsname{62}
\expandafter\def\csname res@llmjp@e0@Full@hubbranch\endcsname{76}
\expandafter\def\csname res@llmjp@e0@Full@topstopone\endcsname{3}
\expandafter\def\csname res@llmjp@e0@Full@topbranchone\endcsname{35}
\expandafter\def\csname res@llmjp@e0@Full@polar\endcsname{86}
\expandafter\def\csname res@llmjp@e0@Full@spacemass\endcsname{0.10}
\expandafter\def\csname res@all@e0@Full@topstopmax\endcsname{9}
\expandafter\def\csname res@llama@e0@any@spacebranchmin\endcsname{64}
\expandafter\def\csname res@llama@e0@any@spacebranchmax\endcsname{87}
\expandafter\def\csname res@qwen@e0@any@spacebranchmin\endcsname{4}
\expandafter\def\csname res@qwen@e0@any@spacebranchmax\endcsname{52}
\expandafter\def\csname res@llmjp@e0@any@spacebranchmin\endcsname{15}
\expandafter\def\csname res@llmjp@e0@any@spacebranchmax\endcsname{50}
\expandafter\def\csname res@all@e0@16@branchmin\endcsname{4}
\expandafter\def\csname res@all@e0@16@branchmax\endcsname{12}
\expandafter\def\csname res@all@e0@Full@branchmin\endcsname{49}
\expandafter\def\csname res@all@e0@Full@branchmax\endcsname{77}
\expandafter\def\csname res@llama@native@all@recovered\endcsname{0}
\expandafter\def\csname res@llama@native@all@bndtot\endcsname{0}
\expandafter\def\csname res@llama@native@all@silent\endcsname{21}
\expandafter\def\csname res@llama@ratio@16@native\endcsname{0.92}
\expandafter\def\csname res@llama@ratio@64@native\endcsname{0.92}
\expandafter\def\csname res@llama@ratio@256@native\endcsname{0.91}
\expandafter\def\csname res@llama@ratio@1k@native\endcsname{0.91}
\expandafter\def\csname res@llama@ratio@4k@native\endcsname{0.92}
\expandafter\def\csname res@llama@ratio@Full@native\endcsname{0.92}
\expandafter\def\csname res@llama@ratio@16@stepwise\endcsname{0.92}
\expandafter\def\csname res@llama@ratio@64@stepwise\endcsname{0.91}
\expandafter\def\csname res@llama@ratio@256@stepwise\endcsname{0.91}
\expandafter\def\csname res@llama@ratio@1k@stepwise\endcsname{0.91}
\expandafter\def\csname res@llama@ratio@4k@stepwise\endcsname{0.91}
\expandafter\def\csname res@llama@native@16@bpt\endcsname{2.02}
\expandafter\def\csname res@llama@native@16@util\endcsname{.644}
\expandafter\def\csname res@llama@native@16@utilpct\endcsname{64.4}
\expandafter\def\csname res@llama@native@16@kl\endcsname{0}
\expandafter\def\csname res@llama@native@16@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@16@n\endcsname{100}
\expandafter\def\csname res@llama@native@16@tested\endcsname{100}
\expandafter\def\csname res@llama@native@16@err\endcsname{2}
\expandafter\def\csname res@llama@native@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@16@utilk\endcsname{.987}
\expandafter\def\csname res@llama@native@16@bptlo\endcsname{1.91}
\expandafter\def\csname res@llama@native@16@bpthi\endcsname{2.13}
\expandafter\def\csname res@llama@native@16@utillo\endcsname{.629}
\expandafter\def\csname res@llama@native@16@utilhi\endcsname{.659}
\expandafter\def\csname res@llama@native@16@utilklo\endcsname{.973}
\expandafter\def\csname res@llama@native@16@utilkhi\endcsname{1.001}
\expandafter\def\csname res@llama@basic@16@bpt\endcsname{2.25}
\expandafter\def\csname res@llama@basic@16@util\endcsname{.635}
\expandafter\def\csname res@llama@basic@16@utilpct\endcsname{63.5}
\expandafter\def\csname res@llama@basic@16@kl\endcsname{.466}
\expandafter\def\csname res@llama@basic@16@klkappa\endcsname{0.466}
\expandafter\def\csname res@llama@basic@16@n\endcsname{100}
\expandafter\def\csname res@llama@basic@16@tested\endcsname{20}
\expandafter\def\csname res@llama@basic@16@err\endcsname{0}
\expandafter\def\csname res@llama@basic@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@16@utilk\endcsname{1.006}
\expandafter\def\csname res@llama@basic@16@bptlo\endcsname{2.18}
\expandafter\def\csname res@llama@basic@16@bpthi\endcsname{2.32}
\expandafter\def\csname res@llama@basic@16@utillo\endcsname{.620}
\expandafter\def\csname res@llama@basic@16@utilhi\endcsname{.649}
\expandafter\def\csname res@llama@basic@16@utilklo\endcsname{.992}
\expandafter\def\csname res@llama@basic@16@utilkhi\endcsname{1.020}
\expandafter\def\csname res@llama@mwis@16@bpt\endcsname{1.90}
\expandafter\def\csname res@llama@mwis@16@util\endcsname{.602}
\expandafter\def\csname res@llama@mwis@16@utilpct\endcsname{60.2}
\expandafter\def\csname res@llama@mwis@16@kl\endcsname{.052}
\expandafter\def\csname res@llama@mwis@16@klkappa\endcsname{0.052}
\expandafter\def\csname res@llama@mwis@16@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@16@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@16@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@16@utilk\endcsname{.922}
\expandafter\def\csname res@llama@mwis@16@bptlo\endcsname{1.80}
\expandafter\def\csname res@llama@mwis@16@bpthi\endcsname{2.00}
\expandafter\def\csname res@llama@mwis@16@utillo\endcsname{.589}
\expandafter\def\csname res@llama@mwis@16@utilhi\endcsname{.615}
\expandafter\def\csname res@llama@mwis@16@utilklo\endcsname{.908}
\expandafter\def\csname res@llama@mwis@16@utilkhi\endcsname{.935}
\expandafter\def\csname res@llama@stepwise@16@bpt\endcsname{2.03}
\expandafter\def\csname res@llama@stepwise@16@util\endcsname{.645}
\expandafter\def\csname res@llama@stepwise@16@utilpct\endcsname{64.5}
\expandafter\def\csname res@llama@stepwise@16@kl\endcsname{.0019}
\expandafter\def\csname res@llama@stepwise@16@klkappa\endcsname{0.002}
\expandafter\def\csname res@llama@stepwise@16@n\endcsname{100}
\expandafter\def\csname res@llama@stepwise@16@tested\endcsname{20}
\expandafter\def\csname res@llama@stepwise@16@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@16@utilk\endcsname{.987}
\expandafter\def\csname res@llama@stepwise@16@bptlo\endcsname{1.91}
\expandafter\def\csname res@llama@stepwise@16@bpthi\endcsname{2.14}
\expandafter\def\csname res@llama@stepwise@16@utillo\endcsname{.632}
\expandafter\def\csname res@llama@stepwise@16@utilhi\endcsname{.658}
\expandafter\def\csname res@llama@stepwise@16@utilklo\endcsname{.974}
\expandafter\def\csname res@llama@stepwise@16@utilkhi\endcsname{.999}
\expandafter\def\csname res@llama@syncpool@16@bpt\endcsname{1.61}
\expandafter\def\csname res@llama@syncpool@16@util\endcsname{.511}
\expandafter\def\csname res@llama@syncpool@16@utilpct\endcsname{51.1}
\expandafter\def\csname res@llama@syncpool@16@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@16@klkappa\endcsname{0.277}
\expandafter\def\csname res@llama@syncpool@16@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@16@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@16@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@16@utilk\endcsname{.792}
\expandafter\def\csname res@llama@syncpool@16@bptlo\endcsname{1.50}
\expandafter\def\csname res@llama@syncpool@16@bpthi\endcsname{1.72}
\expandafter\def\csname res@llama@syncpool@16@utillo\endcsname{.491}
\expandafter\def\csname res@llama@syncpool@16@utilhi\endcsname{.530}
\expandafter\def\csname res@llama@syncpool@16@utilklo\endcsname{.768}
\expandafter\def\csname res@llama@syncpool@16@utilkhi\endcsname{.815}
\expandafter\def\csname res@llama@coin@16@bpt\endcsname{1.85}
\expandafter\def\csname res@llama@coin@16@util\endcsname{.592}
\expandafter\def\csname res@llama@coin@16@utilpct\endcsname{59.2}
\expandafter\def\csname res@llama@coin@16@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@16@klkappa\endcsname{0.117}
\expandafter\def\csname res@llama@coin@16@n\endcsname{100}
\expandafter\def\csname res@llama@coin@16@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@16@err\endcsname{0}
\expandafter\def\csname res@llama@coin@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@16@utilk\endcsname{.898}
\expandafter\def\csname res@llama@coin@16@bptlo\endcsname{1.75}
\expandafter\def\csname res@llama@coin@16@bpthi\endcsname{1.95}
\expandafter\def\csname res@llama@coin@16@utillo\endcsname{.581}
\expandafter\def\csname res@llama@coin@16@utilhi\endcsname{.604}
\expandafter\def\csname res@llama@coin@16@utilklo\endcsname{.885}
\expandafter\def\csname res@llama@coin@16@utilkhi\endcsname{.910}
\expandafter\def\csname res@llama@hubdrop@16@bpt\endcsname{1.79}
\expandafter\def\csname res@llama@hubdrop@16@util\endcsname{.567}
\expandafter\def\csname res@llama@hubdrop@16@utilpct\endcsname{56.7}
\expandafter\def\csname res@llama@hubdrop@16@kl\endcsname{.0019}
\expandafter\def\csname res@llama@hubdrop@16@klkappa\endcsname{0.167}
\expandafter\def\csname res@llama@hubdrop@16@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@16@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@16@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@16@utilk\endcsname{.866}
\expandafter\def\csname res@llama@hubdrop@16@bptlo\endcsname{1.69}
\expandafter\def\csname res@llama@hubdrop@16@bpthi\endcsname{1.90}
\expandafter\def\csname res@llama@hubdrop@16@utillo\endcsname{.551}
\expandafter\def\csname res@llama@hubdrop@16@utilhi\endcsname{.582}
\expandafter\def\csname res@llama@hubdrop@16@utilklo\endcsname{.847}
\expandafter\def\csname res@llama@hubdrop@16@utilkhi\endcsname{.884}
\expandafter\def\csname res@llama@native@64@bpt\endcsname{2.65}
\expandafter\def\csname res@llama@native@64@util\endcsname{.794}
\expandafter\def\csname res@llama@native@64@utilpct\endcsname{79.4}
\expandafter\def\csname res@llama@native@64@kl\endcsname{0}
\expandafter\def\csname res@llama@native@64@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@64@n\endcsname{100}
\expandafter\def\csname res@llama@native@64@tested\endcsname{100}
\expandafter\def\csname res@llama@native@64@err\endcsname{3}
\expandafter\def\csname res@llama@native@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@64@utilk\endcsname{.985}
\expandafter\def\csname res@llama@native@64@bptlo\endcsname{2.50}
\expandafter\def\csname res@llama@native@64@bpthi\endcsname{2.79}
\expandafter\def\csname res@llama@native@64@utillo\endcsname{.780}
\expandafter\def\csname res@llama@native@64@utilhi\endcsname{.807}
\expandafter\def\csname res@llama@native@64@utilklo\endcsname{.972}
\expandafter\def\csname res@llama@native@64@utilkhi\endcsname{.999}
\expandafter\def\csname res@llama@basic@64@bpt\endcsname{3.25}
\expandafter\def\csname res@llama@basic@64@util\endcsname{.815}
\expandafter\def\csname res@llama@basic@64@utilpct\endcsname{81.5}
\expandafter\def\csname res@llama@basic@64@kl\endcsname{.718}
\expandafter\def\csname res@llama@basic@64@klkappa\endcsname{0.718}
\expandafter\def\csname res@llama@basic@64@n\endcsname{100}
\expandafter\def\csname res@llama@basic@64@tested\endcsname{20}
\expandafter\def\csname res@llama@basic@64@err\endcsname{0}
\expandafter\def\csname res@llama@basic@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@64@utilk\endcsname{1.053}
\expandafter\def\csname res@llama@basic@64@bptlo\endcsname{3.16}
\expandafter\def\csname res@llama@basic@64@bpthi\endcsname{3.34}
\expandafter\def\csname res@llama@basic@64@utillo\endcsname{.801}
\expandafter\def\csname res@llama@basic@64@utilhi\endcsname{.829}
\expandafter\def\csname res@llama@basic@64@utilklo\endcsname{1.039}
\expandafter\def\csname res@llama@basic@64@utilkhi\endcsname{1.068}
\expandafter\def\csname res@llama@mwis@64@bpt\endcsname{2.45}
\expandafter\def\csname res@llama@mwis@64@util\endcsname{.735}
\expandafter\def\csname res@llama@mwis@64@utilpct\endcsname{73.5}
\expandafter\def\csname res@llama@mwis@64@kl\endcsname{.064}
\expandafter\def\csname res@llama@mwis@64@klkappa\endcsname{0.064}
\expandafter\def\csname res@llama@mwis@64@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@64@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@64@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@64@utilk\endcsname{.909}
\expandafter\def\csname res@llama@mwis@64@bptlo\endcsname{2.30}
\expandafter\def\csname res@llama@mwis@64@bpthi\endcsname{2.59}
\expandafter\def\csname res@llama@mwis@64@utillo\endcsname{.723}
\expandafter\def\csname res@llama@mwis@64@utilhi\endcsname{.747}
\expandafter\def\csname res@llama@mwis@64@utilklo\endcsname{.898}
\expandafter\def\csname res@llama@mwis@64@utilkhi\endcsname{.921}
\expandafter\def\csname res@llama@stepwise@64@bpt\endcsname{2.73}
\expandafter\def\csname res@llama@stepwise@64@util\endcsname{.798}
\expandafter\def\csname res@llama@stepwise@64@utilpct\endcsname{79.8}
\expandafter\def\csname res@llama@stepwise@64@kl\endcsname{.0012}
\expandafter\def\csname res@llama@stepwise@64@klkappa\endcsname{0.001}
\expandafter\def\csname res@llama@stepwise@64@n\endcsname{100}
\expandafter\def\csname res@llama@stepwise@64@tested\endcsname{20}
\expandafter\def\csname res@llama@stepwise@64@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@64@utilk\endcsname{.995}
\expandafter\def\csname res@llama@stepwise@64@bptlo\endcsname{2.59}
\expandafter\def\csname res@llama@stepwise@64@bpthi\endcsname{2.87}
\expandafter\def\csname res@llama@stepwise@64@utillo\endcsname{.786}
\expandafter\def\csname res@llama@stepwise@64@utilhi\endcsname{.810}
\expandafter\def\csname res@llama@stepwise@64@utilklo\endcsname{.983}
\expandafter\def\csname res@llama@stepwise@64@utilkhi\endcsname{1.008}
\expandafter\def\csname res@llama@syncpool@64@bpt\endcsname{1.57}
\expandafter\def\csname res@llama@syncpool@64@util\endcsname{.459}
\expandafter\def\csname res@llama@syncpool@64@utilpct\endcsname{45.9}
\expandafter\def\csname res@llama@syncpool@64@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@64@klkappa\endcsname{0.783}
\expandafter\def\csname res@llama@syncpool@64@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@64@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@64@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@64@utilk\endcsname{.575}
\expandafter\def\csname res@llama@syncpool@64@bptlo\endcsname{1.44}
\expandafter\def\csname res@llama@syncpool@64@bpthi\endcsname{1.70}
\expandafter\def\csname res@llama@syncpool@64@utillo\endcsname{.433}
\expandafter\def\csname res@llama@syncpool@64@utilhi\endcsname{.485}
\expandafter\def\csname res@llama@syncpool@64@utilklo\endcsname{.544}
\expandafter\def\csname res@llama@syncpool@64@utilkhi\endcsname{.605}
\expandafter\def\csname res@llama@coin@64@bpt\endcsname{2.52}
\expandafter\def\csname res@llama@coin@64@util\endcsname{.729}
\expandafter\def\csname res@llama@coin@64@utilpct\endcsname{72.9}
\expandafter\def\csname res@llama@coin@64@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@64@klkappa\endcsname{0.149}
\expandafter\def\csname res@llama@coin@64@n\endcsname{100}
\expandafter\def\csname res@llama@coin@64@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@64@err\endcsname{0}
\expandafter\def\csname res@llama@coin@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@64@utilk\endcsname{.911}
\expandafter\def\csname res@llama@coin@64@bptlo\endcsname{2.38}
\expandafter\def\csname res@llama@coin@64@bpthi\endcsname{2.64}
\expandafter\def\csname res@llama@coin@64@utillo\endcsname{.716}
\expandafter\def\csname res@llama@coin@64@utilhi\endcsname{.742}
\expandafter\def\csname res@llama@coin@64@utilklo\endcsname{.898}
\expandafter\def\csname res@llama@coin@64@utilkhi\endcsname{.924}
\expandafter\def\csname res@llama@hubdrop@64@bpt\endcsname{2.37}
\expandafter\def\csname res@llama@hubdrop@64@util\endcsname{.697}
\expandafter\def\csname res@llama@hubdrop@64@utilpct\endcsname{69.7}
\expandafter\def\csname res@llama@hubdrop@64@kl\endcsname{.0032}
\expandafter\def\csname res@llama@hubdrop@64@klkappa\endcsname{0.231}
\expandafter\def\csname res@llama@hubdrop@64@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@64@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@64@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@64@utilk\endcsname{.871}
\expandafter\def\csname res@llama@hubdrop@64@bptlo\endcsname{2.22}
\expandafter\def\csname res@llama@hubdrop@64@bpthi\endcsname{2.49}
\expandafter\def\csname res@llama@hubdrop@64@utillo\endcsname{.682}
\expandafter\def\csname res@llama@hubdrop@64@utilhi\endcsname{.711}
\expandafter\def\csname res@llama@hubdrop@64@utilklo\endcsname{.855}
\expandafter\def\csname res@llama@hubdrop@64@utilkhi\endcsname{.885}
\expandafter\def\csname res@llama@native@256@bpt\endcsname{3.17}
\expandafter\def\csname res@llama@native@256@util\endcsname{.890}
\expandafter\def\csname res@llama@native@256@utilpct\endcsname{89.0}
\expandafter\def\csname res@llama@native@256@kl\endcsname{0}
\expandafter\def\csname res@llama@native@256@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@256@n\endcsname{100}
\expandafter\def\csname res@llama@native@256@tested\endcsname{100}
\expandafter\def\csname res@llama@native@256@err\endcsname{4}
\expandafter\def\csname res@llama@native@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@256@utilk\endcsname{.992}
\expandafter\def\csname res@llama@native@256@bptlo\endcsname{2.98}
\expandafter\def\csname res@llama@native@256@bpthi\endcsname{3.34}
\expandafter\def\csname res@llama@native@256@utillo\endcsname{.878}
\expandafter\def\csname res@llama@native@256@utilhi\endcsname{.902}
\expandafter\def\csname res@llama@native@256@utilklo\endcsname{.980}
\expandafter\def\csname res@llama@native@256@utilkhi\endcsname{1.004}
\expandafter\def\csname res@llama@basic@256@bpt\endcsname{4.35}
\expandafter\def\csname res@llama@basic@256@util\endcsname{.916}
\expandafter\def\csname res@llama@basic@256@utilpct\endcsname{91.6}
\expandafter\def\csname res@llama@basic@256@kl\endcsname{.933}
\expandafter\def\csname res@llama@basic@256@klkappa\endcsname{0.933}
\expandafter\def\csname res@llama@basic@256@n\endcsname{100}
\expandafter\def\csname res@llama@basic@256@tested\endcsname{20}
\expandafter\def\csname res@llama@basic@256@err\endcsname{0}
\expandafter\def\csname res@llama@basic@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@256@utilk\endcsname{1.075}
\expandafter\def\csname res@llama@basic@256@bptlo\endcsname{4.22}
\expandafter\def\csname res@llama@basic@256@bpthi\endcsname{4.46}
\expandafter\def\csname res@llama@basic@256@utillo\endcsname{.904}
\expandafter\def\csname res@llama@basic@256@utilhi\endcsname{.929}
\expandafter\def\csname res@llama@basic@256@utilklo\endcsname{1.062}
\expandafter\def\csname res@llama@basic@256@utilkhi\endcsname{1.089}
\expandafter\def\csname res@llama@mwis@256@bpt\endcsname{2.81}
\expandafter\def\csname res@llama@mwis@256@util\endcsname{.824}
\expandafter\def\csname res@llama@mwis@256@utilpct\endcsname{82.4}
\expandafter\def\csname res@llama@mwis@256@kl\endcsname{.074}
\expandafter\def\csname res@llama@mwis@256@klkappa\endcsname{0.074}
\expandafter\def\csname res@llama@mwis@256@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@256@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@256@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@256@utilk\endcsname{.916}
\expandafter\def\csname res@llama@mwis@256@bptlo\endcsname{2.62}
\expandafter\def\csname res@llama@mwis@256@bpthi\endcsname{2.99}
\expandafter\def\csname res@llama@mwis@256@utillo\endcsname{.810}
\expandafter\def\csname res@llama@mwis@256@utilhi\endcsname{.837}
\expandafter\def\csname res@llama@mwis@256@utilklo\endcsname{.902}
\expandafter\def\csname res@llama@mwis@256@utilkhi\endcsname{.931}
\expandafter\def\csname res@llama@stepwise@256@bpt\endcsname{3.19}
\expandafter\def\csname res@llama@stepwise@256@util\endcsname{.891}
\expandafter\def\csname res@llama@stepwise@256@utilpct\endcsname{89.1}
\expandafter\def\csname res@llama@stepwise@256@kl\endcsname{.002}
\expandafter\def\csname res@llama@stepwise@256@klkappa\endcsname{0.002}
\expandafter\def\csname res@llama@stepwise@256@n\endcsname{100}
\expandafter\def\csname res@llama@stepwise@256@tested\endcsname{20}
\expandafter\def\csname res@llama@stepwise@256@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@256@utilk\endcsname{.996}
\expandafter\def\csname res@llama@stepwise@256@bptlo\endcsname{3.01}
\expandafter\def\csname res@llama@stepwise@256@bpthi\endcsname{3.35}
\expandafter\def\csname res@llama@stepwise@256@utillo\endcsname{.880}
\expandafter\def\csname res@llama@stepwise@256@utilhi\endcsname{.904}
\expandafter\def\csname res@llama@stepwise@256@utilklo\endcsname{.982}
\expandafter\def\csname res@llama@stepwise@256@utilkhi\endcsname{1.009}
\expandafter\def\csname res@llama@syncpool@256@bpt\endcsname{0.85}
\expandafter\def\csname res@llama@syncpool@256@util\endcsname{.241}
\expandafter\def\csname res@llama@syncpool@256@utilpct\endcsname{24.1}
\expandafter\def\csname res@llama@syncpool@256@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@256@klkappa\endcsname{1.555}
\expandafter\def\csname res@llama@syncpool@256@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@256@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@256@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@256@utilk\endcsname{.269}
\expandafter\def\csname res@llama@syncpool@256@bptlo\endcsname{0.77}
\expandafter\def\csname res@llama@syncpool@256@bpthi\endcsname{0.93}
\expandafter\def\csname res@llama@syncpool@256@utillo\endcsname{.223}
\expandafter\def\csname res@llama@syncpool@256@utilhi\endcsname{.260}
\expandafter\def\csname res@llama@syncpool@256@utilklo\endcsname{.249}
\expandafter\def\csname res@llama@syncpool@256@utilkhi\endcsname{.291}
\expandafter\def\csname res@llama@coin@256@bpt\endcsname{2.86}
\expandafter\def\csname res@llama@coin@256@util\endcsname{.810}
\expandafter\def\csname res@llama@coin@256@utilpct\endcsname{81.0}
\expandafter\def\csname res@llama@coin@256@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@256@klkappa\endcsname{0.179}
\expandafter\def\csname res@llama@coin@256@n\endcsname{100}
\expandafter\def\csname res@llama@coin@256@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@256@err\endcsname{0}
\expandafter\def\csname res@llama@coin@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@256@utilk\endcsname{.906}
\expandafter\def\csname res@llama@coin@256@bptlo\endcsname{2.70}
\expandafter\def\csname res@llama@coin@256@bpthi\endcsname{3.01}
\expandafter\def\csname res@llama@coin@256@utillo\endcsname{.798}
\expandafter\def\csname res@llama@coin@256@utilhi\endcsname{.823}
\expandafter\def\csname res@llama@coin@256@utilklo\endcsname{.894}
\expandafter\def\csname res@llama@coin@256@utilkhi\endcsname{.919}
\expandafter\def\csname res@llama@hubdrop@256@bpt\endcsname{2.70}
\expandafter\def\csname res@llama@hubdrop@256@util\endcsname{.764}
\expandafter\def\csname res@llama@hubdrop@256@utilpct\endcsname{76.4}
\expandafter\def\csname res@llama@hubdrop@256@kl\endcsname{.0046}
\expandafter\def\csname res@llama@hubdrop@256@klkappa\endcsname{0.300}
\expandafter\def\csname res@llama@hubdrop@256@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@256@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@256@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@256@utilk\endcsname{.855}
\expandafter\def\csname res@llama@hubdrop@256@bptlo\endcsname{2.52}
\expandafter\def\csname res@llama@hubdrop@256@bpthi\endcsname{2.86}
\expandafter\def\csname res@llama@hubdrop@256@utillo\endcsname{.742}
\expandafter\def\csname res@llama@hubdrop@256@utilhi\endcsname{.784}
\expandafter\def\csname res@llama@hubdrop@256@utilklo\endcsname{.832}
\expandafter\def\csname res@llama@hubdrop@256@utilkhi\endcsname{.875}
\expandafter\def\csname res@llama@native@1k@bpt\endcsname{3.51}
\expandafter\def\csname res@llama@native@1k@util\endcsname{.944}
\expandafter\def\csname res@llama@native@1k@utilpct\endcsname{94.4}
\expandafter\def\csname res@llama@native@1k@kl\endcsname{0}
\expandafter\def\csname res@llama@native@1k@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@1k@n\endcsname{100}
\expandafter\def\csname res@llama@native@1k@tested\endcsname{100}
\expandafter\def\csname res@llama@native@1k@err\endcsname{5}
\expandafter\def\csname res@llama@native@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@1k@utilk\endcsname{.995}
\expandafter\def\csname res@llama@native@1k@bptlo\endcsname{3.32}
\expandafter\def\csname res@llama@native@1k@bpthi\endcsname{3.69}
\expandafter\def\csname res@llama@native@1k@utillo\endcsname{.934}
\expandafter\def\csname res@llama@native@1k@utilhi\endcsname{.956}
\expandafter\def\csname res@llama@native@1k@utilklo\endcsname{.984}
\expandafter\def\csname res@llama@native@1k@utilkhi\endcsname{1.007}
\expandafter\def\csname res@llama@basic@1k@bpt\endcsname{5.22}
\expandafter\def\csname res@llama@basic@1k@util\endcsname{.984}
\expandafter\def\csname res@llama@basic@1k@utilpct\endcsname{98.4}
\expandafter\def\csname res@llama@basic@1k@kl\endcsname{1.05}
\expandafter\def\csname res@llama@basic@1k@klkappa\endcsname{1.055}
\expandafter\def\csname res@llama@basic@1k@n\endcsname{100}
\expandafter\def\csname res@llama@basic@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@basic@1k@err\endcsname{0}
\expandafter\def\csname res@llama@basic@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@1k@utilk\endcsname{1.072}
\expandafter\def\csname res@llama@basic@1k@bptlo\endcsname{5.04}
\expandafter\def\csname res@llama@basic@1k@bpthi\endcsname{5.39}
\expandafter\def\csname res@llama@basic@1k@utillo\endcsname{.970}
\expandafter\def\csname res@llama@basic@1k@utilhi\endcsname{.997}
\expandafter\def\csname res@llama@basic@1k@utilklo\endcsname{1.057}
\expandafter\def\csname res@llama@basic@1k@utilkhi\endcsname{1.087}
\expandafter\def\csname res@llama@mwis@1k@bpt\endcsname{3.14}
\expandafter\def\csname res@llama@mwis@1k@util\endcsname{.878}
\expandafter\def\csname res@llama@mwis@1k@utilpct\endcsname{87.8}
\expandafter\def\csname res@llama@mwis@1k@kl\endcsname{.083}
\expandafter\def\csname res@llama@mwis@1k@klkappa\endcsname{0.083}
\expandafter\def\csname res@llama@mwis@1k@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@1k@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@1k@utilk\endcsname{.920}
\expandafter\def\csname res@llama@mwis@1k@bptlo\endcsname{2.95}
\expandafter\def\csname res@llama@mwis@1k@bpthi\endcsname{3.31}
\expandafter\def\csname res@llama@mwis@1k@utillo\endcsname{.866}
\expandafter\def\csname res@llama@mwis@1k@utilhi\endcsname{.891}
\expandafter\def\csname res@llama@mwis@1k@utilklo\endcsname{.907}
\expandafter\def\csname res@llama@mwis@1k@utilkhi\endcsname{.933}
\expandafter\def\csname res@llama@stepwise@1k@bpt\endcsname{3.47}
\expandafter\def\csname res@llama@stepwise@1k@util\endcsname{.945}
\expandafter\def\csname res@llama@stepwise@1k@utilpct\endcsname{94.5}
\expandafter\def\csname res@llama@stepwise@1k@kl\endcsname{.0043}
\expandafter\def\csname res@llama@stepwise@1k@klkappa\endcsname{0.004}
\expandafter\def\csname res@llama@stepwise@1k@n\endcsname{100}
\expandafter\def\csname res@llama@stepwise@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@stepwise@1k@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@1k@utilk\endcsname{.997}
\expandafter\def\csname res@llama@stepwise@1k@bptlo\endcsname{3.25}
\expandafter\def\csname res@llama@stepwise@1k@bpthi\endcsname{3.68}
\expandafter\def\csname res@llama@stepwise@1k@utillo\endcsname{.931}
\expandafter\def\csname res@llama@stepwise@1k@utilhi\endcsname{.959}
\expandafter\def\csname res@llama@stepwise@1k@utilklo\endcsname{.982}
\expandafter\def\csname res@llama@stepwise@1k@utilkhi\endcsname{1.012}
\expandafter\def\csname res@llama@syncpool@1k@bpt\endcsname{0.52}
\expandafter\def\csname res@llama@syncpool@1k@util\endcsname{.139}
\expandafter\def\csname res@llama@syncpool@1k@utilpct\endcsname{13.9}
\expandafter\def\csname res@llama@syncpool@1k@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@1k@klkappa\endcsname{2.072}
\expandafter\def\csname res@llama@syncpool@1k@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@1k@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@1k@utilk\endcsname{.147}
\expandafter\def\csname res@llama@syncpool@1k@bptlo\endcsname{0.45}
\expandafter\def\csname res@llama@syncpool@1k@bpthi\endcsname{0.60}
\expandafter\def\csname res@llama@syncpool@1k@utillo\endcsname{.121}
\expandafter\def\csname res@llama@syncpool@1k@utilhi\endcsname{.158}
\expandafter\def\csname res@llama@syncpool@1k@utilklo\endcsname{.128}
\expandafter\def\csname res@llama@syncpool@1k@utilkhi\endcsname{.167}
\expandafter\def\csname res@llama@coin@1k@bpt\endcsname{3.21}
\expandafter\def\csname res@llama@coin@1k@util\endcsname{.861}
\expandafter\def\csname res@llama@coin@1k@utilpct\endcsname{86.1}
\expandafter\def\csname res@llama@coin@1k@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@1k@klkappa\endcsname{0.209}
\expandafter\def\csname res@llama@coin@1k@n\endcsname{100}
\expandafter\def\csname res@llama@coin@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@1k@err\endcsname{0}
\expandafter\def\csname res@llama@coin@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@1k@utilk\endcsname{.907}
\expandafter\def\csname res@llama@coin@1k@bptlo\endcsname{3.02}
\expandafter\def\csname res@llama@coin@1k@bpthi\endcsname{3.37}
\expandafter\def\csname res@llama@coin@1k@utillo\endcsname{.848}
\expandafter\def\csname res@llama@coin@1k@utilhi\endcsname{.874}
\expandafter\def\csname res@llama@coin@1k@utilklo\endcsname{.893}
\expandafter\def\csname res@llama@coin@1k@utilkhi\endcsname{.920}
\expandafter\def\csname res@llama@hubdrop@1k@bpt\endcsname{2.89}
\expandafter\def\csname res@llama@hubdrop@1k@util\endcsname{.799}
\expandafter\def\csname res@llama@hubdrop@1k@utilpct\endcsname{79.9}
\expandafter\def\csname res@llama@hubdrop@1k@kl\endcsname{.0058}
\expandafter\def\csname res@llama@hubdrop@1k@klkappa\endcsname{0.354}
\expandafter\def\csname res@llama@hubdrop@1k@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@1k@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@1k@utilk\endcsname{.840}
\expandafter\def\csname res@llama@hubdrop@1k@bptlo\endcsname{2.71}
\expandafter\def\csname res@llama@hubdrop@1k@bpthi\endcsname{3.07}
\expandafter\def\csname res@llama@hubdrop@1k@utillo\endcsname{.777}
\expandafter\def\csname res@llama@hubdrop@1k@utilhi\endcsname{.817}
\expandafter\def\csname res@llama@hubdrop@1k@utilklo\endcsname{.819}
\expandafter\def\csname res@llama@hubdrop@1k@utilkhi\endcsname{.858}
\expandafter\def\csname res@llama@native@4k@bpt\endcsname{3.61}
\expandafter\def\csname res@llama@native@4k@util\endcsname{.971}
\expandafter\def\csname res@llama@native@4k@utilpct\endcsname{97.1}
\expandafter\def\csname res@llama@native@4k@kl\endcsname{0}
\expandafter\def\csname res@llama@native@4k@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@4k@n\endcsname{100}
\expandafter\def\csname res@llama@native@4k@tested\endcsname{100}
\expandafter\def\csname res@llama@native@4k@err\endcsname{5}
\expandafter\def\csname res@llama@native@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@4k@utilk\endcsname{.988}
\expandafter\def\csname res@llama@native@4k@bptlo\endcsname{3.39}
\expandafter\def\csname res@llama@native@4k@bpthi\endcsname{3.82}
\expandafter\def\csname res@llama@native@4k@utillo\endcsname{.958}
\expandafter\def\csname res@llama@native@4k@utilhi\endcsname{.985}
\expandafter\def\csname res@llama@native@4k@utilklo\endcsname{.975}
\expandafter\def\csname res@llama@native@4k@utilkhi\endcsname{1.002}
\expandafter\def\csname res@llama@basic@4k@bpt\endcsname{5.55}
\expandafter\def\csname res@llama@basic@4k@util\endcsname{.984}
\expandafter\def\csname res@llama@basic@4k@utilpct\endcsname{98.4}
\expandafter\def\csname res@llama@basic@4k@kl\endcsname{1.02}
\expandafter\def\csname res@llama@basic@4k@klkappa\endcsname{1.023}
\expandafter\def\csname res@llama@basic@4k@n\endcsname{100}
\expandafter\def\csname res@llama@basic@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@basic@4k@err\endcsname{0}
\expandafter\def\csname res@llama@basic@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@4k@utilk\endcsname{1.023}
\expandafter\def\csname res@llama@basic@4k@bptlo\endcsname{5.23}
\expandafter\def\csname res@llama@basic@4k@bpthi\endcsname{5.87}
\expandafter\def\csname res@llama@basic@4k@utillo\endcsname{.970}
\expandafter\def\csname res@llama@basic@4k@utilhi\endcsname{.997}
\expandafter\def\csname res@llama@basic@4k@utilklo\endcsname{1.008}
\expandafter\def\csname res@llama@basic@4k@utilkhi\endcsname{1.039}
\expandafter\def\csname res@llama@mwis@4k@bpt\endcsname{3.34}
\expandafter\def\csname res@llama@mwis@4k@util\endcsname{.901}
\expandafter\def\csname res@llama@mwis@4k@utilpct\endcsname{90.1}
\expandafter\def\csname res@llama@mwis@4k@kl\endcsname{.088}
\expandafter\def\csname res@llama@mwis@4k@klkappa\endcsname{0.088}
\expandafter\def\csname res@llama@mwis@4k@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@4k@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@4k@utilk\endcsname{.916}
\expandafter\def\csname res@llama@mwis@4k@bptlo\endcsname{3.13}
\expandafter\def\csname res@llama@mwis@4k@bpthi\endcsname{3.54}
\expandafter\def\csname res@llama@mwis@4k@utillo\endcsname{.887}
\expandafter\def\csname res@llama@mwis@4k@utilhi\endcsname{.914}
\expandafter\def\csname res@llama@mwis@4k@utilklo\endcsname{.902}
\expandafter\def\csname res@llama@mwis@4k@utilkhi\endcsname{.930}
\expandafter\def\csname res@llama@stepwise@4k@bpt\endcsname{3.69}
\expandafter\def\csname res@llama@stepwise@4k@util\endcsname{.976}
\expandafter\def\csname res@llama@stepwise@4k@utilpct\endcsname{97.6}
\expandafter\def\csname res@llama@stepwise@4k@kl\endcsname{.0043}
\expandafter\def\csname res@llama@stepwise@4k@klkappa\endcsname{0.004}
\expandafter\def\csname res@llama@stepwise@4k@n\endcsname{100}
\expandafter\def\csname res@llama@stepwise@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@stepwise@4k@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@4k@utilk\endcsname{.993}
\expandafter\def\csname res@llama@stepwise@4k@bptlo\endcsname{3.47}
\expandafter\def\csname res@llama@stepwise@4k@bpthi\endcsname{3.90}
\expandafter\def\csname res@llama@stepwise@4k@utillo\endcsname{.963}
\expandafter\def\csname res@llama@stepwise@4k@utilhi\endcsname{.989}
\expandafter\def\csname res@llama@stepwise@4k@utilklo\endcsname{.979}
\expandafter\def\csname res@llama@stepwise@4k@utilkhi\endcsname{1.006}
\expandafter\def\csname res@llama@syncpool@4k@bpt\endcsname{0.49}
\expandafter\def\csname res@llama@syncpool@4k@util\endcsname{.131}
\expandafter\def\csname res@llama@syncpool@4k@utilpct\endcsname{13.1}
\expandafter\def\csname res@llama@syncpool@4k@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@4k@klkappa\endcsname{2.190}
\expandafter\def\csname res@llama@syncpool@4k@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@4k@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@4k@utilk\endcsname{.134}
\expandafter\def\csname res@llama@syncpool@4k@bptlo\endcsname{0.44}
\expandafter\def\csname res@llama@syncpool@4k@bpthi\endcsname{0.56}
\expandafter\def\csname res@llama@syncpool@4k@utillo\endcsname{.118}
\expandafter\def\csname res@llama@syncpool@4k@utilhi\endcsname{.146}
\expandafter\def\csname res@llama@syncpool@4k@utilklo\endcsname{.120}
\expandafter\def\csname res@llama@syncpool@4k@utilkhi\endcsname{.148}
\expandafter\def\csname res@llama@coin@4k@bpt\endcsname{3.35}
\expandafter\def\csname res@llama@coin@4k@util\endcsname{.891}
\expandafter\def\csname res@llama@coin@4k@utilpct\endcsname{89.1}
\expandafter\def\csname res@llama@coin@4k@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@4k@klkappa\endcsname{0.223}
\expandafter\def\csname res@llama@coin@4k@n\endcsname{100}
\expandafter\def\csname res@llama@coin@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@4k@err\endcsname{0}
\expandafter\def\csname res@llama@coin@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@4k@utilk\endcsname{.907}
\expandafter\def\csname res@llama@coin@4k@bptlo\endcsname{3.16}
\expandafter\def\csname res@llama@coin@4k@bpthi\endcsname{3.53}
\expandafter\def\csname res@llama@coin@4k@utillo\endcsname{.878}
\expandafter\def\csname res@llama@coin@4k@utilhi\endcsname{.904}
\expandafter\def\csname res@llama@coin@4k@utilklo\endcsname{.894}
\expandafter\def\csname res@llama@coin@4k@utilkhi\endcsname{.920}
\expandafter\def\csname res@llama@hubdrop@4k@bpt\endcsname{3.04}
\expandafter\def\csname res@llama@hubdrop@4k@util\endcsname{.810}
\expandafter\def\csname res@llama@hubdrop@4k@utilpct\endcsname{81.0}
\expandafter\def\csname res@llama@hubdrop@4k@kl\endcsname{.0066}
\expandafter\def\csname res@llama@hubdrop@4k@klkappa\endcsname{0.411}
\expandafter\def\csname res@llama@hubdrop@4k@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@4k@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@4k@utilk\endcsname{.825}
\expandafter\def\csname res@llama@hubdrop@4k@bptlo\endcsname{2.84}
\expandafter\def\csname res@llama@hubdrop@4k@bpthi\endcsname{3.23}
\expandafter\def\csname res@llama@hubdrop@4k@utillo\endcsname{.784}
\expandafter\def\csname res@llama@hubdrop@4k@utilhi\endcsname{.833}
\expandafter\def\csname res@llama@hubdrop@4k@utilklo\endcsname{.800}
\expandafter\def\csname res@llama@hubdrop@4k@utilkhi\endcsname{.847}
\expandafter\def\csname res@llama@native@Full@bpt\endcsname{3.79}
\expandafter\def\csname res@llama@native@Full@util\endcsname{.985}
\expandafter\def\csname res@llama@native@Full@utilpct\endcsname{98.5}
\expandafter\def\csname res@llama@native@Full@kl\endcsname{0}
\expandafter\def\csname res@llama@native@Full@klkappa\endcsname{0.000}
\expandafter\def\csname res@llama@native@Full@n\endcsname{100}
\expandafter\def\csname res@llama@native@Full@tested\endcsname{100}
\expandafter\def\csname res@llama@native@Full@err\endcsname{4}
\expandafter\def\csname res@llama@native@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@native@Full@utilk\endcsname{.985}
\expandafter\def\csname res@llama@native@Full@bptlo\endcsname{3.56}
\expandafter\def\csname res@llama@native@Full@bpthi\endcsname{4.00}
\expandafter\def\csname res@llama@native@Full@utillo\endcsname{.972}
\expandafter\def\csname res@llama@native@Full@utilhi\endcsname{.999}
\expandafter\def\csname res@llama@native@Full@utilklo\endcsname{.972}
\expandafter\def\csname res@llama@native@Full@utilkhi\endcsname{.999}
\expandafter\def\csname res@llama@mwis@Full@bpt\endcsname{3.24}
\expandafter\def\csname res@llama@mwis@Full@util\endcsname{.897}
\expandafter\def\csname res@llama@mwis@Full@utilpct\endcsname{89.7}
\expandafter\def\csname res@llama@mwis@Full@kl\endcsname{.088}
\expandafter\def\csname res@llama@mwis@Full@klkappa\endcsname{0.088}
\expandafter\def\csname res@llama@mwis@Full@n\endcsname{100}
\expandafter\def\csname res@llama@mwis@Full@tested\endcsname{20}
\expandafter\def\csname res@llama@mwis@Full@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@Full@utilk\endcsname{.897}
\expandafter\def\csname res@llama@mwis@Full@bptlo\endcsname{3.03}
\expandafter\def\csname res@llama@mwis@Full@bpthi\endcsname{3.45}
\expandafter\def\csname res@llama@mwis@Full@utillo\endcsname{.882}
\expandafter\def\csname res@llama@mwis@Full@utilhi\endcsname{.912}
\expandafter\def\csname res@llama@mwis@Full@utilklo\endcsname{.882}
\expandafter\def\csname res@llama@mwis@Full@utilkhi\endcsname{.912}
\expandafter\def\csname res@llama@syncpool@Full@bpt\endcsname{0.52}
\expandafter\def\csname res@llama@syncpool@Full@util\endcsname{.133}
\expandafter\def\csname res@llama@syncpool@Full@utilpct\endcsname{13.3}
\expandafter\def\csname res@llama@syncpool@Full@kl\endcsname{0}
\expandafter\def\csname res@llama@syncpool@Full@klkappa\endcsname{2.326}
\expandafter\def\csname res@llama@syncpool@Full@n\endcsname{100}
\expandafter\def\csname res@llama@syncpool@Full@tested\endcsname{20}
\expandafter\def\csname res@llama@syncpool@Full@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@Full@utilk\endcsname{.133}
\expandafter\def\csname res@llama@syncpool@Full@bptlo\endcsname{0.45}
\expandafter\def\csname res@llama@syncpool@Full@bpthi\endcsname{0.59}
\expandafter\def\csname res@llama@syncpool@Full@utillo\endcsname{.119}
\expandafter\def\csname res@llama@syncpool@Full@utilhi\endcsname{.149}
\expandafter\def\csname res@llama@syncpool@Full@utilklo\endcsname{.119}
\expandafter\def\csname res@llama@syncpool@Full@utilkhi\endcsname{.149}
\expandafter\def\csname res@llama@coin@Full@bpt\endcsname{3.52}
\expandafter\def\csname res@llama@coin@Full@util\endcsname{.910}
\expandafter\def\csname res@llama@coin@Full@utilpct\endcsname{91.0}
\expandafter\def\csname res@llama@coin@Full@kl\endcsname{0}
\expandafter\def\csname res@llama@coin@Full@klkappa\endcsname{0.243}
\expandafter\def\csname res@llama@coin@Full@n\endcsname{100}
\expandafter\def\csname res@llama@coin@Full@tested\endcsname{20}
\expandafter\def\csname res@llama@coin@Full@err\endcsname{0}
\expandafter\def\csname res@llama@coin@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@Full@utilk\endcsname{.910}
\expandafter\def\csname res@llama@coin@Full@bptlo\endcsname{3.32}
\expandafter\def\csname res@llama@coin@Full@bpthi\endcsname{3.73}
\expandafter\def\csname res@llama@coin@Full@utillo\endcsname{.898}
\expandafter\def\csname res@llama@coin@Full@utilhi\endcsname{.923}
\expandafter\def\csname res@llama@coin@Full@utilklo\endcsname{.898}
\expandafter\def\csname res@llama@coin@Full@utilkhi\endcsname{.923}
\expandafter\def\csname res@llama@hubdrop@Full@bpt\endcsname{3.20}
\expandafter\def\csname res@llama@hubdrop@Full@util\endcsname{.832}
\expandafter\def\csname res@llama@hubdrop@Full@utilpct\endcsname{83.2}
\expandafter\def\csname res@llama@hubdrop@Full@kl\endcsname{.0073}
\expandafter\def\csname res@llama@hubdrop@Full@klkappa\endcsname{0.442}
\expandafter\def\csname res@llama@hubdrop@Full@n\endcsname{100}
\expandafter\def\csname res@llama@hubdrop@Full@tested\endcsname{20}
\expandafter\def\csname res@llama@hubdrop@Full@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@Full@utilk\endcsname{.832}
\expandafter\def\csname res@llama@hubdrop@Full@bptlo\endcsname{2.99}
\expandafter\def\csname res@llama@hubdrop@Full@bpthi\endcsname{3.38}
\expandafter\def\csname res@llama@hubdrop@Full@utillo\endcsname{.809}
\expandafter\def\csname res@llama@hubdrop@Full@utilhi\endcsname{.852}
\expandafter\def\csname res@llama@hubdrop@Full@utilklo\endcsname{.809}
\expandafter\def\csname res@llama@hubdrop@Full@utilkhi\endcsname{.852}
\expandafter\def\csname res@llama@las@16@bpt\endcsname{1.98}
\expandafter\def\csname res@llama@las@16@util\endcsname{.631}
\expandafter\def\csname res@llama@las@16@utilpct\endcsname{63.1}
\expandafter\def\csname res@llama@las@16@kl\endcsname{0}
\expandafter\def\csname res@llama@las@16@n\endcsname{100}
\expandafter\def\csname res@llama@las@16@tested\endcsname{20}
\expandafter\def\csname res@llama@las@16@err\endcsname{0}
\expandafter\def\csname res@llama@las@16@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@16@utilk\endcsname{.973}
\expandafter\def\csname res@llama@las@16@bptlo\endcsname{1.85}
\expandafter\def\csname res@llama@las@16@bpthi\endcsname{2.10}
\expandafter\def\csname res@llama@las@16@utillo\endcsname{.617}
\expandafter\def\csname res@llama@las@16@utilhi\endcsname{.646}
\expandafter\def\csname res@llama@las@16@utilklo\endcsname{.958}
\expandafter\def\csname res@llama@las@16@utilkhi\endcsname{.986}
\expandafter\def\csname res@llama@las@64@bpt\endcsname{2.68}
\expandafter\def\csname res@llama@las@64@util\endcsname{.785}
\expandafter\def\csname res@llama@las@64@utilpct\endcsname{78.5}
\expandafter\def\csname res@llama@las@64@kl\endcsname{0}
\expandafter\def\csname res@llama@las@64@n\endcsname{100}
\expandafter\def\csname res@llama@las@64@tested\endcsname{20}
\expandafter\def\csname res@llama@las@64@err\endcsname{0}
\expandafter\def\csname res@llama@las@64@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@64@utilk\endcsname{.982}
\expandafter\def\csname res@llama@las@64@bptlo\endcsname{2.51}
\expandafter\def\csname res@llama@las@64@bpthi\endcsname{2.82}
\expandafter\def\csname res@llama@las@64@utillo\endcsname{.772}
\expandafter\def\csname res@llama@las@64@utilhi\endcsname{.798}
\expandafter\def\csname res@llama@las@64@utilklo\endcsname{.968}
\expandafter\def\csname res@llama@las@64@utilkhi\endcsname{.995}
\expandafter\def\csname res@llama@las@256@bpt\endcsname{3.12}
\expandafter\def\csname res@llama@las@256@util\endcsname{.885}
\expandafter\def\csname res@llama@las@256@utilpct\endcsname{88.5}
\expandafter\def\csname res@llama@las@256@kl\endcsname{0}
\expandafter\def\csname res@llama@las@256@n\endcsname{100}
\expandafter\def\csname res@llama@las@256@tested\endcsname{20}
\expandafter\def\csname res@llama@las@256@err\endcsname{0}
\expandafter\def\csname res@llama@las@256@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@256@utilk\endcsname{.984}
\expandafter\def\csname res@llama@las@256@bptlo\endcsname{2.94}
\expandafter\def\csname res@llama@las@256@bpthi\endcsname{3.30}
\expandafter\def\csname res@llama@las@256@utillo\endcsname{.872}
\expandafter\def\csname res@llama@las@256@utilhi\endcsname{.899}
\expandafter\def\csname res@llama@las@256@utilklo\endcsname{.969}
\expandafter\def\csname res@llama@las@256@utilkhi\endcsname{1.000}
\expandafter\def\csname res@llama@las@1k@bpt\endcsname{3.44}
\expandafter\def\csname res@llama@las@1k@util\endcsname{.923}
\expandafter\def\csname res@llama@las@1k@utilpct\endcsname{92.3}
\expandafter\def\csname res@llama@las@1k@kl\endcsname{0}
\expandafter\def\csname res@llama@las@1k@n\endcsname{100}
\expandafter\def\csname res@llama@las@1k@tested\endcsname{20}
\expandafter\def\csname res@llama@las@1k@err\endcsname{0}
\expandafter\def\csname res@llama@las@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@1k@utilk\endcsname{.975}
\expandafter\def\csname res@llama@las@1k@bptlo\endcsname{3.23}
\expandafter\def\csname res@llama@las@1k@bpthi\endcsname{3.63}
\expandafter\def\csname res@llama@las@1k@utillo\endcsname{.909}
\expandafter\def\csname res@llama@las@1k@utilhi\endcsname{.937}
\expandafter\def\csname res@llama@las@1k@utilklo\endcsname{.959}
\expandafter\def\csname res@llama@las@1k@utilkhi\endcsname{.990}
\expandafter\def\csname res@llama@las@4k@bpt\endcsname{3.71}
\expandafter\def\csname res@llama@las@4k@util\endcsname{.979}
\expandafter\def\csname res@llama@las@4k@utilpct\endcsname{97.9}
\expandafter\def\csname res@llama@las@4k@kl\endcsname{0}
\expandafter\def\csname res@llama@las@4k@n\endcsname{100}
\expandafter\def\csname res@llama@las@4k@tested\endcsname{20}
\expandafter\def\csname res@llama@las@4k@err\endcsname{0}
\expandafter\def\csname res@llama@las@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@4k@utilk\endcsname{.998}
\expandafter\def\csname res@llama@las@4k@bptlo\endcsname{3.46}
\expandafter\def\csname res@llama@las@4k@bpthi\endcsname{3.94}
\expandafter\def\csname res@llama@las@4k@utillo\endcsname{.966}
\expandafter\def\csname res@llama@las@4k@utilhi\endcsname{.993}
\expandafter\def\csname res@llama@las@4k@utilklo\endcsname{.984}
\expandafter\def\csname res@llama@las@4k@utilkhi\endcsname{1.012}
\expandafter\def\csname res@llama@las@Full@bpt\endcsname{3.79}
\expandafter\def\csname res@llama@las@Full@util\endcsname{.979}
\expandafter\def\csname res@llama@las@Full@utilpct\endcsname{97.9}
\expandafter\def\csname res@llama@las@Full@kl\endcsname{0}
\expandafter\def\csname res@llama@las@Full@n\endcsname{100}
\expandafter\def\csname res@llama@las@Full@tested\endcsname{20}
\expandafter\def\csname res@llama@las@Full@err\endcsname{0}
\expandafter\def\csname res@llama@las@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@Full@utilk\endcsname{.979}
\expandafter\def\csname res@llama@las@Full@bptlo\endcsname{3.54}
\expandafter\def\csname res@llama@las@Full@bpthi\endcsname{4.05}
\expandafter\def\csname res@llama@las@Full@utillo\endcsname{.965}
\expandafter\def\csname res@llama@las@Full@utilhi\endcsname{.994}
\expandafter\def\csname res@llama@las@Full@utilklo\endcsname{.965}
\expandafter\def\csname res@llama@las@Full@utilkhi\endcsname{.994}
\expandafter\def\csname res@llama@native@all@err\endcsname{23}
\expandafter\def\csname res@llama@native@all@tested\endcsname{600}
\expandafter\def\csname res@llama@native@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@basic@all@err\endcsname{0}
\expandafter\def\csname res@llama@basic@all@tested\endcsname{100}
\expandafter\def\csname res@llama@basic@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@mwis@all@err\endcsname{0}
\expandafter\def\csname res@llama@mwis@all@tested\endcsname{120}
\expandafter\def\csname res@llama@mwis@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@stepwise@all@err\endcsname{0}
\expandafter\def\csname res@llama@stepwise@all@tested\endcsname{100}
\expandafter\def\csname res@llama@stepwise@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@all@err\endcsname{0}
\expandafter\def\csname res@llama@hubdrop@all@tested\endcsname{120}
\expandafter\def\csname res@llama@hubdrop@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@syncpool@all@err\endcsname{0}
\expandafter\def\csname res@llama@syncpool@all@tested\endcsname{120}
\expandafter\def\csname res@llama@syncpool@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@all@err\endcsname{0}
\expandafter\def\csname res@llama@las@all@tested\endcsname{120}
\expandafter\def\csname res@llama@las@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@coin@all@err\endcsname{0}
\expandafter\def\csname res@llama@coin@all@tested\endcsname{120}
\expandafter\def\csname res@llama@coin@all@incomplete\endcsname{0}
\expandafter\def\csname res@llama@las@Full@utilgap\endcsname{7.0}
\expandafter\def\csname res@llama@native@all@oop\endcsname{2}
\expandafter\def\csname res@llama@native@all@prompt\endcsname{0}
\expandafter\def\csname res@llama@native@Full@silent\endcsname{4}
\expandafter\def\csname res@llama@gain@16@meas\endcsname{1.16}
\expandafter\def\csname res@llama@coin@16@utilvsH\endcsname{59}
\expandafter\def\csname res@llama@gain@16@pred\endcsname{1.14}
\expandafter\def\csname res@llama@gain@16@predtraj\endcsname{1.15}
\expandafter\def\csname res@llama@gain@16@lo\endcsname{1.12}
\expandafter\def\csname res@llama@gain@16@hi\endcsname{1.20}
\expandafter\def\csname res@llama@gain@64@meas\endcsname{1.59}
\expandafter\def\csname res@llama@coin@64@utilvsH\endcsname{73}
\expandafter\def\csname res@llama@gain@64@pred\endcsname{1.68}
\expandafter\def\csname res@llama@gain@64@predtraj\endcsname{1.54}
\expandafter\def\csname res@llama@gain@64@lo\endcsname{1.50}
\expandafter\def\csname res@llama@gain@64@hi\endcsname{1.68}
\expandafter\def\csname res@llama@gain@256@meas\endcsname{3.37}
\expandafter\def\csname res@llama@coin@256@utilvsH\endcsname{81}
\expandafter\def\csname res@llama@gain@256@pred\endcsname{3.16}
\expandafter\def\csname res@llama@gain@256@predtraj\endcsname{3.21}
\expandafter\def\csname res@llama@gain@256@lo\endcsname{3.12}
\expandafter\def\csname res@llama@gain@256@hi\endcsname{3.64}
\expandafter\def\csname res@llama@gain@1k@meas\endcsname{6.20}
\expandafter\def\csname res@llama@coin@1k@utilvsH\endcsname{86}
\expandafter\def\csname res@llama@gain@1k@pred\endcsname{6.43}
\expandafter\def\csname res@llama@gain@1k@predtraj\endcsname{5.86}
\expandafter\def\csname res@llama@gain@1k@lo\endcsname{5.43}
\expandafter\def\csname res@llama@gain@1k@hi\endcsname{7.08}
\expandafter\def\csname res@llama@gain@4k@meas\endcsname{6.80}
\expandafter\def\csname res@llama@coin@4k@utilvsH\endcsname{89}
\expandafter\def\csname res@llama@gain@4k@pred\endcsname{6.20}
\expandafter\def\csname res@llama@gain@4k@predtraj\endcsname{6.08}
\expandafter\def\csname res@llama@gain@4k@lo\endcsname{6.07}
\expandafter\def\csname res@llama@gain@4k@hi\endcsname{7.57}
\expandafter\def\csname res@llama@gain@Full@meas\endcsname{6.83}
\expandafter\def\csname res@llama@coin@Full@utilvsH\endcsname{91}
\expandafter\def\csname res@llama@gain@Full@pred\endcsname{6.41}
\expandafter\def\csname res@llama@gain@Full@predtraj\endcsname{6.26}
\expandafter\def\csname res@llama@gain@Full@lo\endcsname{6.06}
\expandafter\def\csname res@llama@gain@Full@hi\endcsname{7.66}
\expandafter\def\csname res@qwen@native@all@recovered\endcsname{0}
\expandafter\def\csname res@qwen@native@all@bndtot\endcsname{0}
\expandafter\def\csname res@qwen@native@all@silent\endcsname{56}
\expandafter\def\csname res@qwen@ratio@16@native\endcsname{0.92}
\expandafter\def\csname res@qwen@ratio@64@native\endcsname{0.90}
\expandafter\def\csname res@qwen@ratio@256@native\endcsname{0.93}
\expandafter\def\csname res@qwen@ratio@1k@native\endcsname{0.92}
\expandafter\def\csname res@qwen@ratio@4k@native\endcsname{0.92}
\expandafter\def\csname res@qwen@ratio@Full@native\endcsname{0.93}
\expandafter\def\csname res@qwen@ratio@16@stepwise\endcsname{0.94}
\expandafter\def\csname res@qwen@ratio@64@stepwise\endcsname{0.92}
\expandafter\def\csname res@qwen@ratio@256@stepwise\endcsname{0.93}
\expandafter\def\csname res@qwen@ratio@1k@stepwise\endcsname{0.92}
\expandafter\def\csname res@qwen@ratio@4k@stepwise\endcsname{0.92}
\expandafter\def\csname res@qwen@native@16@bpt\endcsname{1.73}
\expandafter\def\csname res@qwen@native@16@util\endcsname{.628}
\expandafter\def\csname res@qwen@native@16@utilpct\endcsname{62.8}
\expandafter\def\csname res@qwen@native@16@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@16@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@16@n\endcsname{100}
\expandafter\def\csname res@qwen@native@16@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@16@err\endcsname{3}
\expandafter\def\csname res@qwen@native@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@16@utilk\endcsname{.993}
\expandafter\def\csname res@qwen@native@16@bptlo\endcsname{1.62}
\expandafter\def\csname res@qwen@native@16@bpthi\endcsname{1.83}
\expandafter\def\csname res@qwen@native@16@utillo\endcsname{.612}
\expandafter\def\csname res@qwen@native@16@utilhi\endcsname{.645}
\expandafter\def\csname res@qwen@native@16@utilklo\endcsname{.979}
\expandafter\def\csname res@qwen@native@16@utilkhi\endcsname{1.008}
\expandafter\def\csname res@qwen@basic@16@bpt\endcsname{1.95}
\expandafter\def\csname res@qwen@basic@16@util\endcsname{.616}
\expandafter\def\csname res@qwen@basic@16@utilpct\endcsname{61.6}
\expandafter\def\csname res@qwen@basic@16@kl\endcsname{.612}
\expandafter\def\csname res@qwen@basic@16@klkappa\endcsname{0.612}
\expandafter\def\csname res@qwen@basic@16@n\endcsname{100}
\expandafter\def\csname res@qwen@basic@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@basic@16@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@basic@16@utilk\endcsname{1.012}
\expandafter\def\csname res@qwen@basic@16@bptlo\endcsname{1.85}
\expandafter\def\csname res@qwen@basic@16@bpthi\endcsname{2.04}
\expandafter\def\csname res@qwen@basic@16@utillo\endcsname{.600}
\expandafter\def\csname res@qwen@basic@16@utilhi\endcsname{.632}
\expandafter\def\csname res@qwen@basic@16@utilklo\endcsname{.994}
\expandafter\def\csname res@qwen@basic@16@utilkhi\endcsname{1.029}
\expandafter\def\csname res@qwen@mwis@16@bpt\endcsname{1.47}
\expandafter\def\csname res@qwen@mwis@16@util\endcsname{.563}
\expandafter\def\csname res@qwen@mwis@16@utilpct\endcsname{56.3}
\expandafter\def\csname res@qwen@mwis@16@kl\endcsname{.049}
\expandafter\def\csname res@qwen@mwis@16@klkappa\endcsname{0.049}
\expandafter\def\csname res@qwen@mwis@16@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@16@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@16@utilk\endcsname{.888}
\expandafter\def\csname res@qwen@mwis@16@bptlo\endcsname{1.37}
\expandafter\def\csname res@qwen@mwis@16@bpthi\endcsname{1.56}
\expandafter\def\csname res@qwen@mwis@16@utillo\endcsname{.548}
\expandafter\def\csname res@qwen@mwis@16@utilhi\endcsname{.577}
\expandafter\def\csname res@qwen@mwis@16@utilklo\endcsname{.872}
\expandafter\def\csname res@qwen@mwis@16@utilkhi\endcsname{.903}
\expandafter\def\csname res@qwen@stepwise@16@bpt\endcsname{1.74}
\expandafter\def\csname res@qwen@stepwise@16@util\endcsname{.613}
\expandafter\def\csname res@qwen@stepwise@16@utilpct\endcsname{61.3}
\expandafter\def\csname res@qwen@stepwise@16@kl\endcsname{.026}
\expandafter\def\csname res@qwen@stepwise@16@klkappa\endcsname{0.026}
\expandafter\def\csname res@qwen@stepwise@16@n\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@stepwise@16@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@16@utilk\endcsname{.975}
\expandafter\def\csname res@qwen@stepwise@16@bptlo\endcsname{1.64}
\expandafter\def\csname res@qwen@stepwise@16@bpthi\endcsname{1.83}
\expandafter\def\csname res@qwen@stepwise@16@utillo\endcsname{.599}
\expandafter\def\csname res@qwen@stepwise@16@utilhi\endcsname{.628}
\expandafter\def\csname res@qwen@stepwise@16@utilklo\endcsname{.962}
\expandafter\def\csname res@qwen@stepwise@16@utilkhi\endcsname{.989}
\expandafter\def\csname res@qwen@syncpool@16@bpt\endcsname{1.47}
\expandafter\def\csname res@qwen@syncpool@16@util\endcsname{.552}
\expandafter\def\csname res@qwen@syncpool@16@utilpct\endcsname{55.2}
\expandafter\def\csname res@qwen@syncpool@16@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@16@klkappa\endcsname{0.148}
\expandafter\def\csname res@qwen@syncpool@16@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@16@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@16@utilk\endcsname{.861}
\expandafter\def\csname res@qwen@syncpool@16@bptlo\endcsname{1.37}
\expandafter\def\csname res@qwen@syncpool@16@bpthi\endcsname{1.56}
\expandafter\def\csname res@qwen@syncpool@16@utillo\endcsname{.537}
\expandafter\def\csname res@qwen@syncpool@16@utilhi\endcsname{.569}
\expandafter\def\csname res@qwen@syncpool@16@utilklo\endcsname{.843}
\expandafter\def\csname res@qwen@syncpool@16@utilkhi\endcsname{.878}
\expandafter\def\csname res@qwen@coin@16@bpt\endcsname{1.58}
\expandafter\def\csname res@qwen@coin@16@util\endcsname{.577}
\expandafter\def\csname res@qwen@coin@16@utilpct\endcsname{57.7}
\expandafter\def\csname res@qwen@coin@16@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@16@klkappa\endcsname{0.108}
\expandafter\def\csname res@qwen@coin@16@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@16@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@16@utilk\endcsname{.894}
\expandafter\def\csname res@qwen@coin@16@bptlo\endcsname{1.48}
\expandafter\def\csname res@qwen@coin@16@bpthi\endcsname{1.67}
\expandafter\def\csname res@qwen@coin@16@utillo\endcsname{.561}
\expandafter\def\csname res@qwen@coin@16@utilhi\endcsname{.593}
\expandafter\def\csname res@qwen@coin@16@utilklo\endcsname{.875}
\expandafter\def\csname res@qwen@coin@16@utilkhi\endcsname{.912}
\expandafter\def\csname res@qwen@hubdrop@16@bpt\endcsname{1.44}
\expandafter\def\csname res@qwen@hubdrop@16@util\endcsname{.540}
\expandafter\def\csname res@qwen@hubdrop@16@utilpct\endcsname{54.0}
\expandafter\def\csname res@qwen@hubdrop@16@kl\endcsname{.0011}
\expandafter\def\csname res@qwen@hubdrop@16@klkappa\endcsname{0.130}
\expandafter\def\csname res@qwen@hubdrop@16@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@16@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@16@utilk\endcsname{.867}
\expandafter\def\csname res@qwen@hubdrop@16@bptlo\endcsname{1.34}
\expandafter\def\csname res@qwen@hubdrop@16@bpthi\endcsname{1.54}
\expandafter\def\csname res@qwen@hubdrop@16@utillo\endcsname{.526}
\expandafter\def\csname res@qwen@hubdrop@16@utilhi\endcsname{.556}
\expandafter\def\csname res@qwen@hubdrop@16@utilklo\endcsname{.849}
\expandafter\def\csname res@qwen@hubdrop@16@utilkhi\endcsname{.885}
\expandafter\def\csname res@qwen@native@64@bpt\endcsname{2.28}
\expandafter\def\csname res@qwen@native@64@util\endcsname{.764}
\expandafter\def\csname res@qwen@native@64@utilpct\endcsname{76.4}
\expandafter\def\csname res@qwen@native@64@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@64@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@64@n\endcsname{100}
\expandafter\def\csname res@qwen@native@64@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@64@err\endcsname{4}
\expandafter\def\csname res@qwen@native@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@64@utilk\endcsname{.984}
\expandafter\def\csname res@qwen@native@64@bptlo\endcsname{2.13}
\expandafter\def\csname res@qwen@native@64@bpthi\endcsname{2.41}
\expandafter\def\csname res@qwen@native@64@utillo\endcsname{.751}
\expandafter\def\csname res@qwen@native@64@utilhi\endcsname{.780}
\expandafter\def\csname res@qwen@native@64@utilklo\endcsname{.971}
\expandafter\def\csname res@qwen@native@64@utilkhi\endcsname{.997}
\expandafter\def\csname res@qwen@basic@64@bpt\endcsname{3.12}
\expandafter\def\csname res@qwen@basic@64@util\endcsname{.805}
\expandafter\def\csname res@qwen@basic@64@utilpct\endcsname{80.5}
\expandafter\def\csname res@qwen@basic@64@kl\endcsname{.739}
\expandafter\def\csname res@qwen@basic@64@klkappa\endcsname{0.739}
\expandafter\def\csname res@qwen@basic@64@n\endcsname{100}
\expandafter\def\csname res@qwen@basic@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@basic@64@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@basic@64@utilk\endcsname{1.086}
\expandafter\def\csname res@qwen@basic@64@bptlo\endcsname{2.99}
\expandafter\def\csname res@qwen@basic@64@bpthi\endcsname{3.24}
\expandafter\def\csname res@qwen@basic@64@utillo\endcsname{.792}
\expandafter\def\csname res@qwen@basic@64@utilhi\endcsname{.818}
\expandafter\def\csname res@qwen@basic@64@utilklo\endcsname{1.068}
\expandafter\def\csname res@qwen@basic@64@utilkhi\endcsname{1.103}
\expandafter\def\csname res@qwen@mwis@64@bpt\endcsname{2.09}
\expandafter\def\csname res@qwen@mwis@64@util\endcsname{.696}
\expandafter\def\csname res@qwen@mwis@64@utilpct\endcsname{69.6}
\expandafter\def\csname res@qwen@mwis@64@kl\endcsname{.059}
\expandafter\def\csname res@qwen@mwis@64@klkappa\endcsname{0.059}
\expandafter\def\csname res@qwen@mwis@64@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@64@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@64@utilk\endcsname{.907}
\expandafter\def\csname res@qwen@mwis@64@bptlo\endcsname{1.94}
\expandafter\def\csname res@qwen@mwis@64@bpthi\endcsname{2.23}
\expandafter\def\csname res@qwen@mwis@64@utillo\endcsname{.682}
\expandafter\def\csname res@qwen@mwis@64@utilhi\endcsname{.709}
\expandafter\def\csname res@qwen@mwis@64@utilklo\endcsname{.893}
\expandafter\def\csname res@qwen@mwis@64@utilkhi\endcsname{.922}
\expandafter\def\csname res@qwen@stepwise@64@bpt\endcsname{2.41}
\expandafter\def\csname res@qwen@stepwise@64@util\endcsname{.750}
\expandafter\def\csname res@qwen@stepwise@64@utilpct\endcsname{75.0}
\expandafter\def\csname res@qwen@stepwise@64@kl\endcsname{.021}
\expandafter\def\csname res@qwen@stepwise@64@klkappa\endcsname{0.021}
\expandafter\def\csname res@qwen@stepwise@64@n\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@stepwise@64@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@64@utilk\endcsname{.977}
\expandafter\def\csname res@qwen@stepwise@64@bptlo\endcsname{2.28}
\expandafter\def\csname res@qwen@stepwise@64@bpthi\endcsname{2.55}
\expandafter\def\csname res@qwen@stepwise@64@utillo\endcsname{.735}
\expandafter\def\csname res@qwen@stepwise@64@utilhi\endcsname{.764}
\expandafter\def\csname res@qwen@stepwise@64@utilklo\endcsname{.961}
\expandafter\def\csname res@qwen@stepwise@64@utilkhi\endcsname{.992}
\expandafter\def\csname res@qwen@syncpool@64@bpt\endcsname{2.05}
\expandafter\def\csname res@qwen@syncpool@64@util\endcsname{.664}
\expandafter\def\csname res@qwen@syncpool@64@utilpct\endcsname{66.4}
\expandafter\def\csname res@qwen@syncpool@64@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@64@klkappa\endcsname{0.216}
\expandafter\def\csname res@qwen@syncpool@64@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@64@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@64@utilk\endcsname{.860}
\expandafter\def\csname res@qwen@syncpool@64@bptlo\endcsname{1.91}
\expandafter\def\csname res@qwen@syncpool@64@bpthi\endcsname{2.17}
\expandafter\def\csname res@qwen@syncpool@64@utillo\endcsname{.649}
\expandafter\def\csname res@qwen@syncpool@64@utilhi\endcsname{.679}
\expandafter\def\csname res@qwen@syncpool@64@utilklo\endcsname{.842}
\expandafter\def\csname res@qwen@syncpool@64@utilkhi\endcsname{.877}
\expandafter\def\csname res@qwen@coin@64@bpt\endcsname{2.18}
\expandafter\def\csname res@qwen@coin@64@util\endcsname{.690}
\expandafter\def\csname res@qwen@coin@64@utilpct\endcsname{69.0}
\expandafter\def\csname res@qwen@coin@64@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@64@klkappa\endcsname{0.143}
\expandafter\def\csname res@qwen@coin@64@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@64@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@64@utilk\endcsname{.895}
\expandafter\def\csname res@qwen@coin@64@bptlo\endcsname{2.04}
\expandafter\def\csname res@qwen@coin@64@bpthi\endcsname{2.31}
\expandafter\def\csname res@qwen@coin@64@utillo\endcsname{.677}
\expandafter\def\csname res@qwen@coin@64@utilhi\endcsname{.704}
\expandafter\def\csname res@qwen@coin@64@utilklo\endcsname{.880}
\expandafter\def\csname res@qwen@coin@64@utilkhi\endcsname{.911}
\expandafter\def\csname res@qwen@hubdrop@64@bpt\endcsname{1.98}
\expandafter\def\csname res@qwen@hubdrop@64@util\endcsname{.675}
\expandafter\def\csname res@qwen@hubdrop@64@utilpct\endcsname{67.5}
\expandafter\def\csname res@qwen@hubdrop@64@kl\endcsname{.0016}
\expandafter\def\csname res@qwen@hubdrop@64@klkappa\endcsname{0.182}
\expandafter\def\csname res@qwen@hubdrop@64@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@64@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@64@utilk\endcsname{.866}
\expandafter\def\csname res@qwen@hubdrop@64@bptlo\endcsname{1.84}
\expandafter\def\csname res@qwen@hubdrop@64@bpthi\endcsname{2.11}
\expandafter\def\csname res@qwen@hubdrop@64@utillo\endcsname{.662}
\expandafter\def\csname res@qwen@hubdrop@64@utilhi\endcsname{.688}
\expandafter\def\csname res@qwen@hubdrop@64@utilklo\endcsname{.852}
\expandafter\def\csname res@qwen@hubdrop@64@utilkhi\endcsname{.880}
\expandafter\def\csname res@qwen@native@256@bpt\endcsname{2.85}
\expandafter\def\csname res@qwen@native@256@util\endcsname{.857}
\expandafter\def\csname res@qwen@native@256@utilpct\endcsname{85.7}
\expandafter\def\csname res@qwen@native@256@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@256@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@256@n\endcsname{100}
\expandafter\def\csname res@qwen@native@256@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@256@err\endcsname{12}
\expandafter\def\csname res@qwen@native@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@256@utilk\endcsname{.983}
\expandafter\def\csname res@qwen@native@256@bptlo\endcsname{2.65}
\expandafter\def\csname res@qwen@native@256@bpthi\endcsname{3.06}
\expandafter\def\csname res@qwen@native@256@utillo\endcsname{.845}
\expandafter\def\csname res@qwen@native@256@utilhi\endcsname{.870}
\expandafter\def\csname res@qwen@native@256@utilklo\endcsname{.969}
\expandafter\def\csname res@qwen@native@256@utilkhi\endcsname{.997}
\expandafter\def\csname res@qwen@basic@256@bpt\endcsname{3.98}
\expandafter\def\csname res@qwen@basic@256@util\endcsname{.903}
\expandafter\def\csname res@qwen@basic@256@utilpct\endcsname{90.3}
\expandafter\def\csname res@qwen@basic@256@kl\endcsname{.841}
\expandafter\def\csname res@qwen@basic@256@klkappa\endcsname{0.841}
\expandafter\def\csname res@qwen@basic@256@n\endcsname{100}
\expandafter\def\csname res@qwen@basic@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@basic@256@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@basic@256@utilk\endcsname{1.086}
\expandafter\def\csname res@qwen@basic@256@bptlo\endcsname{3.80}
\expandafter\def\csname res@qwen@basic@256@bpthi\endcsname{4.15}
\expandafter\def\csname res@qwen@basic@256@utillo\endcsname{.890}
\expandafter\def\csname res@qwen@basic@256@utilhi\endcsname{.915}
\expandafter\def\csname res@qwen@basic@256@utilklo\endcsname{1.069}
\expandafter\def\csname res@qwen@basic@256@utilkhi\endcsname{1.103}
\expandafter\def\csname res@qwen@mwis@256@bpt\endcsname{2.49}
\expandafter\def\csname res@qwen@mwis@256@util\endcsname{.790}
\expandafter\def\csname res@qwen@mwis@256@utilpct\endcsname{79.0}
\expandafter\def\csname res@qwen@mwis@256@kl\endcsname{.070}
\expandafter\def\csname res@qwen@mwis@256@klkappa\endcsname{0.070}
\expandafter\def\csname res@qwen@mwis@256@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@256@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@256@utilk\endcsname{.907}
\expandafter\def\csname res@qwen@mwis@256@bptlo\endcsname{2.33}
\expandafter\def\csname res@qwen@mwis@256@bpthi\endcsname{2.66}
\expandafter\def\csname res@qwen@mwis@256@utillo\endcsname{.778}
\expandafter\def\csname res@qwen@mwis@256@utilhi\endcsname{.802}
\expandafter\def\csname res@qwen@mwis@256@utilklo\endcsname{.893}
\expandafter\def\csname res@qwen@mwis@256@utilkhi\endcsname{.921}
\expandafter\def\csname res@qwen@stepwise@256@bpt\endcsname{2.94}
\expandafter\def\csname res@qwen@stepwise@256@util\endcsname{.857}
\expandafter\def\csname res@qwen@stepwise@256@utilpct\endcsname{85.7}
\expandafter\def\csname res@qwen@stepwise@256@kl\endcsname{.029}
\expandafter\def\csname res@qwen@stepwise@256@klkappa\endcsname{0.029}
\expandafter\def\csname res@qwen@stepwise@256@n\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@stepwise@256@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@256@utilk\endcsname{.982}
\expandafter\def\csname res@qwen@stepwise@256@bptlo\endcsname{2.78}
\expandafter\def\csname res@qwen@stepwise@256@bpthi\endcsname{3.09}
\expandafter\def\csname res@qwen@stepwise@256@utillo\endcsname{.844}
\expandafter\def\csname res@qwen@stepwise@256@utilhi\endcsname{.871}
\expandafter\def\csname res@qwen@stepwise@256@utilklo\endcsname{.969}
\expandafter\def\csname res@qwen@stepwise@256@utilkhi\endcsname{.996}
\expandafter\def\csname res@qwen@syncpool@256@bpt\endcsname{2.55}
\expandafter\def\csname res@qwen@syncpool@256@util\endcsname{.734}
\expandafter\def\csname res@qwen@syncpool@256@utilpct\endcsname{73.4}
\expandafter\def\csname res@qwen@syncpool@256@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@256@klkappa\endcsname{0.316}
\expandafter\def\csname res@qwen@syncpool@256@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@256@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@256@utilk\endcsname{.844}
\expandafter\def\csname res@qwen@syncpool@256@bptlo\endcsname{2.39}
\expandafter\def\csname res@qwen@syncpool@256@bpthi\endcsname{2.71}
\expandafter\def\csname res@qwen@syncpool@256@utillo\endcsname{.720}
\expandafter\def\csname res@qwen@syncpool@256@utilhi\endcsname{.747}
\expandafter\def\csname res@qwen@syncpool@256@utilklo\endcsname{.828}
\expandafter\def\csname res@qwen@syncpool@256@utilkhi\endcsname{.860}
\expandafter\def\csname res@qwen@coin@256@bpt\endcsname{2.68}
\expandafter\def\csname res@qwen@coin@256@util\endcsname{.801}
\expandafter\def\csname res@qwen@coin@256@utilpct\endcsname{80.1}
\expandafter\def\csname res@qwen@coin@256@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@256@klkappa\endcsname{0.169}
\expandafter\def\csname res@qwen@coin@256@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@256@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@256@utilk\endcsname{.919}
\expandafter\def\csname res@qwen@coin@256@bptlo\endcsname{2.51}
\expandafter\def\csname res@qwen@coin@256@bpthi\endcsname{2.84}
\expandafter\def\csname res@qwen@coin@256@utillo\endcsname{.790}
\expandafter\def\csname res@qwen@coin@256@utilhi\endcsname{.812}
\expandafter\def\csname res@qwen@coin@256@utilklo\endcsname{.905}
\expandafter\def\csname res@qwen@coin@256@utilkhi\endcsname{.932}
\expandafter\def\csname res@qwen@hubdrop@256@bpt\endcsname{2.52}
\expandafter\def\csname res@qwen@hubdrop@256@util\endcsname{.749}
\expandafter\def\csname res@qwen@hubdrop@256@utilpct\endcsname{74.9}
\expandafter\def\csname res@qwen@hubdrop@256@kl\endcsname{.0021}
\expandafter\def\csname res@qwen@hubdrop@256@klkappa\endcsname{0.241}
\expandafter\def\csname res@qwen@hubdrop@256@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@256@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@256@utilk\endcsname{.861}
\expandafter\def\csname res@qwen@hubdrop@256@bptlo\endcsname{2.36}
\expandafter\def\csname res@qwen@hubdrop@256@bpthi\endcsname{2.67}
\expandafter\def\csname res@qwen@hubdrop@256@utillo\endcsname{.735}
\expandafter\def\csname res@qwen@hubdrop@256@utilhi\endcsname{.763}
\expandafter\def\csname res@qwen@hubdrop@256@utilklo\endcsname{.845}
\expandafter\def\csname res@qwen@hubdrop@256@utilkhi\endcsname{.876}
\expandafter\def\csname res@qwen@native@1k@bpt\endcsname{3.32}
\expandafter\def\csname res@qwen@native@1k@util\endcsname{.937}
\expandafter\def\csname res@qwen@native@1k@utilpct\endcsname{93.7}
\expandafter\def\csname res@qwen@native@1k@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@1k@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@native@1k@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@1k@err\endcsname{16}
\expandafter\def\csname res@qwen@native@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@1k@utilk\endcsname{.996}
\expandafter\def\csname res@qwen@native@1k@bptlo\endcsname{3.11}
\expandafter\def\csname res@qwen@native@1k@bpthi\endcsname{3.54}
\expandafter\def\csname res@qwen@native@1k@utillo\endcsname{.926}
\expandafter\def\csname res@qwen@native@1k@utilhi\endcsname{.949}
\expandafter\def\csname res@qwen@native@1k@utilklo\endcsname{.983}
\expandafter\def\csname res@qwen@native@1k@utilkhi\endcsname{1.009}
\expandafter\def\csname res@qwen@basic@1k@bpt\endcsname{4.78}
\expandafter\def\csname res@qwen@basic@1k@util\endcsname{.930}
\expandafter\def\csname res@qwen@basic@1k@utilpct\endcsname{93.0}
\expandafter\def\csname res@qwen@basic@1k@kl\endcsname{.792}
\expandafter\def\csname res@qwen@basic@1k@klkappa\endcsname{0.792}
\expandafter\def\csname res@qwen@basic@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@basic@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@basic@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@1k@incomplete\endcsname{1}
\expandafter\def\csname res@qwen@basic@1k@utilk\endcsname{1.029}
\expandafter\def\csname res@qwen@basic@1k@bptlo\endcsname{4.48}
\expandafter\def\csname res@qwen@basic@1k@bpthi\endcsname{5.07}
\expandafter\def\csname res@qwen@basic@1k@utillo\endcsname{.887}
\expandafter\def\csname res@qwen@basic@1k@utilhi\endcsname{.960}
\expandafter\def\csname res@qwen@basic@1k@utilklo\endcsname{.981}
\expandafter\def\csname res@qwen@basic@1k@utilkhi\endcsname{1.061}
\expandafter\def\csname res@qwen@mwis@1k@bpt\endcsname{2.86}
\expandafter\def\csname res@qwen@mwis@1k@util\endcsname{.846}
\expandafter\def\csname res@qwen@mwis@1k@utilpct\endcsname{84.6}
\expandafter\def\csname res@qwen@mwis@1k@kl\endcsname{.082}
\expandafter\def\csname res@qwen@mwis@1k@klkappa\endcsname{0.082}
\expandafter\def\csname res@qwen@mwis@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@1k@utilk\endcsname{.900}
\expandafter\def\csname res@qwen@mwis@1k@bptlo\endcsname{2.63}
\expandafter\def\csname res@qwen@mwis@1k@bpthi\endcsname{3.09}
\expandafter\def\csname res@qwen@mwis@1k@utillo\endcsname{.832}
\expandafter\def\csname res@qwen@mwis@1k@utilhi\endcsname{.859}
\expandafter\def\csname res@qwen@mwis@1k@utilklo\endcsname{.884}
\expandafter\def\csname res@qwen@mwis@1k@utilkhi\endcsname{.914}
\expandafter\def\csname res@qwen@stepwise@1k@bpt\endcsname{3.43}
\expandafter\def\csname res@qwen@stepwise@1k@util\endcsname{.934}
\expandafter\def\csname res@qwen@stepwise@1k@utilpct\endcsname{93.4}
\expandafter\def\csname res@qwen@stepwise@1k@kl\endcsname{.024}
\expandafter\def\csname res@qwen@stepwise@1k@klkappa\endcsname{0.024}
\expandafter\def\csname res@qwen@stepwise@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@stepwise@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@1k@utilk\endcsname{.993}
\expandafter\def\csname res@qwen@stepwise@1k@bptlo\endcsname{3.23}
\expandafter\def\csname res@qwen@stepwise@1k@bpthi\endcsname{3.65}
\expandafter\def\csname res@qwen@stepwise@1k@utillo\endcsname{.920}
\expandafter\def\csname res@qwen@stepwise@1k@utilhi\endcsname{.947}
\expandafter\def\csname res@qwen@stepwise@1k@utilklo\endcsname{.978}
\expandafter\def\csname res@qwen@stepwise@1k@utilkhi\endcsname{1.008}
\expandafter\def\csname res@qwen@syncpool@1k@bpt\endcsname{2.86}
\expandafter\def\csname res@qwen@syncpool@1k@util\endcsname{.788}
\expandafter\def\csname res@qwen@syncpool@1k@utilpct\endcsname{78.8}
\expandafter\def\csname res@qwen@syncpool@1k@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@1k@klkappa\endcsname{0.395}
\expandafter\def\csname res@qwen@syncpool@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@1k@utilk\endcsname{.840}
\expandafter\def\csname res@qwen@syncpool@1k@bptlo\endcsname{2.65}
\expandafter\def\csname res@qwen@syncpool@1k@bpthi\endcsname{3.07}
\expandafter\def\csname res@qwen@syncpool@1k@utillo\endcsname{.771}
\expandafter\def\csname res@qwen@syncpool@1k@utilhi\endcsname{.803}
\expandafter\def\csname res@qwen@syncpool@1k@utilklo\endcsname{.821}
\expandafter\def\csname res@qwen@syncpool@1k@utilkhi\endcsname{.857}
\expandafter\def\csname res@qwen@coin@1k@bpt\endcsname{3.09}
\expandafter\def\csname res@qwen@coin@1k@util\endcsname{.862}
\expandafter\def\csname res@qwen@coin@1k@utilpct\endcsname{86.2}
\expandafter\def\csname res@qwen@coin@1k@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@1k@klkappa\endcsname{0.186}
\expandafter\def\csname res@qwen@coin@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@1k@utilk\endcsname{.919}
\expandafter\def\csname res@qwen@coin@1k@bptlo\endcsname{2.87}
\expandafter\def\csname res@qwen@coin@1k@bpthi\endcsname{3.30}
\expandafter\def\csname res@qwen@coin@1k@utillo\endcsname{.850}
\expandafter\def\csname res@qwen@coin@1k@utilhi\endcsname{.875}
\expandafter\def\csname res@qwen@coin@1k@utilklo\endcsname{.906}
\expandafter\def\csname res@qwen@coin@1k@utilkhi\endcsname{.933}
\expandafter\def\csname res@qwen@hubdrop@1k@bpt\endcsname{2.74}
\expandafter\def\csname res@qwen@hubdrop@1k@util\endcsname{.811}
\expandafter\def\csname res@qwen@hubdrop@1k@utilpct\endcsname{81.1}
\expandafter\def\csname res@qwen@hubdrop@1k@kl\endcsname{.0024}
\expandafter\def\csname res@qwen@hubdrop@1k@klkappa\endcsname{0.279}
\expandafter\def\csname res@qwen@hubdrop@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@1k@utilk\endcsname{.860}
\expandafter\def\csname res@qwen@hubdrop@1k@bptlo\endcsname{2.56}
\expandafter\def\csname res@qwen@hubdrop@1k@bpthi\endcsname{2.92}
\expandafter\def\csname res@qwen@hubdrop@1k@utillo\endcsname{.798}
\expandafter\def\csname res@qwen@hubdrop@1k@utilhi\endcsname{.823}
\expandafter\def\csname res@qwen@hubdrop@1k@utilklo\endcsname{.846}
\expandafter\def\csname res@qwen@hubdrop@1k@utilkhi\endcsname{.873}
\expandafter\def\csname res@qwen@native@4k@bpt\endcsname{3.76}
\expandafter\def\csname res@qwen@native@4k@util\endcsname{.969}
\expandafter\def\csname res@qwen@native@4k@utilpct\endcsname{96.9}
\expandafter\def\csname res@qwen@native@4k@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@4k@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@native@4k@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@4k@err\endcsname{16}
\expandafter\def\csname res@qwen@native@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@4k@utilk\endcsname{.990}
\expandafter\def\csname res@qwen@native@4k@bptlo\endcsname{3.49}
\expandafter\def\csname res@qwen@native@4k@bpthi\endcsname{4.04}
\expandafter\def\csname res@qwen@native@4k@utillo\endcsname{.957}
\expandafter\def\csname res@qwen@native@4k@utilhi\endcsname{.981}
\expandafter\def\csname res@qwen@native@4k@utilklo\endcsname{.976}
\expandafter\def\csname res@qwen@native@4k@utilkhi\endcsname{1.003}
\expandafter\def\csname res@qwen@basic@4k@bpt\endcsname{4.70}
\expandafter\def\csname res@qwen@basic@4k@util\endcsname{.951}
\expandafter\def\csname res@qwen@basic@4k@utilpct\endcsname{95.1}
\expandafter\def\csname res@qwen@basic@4k@kl\endcsname{.811}
\expandafter\def\csname res@qwen@basic@4k@klkappa\endcsname{0.811}
\expandafter\def\csname res@qwen@basic@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@basic@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@basic@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@4k@incomplete\endcsname{1}
\expandafter\def\csname res@qwen@basic@4k@utilk\endcsname{.988}
\expandafter\def\csname res@qwen@basic@4k@bptlo\endcsname{4.35}
\expandafter\def\csname res@qwen@basic@4k@bpthi\endcsname{5.04}
\expandafter\def\csname res@qwen@basic@4k@utillo\endcsname{.904}
\expandafter\def\csname res@qwen@basic@4k@utilhi\endcsname{.982}
\expandafter\def\csname res@qwen@basic@4k@utilklo\endcsname{.940}
\expandafter\def\csname res@qwen@basic@4k@utilkhi\endcsname{1.020}
\expandafter\def\csname res@qwen@mwis@4k@bpt\endcsname{3.07}
\expandafter\def\csname res@qwen@mwis@4k@util\endcsname{.879}
\expandafter\def\csname res@qwen@mwis@4k@utilpct\endcsname{87.9}
\expandafter\def\csname res@qwen@mwis@4k@kl\endcsname{.086}
\expandafter\def\csname res@qwen@mwis@4k@klkappa\endcsname{0.086}
\expandafter\def\csname res@qwen@mwis@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@4k@utilk\endcsname{.897}
\expandafter\def\csname res@qwen@mwis@4k@bptlo\endcsname{2.82}
\expandafter\def\csname res@qwen@mwis@4k@bpthi\endcsname{3.33}
\expandafter\def\csname res@qwen@mwis@4k@utillo\endcsname{.865}
\expandafter\def\csname res@qwen@mwis@4k@utilhi\endcsname{.894}
\expandafter\def\csname res@qwen@mwis@4k@utilklo\endcsname{.881}
\expandafter\def\csname res@qwen@mwis@4k@utilkhi\endcsname{.912}
\expandafter\def\csname res@qwen@stepwise@4k@bpt\endcsname{3.97}
\expandafter\def\csname res@qwen@stepwise@4k@util\endcsname{.973}
\expandafter\def\csname res@qwen@stepwise@4k@utilpct\endcsname{97.3}
\expandafter\def\csname res@qwen@stepwise@4k@kl\endcsname{.022}
\expandafter\def\csname res@qwen@stepwise@4k@klkappa\endcsname{0.022}
\expandafter\def\csname res@qwen@stepwise@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@stepwise@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@4k@utilk\endcsname{.994}
\expandafter\def\csname res@qwen@stepwise@4k@bptlo\endcsname{3.67}
\expandafter\def\csname res@qwen@stepwise@4k@bpthi\endcsname{4.29}
\expandafter\def\csname res@qwen@stepwise@4k@utillo\endcsname{.961}
\expandafter\def\csname res@qwen@stepwise@4k@utilhi\endcsname{.984}
\expandafter\def\csname res@qwen@stepwise@4k@utilklo\endcsname{.981}
\expandafter\def\csname res@qwen@stepwise@4k@utilkhi\endcsname{1.006}
\expandafter\def\csname res@qwen@syncpool@4k@bpt\endcsname{2.99}
\expandafter\def\csname res@qwen@syncpool@4k@util\endcsname{.767}
\expandafter\def\csname res@qwen@syncpool@4k@utilpct\endcsname{76.7}
\expandafter\def\csname res@qwen@syncpool@4k@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@4k@klkappa\endcsname{0.583}
\expandafter\def\csname res@qwen@syncpool@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@4k@utilk\endcsname{.783}
\expandafter\def\csname res@qwen@syncpool@4k@bptlo\endcsname{2.76}
\expandafter\def\csname res@qwen@syncpool@4k@bpthi\endcsname{3.21}
\expandafter\def\csname res@qwen@syncpool@4k@utillo\endcsname{.744}
\expandafter\def\csname res@qwen@syncpool@4k@utilhi\endcsname{.787}
\expandafter\def\csname res@qwen@syncpool@4k@utilklo\endcsname{.759}
\expandafter\def\csname res@qwen@syncpool@4k@utilkhi\endcsname{.804}
\expandafter\def\csname res@qwen@coin@4k@bpt\endcsname{3.40}
\expandafter\def\csname res@qwen@coin@4k@util\endcsname{.891}
\expandafter\def\csname res@qwen@coin@4k@utilpct\endcsname{89.1}
\expandafter\def\csname res@qwen@coin@4k@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@4k@klkappa\endcsname{0.205}
\expandafter\def\csname res@qwen@coin@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@4k@utilk\endcsname{.909}
\expandafter\def\csname res@qwen@coin@4k@bptlo\endcsname{3.13}
\expandafter\def\csname res@qwen@coin@4k@bpthi\endcsname{3.68}
\expandafter\def\csname res@qwen@coin@4k@utillo\endcsname{.878}
\expandafter\def\csname res@qwen@coin@4k@utilhi\endcsname{.903}
\expandafter\def\csname res@qwen@coin@4k@utilklo\endcsname{.895}
\expandafter\def\csname res@qwen@coin@4k@utilkhi\endcsname{.923}
\expandafter\def\csname res@qwen@hubdrop@4k@bpt\endcsname{3.26}
\expandafter\def\csname res@qwen@hubdrop@4k@util\endcsname{.840}
\expandafter\def\csname res@qwen@hubdrop@4k@utilpct\endcsname{84.0}
\expandafter\def\csname res@qwen@hubdrop@4k@kl\endcsname{.0028}
\expandafter\def\csname res@qwen@hubdrop@4k@klkappa\endcsname{0.359}
\expandafter\def\csname res@qwen@hubdrop@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@4k@utilk\endcsname{.858}
\expandafter\def\csname res@qwen@hubdrop@4k@bptlo\endcsname{3.01}
\expandafter\def\csname res@qwen@hubdrop@4k@bpthi\endcsname{3.48}
\expandafter\def\csname res@qwen@hubdrop@4k@utillo\endcsname{.828}
\expandafter\def\csname res@qwen@hubdrop@4k@utilhi\endcsname{.853}
\expandafter\def\csname res@qwen@hubdrop@4k@utilklo\endcsname{.844}
\expandafter\def\csname res@qwen@hubdrop@4k@utilkhi\endcsname{.871}
\expandafter\def\csname res@qwen@native@Full@bpt\endcsname{4.05}
\expandafter\def\csname res@qwen@native@Full@util\endcsname{.992}
\expandafter\def\csname res@qwen@native@Full@utilpct\endcsname{99.2}
\expandafter\def\csname res@qwen@native@Full@kl\endcsname{0}
\expandafter\def\csname res@qwen@native@Full@klkappa\endcsname{0.000}
\expandafter\def\csname res@qwen@native@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@native@Full@tested\endcsname{100}
\expandafter\def\csname res@qwen@native@Full@err\endcsname{16}
\expandafter\def\csname res@qwen@native@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@native@Full@utilk\endcsname{.992}
\expandafter\def\csname res@qwen@native@Full@bptlo\endcsname{3.73}
\expandafter\def\csname res@qwen@native@Full@bpthi\endcsname{4.36}
\expandafter\def\csname res@qwen@native@Full@utillo\endcsname{.979}
\expandafter\def\csname res@qwen@native@Full@utilhi\endcsname{1.004}
\expandafter\def\csname res@qwen@native@Full@utilklo\endcsname{.979}
\expandafter\def\csname res@qwen@native@Full@utilkhi\endcsname{1.004}
\expandafter\def\csname res@qwen@mwis@Full@bpt\endcsname{3.23}
\expandafter\def\csname res@qwen@mwis@Full@util\endcsname{.892}
\expandafter\def\csname res@qwen@mwis@Full@utilpct\endcsname{89.2}
\expandafter\def\csname res@qwen@mwis@Full@kl\endcsname{.091}
\expandafter\def\csname res@qwen@mwis@Full@klkappa\endcsname{0.091}
\expandafter\def\csname res@qwen@mwis@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@mwis@Full@tested\endcsname{20}
\expandafter\def\csname res@qwen@mwis@Full@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@mwis@Full@utilk\endcsname{.892}
\expandafter\def\csname res@qwen@mwis@Full@bptlo\endcsname{2.96}
\expandafter\def\csname res@qwen@mwis@Full@bpthi\endcsname{3.50}
\expandafter\def\csname res@qwen@mwis@Full@utillo\endcsname{.879}
\expandafter\def\csname res@qwen@mwis@Full@utilhi\endcsname{.906}
\expandafter\def\csname res@qwen@mwis@Full@utilklo\endcsname{.879}
\expandafter\def\csname res@qwen@mwis@Full@utilkhi\endcsname{.906}
\expandafter\def\csname res@qwen@syncpool@Full@bpt\endcsname{1.63}
\expandafter\def\csname res@qwen@syncpool@Full@util\endcsname{.423}
\expandafter\def\csname res@qwen@syncpool@Full@utilpct\endcsname{42.3}
\expandafter\def\csname res@qwen@syncpool@Full@kl\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@Full@klkappa\endcsname{1.522}
\expandafter\def\csname res@qwen@syncpool@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@syncpool@Full@tested\endcsname{20}
\expandafter\def\csname res@qwen@syncpool@Full@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@Full@utilk\endcsname{.423}
\expandafter\def\csname res@qwen@syncpool@Full@bptlo\endcsname{1.53}
\expandafter\def\csname res@qwen@syncpool@Full@bpthi\endcsname{1.73}
\expandafter\def\csname res@qwen@syncpool@Full@utillo\endcsname{.409}
\expandafter\def\csname res@qwen@syncpool@Full@utilhi\endcsname{.437}
\expandafter\def\csname res@qwen@syncpool@Full@utilklo\endcsname{.409}
\expandafter\def\csname res@qwen@syncpool@Full@utilkhi\endcsname{.437}
\expandafter\def\csname res@qwen@coin@Full@bpt\endcsname{3.85}
\expandafter\def\csname res@qwen@coin@Full@util\endcsname{.923}
\expandafter\def\csname res@qwen@coin@Full@utilpct\endcsname{92.3}
\expandafter\def\csname res@qwen@coin@Full@kl\endcsname{0}
\expandafter\def\csname res@qwen@coin@Full@klkappa\endcsname{0.231}
\expandafter\def\csname res@qwen@coin@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@coin@Full@tested\endcsname{20}
\expandafter\def\csname res@qwen@coin@Full@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@Full@utilk\endcsname{.923}
\expandafter\def\csname res@qwen@coin@Full@bptlo\endcsname{3.54}
\expandafter\def\csname res@qwen@coin@Full@bpthi\endcsname{4.16}
\expandafter\def\csname res@qwen@coin@Full@utillo\endcsname{.909}
\expandafter\def\csname res@qwen@coin@Full@utilhi\endcsname{.936}
\expandafter\def\csname res@qwen@coin@Full@utilklo\endcsname{.909}
\expandafter\def\csname res@qwen@coin@Full@utilkhi\endcsname{.936}
\expandafter\def\csname res@qwen@hubdrop@Full@bpt\endcsname{3.25}
\expandafter\def\csname res@qwen@hubdrop@Full@util\endcsname{.844}
\expandafter\def\csname res@qwen@hubdrop@Full@utilpct\endcsname{84.4}
\expandafter\def\csname res@qwen@hubdrop@Full@kl\endcsname{.0029}
\expandafter\def\csname res@qwen@hubdrop@Full@klkappa\endcsname{0.378}
\expandafter\def\csname res@qwen@hubdrop@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@hubdrop@Full@tested\endcsname{20}
\expandafter\def\csname res@qwen@hubdrop@Full@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@Full@utilk\endcsname{.844}
\expandafter\def\csname res@qwen@hubdrop@Full@bptlo\endcsname{3.01}
\expandafter\def\csname res@qwen@hubdrop@Full@bpthi\endcsname{3.53}
\expandafter\def\csname res@qwen@hubdrop@Full@utillo\endcsname{.828}
\expandafter\def\csname res@qwen@hubdrop@Full@utilhi\endcsname{.859}
\expandafter\def\csname res@qwen@hubdrop@Full@utilklo\endcsname{.828}
\expandafter\def\csname res@qwen@hubdrop@Full@utilkhi\endcsname{.859}
\expandafter\def\csname res@qwen@las@16@bpt\endcsname{1.67}
\expandafter\def\csname res@qwen@las@16@util\endcsname{.620}
\expandafter\def\csname res@qwen@las@16@utilpct\endcsname{62.0}
\expandafter\def\csname res@qwen@las@16@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@16@n\endcsname{100}
\expandafter\def\csname res@qwen@las@16@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@16@err\endcsname{0}
\expandafter\def\csname res@qwen@las@16@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@16@utilk\endcsname{.979}
\expandafter\def\csname res@qwen@las@16@bptlo\endcsname{1.57}
\expandafter\def\csname res@qwen@las@16@bpthi\endcsname{1.77}
\expandafter\def\csname res@qwen@las@16@utillo\endcsname{.606}
\expandafter\def\csname res@qwen@las@16@utilhi\endcsname{.635}
\expandafter\def\csname res@qwen@las@16@utilklo\endcsname{.963}
\expandafter\def\csname res@qwen@las@16@utilkhi\endcsname{.994}
\expandafter\def\csname res@qwen@las@64@bpt\endcsname{2.31}
\expandafter\def\csname res@qwen@las@64@util\endcsname{.758}
\expandafter\def\csname res@qwen@las@64@utilpct\endcsname{75.8}
\expandafter\def\csname res@qwen@las@64@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@64@n\endcsname{100}
\expandafter\def\csname res@qwen@las@64@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@64@err\endcsname{0}
\expandafter\def\csname res@qwen@las@64@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@64@utilk\endcsname{.973}
\expandafter\def\csname res@qwen@las@64@bptlo\endcsname{2.17}
\expandafter\def\csname res@qwen@las@64@bpthi\endcsname{2.46}
\expandafter\def\csname res@qwen@las@64@utillo\endcsname{.745}
\expandafter\def\csname res@qwen@las@64@utilhi\endcsname{.770}
\expandafter\def\csname res@qwen@las@64@utilklo\endcsname{.958}
\expandafter\def\csname res@qwen@las@64@utilkhi\endcsname{.986}
\expandafter\def\csname res@qwen@las@256@bpt\endcsname{2.85}
\expandafter\def\csname res@qwen@las@256@util\endcsname{.850}
\expandafter\def\csname res@qwen@las@256@utilpct\endcsname{85.0}
\expandafter\def\csname res@qwen@las@256@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@256@n\endcsname{100}
\expandafter\def\csname res@qwen@las@256@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@256@err\endcsname{0}
\expandafter\def\csname res@qwen@las@256@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@256@utilk\endcsname{.977}
\expandafter\def\csname res@qwen@las@256@bptlo\endcsname{2.67}
\expandafter\def\csname res@qwen@las@256@bpthi\endcsname{3.03}
\expandafter\def\csname res@qwen@las@256@utillo\endcsname{.838}
\expandafter\def\csname res@qwen@las@256@utilhi\endcsname{.862}
\expandafter\def\csname res@qwen@las@256@utilklo\endcsname{.964}
\expandafter\def\csname res@qwen@las@256@utilkhi\endcsname{.990}
\expandafter\def\csname res@qwen@las@1k@bpt\endcsname{3.34}
\expandafter\def\csname res@qwen@las@1k@util\endcsname{.932}
\expandafter\def\csname res@qwen@las@1k@utilpct\endcsname{93.2}
\expandafter\def\csname res@qwen@las@1k@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@1k@n\endcsname{100}
\expandafter\def\csname res@qwen@las@1k@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@1k@err\endcsname{0}
\expandafter\def\csname res@qwen@las@1k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@1k@utilk\endcsname{.995}
\expandafter\def\csname res@qwen@las@1k@bptlo\endcsname{3.11}
\expandafter\def\csname res@qwen@las@1k@bpthi\endcsname{3.58}
\expandafter\def\csname res@qwen@las@1k@utillo\endcsname{.919}
\expandafter\def\csname res@qwen@las@1k@utilhi\endcsname{.945}
\expandafter\def\csname res@qwen@las@1k@utilklo\endcsname{.981}
\expandafter\def\csname res@qwen@las@1k@utilkhi\endcsname{1.010}
\expandafter\def\csname res@qwen@las@4k@bpt\endcsname{3.79}
\expandafter\def\csname res@qwen@las@4k@util\endcsname{.967}
\expandafter\def\csname res@qwen@las@4k@utilpct\endcsname{96.7}
\expandafter\def\csname res@qwen@las@4k@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@4k@n\endcsname{100}
\expandafter\def\csname res@qwen@las@4k@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@4k@err\endcsname{0}
\expandafter\def\csname res@qwen@las@4k@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@4k@utilk\endcsname{.987}
\expandafter\def\csname res@qwen@las@4k@bptlo\endcsname{3.49}
\expandafter\def\csname res@qwen@las@4k@bpthi\endcsname{4.09}
\expandafter\def\csname res@qwen@las@4k@utillo\endcsname{.954}
\expandafter\def\csname res@qwen@las@4k@utilhi\endcsname{.980}
\expandafter\def\csname res@qwen@las@4k@utilklo\endcsname{.973}
\expandafter\def\csname res@qwen@las@4k@utilkhi\endcsname{1.001}
\expandafter\def\csname res@qwen@las@Full@bpt\endcsname{4.02}
\expandafter\def\csname res@qwen@las@Full@util\endcsname{.983}
\expandafter\def\csname res@qwen@las@Full@utilpct\endcsname{98.3}
\expandafter\def\csname res@qwen@las@Full@kl\endcsname{0}
\expandafter\def\csname res@qwen@las@Full@n\endcsname{100}
\expandafter\def\csname res@qwen@las@Full@tested\endcsname{20}
\expandafter\def\csname res@qwen@las@Full@err\endcsname{0}
\expandafter\def\csname res@qwen@las@Full@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@Full@utilk\endcsname{.983}
\expandafter\def\csname res@qwen@las@Full@bptlo\endcsname{3.72}
\expandafter\def\csname res@qwen@las@Full@bpthi\endcsname{4.32}
\expandafter\def\csname res@qwen@las@Full@utillo\endcsname{.970}
\expandafter\def\csname res@qwen@las@Full@utilhi\endcsname{.995}
\expandafter\def\csname res@qwen@las@Full@utilklo\endcsname{.970}
\expandafter\def\csname res@qwen@las@Full@utilkhi\endcsname{.995}
\expandafter\def\csname res@qwen@native@all@err\endcsname{67}
\expandafter\def\csname res@qwen@native@all@tested\endcsname{600}
\expandafter\def\csname res@qwen@native@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@basic@all@err\endcsname{0}
\expandafter\def\csname res@qwen@basic@all@tested\endcsname{100}
\expandafter\def\csname res@qwen@basic@all@incomplete\endcsname{2}
\expandafter\def\csname res@qwen@mwis@all@err\endcsname{0}
\expandafter\def\csname res@qwen@mwis@all@tested\endcsname{120}
\expandafter\def\csname res@qwen@mwis@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@all@err\endcsname{0}
\expandafter\def\csname res@qwen@stepwise@all@tested\endcsname{100}
\expandafter\def\csname res@qwen@stepwise@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@all@err\endcsname{0}
\expandafter\def\csname res@qwen@hubdrop@all@tested\endcsname{120}
\expandafter\def\csname res@qwen@hubdrop@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@all@err\endcsname{0}
\expandafter\def\csname res@qwen@syncpool@all@tested\endcsname{120}
\expandafter\def\csname res@qwen@syncpool@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@all@err\endcsname{0}
\expandafter\def\csname res@qwen@las@all@tested\endcsname{120}
\expandafter\def\csname res@qwen@las@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@coin@all@err\endcsname{0}
\expandafter\def\csname res@qwen@coin@all@tested\endcsname{120}
\expandafter\def\csname res@qwen@coin@all@incomplete\endcsname{0}
\expandafter\def\csname res@qwen@las@Full@utilgap\endcsname{6.0}
\expandafter\def\csname res@qwen@native@all@oop\endcsname{11}
\expandafter\def\csname res@qwen@native@all@prompt\endcsname{0}
\expandafter\def\csname res@qwen@native@Full@silent\endcsname{16}
\expandafter\def\csname res@qwen@gain@16@meas\endcsname{1.04}
\expandafter\def\csname res@qwen@coin@16@utilvsH\endcsname{58}
\expandafter\def\csname res@qwen@gain@16@pred\endcsname{1.05}
\expandafter\def\csname res@qwen@gain@16@predtraj\endcsname{1.04}
\expandafter\def\csname res@qwen@gain@16@lo\endcsname{1.01}
\expandafter\def\csname res@qwen@gain@16@hi\endcsname{1.08}
\expandafter\def\csname res@qwen@gain@64@meas\endcsname{1.04}
\expandafter\def\csname res@qwen@coin@64@utilvsH\endcsname{69}
\expandafter\def\csname res@qwen@gain@64@pred\endcsname{1.07}
\expandafter\def\csname res@qwen@gain@64@predtraj\endcsname{1.06}
\expandafter\def\csname res@qwen@gain@64@lo\endcsname{1.01}
\expandafter\def\csname res@qwen@gain@64@hi\endcsname{1.07}
\expandafter\def\csname res@qwen@gain@256@meas\endcsname{1.09}
\expandafter\def\csname res@qwen@coin@256@utilvsH\endcsname{80}
\expandafter\def\csname res@qwen@gain@256@pred\endcsname{1.08}
\expandafter\def\csname res@qwen@gain@256@predtraj\endcsname{1.07}
\expandafter\def\csname res@qwen@gain@256@lo\endcsname{1.07}
\expandafter\def\csname res@qwen@gain@256@hi\endcsname{1.12}
\expandafter\def\csname res@qwen@gain@1k@meas\endcsname{1.09}
\expandafter\def\csname res@qwen@coin@1k@utilvsH\endcsname{86}
\expandafter\def\csname res@qwen@gain@1k@pred\endcsname{1.11}
\expandafter\def\csname res@qwen@gain@1k@predtraj\endcsname{1.10}
\expandafter\def\csname res@qwen@gain@1k@lo\endcsname{1.07}
\expandafter\def\csname res@qwen@gain@1k@hi\endcsname{1.12}
\expandafter\def\csname res@qwen@gain@4k@meas\endcsname{1.16}
\expandafter\def\csname res@qwen@coin@4k@utilvsH\endcsname{89}
\expandafter\def\csname res@qwen@gain@4k@pred\endcsname{1.16}
\expandafter\def\csname res@qwen@gain@4k@predtraj\endcsname{1.17}
\expandafter\def\csname res@qwen@gain@4k@lo\endcsname{1.13}
\expandafter\def\csname res@qwen@gain@4k@hi\endcsname{1.20}
\expandafter\def\csname res@qwen@gain@Full@meas\endcsname{2.18}
\expandafter\def\csname res@qwen@coin@Full@utilvsH\endcsname{92}
\expandafter\def\csname res@qwen@gain@Full@pred\endcsname{2.14}
\expandafter\def\csname res@qwen@gain@Full@predtraj\endcsname{2.16}
\expandafter\def\csname res@qwen@gain@Full@lo\endcsname{2.11}
\expandafter\def\csname res@qwen@gain@Full@hi\endcsname{2.25}
\expandafter\def\csname res@llmjp@native@all@recovered\endcsname{0}
\expandafter\def\csname res@llmjp@native@all@bndtot\endcsname{0}
\expandafter\def\csname res@llmjp@native@all@silent\endcsname{56}
\expandafter\def\csname res@llmjp@ratio@16@native\endcsname{0.90}
\expandafter\def\csname res@llmjp@ratio@64@native\endcsname{0.90}
\expandafter\def\csname res@llmjp@ratio@256@native\endcsname{0.93}
\expandafter\def\csname res@llmjp@ratio@1k@native\endcsname{0.92}
\expandafter\def\csname res@llmjp@ratio@4k@native\endcsname{0.92}
\expandafter\def\csname res@llmjp@ratio@Full@native\endcsname{0.93}
\expandafter\def\csname res@llmjp@ratio@16@stepwise\endcsname{0.92}
\expandafter\def\csname res@llmjp@ratio@64@stepwise\endcsname{0.90}
\expandafter\def\csname res@llmjp@ratio@256@stepwise\endcsname{0.94}
\expandafter\def\csname res@llmjp@ratio@1k@stepwise\endcsname{0.92}
\expandafter\def\csname res@llmjp@ratio@4k@stepwise\endcsname{0.91}
\expandafter\def\csname res@llmjp@native@16@bpt\endcsname{1.72}
\expandafter\def\csname res@llmjp@native@16@util\endcsname{.569}
\expandafter\def\csname res@llmjp@native@16@utilpct\endcsname{56.9}
\expandafter\def\csname res@llmjp@native@16@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@16@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@16@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@16@err\endcsname{7}
\expandafter\def\csname res@llmjp@native@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@16@utilk\endcsname{.989}
\expandafter\def\csname res@llmjp@native@16@bptlo\endcsname{1.62}
\expandafter\def\csname res@llmjp@native@16@bpthi\endcsname{1.81}
\expandafter\def\csname res@llmjp@native@16@utillo\endcsname{.554}
\expandafter\def\csname res@llmjp@native@16@utilhi\endcsname{.584}
\expandafter\def\csname res@llmjp@native@16@utilklo\endcsname{.974}
\expandafter\def\csname res@llmjp@native@16@utilkhi\endcsname{1.006}
\expandafter\def\csname res@llmjp@basic@16@bpt\endcsname{1.81}
\expandafter\def\csname res@llmjp@basic@16@util\endcsname{.560}
\expandafter\def\csname res@llmjp@basic@16@utilpct\endcsname{56.0}
\expandafter\def\csname res@llmjp@basic@16@kl\endcsname{.456}
\expandafter\def\csname res@llmjp@basic@16@klkappa\endcsname{0.456}
\expandafter\def\csname res@llmjp@basic@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@basic@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@basic@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@16@utilk\endcsname{.982}
\expandafter\def\csname res@llmjp@basic@16@bptlo\endcsname{1.71}
\expandafter\def\csname res@llmjp@basic@16@bpthi\endcsname{1.90}
\expandafter\def\csname res@llmjp@basic@16@utillo\endcsname{.544}
\expandafter\def\csname res@llmjp@basic@16@utilhi\endcsname{.577}
\expandafter\def\csname res@llmjp@basic@16@utilklo\endcsname{.964}
\expandafter\def\csname res@llmjp@basic@16@utilkhi\endcsname{1.000}
\expandafter\def\csname res@llmjp@mwis@16@bpt\endcsname{1.45}
\expandafter\def\csname res@llmjp@mwis@16@util\endcsname{.518}
\expandafter\def\csname res@llmjp@mwis@16@utilpct\endcsname{51.8}
\expandafter\def\csname res@llmjp@mwis@16@kl\endcsname{.045}
\expandafter\def\csname res@llmjp@mwis@16@klkappa\endcsname{0.045}
\expandafter\def\csname res@llmjp@mwis@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@16@utilk\endcsname{.885}
\expandafter\def\csname res@llmjp@mwis@16@bptlo\endcsname{1.35}
\expandafter\def\csname res@llmjp@mwis@16@bpthi\endcsname{1.54}
\expandafter\def\csname res@llmjp@mwis@16@utillo\endcsname{.505}
\expandafter\def\csname res@llmjp@mwis@16@utilhi\endcsname{.531}
\expandafter\def\csname res@llmjp@mwis@16@utilklo\endcsname{.869}
\expandafter\def\csname res@llmjp@mwis@16@utilkhi\endcsname{.900}
\expandafter\def\csname res@llmjp@stepwise@16@bpt\endcsname{1.65}
\expandafter\def\csname res@llmjp@stepwise@16@util\endcsname{.561}
\expandafter\def\csname res@llmjp@stepwise@16@utilpct\endcsname{56.1}
\expandafter\def\csname res@llmjp@stepwise@16@kl\endcsname{.0029}
\expandafter\def\csname res@llmjp@stepwise@16@klkappa\endcsname{0.003}
\expandafter\def\csname res@llmjp@stepwise@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@stepwise@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@16@utilk\endcsname{.975}
\expandafter\def\csname res@llmjp@stepwise@16@bptlo\endcsname{1.55}
\expandafter\def\csname res@llmjp@stepwise@16@bpthi\endcsname{1.75}
\expandafter\def\csname res@llmjp@stepwise@16@utillo\endcsname{.546}
\expandafter\def\csname res@llmjp@stepwise@16@utilhi\endcsname{.576}
\expandafter\def\csname res@llmjp@stepwise@16@utilklo\endcsname{.960}
\expandafter\def\csname res@llmjp@stepwise@16@utilkhi\endcsname{.991}
\expandafter\def\csname res@llmjp@syncpool@16@bpt\endcsname{1.39}
\expandafter\def\csname res@llmjp@syncpool@16@util\endcsname{.495}
\expandafter\def\csname res@llmjp@syncpool@16@utilpct\endcsname{49.5}
\expandafter\def\csname res@llmjp@syncpool@16@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@16@klkappa\endcsname{0.158}
\expandafter\def\csname res@llmjp@syncpool@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@16@utilk\endcsname{.846}
\expandafter\def\csname res@llmjp@syncpool@16@bptlo\endcsname{1.29}
\expandafter\def\csname res@llmjp@syncpool@16@bpthi\endcsname{1.48}
\expandafter\def\csname res@llmjp@syncpool@16@utillo\endcsname{.481}
\expandafter\def\csname res@llmjp@syncpool@16@utilhi\endcsname{.511}
\expandafter\def\csname res@llmjp@syncpool@16@utilklo\endcsname{.828}
\expandafter\def\csname res@llmjp@syncpool@16@utilkhi\endcsname{.863}
\expandafter\def\csname res@llmjp@coin@16@bpt\endcsname{1.52}
\expandafter\def\csname res@llmjp@coin@16@util\endcsname{.514}
\expandafter\def\csname res@llmjp@coin@16@utilpct\endcsname{51.4}
\expandafter\def\csname res@llmjp@coin@16@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@16@klkappa\endcsname{0.103}
\expandafter\def\csname res@llmjp@coin@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@16@utilk\endcsname{.884}
\expandafter\def\csname res@llmjp@coin@16@bptlo\endcsname{1.43}
\expandafter\def\csname res@llmjp@coin@16@bpthi\endcsname{1.60}
\expandafter\def\csname res@llmjp@coin@16@utillo\endcsname{.500}
\expandafter\def\csname res@llmjp@coin@16@utilhi\endcsname{.528}
\expandafter\def\csname res@llmjp@coin@16@utilklo\endcsname{.868}
\expandafter\def\csname res@llmjp@coin@16@utilkhi\endcsname{.899}
\expandafter\def\csname res@llmjp@hubdrop@16@bpt\endcsname{1.35}
\expandafter\def\csname res@llmjp@hubdrop@16@util\endcsname{.499}
\expandafter\def\csname res@llmjp@hubdrop@16@utilpct\endcsname{49.9}
\expandafter\def\csname res@llmjp@hubdrop@16@kl\endcsname{.0011}
\expandafter\def\csname res@llmjp@hubdrop@16@klkappa\endcsname{0.121}
\expandafter\def\csname res@llmjp@hubdrop@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@16@utilk\endcsname{.861}
\expandafter\def\csname res@llmjp@hubdrop@16@bptlo\endcsname{1.26}
\expandafter\def\csname res@llmjp@hubdrop@16@bpthi\endcsname{1.44}
\expandafter\def\csname res@llmjp@hubdrop@16@utillo\endcsname{.483}
\expandafter\def\csname res@llmjp@hubdrop@16@utilhi\endcsname{.514}
\expandafter\def\csname res@llmjp@hubdrop@16@utilklo\endcsname{.842}
\expandafter\def\csname res@llmjp@hubdrop@16@utilkhi\endcsname{.878}
\expandafter\def\csname res@llmjp@native@64@bpt\endcsname{2.36}
\expandafter\def\csname res@llmjp@native@64@util\endcsname{.737}
\expandafter\def\csname res@llmjp@native@64@utilpct\endcsname{73.7}
\expandafter\def\csname res@llmjp@native@64@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@64@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@64@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@64@err\endcsname{6}
\expandafter\def\csname res@llmjp@native@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@64@utilk\endcsname{.994}
\expandafter\def\csname res@llmjp@native@64@bptlo\endcsname{2.22}
\expandafter\def\csname res@llmjp@native@64@bpthi\endcsname{2.49}
\expandafter\def\csname res@llmjp@native@64@utillo\endcsname{.723}
\expandafter\def\csname res@llmjp@native@64@utilhi\endcsname{.753}
\expandafter\def\csname res@llmjp@native@64@utilklo\endcsname{.981}
\expandafter\def\csname res@llmjp@native@64@utilkhi\endcsname{1.008}
\expandafter\def\csname res@llmjp@basic@64@bpt\endcsname{2.77}
\expandafter\def\csname res@llmjp@basic@64@util\endcsname{.733}
\expandafter\def\csname res@llmjp@basic@64@utilpct\endcsname{73.3}
\expandafter\def\csname res@llmjp@basic@64@kl\endcsname{.596}
\expandafter\def\csname res@llmjp@basic@64@klkappa\endcsname{0.596}
\expandafter\def\csname res@llmjp@basic@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@basic@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@basic@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@64@utilk\endcsname{1.028}
\expandafter\def\csname res@llmjp@basic@64@bptlo\endcsname{2.65}
\expandafter\def\csname res@llmjp@basic@64@bpthi\endcsname{2.89}
\expandafter\def\csname res@llmjp@basic@64@utillo\endcsname{.718}
\expandafter\def\csname res@llmjp@basic@64@utilhi\endcsname{.748}
\expandafter\def\csname res@llmjp@basic@64@utilklo\endcsname{1.011}
\expandafter\def\csname res@llmjp@basic@64@utilkhi\endcsname{1.044}
\expandafter\def\csname res@llmjp@mwis@64@bpt\endcsname{2.10}
\expandafter\def\csname res@llmjp@mwis@64@util\endcsname{.676}
\expandafter\def\csname res@llmjp@mwis@64@utilpct\endcsname{67.6}
\expandafter\def\csname res@llmjp@mwis@64@kl\endcsname{.059}
\expandafter\def\csname res@llmjp@mwis@64@klkappa\endcsname{0.059}
\expandafter\def\csname res@llmjp@mwis@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@64@utilk\endcsname{.918}
\expandafter\def\csname res@llmjp@mwis@64@bptlo\endcsname{1.98}
\expandafter\def\csname res@llmjp@mwis@64@bpthi\endcsname{2.22}
\expandafter\def\csname res@llmjp@mwis@64@utillo\endcsname{.661}
\expandafter\def\csname res@llmjp@mwis@64@utilhi\endcsname{.692}
\expandafter\def\csname res@llmjp@mwis@64@utilklo\endcsname{.904}
\expandafter\def\csname res@llmjp@mwis@64@utilkhi\endcsname{.932}
\expandafter\def\csname res@llmjp@stepwise@64@bpt\endcsname{2.33}
\expandafter\def\csname res@llmjp@stepwise@64@util\endcsname{.736}
\expandafter\def\csname res@llmjp@stepwise@64@utilpct\endcsname{73.6}
\expandafter\def\csname res@llmjp@stepwise@64@kl\endcsname{.0022}
\expandafter\def\csname res@llmjp@stepwise@64@klkappa\endcsname{0.002}
\expandafter\def\csname res@llmjp@stepwise@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@stepwise@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@64@utilk\endcsname{.988}
\expandafter\def\csname res@llmjp@stepwise@64@bptlo\endcsname{2.19}
\expandafter\def\csname res@llmjp@stepwise@64@bpthi\endcsname{2.46}
\expandafter\def\csname res@llmjp@stepwise@64@utillo\endcsname{.721}
\expandafter\def\csname res@llmjp@stepwise@64@utilhi\endcsname{.749}
\expandafter\def\csname res@llmjp@stepwise@64@utilklo\endcsname{.975}
\expandafter\def\csname res@llmjp@stepwise@64@utilkhi\endcsname{1.002}
\expandafter\def\csname res@llmjp@syncpool@64@bpt\endcsname{1.93}
\expandafter\def\csname res@llmjp@syncpool@64@util\endcsname{.604}
\expandafter\def\csname res@llmjp@syncpool@64@utilpct\endcsname{60.4}
\expandafter\def\csname res@llmjp@syncpool@64@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@64@klkappa\endcsname{0.286}
\expandafter\def\csname res@llmjp@syncpool@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@64@utilk\endcsname{.819}
\expandafter\def\csname res@llmjp@syncpool@64@bptlo\endcsname{1.82}
\expandafter\def\csname res@llmjp@syncpool@64@bpthi\endcsname{2.04}
\expandafter\def\csname res@llmjp@syncpool@64@utillo\endcsname{.589}
\expandafter\def\csname res@llmjp@syncpool@64@utilhi\endcsname{.619}
\expandafter\def\csname res@llmjp@syncpool@64@utilklo\endcsname{.801}
\expandafter\def\csname res@llmjp@syncpool@64@utilkhi\endcsname{.836}
\expandafter\def\csname res@llmjp@coin@64@bpt\endcsname{2.06}
\expandafter\def\csname res@llmjp@coin@64@util\endcsname{.664}
\expandafter\def\csname res@llmjp@coin@64@utilpct\endcsname{66.4}
\expandafter\def\csname res@llmjp@coin@64@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@64@klkappa\endcsname{0.125}
\expandafter\def\csname res@llmjp@coin@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@64@utilk\endcsname{.903}
\expandafter\def\csname res@llmjp@coin@64@bptlo\endcsname{1.94}
\expandafter\def\csname res@llmjp@coin@64@bpthi\endcsname{2.19}
\expandafter\def\csname res@llmjp@coin@64@utillo\endcsname{.649}
\expandafter\def\csname res@llmjp@coin@64@utilhi\endcsname{.678}
\expandafter\def\csname res@llmjp@coin@64@utilklo\endcsname{.889}
\expandafter\def\csname res@llmjp@coin@64@utilkhi\endcsname{.917}
\expandafter\def\csname res@llmjp@hubdrop@64@bpt\endcsname{1.97}
\expandafter\def\csname res@llmjp@hubdrop@64@util\endcsname{.644}
\expandafter\def\csname res@llmjp@hubdrop@64@utilpct\endcsname{64.4}
\expandafter\def\csname res@llmjp@hubdrop@64@kl\endcsname{.0018}
\expandafter\def\csname res@llmjp@hubdrop@64@klkappa\endcsname{0.181}
\expandafter\def\csname res@llmjp@hubdrop@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@64@utilk\endcsname{.869}
\expandafter\def\csname res@llmjp@hubdrop@64@bptlo\endcsname{1.85}
\expandafter\def\csname res@llmjp@hubdrop@64@bpthi\endcsname{2.08}
\expandafter\def\csname res@llmjp@hubdrop@64@utillo\endcsname{.631}
\expandafter\def\csname res@llmjp@hubdrop@64@utilhi\endcsname{.658}
\expandafter\def\csname res@llmjp@hubdrop@64@utilklo\endcsname{.856}
\expandafter\def\csname res@llmjp@hubdrop@64@utilkhi\endcsname{.883}
\expandafter\def\csname res@llmjp@native@256@bpt\endcsname{2.85}
\expandafter\def\csname res@llmjp@native@256@util\endcsname{.830}
\expandafter\def\csname res@llmjp@native@256@utilpct\endcsname{83.0}
\expandafter\def\csname res@llmjp@native@256@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@256@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@256@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@256@err\endcsname{11}
\expandafter\def\csname res@llmjp@native@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@256@utilk\endcsname{.976}
\expandafter\def\csname res@llmjp@native@256@bptlo\endcsname{2.68}
\expandafter\def\csname res@llmjp@native@256@bpthi\endcsname{3.01}
\expandafter\def\csname res@llmjp@native@256@utillo\endcsname{.815}
\expandafter\def\csname res@llmjp@native@256@utilhi\endcsname{.845}
\expandafter\def\csname res@llmjp@native@256@utilklo\endcsname{.962}
\expandafter\def\csname res@llmjp@native@256@utilkhi\endcsname{.990}
\expandafter\def\csname res@llmjp@basic@256@bpt\endcsname{3.53}
\expandafter\def\csname res@llmjp@basic@256@util\endcsname{.852}
\expandafter\def\csname res@llmjp@basic@256@utilpct\endcsname{85.2}
\expandafter\def\csname res@llmjp@basic@256@kl\endcsname{.689}
\expandafter\def\csname res@llmjp@basic@256@klkappa\endcsname{0.689}
\expandafter\def\csname res@llmjp@basic@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@basic@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@basic@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@256@utilk\endcsname{1.044}
\expandafter\def\csname res@llmjp@basic@256@bptlo\endcsname{3.38}
\expandafter\def\csname res@llmjp@basic@256@bpthi\endcsname{3.68}
\expandafter\def\csname res@llmjp@basic@256@utillo\endcsname{.835}
\expandafter\def\csname res@llmjp@basic@256@utilhi\endcsname{.868}
\expandafter\def\csname res@llmjp@basic@256@utilklo\endcsname{1.027}
\expandafter\def\csname res@llmjp@basic@256@utilkhi\endcsname{1.060}
\expandafter\def\csname res@llmjp@mwis@256@bpt\endcsname{2.52}
\expandafter\def\csname res@llmjp@mwis@256@util\endcsname{.772}
\expandafter\def\csname res@llmjp@mwis@256@utilpct\endcsname{77.2}
\expandafter\def\csname res@llmjp@mwis@256@kl\endcsname{.067}
\expandafter\def\csname res@llmjp@mwis@256@klkappa\endcsname{0.067}
\expandafter\def\csname res@llmjp@mwis@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@256@utilk\endcsname{.912}
\expandafter\def\csname res@llmjp@mwis@256@bptlo\endcsname{2.38}
\expandafter\def\csname res@llmjp@mwis@256@bpthi\endcsname{2.66}
\expandafter\def\csname res@llmjp@mwis@256@utillo\endcsname{.759}
\expandafter\def\csname res@llmjp@mwis@256@utilhi\endcsname{.784}
\expandafter\def\csname res@llmjp@mwis@256@utilklo\endcsname{.898}
\expandafter\def\csname res@llmjp@mwis@256@utilkhi\endcsname{.926}
\expandafter\def\csname res@llmjp@stepwise@256@bpt\endcsname{2.83}
\expandafter\def\csname res@llmjp@stepwise@256@util\endcsname{.823}
\expandafter\def\csname res@llmjp@stepwise@256@utilpct\endcsname{82.3}
\expandafter\def\csname res@llmjp@stepwise@256@kl\endcsname{.0027}
\expandafter\def\csname res@llmjp@stepwise@256@klkappa\endcsname{0.003}
\expandafter\def\csname res@llmjp@stepwise@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@stepwise@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@256@utilk\endcsname{.982}
\expandafter\def\csname res@llmjp@stepwise@256@bptlo\endcsname{2.67}
\expandafter\def\csname res@llmjp@stepwise@256@bpthi\endcsname{2.99}
\expandafter\def\csname res@llmjp@stepwise@256@utillo\endcsname{.810}
\expandafter\def\csname res@llmjp@stepwise@256@utilhi\endcsname{.837}
\expandafter\def\csname res@llmjp@stepwise@256@utilklo\endcsname{.968}
\expandafter\def\csname res@llmjp@stepwise@256@utilkhi\endcsname{.995}
\expandafter\def\csname res@llmjp@syncpool@256@bpt\endcsname{2.26}
\expandafter\def\csname res@llmjp@syncpool@256@util\endcsname{.661}
\expandafter\def\csname res@llmjp@syncpool@256@utilpct\endcsname{66.1}
\expandafter\def\csname res@llmjp@syncpool@256@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@256@klkappa\endcsname{0.426}
\expandafter\def\csname res@llmjp@syncpool@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@256@utilk\endcsname{.781}
\expandafter\def\csname res@llmjp@syncpool@256@bptlo\endcsname{2.13}
\expandafter\def\csname res@llmjp@syncpool@256@bpthi\endcsname{2.40}
\expandafter\def\csname res@llmjp@syncpool@256@utillo\endcsname{.641}
\expandafter\def\csname res@llmjp@syncpool@256@utilhi\endcsname{.682}
\expandafter\def\csname res@llmjp@syncpool@256@utilklo\endcsname{.756}
\expandafter\def\csname res@llmjp@syncpool@256@utilkhi\endcsname{.806}
\expandafter\def\csname res@llmjp@coin@256@bpt\endcsname{2.76}
\expandafter\def\csname res@llmjp@coin@256@util\endcsname{.774}
\expandafter\def\csname res@llmjp@coin@256@utilpct\endcsname{77.4}
\expandafter\def\csname res@llmjp@coin@256@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@256@klkappa\endcsname{0.168}
\expandafter\def\csname res@llmjp@coin@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@256@utilk\endcsname{.921}
\expandafter\def\csname res@llmjp@coin@256@bptlo\endcsname{2.61}
\expandafter\def\csname res@llmjp@coin@256@bpthi\endcsname{2.91}
\expandafter\def\csname res@llmjp@coin@256@utillo\endcsname{.761}
\expandafter\def\csname res@llmjp@coin@256@utilhi\endcsname{.789}
\expandafter\def\csname res@llmjp@coin@256@utilklo\endcsname{.907}
\expandafter\def\csname res@llmjp@coin@256@utilkhi\endcsname{.936}
\expandafter\def\csname res@llmjp@hubdrop@256@bpt\endcsname{2.47}
\expandafter\def\csname res@llmjp@hubdrop@256@util\endcsname{.720}
\expandafter\def\csname res@llmjp@hubdrop@256@utilpct\endcsname{72.0}
\expandafter\def\csname res@llmjp@hubdrop@256@kl\endcsname{.0027}
\expandafter\def\csname res@llmjp@hubdrop@256@klkappa\endcsname{0.249}
\expandafter\def\csname res@llmjp@hubdrop@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@256@utilk\endcsname{.851}
\expandafter\def\csname res@llmjp@hubdrop@256@bptlo\endcsname{2.34}
\expandafter\def\csname res@llmjp@hubdrop@256@bpthi\endcsname{2.60}
\expandafter\def\csname res@llmjp@hubdrop@256@utillo\endcsname{.706}
\expandafter\def\csname res@llmjp@hubdrop@256@utilhi\endcsname{.734}
\expandafter\def\csname res@llmjp@hubdrop@256@utilklo\endcsname{.837}
\expandafter\def\csname res@llmjp@hubdrop@256@utilkhi\endcsname{.866}
\expandafter\def\csname res@llmjp@native@1k@bpt\endcsname{3.47}
\expandafter\def\csname res@llmjp@native@1k@util\endcsname{.911}
\expandafter\def\csname res@llmjp@native@1k@utilpct\endcsname{91.1}
\expandafter\def\csname res@llmjp@native@1k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@1k@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@1k@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@1k@err\endcsname{12}
\expandafter\def\csname res@llmjp@native@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@1k@utilk\endcsname{.996}
\expandafter\def\csname res@llmjp@native@1k@bptlo\endcsname{3.28}
\expandafter\def\csname res@llmjp@native@1k@bpthi\endcsname{3.66}
\expandafter\def\csname res@llmjp@native@1k@utillo\endcsname{.898}
\expandafter\def\csname res@llmjp@native@1k@utilhi\endcsname{.923}
\expandafter\def\csname res@llmjp@native@1k@utilklo\endcsname{.983}
\expandafter\def\csname res@llmjp@native@1k@utilkhi\endcsname{1.009}
\expandafter\def\csname res@llmjp@basic@1k@bpt\endcsname{4.12}
\expandafter\def\csname res@llmjp@basic@1k@util\endcsname{.904}
\expandafter\def\csname res@llmjp@basic@1k@utilpct\endcsname{90.4}
\expandafter\def\csname res@llmjp@basic@1k@kl\endcsname{.698}
\expandafter\def\csname res@llmjp@basic@1k@klkappa\endcsname{0.698}
\expandafter\def\csname res@llmjp@basic@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@basic@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@basic@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@1k@utilk\endcsname{1.011}
\expandafter\def\csname res@llmjp@basic@1k@bptlo\endcsname{3.92}
\expandafter\def\csname res@llmjp@basic@1k@bpthi\endcsname{4.31}
\expandafter\def\csname res@llmjp@basic@1k@utillo\endcsname{.888}
\expandafter\def\csname res@llmjp@basic@1k@utilhi\endcsname{.919}
\expandafter\def\csname res@llmjp@basic@1k@utilklo\endcsname{.994}
\expandafter\def\csname res@llmjp@basic@1k@utilkhi\endcsname{1.027}
\expandafter\def\csname res@llmjp@mwis@1k@bpt\endcsname{2.98}
\expandafter\def\csname res@llmjp@mwis@1k@util\endcsname{.821}
\expandafter\def\csname res@llmjp@mwis@1k@utilpct\endcsname{82.1}
\expandafter\def\csname res@llmjp@mwis@1k@kl\endcsname{.084}
\expandafter\def\csname res@llmjp@mwis@1k@klkappa\endcsname{0.084}
\expandafter\def\csname res@llmjp@mwis@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@1k@utilk\endcsname{.894}
\expandafter\def\csname res@llmjp@mwis@1k@bptlo\endcsname{2.80}
\expandafter\def\csname res@llmjp@mwis@1k@bpthi\endcsname{3.15}
\expandafter\def\csname res@llmjp@mwis@1k@utillo\endcsname{.807}
\expandafter\def\csname res@llmjp@mwis@1k@utilhi\endcsname{.835}
\expandafter\def\csname res@llmjp@mwis@1k@utilklo\endcsname{.878}
\expandafter\def\csname res@llmjp@mwis@1k@utilkhi\endcsname{.909}
\expandafter\def\csname res@llmjp@stepwise@1k@bpt\endcsname{3.46}
\expandafter\def\csname res@llmjp@stepwise@1k@util\endcsname{.911}
\expandafter\def\csname res@llmjp@stepwise@1k@utilpct\endcsname{91.1}
\expandafter\def\csname res@llmjp@stepwise@1k@kl\endcsname{.0021}
\expandafter\def\csname res@llmjp@stepwise@1k@klkappa\endcsname{0.002}
\expandafter\def\csname res@llmjp@stepwise@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@stepwise@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@1k@utilk\endcsname{.991}
\expandafter\def\csname res@llmjp@stepwise@1k@bptlo\endcsname{3.27}
\expandafter\def\csname res@llmjp@stepwise@1k@bpthi\endcsname{3.65}
\expandafter\def\csname res@llmjp@stepwise@1k@utillo\endcsname{.898}
\expandafter\def\csname res@llmjp@stepwise@1k@utilhi\endcsname{.924}
\expandafter\def\csname res@llmjp@stepwise@1k@utilklo\endcsname{.976}
\expandafter\def\csname res@llmjp@stepwise@1k@utilkhi\endcsname{1.005}
\expandafter\def\csname res@llmjp@syncpool@1k@bpt\endcsname{2.42}
\expandafter\def\csname res@llmjp@syncpool@1k@util\endcsname{.640}
\expandafter\def\csname res@llmjp@syncpool@1k@utilpct\endcsname{64.0}
\expandafter\def\csname res@llmjp@syncpool@1k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@1k@klkappa\endcsname{0.710}
\expandafter\def\csname res@llmjp@syncpool@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@1k@utilk\endcsname{.697}
\expandafter\def\csname res@llmjp@syncpool@1k@bptlo\endcsname{2.27}
\expandafter\def\csname res@llmjp@syncpool@1k@bpthi\endcsname{2.57}
\expandafter\def\csname res@llmjp@syncpool@1k@utillo\endcsname{.611}
\expandafter\def\csname res@llmjp@syncpool@1k@utilhi\endcsname{.667}
\expandafter\def\csname res@llmjp@syncpool@1k@utilklo\endcsname{.665}
\expandafter\def\csname res@llmjp@syncpool@1k@utilkhi\endcsname{.726}
\expandafter\def\csname res@llmjp@coin@1k@bpt\endcsname{3.12}
\expandafter\def\csname res@llmjp@coin@1k@util\endcsname{.836}
\expandafter\def\csname res@llmjp@coin@1k@utilpct\endcsname{83.6}
\expandafter\def\csname res@llmjp@coin@1k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@1k@klkappa\endcsname{0.189}
\expandafter\def\csname res@llmjp@coin@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@1k@utilk\endcsname{.910}
\expandafter\def\csname res@llmjp@coin@1k@bptlo\endcsname{2.95}
\expandafter\def\csname res@llmjp@coin@1k@bpthi\endcsname{3.29}
\expandafter\def\csname res@llmjp@coin@1k@utillo\endcsname{.823}
\expandafter\def\csname res@llmjp@coin@1k@utilhi\endcsname{.848}
\expandafter\def\csname res@llmjp@coin@1k@utilklo\endcsname{.895}
\expandafter\def\csname res@llmjp@coin@1k@utilkhi\endcsname{.924}
\expandafter\def\csname res@llmjp@hubdrop@1k@bpt\endcsname{2.79}
\expandafter\def\csname res@llmjp@hubdrop@1k@util\endcsname{.776}
\expandafter\def\csname res@llmjp@hubdrop@1k@utilpct\endcsname{77.6}
\expandafter\def\csname res@llmjp@hubdrop@1k@kl\endcsname{.0032}
\expandafter\def\csname res@llmjp@hubdrop@1k@klkappa\endcsname{0.305}
\expandafter\def\csname res@llmjp@hubdrop@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@1k@utilk\endcsname{.845}
\expandafter\def\csname res@llmjp@hubdrop@1k@bptlo\endcsname{2.64}
\expandafter\def\csname res@llmjp@hubdrop@1k@bpthi\endcsname{2.94}
\expandafter\def\csname res@llmjp@hubdrop@1k@utillo\endcsname{.763}
\expandafter\def\csname res@llmjp@hubdrop@1k@utilhi\endcsname{.789}
\expandafter\def\csname res@llmjp@hubdrop@1k@utilklo\endcsname{.832}
\expandafter\def\csname res@llmjp@hubdrop@1k@utilkhi\endcsname{.858}
\expandafter\def\csname res@llmjp@native@4k@bpt\endcsname{3.77}
\expandafter\def\csname res@llmjp@native@4k@util\endcsname{.956}
\expandafter\def\csname res@llmjp@native@4k@utilpct\endcsname{95.6}
\expandafter\def\csname res@llmjp@native@4k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@4k@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@4k@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@4k@err\endcsname{19}
\expandafter\def\csname res@llmjp@native@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@4k@utilk\endcsname{.992}
\expandafter\def\csname res@llmjp@native@4k@bptlo\endcsname{3.54}
\expandafter\def\csname res@llmjp@native@4k@bpthi\endcsname{3.99}
\expandafter\def\csname res@llmjp@native@4k@utillo\endcsname{.941}
\expandafter\def\csname res@llmjp@native@4k@utilhi\endcsname{.971}
\expandafter\def\csname res@llmjp@native@4k@utilklo\endcsname{.977}
\expandafter\def\csname res@llmjp@native@4k@utilkhi\endcsname{1.007}
\expandafter\def\csname res@llmjp@basic@4k@bpt\endcsname{4.39}
\expandafter\def\csname res@llmjp@basic@4k@util\endcsname{.938}
\expandafter\def\csname res@llmjp@basic@4k@utilpct\endcsname{93.8}
\expandafter\def\csname res@llmjp@basic@4k@kl\endcsname{.708}
\expandafter\def\csname res@llmjp@basic@4k@klkappa\endcsname{0.708}
\expandafter\def\csname res@llmjp@basic@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@basic@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@basic@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@4k@utilk\endcsname{.979}
\expandafter\def\csname res@llmjp@basic@4k@bptlo\endcsname{4.15}
\expandafter\def\csname res@llmjp@basic@4k@bpthi\endcsname{4.63}
\expandafter\def\csname res@llmjp@basic@4k@utillo\endcsname{.920}
\expandafter\def\csname res@llmjp@basic@4k@utilhi\endcsname{.956}
\expandafter\def\csname res@llmjp@basic@4k@utilklo\endcsname{.961}
\expandafter\def\csname res@llmjp@basic@4k@utilkhi\endcsname{.997}
\expandafter\def\csname res@llmjp@mwis@4k@bpt\endcsname{3.15}
\expandafter\def\csname res@llmjp@mwis@4k@util\endcsname{.867}
\expandafter\def\csname res@llmjp@mwis@4k@utilpct\endcsname{86.7}
\expandafter\def\csname res@llmjp@mwis@4k@kl\endcsname{.085}
\expandafter\def\csname res@llmjp@mwis@4k@klkappa\endcsname{0.085}
\expandafter\def\csname res@llmjp@mwis@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@4k@utilk\endcsname{.893}
\expandafter\def\csname res@llmjp@mwis@4k@bptlo\endcsname{2.97}
\expandafter\def\csname res@llmjp@mwis@4k@bpthi\endcsname{3.34}
\expandafter\def\csname res@llmjp@mwis@4k@utillo\endcsname{.853}
\expandafter\def\csname res@llmjp@mwis@4k@utilhi\endcsname{.880}
\expandafter\def\csname res@llmjp@mwis@4k@utilklo\endcsname{.878}
\expandafter\def\csname res@llmjp@mwis@4k@utilkhi\endcsname{.907}
\expandafter\def\csname res@llmjp@stepwise@4k@bpt\endcsname{3.65}
\expandafter\def\csname res@llmjp@stepwise@4k@util\endcsname{.963}
\expandafter\def\csname res@llmjp@stepwise@4k@utilpct\endcsname{96.3}
\expandafter\def\csname res@llmjp@stepwise@4k@kl\endcsname{.003}
\expandafter\def\csname res@llmjp@stepwise@4k@klkappa\endcsname{0.003}
\expandafter\def\csname res@llmjp@stepwise@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@stepwise@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@4k@utilk\endcsname{.997}
\expandafter\def\csname res@llmjp@stepwise@4k@bptlo\endcsname{3.44}
\expandafter\def\csname res@llmjp@stepwise@4k@bpthi\endcsname{3.87}
\expandafter\def\csname res@llmjp@stepwise@4k@utillo\endcsname{.949}
\expandafter\def\csname res@llmjp@stepwise@4k@utilhi\endcsname{.979}
\expandafter\def\csname res@llmjp@stepwise@4k@utilklo\endcsname{.982}
\expandafter\def\csname res@llmjp@stepwise@4k@utilkhi\endcsname{1.013}
\expandafter\def\csname res@llmjp@syncpool@4k@bpt\endcsname{2.13}
\expandafter\def\csname res@llmjp@syncpool@4k@util\endcsname{.552}
\expandafter\def\csname res@llmjp@syncpool@4k@utilpct\endcsname{55.2}
\expandafter\def\csname res@llmjp@syncpool@4k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@4k@klkappa\endcsname{1.062}
\expandafter\def\csname res@llmjp@syncpool@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@4k@utilk\endcsname{.572}
\expandafter\def\csname res@llmjp@syncpool@4k@bptlo\endcsname{1.97}
\expandafter\def\csname res@llmjp@syncpool@4k@bpthi\endcsname{2.29}
\expandafter\def\csname res@llmjp@syncpool@4k@utillo\endcsname{.520}
\expandafter\def\csname res@llmjp@syncpool@4k@utilhi\endcsname{.581}
\expandafter\def\csname res@llmjp@syncpool@4k@utilklo\endcsname{.538}
\expandafter\def\csname res@llmjp@syncpool@4k@utilkhi\endcsname{.603}
\expandafter\def\csname res@llmjp@coin@4k@bpt\endcsname{3.52}
\expandafter\def\csname res@llmjp@coin@4k@util\endcsname{.876}
\expandafter\def\csname res@llmjp@coin@4k@utilpct\endcsname{87.6}
\expandafter\def\csname res@llmjp@coin@4k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@4k@klkappa\endcsname{0.218}
\expandafter\def\csname res@llmjp@coin@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@4k@utilk\endcsname{.907}
\expandafter\def\csname res@llmjp@coin@4k@bptlo\endcsname{3.32}
\expandafter\def\csname res@llmjp@coin@4k@bpthi\endcsname{3.72}
\expandafter\def\csname res@llmjp@coin@4k@utillo\endcsname{.863}
\expandafter\def\csname res@llmjp@coin@4k@utilhi\endcsname{.890}
\expandafter\def\csname res@llmjp@coin@4k@utilklo\endcsname{.893}
\expandafter\def\csname res@llmjp@coin@4k@utilkhi\endcsname{.920}
\expandafter\def\csname res@llmjp@hubdrop@4k@bpt\endcsname{3.21}
\expandafter\def\csname res@llmjp@hubdrop@4k@util\endcsname{.795}
\expandafter\def\csname res@llmjp@hubdrop@4k@utilpct\endcsname{79.5}
\expandafter\def\csname res@llmjp@hubdrop@4k@kl\endcsname{.0043}
\expandafter\def\csname res@llmjp@hubdrop@4k@klkappa\endcsname{0.410}
\expandafter\def\csname res@llmjp@hubdrop@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@4k@incomplete\endcsname{1}
\expandafter\def\csname res@llmjp@hubdrop@4k@utilk\endcsname{.824}
\expandafter\def\csname res@llmjp@hubdrop@4k@bptlo\endcsname{3.02}
\expandafter\def\csname res@llmjp@hubdrop@4k@bpthi\endcsname{3.39}
\expandafter\def\csname res@llmjp@hubdrop@4k@utillo\endcsname{.757}
\expandafter\def\csname res@llmjp@hubdrop@4k@utilhi\endcsname{.821}
\expandafter\def\csname res@llmjp@hubdrop@4k@utilklo\endcsname{.791}
\expandafter\def\csname res@llmjp@hubdrop@4k@utilkhi\endcsname{.847}
\expandafter\def\csname res@llmjp@native@Full@bpt\endcsname{4.03}
\expandafter\def\csname res@llmjp@native@Full@util\endcsname{.989}
\expandafter\def\csname res@llmjp@native@Full@utilpct\endcsname{98.9}
\expandafter\def\csname res@llmjp@native@Full@kl\endcsname{0}
\expandafter\def\csname res@llmjp@native@Full@klkappa\endcsname{0.000}
\expandafter\def\csname res@llmjp@native@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@native@Full@tested\endcsname{100}
\expandafter\def\csname res@llmjp@native@Full@err\endcsname{17}
\expandafter\def\csname res@llmjp@native@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@native@Full@utilk\endcsname{.989}
\expandafter\def\csname res@llmjp@native@Full@bptlo\endcsname{3.75}
\expandafter\def\csname res@llmjp@native@Full@bpthi\endcsname{4.31}
\expandafter\def\csname res@llmjp@native@Full@utillo\endcsname{.975}
\expandafter\def\csname res@llmjp@native@Full@utilhi\endcsname{1.003}
\expandafter\def\csname res@llmjp@native@Full@utilklo\endcsname{.975}
\expandafter\def\csname res@llmjp@native@Full@utilkhi\endcsname{1.003}
\expandafter\def\csname res@llmjp@mwis@Full@bpt\endcsname{3.37}
\expandafter\def\csname res@llmjp@mwis@Full@util\endcsname{.873}
\expandafter\def\csname res@llmjp@mwis@Full@utilpct\endcsname{87.3}
\expandafter\def\csname res@llmjp@mwis@Full@kl\endcsname{.097}
\expandafter\def\csname res@llmjp@mwis@Full@klkappa\endcsname{0.097}
\expandafter\def\csname res@llmjp@mwis@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@mwis@Full@tested\endcsname{20}
\expandafter\def\csname res@llmjp@mwis@Full@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@Full@incomplete\endcsname{1}
\expandafter\def\csname res@llmjp@mwis@Full@utilk\endcsname{.873}
\expandafter\def\csname res@llmjp@mwis@Full@bptlo\endcsname{3.16}
\expandafter\def\csname res@llmjp@mwis@Full@bpthi\endcsname{3.57}
\expandafter\def\csname res@llmjp@mwis@Full@utillo\endcsname{.843}
\expandafter\def\csname res@llmjp@mwis@Full@utilhi\endcsname{.894}
\expandafter\def\csname res@llmjp@mwis@Full@utilklo\endcsname{.843}
\expandafter\def\csname res@llmjp@mwis@Full@utilkhi\endcsname{.894}
\expandafter\def\csname res@llmjp@syncpool@Full@bpt\endcsname{1.40}
\expandafter\def\csname res@llmjp@syncpool@Full@util\endcsname{.336}
\expandafter\def\csname res@llmjp@syncpool@Full@utilpct\endcsname{33.6}
\expandafter\def\csname res@llmjp@syncpool@Full@kl\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@Full@klkappa\endcsname{1.889}
\expandafter\def\csname res@llmjp@syncpool@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@syncpool@Full@tested\endcsname{20}
\expandafter\def\csname res@llmjp@syncpool@Full@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@Full@utilk\endcsname{.336}
\expandafter\def\csname res@llmjp@syncpool@Full@bptlo\endcsname{1.32}
\expandafter\def\csname res@llmjp@syncpool@Full@bpthi\endcsname{1.49}
\expandafter\def\csname res@llmjp@syncpool@Full@utillo\endcsname{.318}
\expandafter\def\csname res@llmjp@syncpool@Full@utilhi\endcsname{.354}
\expandafter\def\csname res@llmjp@syncpool@Full@utilklo\endcsname{.318}
\expandafter\def\csname res@llmjp@syncpool@Full@utilkhi\endcsname{.354}
\expandafter\def\csname res@llmjp@coin@Full@bpt\endcsname{3.90}
\expandafter\def\csname res@llmjp@coin@Full@util\endcsname{.920}
\expandafter\def\csname res@llmjp@coin@Full@utilpct\endcsname{92.0}
\expandafter\def\csname res@llmjp@coin@Full@kl\endcsname{0}
\expandafter\def\csname res@llmjp@coin@Full@klkappa\endcsname{0.241}
\expandafter\def\csname res@llmjp@coin@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@coin@Full@tested\endcsname{20}
\expandafter\def\csname res@llmjp@coin@Full@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@Full@utilk\endcsname{.920}
\expandafter\def\csname res@llmjp@coin@Full@bptlo\endcsname{3.65}
\expandafter\def\csname res@llmjp@coin@Full@bpthi\endcsname{4.14}
\expandafter\def\csname res@llmjp@coin@Full@utillo\endcsname{.907}
\expandafter\def\csname res@llmjp@coin@Full@utilhi\endcsname{.932}
\expandafter\def\csname res@llmjp@coin@Full@utilklo\endcsname{.907}
\expandafter\def\csname res@llmjp@coin@Full@utilkhi\endcsname{.932}
\expandafter\def\csname res@llmjp@hubdrop@Full@bpt\endcsname{3.55}
\expandafter\def\csname res@llmjp@hubdrop@Full@util\endcsname{.832}
\expandafter\def\csname res@llmjp@hubdrop@Full@utilpct\endcsname{83.2}
\expandafter\def\csname res@llmjp@hubdrop@Full@kl\endcsname{.0046}
\expandafter\def\csname res@llmjp@hubdrop@Full@klkappa\endcsname{0.459}
\expandafter\def\csname res@llmjp@hubdrop@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@hubdrop@Full@tested\endcsname{20}
\expandafter\def\csname res@llmjp@hubdrop@Full@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@Full@utilk\endcsname{.832}
\expandafter\def\csname res@llmjp@hubdrop@Full@bptlo\endcsname{3.37}
\expandafter\def\csname res@llmjp@hubdrop@Full@bpthi\endcsname{3.76}
\expandafter\def\csname res@llmjp@hubdrop@Full@utillo\endcsname{.818}
\expandafter\def\csname res@llmjp@hubdrop@Full@utilhi\endcsname{.846}
\expandafter\def\csname res@llmjp@hubdrop@Full@utilklo\endcsname{.818}
\expandafter\def\csname res@llmjp@hubdrop@Full@utilkhi\endcsname{.846}
\expandafter\def\csname res@llmjp@las@16@bpt\endcsname{1.69}
\expandafter\def\csname res@llmjp@las@16@util\endcsname{.572}
\expandafter\def\csname res@llmjp@las@16@utilpct\endcsname{57.2}
\expandafter\def\csname res@llmjp@las@16@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@16@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@16@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@16@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@16@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@16@utilk\endcsname{.986}
\expandafter\def\csname res@llmjp@las@16@bptlo\endcsname{1.59}
\expandafter\def\csname res@llmjp@las@16@bpthi\endcsname{1.79}
\expandafter\def\csname res@llmjp@las@16@utillo\endcsname{.558}
\expandafter\def\csname res@llmjp@las@16@utilhi\endcsname{.587}
\expandafter\def\csname res@llmjp@las@16@utilklo\endcsname{.969}
\expandafter\def\csname res@llmjp@las@16@utilkhi\endcsname{1.001}
\expandafter\def\csname res@llmjp@las@64@bpt\endcsname{2.31}
\expandafter\def\csname res@llmjp@las@64@util\endcsname{.716}
\expandafter\def\csname res@llmjp@las@64@utilpct\endcsname{71.6}
\expandafter\def\csname res@llmjp@las@64@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@64@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@64@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@64@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@64@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@64@utilk\endcsname{.975}
\expandafter\def\csname res@llmjp@las@64@bptlo\endcsname{2.19}
\expandafter\def\csname res@llmjp@las@64@bpthi\endcsname{2.44}
\expandafter\def\csname res@llmjp@las@64@utillo\endcsname{.701}
\expandafter\def\csname res@llmjp@las@64@utilhi\endcsname{.732}
\expandafter\def\csname res@llmjp@las@64@utilklo\endcsname{.961}
\expandafter\def\csname res@llmjp@las@64@utilkhi\endcsname{.990}
\expandafter\def\csname res@llmjp@las@256@bpt\endcsname{2.87}
\expandafter\def\csname res@llmjp@las@256@util\endcsname{.834}
\expandafter\def\csname res@llmjp@las@256@utilpct\endcsname{83.4}
\expandafter\def\csname res@llmjp@las@256@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@256@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@256@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@256@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@256@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@256@utilk\endcsname{.991}
\expandafter\def\csname res@llmjp@las@256@bptlo\endcsname{2.69}
\expandafter\def\csname res@llmjp@las@256@bpthi\endcsname{3.05}
\expandafter\def\csname res@llmjp@las@256@utillo\endcsname{.819}
\expandafter\def\csname res@llmjp@las@256@utilhi\endcsname{.849}
\expandafter\def\csname res@llmjp@las@256@utilklo\endcsname{.977}
\expandafter\def\csname res@llmjp@las@256@utilkhi\endcsname{1.005}
\expandafter\def\csname res@llmjp@las@1k@bpt\endcsname{3.34}
\expandafter\def\csname res@llmjp@las@1k@util\endcsname{.912}
\expandafter\def\csname res@llmjp@las@1k@utilpct\endcsname{91.2}
\expandafter\def\csname res@llmjp@las@1k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@1k@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@1k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@1k@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@1k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@1k@utilk\endcsname{.995}
\expandafter\def\csname res@llmjp@las@1k@bptlo\endcsname{3.15}
\expandafter\def\csname res@llmjp@las@1k@bpthi\endcsname{3.53}
\expandafter\def\csname res@llmjp@las@1k@utillo\endcsname{.898}
\expandafter\def\csname res@llmjp@las@1k@utilhi\endcsname{.926}
\expandafter\def\csname res@llmjp@las@1k@utilklo\endcsname{.982}
\expandafter\def\csname res@llmjp@las@1k@utilkhi\endcsname{1.010}
\expandafter\def\csname res@llmjp@las@4k@bpt\endcsname{3.90}
\expandafter\def\csname res@llmjp@las@4k@util\endcsname{.955}
\expandafter\def\csname res@llmjp@las@4k@utilpct\endcsname{95.5}
\expandafter\def\csname res@llmjp@las@4k@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@4k@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@4k@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@4k@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@4k@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@4k@utilk\endcsname{.990}
\expandafter\def\csname res@llmjp@las@4k@bptlo\endcsname{3.68}
\expandafter\def\csname res@llmjp@las@4k@bpthi\endcsname{4.13}
\expandafter\def\csname res@llmjp@las@4k@utillo\endcsname{.940}
\expandafter\def\csname res@llmjp@las@4k@utilhi\endcsname{.971}
\expandafter\def\csname res@llmjp@las@4k@utilklo\endcsname{.974}
\expandafter\def\csname res@llmjp@las@4k@utilkhi\endcsname{1.006}
\expandafter\def\csname res@llmjp@las@Full@bpt\endcsname{4.01}
\expandafter\def\csname res@llmjp@las@Full@util\endcsname{.984}
\expandafter\def\csname res@llmjp@las@Full@utilpct\endcsname{98.4}
\expandafter\def\csname res@llmjp@las@Full@kl\endcsname{0}
\expandafter\def\csname res@llmjp@las@Full@n\endcsname{100}
\expandafter\def\csname res@llmjp@las@Full@tested\endcsname{20}
\expandafter\def\csname res@llmjp@las@Full@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@Full@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@Full@utilk\endcsname{.984}
\expandafter\def\csname res@llmjp@las@Full@bptlo\endcsname{3.76}
\expandafter\def\csname res@llmjp@las@Full@bpthi\endcsname{4.26}
\expandafter\def\csname res@llmjp@las@Full@utillo\endcsname{.969}
\expandafter\def\csname res@llmjp@las@Full@utilhi\endcsname{.999}
\expandafter\def\csname res@llmjp@las@Full@utilklo\endcsname{.969}
\expandafter\def\csname res@llmjp@las@Full@utilkhi\endcsname{.999}
\expandafter\def\csname res@llmjp@native@all@err\endcsname{72}
\expandafter\def\csname res@llmjp@native@all@tested\endcsname{600}
\expandafter\def\csname res@llmjp@native@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@basic@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@basic@all@tested\endcsname{100}
\expandafter\def\csname res@llmjp@basic@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@mwis@all@tested\endcsname{120}
\expandafter\def\csname res@llmjp@mwis@all@incomplete\endcsname{1}
\expandafter\def\csname res@llmjp@stepwise@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@stepwise@all@tested\endcsname{100}
\expandafter\def\csname res@llmjp@stepwise@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@hubdrop@all@tested\endcsname{120}
\expandafter\def\csname res@llmjp@hubdrop@all@incomplete\endcsname{1}
\expandafter\def\csname res@llmjp@syncpool@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@syncpool@all@tested\endcsname{120}
\expandafter\def\csname res@llmjp@syncpool@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@las@all@tested\endcsname{120}
\expandafter\def\csname res@llmjp@las@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@coin@all@err\endcsname{0}
\expandafter\def\csname res@llmjp@coin@all@tested\endcsname{120}
\expandafter\def\csname res@llmjp@coin@all@incomplete\endcsname{0}
\expandafter\def\csname res@llmjp@las@Full@utilgap\endcsname{6.4}
\expandafter\def\csname res@llmjp@native@all@oop\endcsname{16}
\expandafter\def\csname res@llmjp@native@all@prompt\endcsname{0}
\expandafter\def\csname res@llmjp@native@Full@silent\endcsname{16}
\expandafter\def\csname res@llmjp@gain@16@meas\endcsname{1.04}
\expandafter\def\csname res@llmjp@coin@16@utilvsH\endcsname{51}
\expandafter\def\csname res@llmjp@gain@16@pred\endcsname{1.06}
\expandafter\def\csname res@llmjp@gain@16@predtraj\endcsname{1.06}
\expandafter\def\csname res@llmjp@gain@16@lo\endcsname{1.00}
\expandafter\def\csname res@llmjp@gain@16@hi\endcsname{1.07}
\expandafter\def\csname res@llmjp@gain@64@meas\endcsname{1.10}
\expandafter\def\csname res@llmjp@coin@64@utilvsH\endcsname{66}
\expandafter\def\csname res@llmjp@gain@64@pred\endcsname{1.14}
\expandafter\def\csname res@llmjp@gain@64@predtraj\endcsname{1.12}
\expandafter\def\csname res@llmjp@gain@64@lo\endcsname{1.07}
\expandafter\def\csname res@llmjp@gain@64@hi\endcsname{1.13}
\expandafter\def\csname res@llmjp@gain@256@meas\endcsname{1.17}
\expandafter\def\csname res@llmjp@coin@256@utilvsH\endcsname{77}
\expandafter\def\csname res@llmjp@gain@256@pred\endcsname{1.24}
\expandafter\def\csname res@llmjp@gain@256@predtraj\endcsname{1.18}
\expandafter\def\csname res@llmjp@gain@256@lo\endcsname{1.13}
\expandafter\def\csname res@llmjp@gain@256@hi\endcsname{1.22}
\expandafter\def\csname res@llmjp@gain@1k@meas\endcsname{1.31}
\expandafter\def\csname res@llmjp@coin@1k@utilvsH\endcsname{84}
\expandafter\def\csname res@llmjp@gain@1k@pred\endcsname{1.31}
\expandafter\def\csname res@llmjp@gain@1k@predtraj\endcsname{1.29}
\expandafter\def\csname res@llmjp@gain@1k@lo\endcsname{1.25}
\expandafter\def\csname res@llmjp@gain@1k@hi\endcsname{1.37}
\expandafter\def\csname res@llmjp@gain@4k@meas\endcsname{1.59}
\expandafter\def\csname res@llmjp@coin@4k@utilvsH\endcsname{88}
\expandafter\def\csname res@llmjp@gain@4k@pred\endcsname{1.60}
\expandafter\def\csname res@llmjp@gain@4k@predtraj\endcsname{1.60}
\expandafter\def\csname res@llmjp@gain@4k@lo\endcsname{1.51}
\expandafter\def\csname res@llmjp@gain@4k@hi\endcsname{1.68}
\expandafter\def\csname res@llmjp@gain@Full@meas\endcsname{2.73}
\expandafter\def\csname res@llmjp@coin@Full@utilvsH\endcsname{92}
\expandafter\def\csname res@llmjp@gain@Full@pred\endcsname{2.53}
\expandafter\def\csname res@llmjp@gain@Full@predtraj\endcsname{2.67}
\expandafter\def\csname res@llmjp@gain@Full@lo\endcsname{2.59}
\expandafter\def\csname res@llmjp@gain@Full@hi\endcsname{2.88}
\expandafter\def\csname res@all@e1@any@nmin\endcsname{100}
\expandafter\def\csname res@all@e1@any@recvmin\endcsname{20}
\expandafter\def\csname res@all@e1@any@recvmax\endcsname{20}
\expandafter\def\csname res@all@e1@any@extratok\endcsname{0}
\expandafter\def\csname res@all@e1@any@badutf8\endcsname{0}
\expandafter\def\csname res@all@gain@16@min\endcsname{1.04}
\expandafter\def\csname res@all@gain@16@max\endcsname{1.16}
\expandafter\def\csname res@all@gain@64@min\endcsname{1.04}
\expandafter\def\csname res@all@gain@64@max\endcsname{1.59}
\expandafter\def\csname res@all@gain@256@min\endcsname{1.09}
\expandafter\def\csname res@all@gain@256@max\endcsname{3.37}
\expandafter\def\csname res@all@gain@1k@min\endcsname{1.09}
\expandafter\def\csname res@all@gain@1k@max\endcsname{6.20}
\expandafter\def\csname res@all@gain@4k@min\endcsname{1.16}
\expandafter\def\csname res@all@gain@4k@max\endcsname{6.80}
\expandafter\def\csname res@all@gain@Full@min\endcsname{2.18}
\expandafter\def\csname res@all@gain@Full@max\endcsname{6.83}
\expandafter\def\csname res@all@ratio@native@min\endcsname{90}
\expandafter\def\csname res@all@ratio@native@max\endcsname{93}
\expandafter\def\csname res@all@ratio@native@median\endcsname{92}
\expandafter\def\csname res@all@ratio@stepwise@min\endcsname{90}
\expandafter\def\csname res@all@ratio@stepwise@max\endcsname{94}
\expandafter\def\csname res@all@ratio@stepwise@median\endcsname{92}
\expandafter\def\csname res@all@cv@coin@min\endcsname{0.07}
\expandafter\def\csname res@all@cv@coin@max\endcsname{0.18}
\expandafter\def\csname res@all@cv@syncpool@min\endcsname{0.11}
\expandafter\def\csname res@all@cv@syncpool@max\endcsname{0.65}
\expandafter\def\csname res@all@gain@dev@total\endcsname{3.4}
\expandafter\def\csname res@all@gain@devmax@total\endcsname{10}
\expandafter\def\csname res@all@gain@dev@msg\endcsname{3.6}
\expandafter\def\csname res@all@gain@devmax@msg\endcsname{12}
\expandafter\def\csname res@all@gain@ci@above\endcsname{1}
\expandafter\def\csname res@all@gain@citraj@above\endcsname{0}
\expandafter\def\csname res@all@gain@ci@below\endcsname{3}
\expandafter\def\csname res@all@gain@citraj@below\endcsname{0}
\expandafter\def\csname res@all@gain@ci@inside\endcsname{14}
\expandafter\def\csname res@all@gain@citraj@inside\endcsname{18}
\expandafter\def\csname res@all@util@ci@max\endcsname{4}
\expandafter\def\csname res@all@util@ci@syncpoolmax\endcsname{14}
\expandafter\def\csname res@all@util@ci@median\endcsname{1.8}
\expandafter\def\csname res@all@ratio@native@medlo\endcsname{91}
\expandafter\def\csname res@all@ratio@native@medhi\endcsname{92}
\expandafter\def\csname res@all@ratio@stepwise@medlo\endcsname{91}
\expandafter\def\csname res@all@ratio@stepwise@medhi\endcsname{92}
\expandafter\def\csname res@all@basic@any@klmax\endcsname{1.05}
\expandafter\def\csname res@all@native@any@n\endcsname{600}
\expandafter\def\csname res@all@ident@cells@n\endcsname{18}
\expandafter\def\csname res@all@ident@ratio@min\endcsname{0.999}
\expandafter\def\csname res@all@ident@ratio@max\endcsname{1.001}
\expandafter\def\csname res@all@ident@eff@min\endcsname{0.97}
\expandafter\def\csname res@all@ident@eff@max\endcsname{1.00}
\expandafter\def\csname res@all@gain@cells@n\endcsname{18}
\expandafter\def\csname res@all@gain@excess@max\endcsname{5}
\expandafter\def\csname res@all@gain@excess@absmax\endcsname{5}
\expandafter\def\csname res@all@native@all@err\endcsname{162}
\expandafter\def\csname res@all@native@all@silent\endcsname{133}
\expandafter\def\csname res@all@native@all@oop\endcsname{29}
\expandafter\def\csname res@all@native@all@prompt\endcsname{0}
\expandafter\def\csname res@all@native@all@totaln\endcsname{1800}
\expandafter\def\csname res@all@native@all@silentpct\endcsname{82}
\expandafter\def\csname res@llama@native@best@bpt\endcsname{3.79}
\expandafter\def\csname res@llama@native@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llama@native@best@klab\endcsname{Full}
\expandafter\def\csname res@llama@basic@best@bpt\endcsname{5.55}
\expandafter\def\csname res@llama@basic@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@llama@basic@best@klab\endcsname{4k}
\expandafter\def\csname res@llama@mwis@best@bpt\endcsname{3.34}
\expandafter\def\csname res@llama@mwis@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@llama@mwis@best@klab\endcsname{4k}
\expandafter\def\csname res@llama@stepwise@best@bpt\endcsname{3.69}
\expandafter\def\csname res@llama@stepwise@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@llama@stepwise@best@klab\endcsname{4k}
\expandafter\def\csname res@llama@hubdrop@best@bpt\endcsname{3.20}
\expandafter\def\csname res@llama@hubdrop@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llama@hubdrop@best@klab\endcsname{Full}
\expandafter\def\csname res@llama@syncpool@best@bpt\endcsname{1.61}
\expandafter\def\csname res@llama@syncpool@best@k\endcsname{$k=16$}
\expandafter\def\csname res@llama@syncpool@best@klab\endcsname{16}
\expandafter\def\csname res@llama@las@best@bpt\endcsname{3.79}
\expandafter\def\csname res@llama@las@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llama@las@best@klab\endcsname{Full}
\expandafter\def\csname res@llama@coin@best@bpt\endcsname{3.52}
\expandafter\def\csname res@llama@coin@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llama@coin@best@klab\endcsname{Full}
\expandafter\def\csname res@llama@bestk@native@ratio\endcsname{0.93}
\expandafter\def\csname res@llama@bestk@native@lo\endcsname{0.88}
\expandafter\def\csname res@llama@bestk@native@hi\endcsname{0.98}
\expandafter\def\csname res@llama@bestk@basic@ratio\endcsname{0.63}
\expandafter\def\csname res@llama@bestk@basic@lo\endcsname{0.58}
\expandafter\def\csname res@llama@bestk@basic@hi\endcsname{0.69}
\expandafter\def\csname res@llama@bestk@mwis@ratio\endcsname{1.05}
\expandafter\def\csname res@llama@bestk@mwis@lo\endcsname{1.00}
\expandafter\def\csname res@llama@bestk@mwis@hi\endcsname{1.10}
\expandafter\def\csname res@llama@bestk@stepwise@ratio\endcsname{0.95}
\expandafter\def\csname res@llama@bestk@stepwise@lo\endcsname{0.91}
\expandafter\def\csname res@llama@bestk@stepwise@hi\endcsname{1.00}
\expandafter\def\csname res@llama@bestk@hubdrop@ratio\endcsname{1.10}
\expandafter\def\csname res@llama@bestk@hubdrop@lo\endcsname{1.04}
\expandafter\def\csname res@llama@bestk@hubdrop@hi\endcsname{1.16}
\expandafter\def\csname res@llama@bestk@syncpool@ratio\endcsname{2.18}
\expandafter\def\csname res@llama@bestk@syncpool@lo\endcsname{2.04}
\expandafter\def\csname res@llama@bestk@syncpool@hi\endcsname{2.35}
\expandafter\def\csname res@llama@bestk@las@ratio\endcsname{0.93}
\expandafter\def\csname res@llama@bestk@las@lo\endcsname{0.89}
\expandafter\def\csname res@llama@bestk@las@hi\endcsname{0.97}
\expandafter\def\csname res@qwen@native@best@bpt\endcsname{4.05}
\expandafter\def\csname res@qwen@native@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@qwen@native@best@klab\endcsname{Full}
\expandafter\def\csname res@qwen@basic@best@bpt\endcsname{4.78}
\expandafter\def\csname res@qwen@basic@best@k\endcsname{$k=1024$}
\expandafter\def\csname res@qwen@basic@best@klab\endcsname{1k}
\expandafter\def\csname res@qwen@mwis@best@bpt\endcsname{3.23}
\expandafter\def\csname res@qwen@mwis@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@qwen@mwis@best@klab\endcsname{Full}
\expandafter\def\csname res@qwen@stepwise@best@bpt\endcsname{3.97}
\expandafter\def\csname res@qwen@stepwise@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@qwen@stepwise@best@klab\endcsname{4k}
\expandafter\def\csname res@qwen@hubdrop@best@bpt\endcsname{3.26}
\expandafter\def\csname res@qwen@hubdrop@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@qwen@hubdrop@best@klab\endcsname{4k}
\expandafter\def\csname res@qwen@syncpool@best@bpt\endcsname{2.99}
\expandafter\def\csname res@qwen@syncpool@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@qwen@syncpool@best@klab\endcsname{4k}
\expandafter\def\csname res@qwen@las@best@bpt\endcsname{4.02}
\expandafter\def\csname res@qwen@las@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@qwen@las@best@klab\endcsname{Full}
\expandafter\def\csname res@qwen@coin@best@bpt\endcsname{3.85}
\expandafter\def\csname res@qwen@coin@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@qwen@coin@best@klab\endcsname{Full}
\expandafter\def\csname res@qwen@bestk@native@ratio\endcsname{0.95}
\expandafter\def\csname res@qwen@bestk@native@lo\endcsname{0.86}
\expandafter\def\csname res@qwen@bestk@native@hi\endcsname{1.04}
\expandafter\def\csname res@qwen@bestk@basic@ratio\endcsname{0.80}
\expandafter\def\csname res@qwen@bestk@basic@lo\endcsname{0.73}
\expandafter\def\csname res@qwen@bestk@basic@hi\endcsname{0.89}
\expandafter\def\csname res@qwen@bestk@mwis@ratio\endcsname{1.19}
\expandafter\def\csname res@qwen@bestk@mwis@lo\endcsname{1.10}
\expandafter\def\csname res@qwen@bestk@mwis@hi\endcsname{1.29}
\expandafter\def\csname res@qwen@bestk@stepwise@ratio\endcsname{0.97}
\expandafter\def\csname res@qwen@bestk@stepwise@lo\endcsname{0.90}
\expandafter\def\csname res@qwen@bestk@stepwise@hi\endcsname{1.05}
\expandafter\def\csname res@qwen@bestk@hubdrop@ratio\endcsname{1.18}
\expandafter\def\csname res@qwen@bestk@hubdrop@lo\endcsname{1.08}
\expandafter\def\csname res@qwen@bestk@hubdrop@hi\endcsname{1.29}
\expandafter\def\csname res@qwen@bestk@syncpool@ratio\endcsname{1.29}
\expandafter\def\csname res@qwen@bestk@syncpool@lo\endcsname{1.16}
\expandafter\def\csname res@qwen@bestk@syncpool@hi\endcsname{1.43}
\expandafter\def\csname res@qwen@bestk@las@ratio\endcsname{0.96}
\expandafter\def\csname res@qwen@bestk@las@lo\endcsname{0.87}
\expandafter\def\csname res@qwen@bestk@las@hi\endcsname{1.04}
\expandafter\def\csname res@llmjp@native@best@bpt\endcsname{4.03}
\expandafter\def\csname res@llmjp@native@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llmjp@native@best@klab\endcsname{Full}
\expandafter\def\csname res@llmjp@basic@best@bpt\endcsname{4.39}
\expandafter\def\csname res@llmjp@basic@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@llmjp@basic@best@klab\endcsname{4k}
\expandafter\def\csname res@llmjp@mwis@best@bpt\endcsname{3.37}
\expandafter\def\csname res@llmjp@mwis@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llmjp@mwis@best@klab\endcsname{Full}
\expandafter\def\csname res@llmjp@stepwise@best@bpt\endcsname{3.65}
\expandafter\def\csname res@llmjp@stepwise@best@k\endcsname{$k=4096$}
\expandafter\def\csname res@llmjp@stepwise@best@klab\endcsname{4k}
\expandafter\def\csname res@llmjp@hubdrop@best@bpt\endcsname{3.55}
\expandafter\def\csname res@llmjp@hubdrop@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llmjp@hubdrop@best@klab\endcsname{Full}
\expandafter\def\csname res@llmjp@syncpool@best@bpt\endcsname{2.42}
\expandafter\def\csname res@llmjp@syncpool@best@k\endcsname{$k=1024$}
\expandafter\def\csname res@llmjp@syncpool@best@klab\endcsname{1k}
\expandafter\def\csname res@llmjp@las@best@bpt\endcsname{4.01}
\expandafter\def\csname res@llmjp@las@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llmjp@las@best@klab\endcsname{Full}
\expandafter\def\csname res@llmjp@coin@best@bpt\endcsname{3.90}
\expandafter\def\csname res@llmjp@coin@best@k\endcsname{the full vocabulary}
\expandafter\def\csname res@llmjp@coin@best@klab\endcsname{Full}
\expandafter\def\csname res@llmjp@bestk@native@ratio\endcsname{0.97}
\expandafter\def\csname res@llmjp@bestk@native@lo\endcsname{0.90}
\expandafter\def\csname res@llmjp@bestk@native@hi\endcsname{1.04}
\expandafter\def\csname res@llmjp@bestk@basic@ratio\endcsname{0.89}
\expandafter\def\csname res@llmjp@bestk@basic@lo\endcsname{0.82}
\expandafter\def\csname res@llmjp@bestk@basic@hi\endcsname{0.96}
\expandafter\def\csname res@llmjp@bestk@mwis@ratio\endcsname{1.16}
\expandafter\def\csname res@llmjp@bestk@mwis@lo\endcsname{1.06}
\expandafter\def\csname res@llmjp@bestk@mwis@hi\endcsname{1.26}
\expandafter\def\csname res@llmjp@bestk@stepwise@ratio\endcsname{1.07}
\expandafter\def\csname res@llmjp@bestk@stepwise@lo\endcsname{0.99}
\expandafter\def\csname res@llmjp@bestk@stepwise@hi\endcsname{1.15}
\expandafter\def\csname res@llmjp@bestk@hubdrop@ratio\endcsname{1.10}
\expandafter\def\csname res@llmjp@bestk@hubdrop@lo\endcsname{1.02}
\expandafter\def\csname res@llmjp@bestk@hubdrop@hi\endcsname{1.19}
\expandafter\def\csname res@llmjp@bestk@syncpool@ratio\endcsname{1.61}
\expandafter\def\csname res@llmjp@bestk@syncpool@lo\endcsname{1.48}
\expandafter\def\csname res@llmjp@bestk@syncpool@hi\endcsname{1.74}
\expandafter\def\csname res@llmjp@bestk@las@ratio\endcsname{0.97}
\expandafter\def\csname res@llmjp@bestk@las@lo\endcsname{0.90}
\expandafter\def\csname res@llmjp@bestk@las@hi\endcsname{1.06}
\expandafter\def\csname res@all@bestk@native@min\endcsname{0.93}
\expandafter\def\csname res@all@bestk@native@max\endcsname{0.97}
\expandafter\def\csname res@all@bestk@native@lomin\endcsname{0.86}
\expandafter\def\csname res@all@bestk@basic@min\endcsname{0.63}
\expandafter\def\csname res@all@bestk@basic@max\endcsname{0.89}
\expandafter\def\csname res@all@bestk@basic@lomin\endcsname{0.58}
\expandafter\def\csname res@all@bestk@mwis@min\endcsname{1.05}
\expandafter\def\csname res@all@bestk@mwis@max\endcsname{1.19}
\expandafter\def\csname res@all@bestk@mwis@lomin\endcsname{1.00}
\expandafter\def\csname res@all@bestk@stepwise@min\endcsname{0.95}
\expandafter\def\csname res@all@bestk@stepwise@max\endcsname{1.07}
\expandafter\def\csname res@all@bestk@stepwise@lomin\endcsname{0.90}
\expandafter\def\csname res@all@bestk@hubdrop@min\endcsname{1.10}
\expandafter\def\csname res@all@bestk@hubdrop@max\endcsname{1.18}
\expandafter\def\csname res@all@bestk@hubdrop@lomin\endcsname{1.02}
\expandafter\def\csname res@all@bestk@syncpool@min\endcsname{1.29}
\expandafter\def\csname res@all@bestk@syncpool@max\endcsname{2.18}
\expandafter\def\csname res@all@bestk@syncpool@lomin\endcsname{1.16}
\expandafter\def\csname res@all@bestk@las@min\endcsname{0.93}
\expandafter\def\csname res@all@bestk@las@max\endcsname{0.97}
\expandafter\def\csname res@all@bestk@las@lomin\endcsname{0.87}
\expandafter\def\csname res@llama@time@native@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@native@16@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@native@16@plan\endcsname{0.5}
\expandafter\def\csname res@llama@time@native@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@native@16@sel\endcsname{2.2}
\expandafter\def\csname res@llama@time@native@16@total\endcsname{17.1}
\expandafter\def\csname res@llama@time@native@16@recv\endcsname{17.0}
\expandafter\def\csname res@llama@time@native@16@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@native@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@basic@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@basic@16@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@basic@16@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@basic@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@basic@16@sel\endcsname{2.4}
\expandafter\def\csname res@llama@time@basic@16@total\endcsname{17.3}
\expandafter\def\csname res@llama@time@basic@16@recv\endcsname{17.3}
\expandafter\def\csname res@llama@time@basic@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@basic@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@basic@16@filter\endcsname{0.2}
\expandafter\def\csname res@llama@time@mwis@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@mwis@16@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@mwis@16@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@mwis@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@mwis@16@sel\endcsname{2.4}
\expandafter\def\csname res@llama@time@mwis@16@total\endcsname{17.3}
\expandafter\def\csname res@llama@time@mwis@16@recv\endcsname{17.4}
\expandafter\def\csname res@llama@time@mwis@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@mwis@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@mwis@16@filter\endcsname{0.2}
\expandafter\def\csname res@llama@time@stepwise@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@stepwise@16@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@stepwise@16@plan\endcsname{2.6}
\expandafter\def\csname res@llama@time@stepwise@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@stepwise@16@sel\endcsname{4.2}
\expandafter\def\csname res@llama@time@stepwise@16@total\endcsname{19.1}
\expandafter\def\csname res@llama@time@stepwise@16@recv\endcsname{19.1}
\expandafter\def\csname res@llama@time@stepwise@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@stepwise@16@filter\endcsname{2.6}
\expandafter\def\csname res@llama@time@syncpool@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@syncpool@16@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@syncpool@16@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@syncpool@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@16@sel\endcsname{2.4}
\expandafter\def\csname res@llama@time@syncpool@16@total\endcsname{17.3}
\expandafter\def\csname res@llama@time@syncpool@16@recv\endcsname{17.4}
\expandafter\def\csname res@llama@time@syncpool@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@syncpool@16@group\endcsname{0.2}
\expandafter\def\csname res@llama@time@syncpool@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@coin@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@coin@16@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@coin@16@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@coin@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@16@sel\endcsname{2.4}
\expandafter\def\csname res@llama@time@coin@16@total\endcsname{17.3}
\expandafter\def\csname res@llama@time@coin@16@recv\endcsname{17.3}
\expandafter\def\csname res@llama@time@coin@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@coin@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@coin@16@prf\endcsname{0.0}
\expandafter\def\csname res@llama@time@coin@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@coin@16@proj\endcsname{0.1}
\expandafter\def\csname res@llama@time@hubdrop@16@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@hubdrop@16@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@hubdrop@16@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@hubdrop@16@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@16@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@hubdrop@16@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@hubdrop@16@recv\endcsname{17.4}
\expandafter\def\csname res@llama@time@hubdrop@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@hubdrop@16@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@hubdrop@16@group\endcsname{0.1}
\expandafter\def\csname res@llama@time@hubdrop@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@las@16@fwd\endcsname{23.1}
\expandafter\def\csname res@llama@time@las@16@law\endcsname{2.9}
\expandafter\def\csname res@llama@time@las@16@plan\endcsname{2.6}
\expandafter\def\csname res@llama@time@las@16@code\endcsname{0.6}
\expandafter\def\csname res@llama@time@las@16@sel\endcsname{6.1}
\expandafter\def\csname res@llama@time@las@16@total\endcsname{29.2}
\expandafter\def\csname res@llama@time@las@16@recv\endcsname{30.2}
\expandafter\def\csname res@llama@time@las@16@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@las@16@topk\endcsname{0.8}
\expandafter\def\csname res@llama@time@las@16@fwdpertok\endcsname{1.56}
\expandafter\def\csname res@llama@time@native@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@native@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@native@64@plan\endcsname{0.6}
\expandafter\def\csname res@llama@time@native@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@native@64@sel\endcsname{2.2}
\expandafter\def\csname res@llama@time@native@64@total\endcsname{17.1}
\expandafter\def\csname res@llama@time@native@64@recv\endcsname{17.1}
\expandafter\def\csname res@llama@time@native@64@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@native@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@basic@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@basic@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@basic@64@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@basic@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@basic@64@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@basic@64@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@basic@64@recv\endcsname{17.4}
\expandafter\def\csname res@llama@time@basic@64@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@basic@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@basic@64@filter\endcsname{0.3}
\expandafter\def\csname res@llama@time@mwis@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@mwis@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@mwis@64@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@mwis@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@mwis@64@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@mwis@64@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@mwis@64@recv\endcsname{17.5}
\expandafter\def\csname res@llama@time@mwis@64@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@mwis@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@mwis@64@filter\endcsname{0.3}
\expandafter\def\csname res@llama@time@stepwise@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@stepwise@64@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@stepwise@64@plan\endcsname{8.1}
\expandafter\def\csname res@llama@time@stepwise@64@code\endcsname{0.5}
\expandafter\def\csname res@llama@time@stepwise@64@sel\endcsname{9.8}
\expandafter\def\csname res@llama@time@stepwise@64@total\endcsname{24.7}
\expandafter\def\csname res@llama@time@stepwise@64@recv\endcsname{24.7}
\expandafter\def\csname res@llama@time@stepwise@64@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@stepwise@64@filter\endcsname{8.1}
\expandafter\def\csname res@llama@time@syncpool@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@syncpool@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@syncpool@64@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@syncpool@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@64@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@syncpool@64@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@syncpool@64@recv\endcsname{17.4}
\expandafter\def\csname res@llama@time@syncpool@64@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@syncpool@64@group\endcsname{0.2}
\expandafter\def\csname res@llama@time@syncpool@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@coin@64@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@coin@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@coin@64@plan\endcsname{0.8}
\expandafter\def\csname res@llama@time@coin@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@64@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@coin@64@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@coin@64@recv\endcsname{17.5}
\expandafter\def\csname res@llama@time@coin@64@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@coin@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@coin@64@prf\endcsname{0.0}
\expandafter\def\csname res@llama@time@coin@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@coin@64@proj\endcsname{0.1}
\expandafter\def\csname res@llama@time@hubdrop@64@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@hubdrop@64@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@hubdrop@64@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@hubdrop@64@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@64@sel\endcsname{2.6}
\expandafter\def\csname res@llama@time@hubdrop@64@total\endcsname{17.6}
\expandafter\def\csname res@llama@time@hubdrop@64@recv\endcsname{17.6}
\expandafter\def\csname res@llama@time@hubdrop@64@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@hubdrop@64@topk\endcsname{0.5}
\expandafter\def\csname res@llama@time@hubdrop@64@group\endcsname{0.1}
\expandafter\def\csname res@llama@time@hubdrop@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@las@64@fwd\endcsname{31.0}
\expandafter\def\csname res@llama@time@las@64@law\endcsname{3.8}
\expandafter\def\csname res@llama@time@las@64@plan\endcsname{4.0}
\expandafter\def\csname res@llama@time@las@64@code\endcsname{0.8}
\expandafter\def\csname res@llama@time@las@64@sel\endcsname{8.6}
\expandafter\def\csname res@llama@time@las@64@total\endcsname{39.6}
\expandafter\def\csname res@llama@time@las@64@recv\endcsname{40.8}
\expandafter\def\csname res@llama@time@las@64@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@las@64@topk\endcsname{1.1}
\expandafter\def\csname res@llama@time@las@64@fwdpertok\endcsname{2.08}
\expandafter\def\csname res@llama@time@native@256@fwd\endcsname{14.8}
\expandafter\def\csname res@llama@time@native@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@native@256@plan\endcsname{0.6}
\expandafter\def\csname res@llama@time@native@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@native@256@sel\endcsname{2.3}
\expandafter\def\csname res@llama@time@native@256@total\endcsname{17.1}
\expandafter\def\csname res@llama@time@native@256@recv\endcsname{17.1}
\expandafter\def\csname res@llama@time@native@256@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@native@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@basic@256@fwd\endcsname{14.8}
\expandafter\def\csname res@llama@time@basic@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@basic@256@plan\endcsname{1.4}
\expandafter\def\csname res@llama@time@basic@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@basic@256@sel\endcsname{3.0}
\expandafter\def\csname res@llama@time@basic@256@total\endcsname{17.8}
\expandafter\def\csname res@llama@time@basic@256@recv\endcsname{17.9}
\expandafter\def\csname res@llama@time@basic@256@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@basic@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@basic@256@filter\endcsname{0.7}
\expandafter\def\csname res@llama@time@mwis@256@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@mwis@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@mwis@256@plan\endcsname{1.0}
\expandafter\def\csname res@llama@time@mwis@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@mwis@256@sel\endcsname{2.7}
\expandafter\def\csname res@llama@time@mwis@256@total\endcsname{17.6}
\expandafter\def\csname res@llama@time@mwis@256@recv\endcsname{17.6}
\expandafter\def\csname res@llama@time@mwis@256@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@mwis@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@mwis@256@filter\endcsname{0.4}
\expandafter\def\csname res@llama@time@stepwise@256@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@stepwise@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@stepwise@256@plan\endcsname{31.1}
\expandafter\def\csname res@llama@time@stepwise@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@stepwise@256@sel\endcsname{32.7}
\expandafter\def\csname res@llama@time@stepwise@256@total\endcsname{47.6}
\expandafter\def\csname res@llama@time@stepwise@256@recv\endcsname{47.6}
\expandafter\def\csname res@llama@time@stepwise@256@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@stepwise@256@filter\endcsname{31.1}
\expandafter\def\csname res@llama@time@syncpool@256@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@syncpool@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@syncpool@256@plan\endcsname{1.0}
\expandafter\def\csname res@llama@time@syncpool@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@256@sel\endcsname{2.6}
\expandafter\def\csname res@llama@time@syncpool@256@total\endcsname{17.5}
\expandafter\def\csname res@llama@time@syncpool@256@recv\endcsname{17.6}
\expandafter\def\csname res@llama@time@syncpool@256@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@syncpool@256@group\endcsname{0.2}
\expandafter\def\csname res@llama@time@syncpool@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@coin@256@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@coin@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@coin@256@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@coin@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@256@sel\endcsname{2.6}
\expandafter\def\csname res@llama@time@coin@256@total\endcsname{17.5}
\expandafter\def\csname res@llama@time@coin@256@recv\endcsname{17.5}
\expandafter\def\csname res@llama@time@coin@256@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@coin@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@coin@256@prf\endcsname{0.0}
\expandafter\def\csname res@llama@time@coin@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@coin@256@proj\endcsname{0.1}
\expandafter\def\csname res@llama@time@hubdrop@256@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@hubdrop@256@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@hubdrop@256@plan\endcsname{1.1}
\expandafter\def\csname res@llama@time@hubdrop@256@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@256@sel\endcsname{2.8}
\expandafter\def\csname res@llama@time@hubdrop@256@total\endcsname{17.6}
\expandafter\def\csname res@llama@time@hubdrop@256@recv\endcsname{17.7}
\expandafter\def\csname res@llama@time@hubdrop@256@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@hubdrop@256@topk\endcsname{0.6}
\expandafter\def\csname res@llama@time@hubdrop@256@group\endcsname{0.2}
\expandafter\def\csname res@llama@time@hubdrop@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@las@256@fwd\endcsname{44.5}
\expandafter\def\csname res@llama@time@las@256@law\endcsname{5.7}
\expandafter\def\csname res@llama@time@las@256@plan\endcsname{6.9}
\expandafter\def\csname res@llama@time@las@256@code\endcsname{1.2}
\expandafter\def\csname res@llama@time@las@256@sel\endcsname{13.8}
\expandafter\def\csname res@llama@time@las@256@total\endcsname{58.3}
\expandafter\def\csname res@llama@time@las@256@recv\endcsname{59.8}
\expandafter\def\csname res@llama@time@las@256@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@las@256@topk\endcsname{1.8}
\expandafter\def\csname res@llama@time@las@256@fwdpertok\endcsname{2.98}
\expandafter\def\csname res@llama@time@native@1k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@native@1k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@native@1k@plan\endcsname{0.9}
\expandafter\def\csname res@llama@time@native@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@native@1k@sel\endcsname{2.5}
\expandafter\def\csname res@llama@time@native@1k@total\endcsname{17.4}
\expandafter\def\csname res@llama@time@native@1k@recv\endcsname{15.8}
\expandafter\def\csname res@llama@time@native@1k@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@native@1k@topk\endcsname{0.8}
\expandafter\def\csname res@llama@time@basic@1k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@basic@1k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@basic@1k@plan\endcsname{5.0}
\expandafter\def\csname res@llama@time@basic@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@basic@1k@sel\endcsname{6.7}
\expandafter\def\csname res@llama@time@basic@1k@total\endcsname{21.5}
\expandafter\def\csname res@llama@time@basic@1k@recv\endcsname{21.0}
\expandafter\def\csname res@llama@time@basic@1k@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@basic@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llama@time@basic@1k@filter\endcsname{3.8}
\expandafter\def\csname res@llama@time@mwis@1k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@mwis@1k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@mwis@1k@plan\endcsname{1.7}
\expandafter\def\csname res@llama@time@mwis@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@mwis@1k@sel\endcsname{3.3}
\expandafter\def\csname res@llama@time@mwis@1k@total\endcsname{18.2}
\expandafter\def\csname res@llama@time@mwis@1k@recv\endcsname{18.2}
\expandafter\def\csname res@llama@time@mwis@1k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@mwis@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llama@time@mwis@1k@filter\endcsname{0.6}
\expandafter\def\csname res@llama@time@stepwise@1k@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@stepwise@1k@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@stepwise@1k@plan\endcsname{127.8}
\expandafter\def\csname res@llama@time@stepwise@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@stepwise@1k@sel\endcsname{129.4}
\expandafter\def\csname res@llama@time@stepwise@1k@total\endcsname{144.4}
\expandafter\def\csname res@llama@time@stepwise@1k@recv\endcsname{144.1}
\expandafter\def\csname res@llama@time@stepwise@1k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@stepwise@1k@filter\endcsname{127.7}
\expandafter\def\csname res@llama@time@syncpool@1k@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@syncpool@1k@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@syncpool@1k@plan\endcsname{1.6}
\expandafter\def\csname res@llama@time@syncpool@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@1k@sel\endcsname{3.2}
\expandafter\def\csname res@llama@time@syncpool@1k@total\endcsname{18.2}
\expandafter\def\csname res@llama@time@syncpool@1k@recv\endcsname{18.2}
\expandafter\def\csname res@llama@time@syncpool@1k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@syncpool@1k@group\endcsname{0.5}
\expandafter\def\csname res@llama@time@syncpool@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llama@time@coin@1k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@coin@1k@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@coin@1k@plan\endcsname{1.3}
\expandafter\def\csname res@llama@time@coin@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@1k@sel\endcsname{3.0}
\expandafter\def\csname res@llama@time@coin@1k@total\endcsname{17.9}
\expandafter\def\csname res@llama@time@coin@1k@recv\endcsname{18.0}
\expandafter\def\csname res@llama@time@coin@1k@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@coin@1k@topk\endcsname{0.8}
\expandafter\def\csname res@llama@time@coin@1k@prf\endcsname{0.0}
\expandafter\def\csname res@llama@time@coin@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@coin@1k@proj\endcsname{0.2}
\expandafter\def\csname res@llama@time@hubdrop@1k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@hubdrop@1k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@hubdrop@1k@plan\endcsname{2.0}
\expandafter\def\csname res@llama@time@hubdrop@1k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@1k@sel\endcsname{3.6}
\expandafter\def\csname res@llama@time@hubdrop@1k@total\endcsname{18.5}
\expandafter\def\csname res@llama@time@hubdrop@1k@recv\endcsname{18.6}
\expandafter\def\csname res@llama@time@hubdrop@1k@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@hubdrop@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llama@time@hubdrop@1k@group\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@llama@time@las@1k@fwd\endcsname{57.8}
\expandafter\def\csname res@llama@time@las@1k@law\endcsname{8.1}
\expandafter\def\csname res@llama@time@las@1k@plan\endcsname{12.2}
\expandafter\def\csname res@llama@time@las@1k@code\endcsname{1.6}
\expandafter\def\csname res@llama@time@las@1k@sel\endcsname{21.9}
\expandafter\def\csname res@llama@time@las@1k@total\endcsname{79.7}
\expandafter\def\csname res@llama@time@las@1k@recv\endcsname{81.9}
\expandafter\def\csname res@llama@time@las@1k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@las@1k@topk\endcsname{3.1}
\expandafter\def\csname res@llama@time@las@1k@fwdpertok\endcsname{3.86}
\expandafter\def\csname res@llama@time@native@4k@fwd\endcsname{14.8}
\expandafter\def\csname res@llama@time@native@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@native@4k@plan\endcsname{1.5}
\expandafter\def\csname res@llama@time@native@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@native@4k@sel\endcsname{3.2}
\expandafter\def\csname res@llama@time@native@4k@total\endcsname{18.0}
\expandafter\def\csname res@llama@time@native@4k@recv\endcsname{18.1}
\expandafter\def\csname res@llama@time@native@4k@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@native@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llama@time@basic@4k@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@basic@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@basic@4k@plan\endcsname{25.5}
\expandafter\def\csname res@llama@time@basic@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@basic@4k@sel\endcsname{27.2}
\expandafter\def\csname res@llama@time@basic@4k@total\endcsname{42.3}
\expandafter\def\csname res@llama@time@basic@4k@recv\endcsname{42.3}
\expandafter\def\csname res@llama@time@basic@4k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@basic@4k@topk\endcsname{1.6}
\expandafter\def\csname res@llama@time@basic@4k@filter\endcsname{23.0}
\expandafter\def\csname res@llama@time@mwis@4k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@mwis@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@mwis@4k@plan\endcsname{3.9}
\expandafter\def\csname res@llama@time@mwis@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@mwis@4k@sel\endcsname{5.5}
\expandafter\def\csname res@llama@time@mwis@4k@total\endcsname{20.5}
\expandafter\def\csname res@llama@time@mwis@4k@recv\endcsname{20.4}
\expandafter\def\csname res@llama@time@mwis@4k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@mwis@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llama@time@mwis@4k@filter\endcsname{1.8}
\expandafter\def\csname res@llama@time@stepwise@4k@fwd\endcsname{15.3}
\expandafter\def\csname res@llama@time@stepwise@4k@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@stepwise@4k@plan\endcsname{513.4}
\expandafter\def\csname res@llama@time@stepwise@4k@code\endcsname{0.5}
\expandafter\def\csname res@llama@time@stepwise@4k@sel\endcsname{515.1}
\expandafter\def\csname res@llama@time@stepwise@4k@total\endcsname{530.4}
\expandafter\def\csname res@llama@time@stepwise@4k@recv\endcsname{528.9}
\expandafter\def\csname res@llama@time@stepwise@4k@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@stepwise@4k@filter\endcsname{513.4}
\expandafter\def\csname res@llama@time@syncpool@4k@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@syncpool@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@syncpool@4k@plan\endcsname{3.4}
\expandafter\def\csname res@llama@time@syncpool@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@4k@sel\endcsname{5.1}
\expandafter\def\csname res@llama@time@syncpool@4k@total\endcsname{20.1}
\expandafter\def\csname res@llama@time@syncpool@4k@recv\endcsname{20.1}
\expandafter\def\csname res@llama@time@syncpool@4k@prefill\endcsname{16.7}
\expandafter\def\csname res@llama@time@syncpool@4k@group\endcsname{1.7}
\expandafter\def\csname res@llama@time@syncpool@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llama@time@coin@4k@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@coin@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@coin@4k@plan\endcsname{2.5}
\expandafter\def\csname res@llama@time@coin@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@4k@sel\endcsname{4.2}
\expandafter\def\csname res@llama@time@coin@4k@total\endcsname{19.2}
\expandafter\def\csname res@llama@time@coin@4k@recv\endcsname{19.2}
\expandafter\def\csname res@llama@time@coin@4k@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@coin@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llama@time@coin@4k@prf\endcsname{0.1}
\expandafter\def\csname res@llama@time@coin@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@llama@time@coin@4k@proj\endcsname{0.7}
\expandafter\def\csname res@llama@time@hubdrop@4k@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@hubdrop@4k@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@hubdrop@4k@plan\endcsname{5.0}
\expandafter\def\csname res@llama@time@hubdrop@4k@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@hubdrop@4k@sel\endcsname{6.7}
\expandafter\def\csname res@llama@time@hubdrop@4k@total\endcsname{21.6}
\expandafter\def\csname res@llama@time@hubdrop@4k@recv\endcsname{21.6}
\expandafter\def\csname res@llama@time@hubdrop@4k@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@hubdrop@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llama@time@hubdrop@4k@group\endcsname{1.6}
\expandafter\def\csname res@llama@time@hubdrop@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@llama@time@las@4k@fwd\endcsname{67.8}
\expandafter\def\csname res@llama@time@las@4k@law\endcsname{12.7}
\expandafter\def\csname res@llama@time@las@4k@plan\endcsname{19.7}
\expandafter\def\csname res@llama@time@las@4k@code\endcsname{1.9}
\expandafter\def\csname res@llama@time@las@4k@sel\endcsname{34.3}
\expandafter\def\csname res@llama@time@las@4k@total\endcsname{102.0}
\expandafter\def\csname res@llama@time@las@4k@recv\endcsname{104.5}
\expandafter\def\csname res@llama@time@las@4k@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@las@4k@topk\endcsname{6.7}
\expandafter\def\csname res@llama@time@las@4k@fwdpertok\endcsname{4.51}
\expandafter\def\csname res@llama@time@native@Full@fwd\endcsname{14.9}
\expandafter\def\csname res@llama@time@native@Full@law\endcsname{1.3}
\expandafter\def\csname res@llama@time@native@Full@plan\endcsname{7.5}
\expandafter\def\csname res@llama@time@native@Full@code\endcsname{0.6}
\expandafter\def\csname res@llama@time@native@Full@sel\endcsname{9.3}
\expandafter\def\csname res@llama@time@native@Full@total\endcsname{24.2}
\expandafter\def\csname res@llama@time@native@Full@recv\endcsname{24.5}
\expandafter\def\csname res@llama@time@native@Full@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@native@Full@topk\endcsname{7.4}
\expandafter\def\csname res@llama@time@mwis@Full@fwd\endcsname{15.2}
\expandafter\def\csname res@llama@time@mwis@Full@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@mwis@Full@plan\endcsname{72.5}
\expandafter\def\csname res@llama@time@mwis@Full@code\endcsname{0.6}
\expandafter\def\csname res@llama@time@mwis@Full@sel\endcsname{74.3}
\expandafter\def\csname res@llama@time@mwis@Full@total\endcsname{89.5}
\expandafter\def\csname res@llama@time@mwis@Full@recv\endcsname{89.2}
\expandafter\def\csname res@llama@time@mwis@Full@prefill\endcsname{16.4}
\expandafter\def\csname res@llama@time@mwis@Full@topk\endcsname{7.4}
\expandafter\def\csname res@llama@time@mwis@Full@filter\endcsname{53.7}
\expandafter\def\csname res@llama@time@syncpool@Full@fwd\endcsname{15.0}
\expandafter\def\csname res@llama@time@syncpool@Full@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@syncpool@Full@plan\endcsname{71.8}
\expandafter\def\csname res@llama@time@syncpool@Full@code\endcsname{0.4}
\expandafter\def\csname res@llama@time@syncpool@Full@sel\endcsname{73.5}
\expandafter\def\csname res@llama@time@syncpool@Full@total\endcsname{88.5}
\expandafter\def\csname res@llama@time@syncpool@Full@recv\endcsname{88.4}
\expandafter\def\csname res@llama@time@syncpool@Full@prefill\endcsname{16.6}
\expandafter\def\csname res@llama@time@syncpool@Full@group\endcsname{58.4}
\expandafter\def\csname res@llama@time@syncpool@Full@topk\endcsname{7.4}
\expandafter\def\csname res@llama@time@coin@Full@fwd\endcsname{15.6}
\expandafter\def\csname res@llama@time@coin@Full@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@coin@Full@plan\endcsname{20.7}
\expandafter\def\csname res@llama@time@coin@Full@code\endcsname{0.6}
\expandafter\def\csname res@llama@time@coin@Full@sel\endcsname{22.5}
\expandafter\def\csname res@llama@time@coin@Full@total\endcsname{38.1}
\expandafter\def\csname res@llama@time@coin@Full@recv\endcsname{38.1}
\expandafter\def\csname res@llama@time@coin@Full@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@coin@Full@topk\endcsname{7.4}
\expandafter\def\csname res@llama@time@coin@Full@prf\endcsname{0.4}
\expandafter\def\csname res@llama@time@coin@Full@keylaw\endcsname{1.2}
\expandafter\def\csname res@llama@time@coin@Full@proj\endcsname{11.6}
\expandafter\def\csname res@llama@time@hubdrop@Full@fwd\endcsname{15.2}
\expandafter\def\csname res@llama@time@hubdrop@Full@law\endcsname{1.2}
\expandafter\def\csname res@llama@time@hubdrop@Full@plan\endcsname{120.7}
\expandafter\def\csname res@llama@time@hubdrop@Full@code\endcsname{0.5}
\expandafter\def\csname res@llama@time@hubdrop@Full@sel\endcsname{122.4}
\expandafter\def\csname res@llama@time@hubdrop@Full@total\endcsname{137.6}
\expandafter\def\csname res@llama@time@hubdrop@Full@recv\endcsname{137.9}
\expandafter\def\csname res@llama@time@hubdrop@Full@prefill\endcsname{16.5}
\expandafter\def\csname res@llama@time@hubdrop@Full@topk\endcsname{7.4}
\expandafter\def\csname res@llama@time@hubdrop@Full@group\endcsname{57.6}
\expandafter\def\csname res@llama@time@hubdrop@Full@keylaw\endcsname{1.3}
\expandafter\def\csname res@llama@time@las@Full@fwd\endcsname{72.2}
\expandafter\def\csname res@llama@time@las@Full@law\endcsname{41.8}
\expandafter\def\csname res@llama@time@las@Full@plan\endcsname{22.3}
\expandafter\def\csname res@llama@time@las@Full@code\endcsname{2.2}
\expandafter\def\csname res@llama@time@las@Full@sel\endcsname{66.3}
\expandafter\def\csname res@llama@time@las@Full@total\endcsname{138.5}
\expandafter\def\csname res@llama@time@las@Full@recv\endcsname{143.1}
\expandafter\def\csname res@llama@time@las@Full@prefill\endcsname{16.7}
\expandafter\def\csname res@llama@time@las@Full@topk\endcsname{33.5}
\expandafter\def\csname res@llama@time@las@Full@fwdpertok\endcsname{4.74}
\expandafter\def\csname res@llama@time@lascoin@Full@ratio\endcsname{3.6}
\expandafter\def\csname res@llama@time@basic@16@relnative\endcsname{1.01}
\expandafter\def\csname res@llama@time@mwis@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@stepwise@16@relnative\endcsname{1.12}
\expandafter\def\csname res@llama@time@syncpool@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@coin@16@relnative\endcsname{1.01}
\expandafter\def\csname res@llama@time@hubdrop@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@las@16@relnative\endcsname{1.71}
\expandafter\def\csname res@llama@time@basic@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@mwis@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@stepwise@64@relnative\endcsname{1.45}
\expandafter\def\csname res@llama@time@syncpool@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@coin@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@hubdrop@64@relnative\endcsname{1.03}
\expandafter\def\csname res@llama@time@las@64@relnative\endcsname{2.32}
\expandafter\def\csname res@llama@time@basic@256@relnative\endcsname{1.04}
\expandafter\def\csname res@llama@time@mwis@256@relnative\endcsname{1.03}
\expandafter\def\csname res@llama@time@stepwise@256@relnative\endcsname{2.79}
\expandafter\def\csname res@llama@time@syncpool@256@relnative\endcsname{1.03}
\expandafter\def\csname res@llama@time@coin@256@relnative\endcsname{1.02}
\expandafter\def\csname res@llama@time@hubdrop@256@relnative\endcsname{1.03}
\expandafter\def\csname res@llama@time@las@256@relnative\endcsname{3.41}
\expandafter\def\csname res@llama@time@basic@1k@relnative\endcsname{1.24}
\expandafter\def\csname res@llama@time@mwis@1k@relnative\endcsname{1.05}
\expandafter\def\csname res@llama@time@stepwise@1k@relnative\endcsname{8.30}
\expandafter\def\csname res@llama@time@syncpool@1k@relnative\endcsname{1.05}
\expandafter\def\csname res@llama@time@coin@1k@relnative\endcsname{1.03}
\expandafter\def\csname res@llama@time@hubdrop@1k@relnative\endcsname{1.07}
\expandafter\def\csname res@llama@time@las@1k@relnative\endcsname{4.58}
\expandafter\def\csname res@llama@time@basic@4k@relnative\endcsname{2.34}
\expandafter\def\csname res@llama@time@mwis@4k@relnative\endcsname{1.14}
\expandafter\def\csname res@llama@time@stepwise@4k@relnative\endcsname{29.43}
\expandafter\def\csname res@llama@time@syncpool@4k@relnative\endcsname{1.11}
\expandafter\def\csname res@llama@time@coin@4k@relnative\endcsname{1.07}
\expandafter\def\csname res@llama@time@hubdrop@4k@relnative\endcsname{1.20}
\expandafter\def\csname res@llama@time@las@4k@relnative\endcsname{5.66}
\expandafter\def\csname res@llama@time@mwis@Full@relnative\endcsname{3.69}
\expandafter\def\csname res@llama@time@syncpool@Full@relnative\endcsname{3.65}
\expandafter\def\csname res@llama@time@coin@Full@relnative\endcsname{1.57}
\expandafter\def\csname res@llama@time@hubdrop@Full@relnative\endcsname{5.68}
\expandafter\def\csname res@llama@time@las@Full@relnative\endcsname{5.72}
\expandafter\def\csname res@llama@time@any@gpu\endcsname{GeForce RTX 5090}
\expandafter\def\csname res@qwen@time@native@16@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@native@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@16@plan\endcsname{0.6}
\expandafter\def\csname res@qwen@time@native@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@native@16@sel\endcsname{2.5}
\expandafter\def\csname res@qwen@time@native@16@total\endcsname{23.8}
\expandafter\def\csname res@qwen@time@native@16@recv\endcsname{22.7}
\expandafter\def\csname res@qwen@time@native@16@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@native@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@basic@16@fwd\endcsname{21.1}
\expandafter\def\csname res@qwen@time@basic@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@basic@16@plan\endcsname{0.8}
\expandafter\def\csname res@qwen@time@basic@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@basic@16@sel\endcsname{2.7}
\expandafter\def\csname res@qwen@time@basic@16@total\endcsname{23.8}
\expandafter\def\csname res@qwen@time@basic@16@recv\endcsname{23.9}
\expandafter\def\csname res@qwen@time@basic@16@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@basic@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@basic@16@filter\endcsname{0.2}
\expandafter\def\csname res@qwen@time@mwis@16@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@mwis@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@mwis@16@plan\endcsname{0.9}
\expandafter\def\csname res@qwen@time@mwis@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@mwis@16@sel\endcsname{2.7}
\expandafter\def\csname res@qwen@time@mwis@16@total\endcsname{23.9}
\expandafter\def\csname res@qwen@time@mwis@16@recv\endcsname{24.0}
\expandafter\def\csname res@qwen@time@mwis@16@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@mwis@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@mwis@16@filter\endcsname{0.2}
\expandafter\def\csname res@qwen@time@stepwise@16@fwd\endcsname{21.1}
\expandafter\def\csname res@qwen@time@stepwise@16@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@stepwise@16@plan\endcsname{2.6}
\expandafter\def\csname res@qwen@time@stepwise@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@stepwise@16@sel\endcsname{4.4}
\expandafter\def\csname res@qwen@time@stepwise@16@total\endcsname{25.5}
\expandafter\def\csname res@qwen@time@stepwise@16@recv\endcsname{25.5}
\expandafter\def\csname res@qwen@time@stepwise@16@prefill\endcsname{22.5}
\expandafter\def\csname res@qwen@time@stepwise@16@filter\endcsname{2.5}
\expandafter\def\csname res@qwen@time@syncpool@16@fwd\endcsname{21.1}
\expandafter\def\csname res@qwen@time@syncpool@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@16@plan\endcsname{0.9}
\expandafter\def\csname res@qwen@time@syncpool@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@16@sel\endcsname{2.7}
\expandafter\def\csname res@qwen@time@syncpool@16@total\endcsname{23.9}
\expandafter\def\csname res@qwen@time@syncpool@16@recv\endcsname{24.0}
\expandafter\def\csname res@qwen@time@syncpool@16@prefill\endcsname{22.5}
\expandafter\def\csname res@qwen@time@syncpool@16@group\endcsname{0.2}
\expandafter\def\csname res@qwen@time@syncpool@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@coin@16@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@coin@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@16@plan\endcsname{0.9}
\expandafter\def\csname res@qwen@time@coin@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@coin@16@sel\endcsname{2.7}
\expandafter\def\csname res@qwen@time@coin@16@total\endcsname{23.9}
\expandafter\def\csname res@qwen@time@coin@16@recv\endcsname{24.1}
\expandafter\def\csname res@qwen@time@coin@16@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@coin@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@coin@16@prf\endcsname{0.0}
\expandafter\def\csname res@qwen@time@coin@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@coin@16@proj\endcsname{0.1}
\expandafter\def\csname res@qwen@time@hubdrop@16@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@hubdrop@16@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@16@plan\endcsname{1.0}
\expandafter\def\csname res@qwen@time@hubdrop@16@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@16@sel\endcsname{2.8}
\expandafter\def\csname res@qwen@time@hubdrop@16@total\endcsname{24.1}
\expandafter\def\csname res@qwen@time@hubdrop@16@recv\endcsname{24.2}
\expandafter\def\csname res@qwen@time@hubdrop@16@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@hubdrop@16@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@hubdrop@16@group\endcsname{0.1}
\expandafter\def\csname res@qwen@time@hubdrop@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@las@16@fwd\endcsname{26.6}
\expandafter\def\csname res@qwen@time@las@16@law\endcsname{2.7}
\expandafter\def\csname res@qwen@time@las@16@plan\endcsname{2.5}
\expandafter\def\csname res@qwen@time@las@16@code\endcsname{0.5}
\expandafter\def\csname res@qwen@time@las@16@sel\endcsname{5.7}
\expandafter\def\csname res@qwen@time@las@16@total\endcsname{32.3}
\expandafter\def\csname res@qwen@time@las@16@recv\endcsname{33.4}
\expandafter\def\csname res@qwen@time@las@16@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@las@16@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@las@16@fwdpertok\endcsname{1.24}
\expandafter\def\csname res@qwen@time@native@64@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@native@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@64@plan\endcsname{0.7}
\expandafter\def\csname res@qwen@time@native@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@native@64@sel\endcsname{2.6}
\expandafter\def\csname res@qwen@time@native@64@total\endcsname{23.9}
\expandafter\def\csname res@qwen@time@native@64@recv\endcsname{21.6}
\expandafter\def\csname res@qwen@time@native@64@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@native@64@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@basic@64@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@basic@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@basic@64@plan\endcsname{1.0}
\expandafter\def\csname res@qwen@time@basic@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@basic@64@sel\endcsname{2.9}
\expandafter\def\csname res@qwen@time@basic@64@total\endcsname{24.2}
\expandafter\def\csname res@qwen@time@basic@64@recv\endcsname{24.2}
\expandafter\def\csname res@qwen@time@basic@64@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@basic@64@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@basic@64@filter\endcsname{0.3}
\expandafter\def\csname res@qwen@time@mwis@64@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@mwis@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@mwis@64@plan\endcsname{1.0}
\expandafter\def\csname res@qwen@time@mwis@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@mwis@64@sel\endcsname{2.9}
\expandafter\def\csname res@qwen@time@mwis@64@total\endcsname{24.2}
\expandafter\def\csname res@qwen@time@mwis@64@recv\endcsname{24.3}
\expandafter\def\csname res@qwen@time@mwis@64@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@mwis@64@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@mwis@64@filter\endcsname{0.3}
\expandafter\def\csname res@qwen@time@stepwise@64@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@stepwise@64@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@stepwise@64@plan\endcsname{7.7}
\expandafter\def\csname res@qwen@time@stepwise@64@code\endcsname{0.5}
\expandafter\def\csname res@qwen@time@stepwise@64@sel\endcsname{9.6}
\expandafter\def\csname res@qwen@time@stepwise@64@total\endcsname{31.0}
\expandafter\def\csname res@qwen@time@stepwise@64@recv\endcsname{31.2}
\expandafter\def\csname res@qwen@time@stepwise@64@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@stepwise@64@filter\endcsname{7.6}
\expandafter\def\csname res@qwen@time@syncpool@64@fwd\endcsname{21.5}
\expandafter\def\csname res@qwen@time@syncpool@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@64@plan\endcsname{1.0}
\expandafter\def\csname res@qwen@time@syncpool@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@64@sel\endcsname{2.8}
\expandafter\def\csname res@qwen@time@syncpool@64@total\endcsname{24.3}
\expandafter\def\csname res@qwen@time@syncpool@64@recv\endcsname{24.4}
\expandafter\def\csname res@qwen@time@syncpool@64@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@syncpool@64@group\endcsname{0.2}
\expandafter\def\csname res@qwen@time@syncpool@64@topk\endcsname{0.6}
\expandafter\def\csname res@qwen@time@coin@64@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@coin@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@64@plan\endcsname{0.9}
\expandafter\def\csname res@qwen@time@coin@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@coin@64@sel\endcsname{2.8}
\expandafter\def\csname res@qwen@time@coin@64@total\endcsname{24.1}
\expandafter\def\csname res@qwen@time@coin@64@recv\endcsname{24.3}
\expandafter\def\csname res@qwen@time@coin@64@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@coin@64@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@coin@64@prf\endcsname{0.0}
\expandafter\def\csname res@qwen@time@coin@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@coin@64@proj\endcsname{0.1}
\expandafter\def\csname res@qwen@time@hubdrop@64@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@hubdrop@64@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@64@plan\endcsname{1.1}
\expandafter\def\csname res@qwen@time@hubdrop@64@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@64@sel\endcsname{2.9}
\expandafter\def\csname res@qwen@time@hubdrop@64@total\endcsname{24.3}
\expandafter\def\csname res@qwen@time@hubdrop@64@recv\endcsname{24.4}
\expandafter\def\csname res@qwen@time@hubdrop@64@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@hubdrop@64@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@hubdrop@64@group\endcsname{0.1}
\expandafter\def\csname res@qwen@time@hubdrop@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@las@64@fwd\endcsname{29.2}
\expandafter\def\csname res@qwen@time@las@64@law\endcsname{3.0}
\expandafter\def\csname res@qwen@time@las@64@plan\endcsname{3.3}
\expandafter\def\csname res@qwen@time@las@64@code\endcsname{0.6}
\expandafter\def\csname res@qwen@time@las@64@sel\endcsname{6.9}
\expandafter\def\csname res@qwen@time@las@64@total\endcsname{36.1}
\expandafter\def\csname res@qwen@time@las@64@recv\endcsname{37.2}
\expandafter\def\csname res@qwen@time@las@64@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@las@64@topk\endcsname{0.9}
\expandafter\def\csname res@qwen@time@las@64@fwdpertok\endcsname{1.37}
\expandafter\def\csname res@qwen@time@native@256@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@native@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@256@plan\endcsname{0.7}
\expandafter\def\csname res@qwen@time@native@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@native@256@sel\endcsname{2.6}
\expandafter\def\csname res@qwen@time@native@256@total\endcsname{23.8}
\expandafter\def\csname res@qwen@time@native@256@recv\endcsname{23.9}
\expandafter\def\csname res@qwen@time@native@256@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@native@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@basic@256@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@basic@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@basic@256@plan\endcsname{1.4}
\expandafter\def\csname res@qwen@time@basic@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@basic@256@sel\endcsname{3.2}
\expandafter\def\csname res@qwen@time@basic@256@total\endcsname{24.5}
\expandafter\def\csname res@qwen@time@basic@256@recv\endcsname{24.7}
\expandafter\def\csname res@qwen@time@basic@256@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@basic@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@basic@256@filter\endcsname{0.6}
\expandafter\def\csname res@qwen@time@mwis@256@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@mwis@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@mwis@256@plan\endcsname{1.1}
\expandafter\def\csname res@qwen@time@mwis@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@mwis@256@sel\endcsname{3.0}
\expandafter\def\csname res@qwen@time@mwis@256@total\endcsname{24.2}
\expandafter\def\csname res@qwen@time@mwis@256@recv\endcsname{24.3}
\expandafter\def\csname res@qwen@time@mwis@256@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@mwis@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@mwis@256@filter\endcsname{0.3}
\expandafter\def\csname res@qwen@time@stepwise@256@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@stepwise@256@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@stepwise@256@plan\endcsname{31.2}
\expandafter\def\csname res@qwen@time@stepwise@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@stepwise@256@sel\endcsname{33.0}
\expandafter\def\csname res@qwen@time@stepwise@256@total\endcsname{54.3}
\expandafter\def\csname res@qwen@time@stepwise@256@recv\endcsname{54.3}
\expandafter\def\csname res@qwen@time@stepwise@256@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@stepwise@256@filter\endcsname{31.1}
\expandafter\def\csname res@qwen@time@syncpool@256@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@syncpool@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@256@plan\endcsname{1.1}
\expandafter\def\csname res@qwen@time@syncpool@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@256@sel\endcsname{3.0}
\expandafter\def\csname res@qwen@time@syncpool@256@total\endcsname{24.3}
\expandafter\def\csname res@qwen@time@syncpool@256@recv\endcsname{24.3}
\expandafter\def\csname res@qwen@time@syncpool@256@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@syncpool@256@group\endcsname{0.3}
\expandafter\def\csname res@qwen@time@syncpool@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@coin@256@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@coin@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@256@plan\endcsname{1.0}
\expandafter\def\csname res@qwen@time@coin@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@coin@256@sel\endcsname{2.9}
\expandafter\def\csname res@qwen@time@coin@256@total\endcsname{24.1}
\expandafter\def\csname res@qwen@time@coin@256@recv\endcsname{24.2}
\expandafter\def\csname res@qwen@time@coin@256@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@coin@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@coin@256@prf\endcsname{0.0}
\expandafter\def\csname res@qwen@time@coin@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@coin@256@proj\endcsname{0.1}
\expandafter\def\csname res@qwen@time@hubdrop@256@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@hubdrop@256@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@256@plan\endcsname{1.2}
\expandafter\def\csname res@qwen@time@hubdrop@256@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@256@sel\endcsname{3.1}
\expandafter\def\csname res@qwen@time@hubdrop@256@total\endcsname{24.3}
\expandafter\def\csname res@qwen@time@hubdrop@256@recv\endcsname{24.4}
\expandafter\def\csname res@qwen@time@hubdrop@256@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@hubdrop@256@topk\endcsname{0.7}
\expandafter\def\csname res@qwen@time@hubdrop@256@group\endcsname{0.2}
\expandafter\def\csname res@qwen@time@hubdrop@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@las@256@fwd\endcsname{32.8}
\expandafter\def\csname res@qwen@time@las@256@law\endcsname{3.5}
\expandafter\def\csname res@qwen@time@las@256@plan\endcsname{5.2}
\expandafter\def\csname res@qwen@time@las@256@code\endcsname{0.6}
\expandafter\def\csname res@qwen@time@las@256@sel\endcsname{9.3}
\expandafter\def\csname res@qwen@time@las@256@total\endcsname{42.1}
\expandafter\def\csname res@qwen@time@las@256@recv\endcsname{43.3}
\expandafter\def\csname res@qwen@time@las@256@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@las@256@topk\endcsname{1.1}
\expandafter\def\csname res@qwen@time@las@256@fwdpertok\endcsname{1.54}
\expandafter\def\csname res@qwen@time@native@1k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@native@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@1k@plan\endcsname{1.1}
\expandafter\def\csname res@qwen@time@native@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@native@1k@sel\endcsname{3.0}
\expandafter\def\csname res@qwen@time@native@1k@total\endcsname{24.2}
\expandafter\def\csname res@qwen@time@native@1k@recv\endcsname{24.2}
\expandafter\def\csname res@qwen@time@native@1k@prefill\endcsname{22.9}
\expandafter\def\csname res@qwen@time@native@1k@topk\endcsname{1.1}
\expandafter\def\csname res@qwen@time@basic@1k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@basic@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@basic@1k@plan\endcsname{4.5}
\expandafter\def\csname res@qwen@time@basic@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@basic@1k@sel\endcsname{6.4}
\expandafter\def\csname res@qwen@time@basic@1k@total\endcsname{27.6}
\expandafter\def\csname res@qwen@time@basic@1k@recv\endcsname{27.0}
\expandafter\def\csname res@qwen@time@basic@1k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@basic@1k@topk\endcsname{1.0}
\expandafter\def\csname res@qwen@time@basic@1k@filter\endcsname{3.2}
\expandafter\def\csname res@qwen@time@mwis@1k@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@mwis@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@mwis@1k@plan\endcsname{1.7}
\expandafter\def\csname res@qwen@time@mwis@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@mwis@1k@sel\endcsname{3.6}
\expandafter\def\csname res@qwen@time@mwis@1k@total\endcsname{24.9}
\expandafter\def\csname res@qwen@time@mwis@1k@recv\endcsname{24.9}
\expandafter\def\csname res@qwen@time@mwis@1k@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@mwis@1k@topk\endcsname{1.0}
\expandafter\def\csname res@qwen@time@mwis@1k@filter\endcsname{0.5}
\expandafter\def\csname res@qwen@time@stepwise@1k@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@stepwise@1k@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@stepwise@1k@plan\endcsname{118.5}
\expandafter\def\csname res@qwen@time@stepwise@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@stepwise@1k@sel\endcsname{120.3}
\expandafter\def\csname res@qwen@time@stepwise@1k@total\endcsname{141.7}
\expandafter\def\csname res@qwen@time@stepwise@1k@recv\endcsname{141.5}
\expandafter\def\csname res@qwen@time@stepwise@1k@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@stepwise@1k@filter\endcsname{118.5}
\expandafter\def\csname res@qwen@time@syncpool@1k@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@syncpool@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@1k@plan\endcsname{1.8}
\expandafter\def\csname res@qwen@time@syncpool@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@1k@sel\endcsname{3.7}
\expandafter\def\csname res@qwen@time@syncpool@1k@total\endcsname{25.0}
\expandafter\def\csname res@qwen@time@syncpool@1k@recv\endcsname{25.1}
\expandafter\def\csname res@qwen@time@syncpool@1k@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@syncpool@1k@group\endcsname{0.6}
\expandafter\def\csname res@qwen@time@syncpool@1k@topk\endcsname{1.0}
\expandafter\def\csname res@qwen@time@coin@1k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@coin@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@1k@plan\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@coin@1k@sel\endcsname{3.3}
\expandafter\def\csname res@qwen@time@coin@1k@total\endcsname{24.6}
\expandafter\def\csname res@qwen@time@coin@1k@recv\endcsname{24.7}
\expandafter\def\csname res@qwen@time@coin@1k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@coin@1k@topk\endcsname{1.0}
\expandafter\def\csname res@qwen@time@coin@1k@prf\endcsname{0.0}
\expandafter\def\csname res@qwen@time@coin@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@coin@1k@proj\endcsname{0.2}
\expandafter\def\csname res@qwen@time@hubdrop@1k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@hubdrop@1k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@1k@plan\endcsname{2.1}
\expandafter\def\csname res@qwen@time@hubdrop@1k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@1k@sel\endcsname{4.0}
\expandafter\def\csname res@qwen@time@hubdrop@1k@total\endcsname{25.2}
\expandafter\def\csname res@qwen@time@hubdrop@1k@recv\endcsname{25.3}
\expandafter\def\csname res@qwen@time@hubdrop@1k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@hubdrop@1k@topk\endcsname{1.1}
\expandafter\def\csname res@qwen@time@hubdrop@1k@group\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@qwen@time@las@1k@fwd\endcsname{36.2}
\expandafter\def\csname res@qwen@time@las@1k@law\endcsname{4.5}
\expandafter\def\csname res@qwen@time@las@1k@plan\endcsname{12.2}
\expandafter\def\csname res@qwen@time@las@1k@code\endcsname{0.7}
\expandafter\def\csname res@qwen@time@las@1k@sel\endcsname{17.4}
\expandafter\def\csname res@qwen@time@las@1k@total\endcsname{53.6}
\expandafter\def\csname res@qwen@time@las@1k@recv\endcsname{55.2}
\expandafter\def\csname res@qwen@time@las@1k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@las@1k@topk\endcsname{1.8}
\expandafter\def\csname res@qwen@time@las@1k@fwdpertok\endcsname{1.70}
\expandafter\def\csname res@qwen@time@native@4k@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@native@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@4k@plan\endcsname{1.6}
\expandafter\def\csname res@qwen@time@native@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@native@4k@sel\endcsname{3.5}
\expandafter\def\csname res@qwen@time@native@4k@total\endcsname{24.9}
\expandafter\def\csname res@qwen@time@native@4k@recv\endcsname{24.9}
\expandafter\def\csname res@qwen@time@native@4k@prefill\endcsname{22.9}
\expandafter\def\csname res@qwen@time@native@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@basic@4k@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@basic@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@basic@4k@plan\endcsname{21.2}
\expandafter\def\csname res@qwen@time@basic@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@basic@4k@sel\endcsname{23.1}
\expandafter\def\csname res@qwen@time@basic@4k@total\endcsname{44.5}
\expandafter\def\csname res@qwen@time@basic@4k@recv\endcsname{44.3}
\expandafter\def\csname res@qwen@time@basic@4k@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@basic@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@basic@4k@filter\endcsname{18.7}
\expandafter\def\csname res@qwen@time@mwis@4k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@mwis@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@mwis@4k@plan\endcsname{3.4}
\expandafter\def\csname res@qwen@time@mwis@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@mwis@4k@sel\endcsname{5.3}
\expandafter\def\csname res@qwen@time@mwis@4k@total\endcsname{26.5}
\expandafter\def\csname res@qwen@time@mwis@4k@recv\endcsname{26.5}
\expandafter\def\csname res@qwen@time@mwis@4k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@mwis@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@mwis@4k@filter\endcsname{1.3}
\expandafter\def\csname res@qwen@time@stepwise@4k@fwd\endcsname{21.6}
\expandafter\def\csname res@qwen@time@stepwise@4k@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@stepwise@4k@plan\endcsname{476.8}
\expandafter\def\csname res@qwen@time@stepwise@4k@code\endcsname{0.5}
\expandafter\def\csname res@qwen@time@stepwise@4k@sel\endcsname{478.6}
\expandafter\def\csname res@qwen@time@stepwise@4k@total\endcsname{500.3}
\expandafter\def\csname res@qwen@time@stepwise@4k@recv\endcsname{500.7}
\expandafter\def\csname res@qwen@time@stepwise@4k@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@stepwise@4k@filter\endcsname{476.7}
\expandafter\def\csname res@qwen@time@syncpool@4k@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@syncpool@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@4k@plan\endcsname{3.8}
\expandafter\def\csname res@qwen@time@syncpool@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@4k@sel\endcsname{5.7}
\expandafter\def\csname res@qwen@time@syncpool@4k@total\endcsname{27.1}
\expandafter\def\csname res@qwen@time@syncpool@4k@recv\endcsname{27.2}
\expandafter\def\csname res@qwen@time@syncpool@4k@prefill\endcsname{23.0}
\expandafter\def\csname res@qwen@time@syncpool@4k@group\endcsname{1.7}
\expandafter\def\csname res@qwen@time@syncpool@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@coin@4k@fwd\endcsname{21.3}
\expandafter\def\csname res@qwen@time@coin@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@4k@plan\endcsname{2.4}
\expandafter\def\csname res@qwen@time@coin@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@coin@4k@sel\endcsname{4.3}
\expandafter\def\csname res@qwen@time@coin@4k@total\endcsname{25.6}
\expandafter\def\csname res@qwen@time@coin@4k@recv\endcsname{25.6}
\expandafter\def\csname res@qwen@time@coin@4k@prefill\endcsname{22.7}
\expandafter\def\csname res@qwen@time@coin@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@coin@4k@prf\endcsname{0.1}
\expandafter\def\csname res@qwen@time@coin@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@qwen@time@coin@4k@proj\endcsname{0.5}
\expandafter\def\csname res@qwen@time@hubdrop@4k@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@hubdrop@4k@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@4k@plan\endcsname{4.6}
\expandafter\def\csname res@qwen@time@hubdrop@4k@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@hubdrop@4k@sel\endcsname{6.5}
\expandafter\def\csname res@qwen@time@hubdrop@4k@total\endcsname{27.7}
\expandafter\def\csname res@qwen@time@hubdrop@4k@recv\endcsname{27.8}
\expandafter\def\csname res@qwen@time@hubdrop@4k@prefill\endcsname{22.5}
\expandafter\def\csname res@qwen@time@hubdrop@4k@topk\endcsname{1.6}
\expandafter\def\csname res@qwen@time@hubdrop@4k@group\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@qwen@time@las@4k@fwd\endcsname{49.3}
\expandafter\def\csname res@qwen@time@las@4k@law\endcsname{7.4}
\expandafter\def\csname res@qwen@time@las@4k@plan\endcsname{36.8}
\expandafter\def\csname res@qwen@time@las@4k@code\endcsname{1.1}
\expandafter\def\csname res@qwen@time@las@4k@sel\endcsname{45.3}
\expandafter\def\csname res@qwen@time@las@4k@total\endcsname{94.6}
\expandafter\def\csname res@qwen@time@las@4k@recv\endcsname{97.2}
\expandafter\def\csname res@qwen@time@las@4k@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@las@4k@topk\endcsname{3.7}
\expandafter\def\csname res@qwen@time@las@4k@fwdpertok\endcsname{2.31}
\expandafter\def\csname res@qwen@time@native@Full@fwd\endcsname{21.2}
\expandafter\def\csname res@qwen@time@native@Full@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@native@Full@plan\endcsname{7.4}
\expandafter\def\csname res@qwen@time@native@Full@code\endcsname{0.6}
\expandafter\def\csname res@qwen@time@native@Full@sel\endcsname{9.5}
\expandafter\def\csname res@qwen@time@native@Full@total\endcsname{30.7}
\expandafter\def\csname res@qwen@time@native@Full@recv\endcsname{31.0}
\expandafter\def\csname res@qwen@time@native@Full@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@native@Full@topk\endcsname{7.3}
\expandafter\def\csname res@qwen@time@mwis@Full@fwd\endcsname{21.6}
\expandafter\def\csname res@qwen@time@mwis@Full@law\endcsname{1.4}
\expandafter\def\csname res@qwen@time@mwis@Full@plan\endcsname{81.9}
\expandafter\def\csname res@qwen@time@mwis@Full@code\endcsname{0.6}
\expandafter\def\csname res@qwen@time@mwis@Full@sel\endcsname{83.9}
\expandafter\def\csname res@qwen@time@mwis@Full@total\endcsname{105.5}
\expandafter\def\csname res@qwen@time@mwis@Full@recv\endcsname{105.3}
\expandafter\def\csname res@qwen@time@mwis@Full@prefill\endcsname{22.6}
\expandafter\def\csname res@qwen@time@mwis@Full@topk\endcsname{7.5}
\expandafter\def\csname res@qwen@time@mwis@Full@filter\endcsname{61.4}
\expandafter\def\csname res@qwen@time@syncpool@Full@fwd\endcsname{21.4}
\expandafter\def\csname res@qwen@time@syncpool@Full@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@syncpool@Full@plan\endcsname{85.2}
\expandafter\def\csname res@qwen@time@syncpool@Full@code\endcsname{0.4}
\expandafter\def\csname res@qwen@time@syncpool@Full@sel\endcsname{87.0}
\expandafter\def\csname res@qwen@time@syncpool@Full@total\endcsname{108.4}
\expandafter\def\csname res@qwen@time@syncpool@Full@recv\endcsname{108.4}
\expandafter\def\csname res@qwen@time@syncpool@Full@prefill\endcsname{22.9}
\expandafter\def\csname res@qwen@time@syncpool@Full@group\endcsname{70.0}
\expandafter\def\csname res@qwen@time@syncpool@Full@topk\endcsname{7.4}
\expandafter\def\csname res@qwen@time@coin@Full@fwd\endcsname{21.5}
\expandafter\def\csname res@qwen@time@coin@Full@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@Full@plan\endcsname{22.1}
\expandafter\def\csname res@qwen@time@coin@Full@code\endcsname{0.6}
\expandafter\def\csname res@qwen@time@coin@Full@sel\endcsname{24.1}
\expandafter\def\csname res@qwen@time@coin@Full@total\endcsname{45.6}
\expandafter\def\csname res@qwen@time@coin@Full@recv\endcsname{45.7}
\expandafter\def\csname res@qwen@time@coin@Full@prefill\endcsname{22.9}
\expandafter\def\csname res@qwen@time@coin@Full@topk\endcsname{7.2}
\expandafter\def\csname res@qwen@time@coin@Full@prf\endcsname{0.5}
\expandafter\def\csname res@qwen@time@coin@Full@keylaw\endcsname{1.5}
\expandafter\def\csname res@qwen@time@coin@Full@proj\endcsname{12.9}
\expandafter\def\csname res@qwen@time@hubdrop@Full@fwd\endcsname{21.8}
\expandafter\def\csname res@qwen@time@hubdrop@Full@law\endcsname{1.5}
\expandafter\def\csname res@qwen@time@hubdrop@Full@plan\endcsname{140.8}
\expandafter\def\csname res@qwen@time@hubdrop@Full@code\endcsname{0.5}
\expandafter\def\csname res@qwen@time@hubdrop@Full@sel\endcsname{142.8}
\expandafter\def\csname res@qwen@time@hubdrop@Full@total\endcsname{164.6}
\expandafter\def\csname res@qwen@time@hubdrop@Full@recv\endcsname{164.8}
\expandafter\def\csname res@qwen@time@hubdrop@Full@prefill\endcsname{22.8}
\expandafter\def\csname res@qwen@time@hubdrop@Full@topk\endcsname{7.6}
\expandafter\def\csname res@qwen@time@hubdrop@Full@group\endcsname{63.5}
\expandafter\def\csname res@qwen@time@hubdrop@Full@keylaw\endcsname{1.8}
\expandafter\def\csname res@qwen@time@las@Full@fwd\endcsname{88.6}
\expandafter\def\csname res@qwen@time@las@Full@law\endcsname{43.1}
\expandafter\def\csname res@qwen@time@las@Full@plan\endcsname{19.4}
\expandafter\def\csname res@qwen@time@las@Full@code\endcsname{1.9}
\expandafter\def\csname res@qwen@time@las@Full@sel\endcsname{64.3}
\expandafter\def\csname res@qwen@time@las@Full@total\endcsname{152.9}
\expandafter\def\csname res@qwen@time@las@Full@recv\endcsname{155.3}
\expandafter\def\csname res@qwen@time@las@Full@prefill\endcsname{23.1}
\expandafter\def\csname res@qwen@time@las@Full@topk\endcsname{34.4}
\expandafter\def\csname res@qwen@time@las@Full@fwdpertok\endcsname{4.13}
\expandafter\def\csname res@qwen@time@lascoin@Full@ratio\endcsname{3.4}
\expandafter\def\csname res@qwen@time@basic@16@relnative\endcsname{1.00}
\expandafter\def\csname res@qwen@time@mwis@16@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@stepwise@16@relnative\endcsname{1.07}
\expandafter\def\csname res@qwen@time@syncpool@16@relnative\endcsname{1.00}
\expandafter\def\csname res@qwen@time@coin@16@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@hubdrop@16@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@las@16@relnative\endcsname{1.36}
\expandafter\def\csname res@qwen@time@basic@64@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@mwis@64@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@stepwise@64@relnative\endcsname{1.30}
\expandafter\def\csname res@qwen@time@syncpool@64@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@coin@64@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@hubdrop@64@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@las@64@relnative\endcsname{1.51}
\expandafter\def\csname res@qwen@time@basic@256@relnative\endcsname{1.03}
\expandafter\def\csname res@qwen@time@mwis@256@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@stepwise@256@relnative\endcsname{2.28}
\expandafter\def\csname res@qwen@time@syncpool@256@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@coin@256@relnative\endcsname{1.01}
\expandafter\def\csname res@qwen@time@hubdrop@256@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@las@256@relnative\endcsname{1.77}
\expandafter\def\csname res@qwen@time@basic@1k@relnative\endcsname{1.14}
\expandafter\def\csname res@qwen@time@mwis@1k@relnative\endcsname{1.03}
\expandafter\def\csname res@qwen@time@stepwise@1k@relnative\endcsname{5.85}
\expandafter\def\csname res@qwen@time@syncpool@1k@relnative\endcsname{1.03}
\expandafter\def\csname res@qwen@time@coin@1k@relnative\endcsname{1.02}
\expandafter\def\csname res@qwen@time@hubdrop@1k@relnative\endcsname{1.04}
\expandafter\def\csname res@qwen@time@las@1k@relnative\endcsname{2.22}
\expandafter\def\csname res@qwen@time@basic@4k@relnative\endcsname{1.79}
\expandafter\def\csname res@qwen@time@mwis@4k@relnative\endcsname{1.07}
\expandafter\def\csname res@qwen@time@stepwise@4k@relnative\endcsname{20.11}
\expandafter\def\csname res@qwen@time@syncpool@4k@relnative\endcsname{1.09}
\expandafter\def\csname res@qwen@time@coin@4k@relnative\endcsname{1.03}
\expandafter\def\csname res@qwen@time@hubdrop@4k@relnative\endcsname{1.11}
\expandafter\def\csname res@qwen@time@las@4k@relnative\endcsname{3.80}
\expandafter\def\csname res@qwen@time@mwis@Full@relnative\endcsname{3.44}
\expandafter\def\csname res@qwen@time@syncpool@Full@relnative\endcsname{3.54}
\expandafter\def\csname res@qwen@time@coin@Full@relnative\endcsname{1.49}
\expandafter\def\csname res@qwen@time@hubdrop@Full@relnative\endcsname{5.37}
\expandafter\def\csname res@qwen@time@las@Full@relnative\endcsname{4.99}
\expandafter\def\csname res@qwen@time@any@gpu\endcsname{GeForce RTX 5090}
\expandafter\def\csname res@llmjp@time@native@16@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@native@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@16@plan\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@native@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@native@16@sel\endcsname{1.9}
\expandafter\def\csname res@llmjp@time@native@16@total\endcsname{16.4}
\expandafter\def\csname res@llmjp@time@native@16@recv\endcsname{15.5}
\expandafter\def\csname res@llmjp@time@native@16@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@native@16@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@16@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@basic@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@basic@16@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@basic@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@16@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@basic@16@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@basic@16@recv\endcsname{16.6}
\expandafter\def\csname res@llmjp@time@basic@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@basic@16@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@16@filter\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@mwis@16@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@mwis@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@16@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@mwis@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@16@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@mwis@16@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@mwis@16@recv\endcsname{16.6}
\expandafter\def\csname res@llmjp@time@mwis@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@mwis@16@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@16@filter\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@stepwise@16@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@stepwise@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@stepwise@16@plan\endcsname{2.2}
\expandafter\def\csname res@llmjp@time@stepwise@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@stepwise@16@sel\endcsname{3.5}
\expandafter\def\csname res@llmjp@time@stepwise@16@total\endcsname{18.0}
\expandafter\def\csname res@llmjp@time@stepwise@16@recv\endcsname{18.0}
\expandafter\def\csname res@llmjp@time@stepwise@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@stepwise@16@filter\endcsname{2.2}
\expandafter\def\csname res@llmjp@time@syncpool@16@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@syncpool@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@16@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@syncpool@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@16@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@syncpool@16@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@syncpool@16@recv\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@syncpool@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@syncpool@16@group\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@syncpool@16@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@coin@16@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@coin@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@16@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@coin@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@16@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@coin@16@total\endcsname{16.6}
\expandafter\def\csname res@llmjp@time@coin@16@recv\endcsname{16.6}
\expandafter\def\csname res@llmjp@time@coin@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@coin@16@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@16@prf\endcsname{0.0}
\expandafter\def\csname res@llmjp@time@coin@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@coin@16@proj\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@hubdrop@16@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@hubdrop@16@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@16@plan\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@hubdrop@16@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@16@sel\endcsname{2.2}
\expandafter\def\csname res@llmjp@time@hubdrop@16@total\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@hubdrop@16@recv\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@hubdrop@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@hubdrop@16@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@hubdrop@16@group\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@hubdrop@16@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@las@16@fwd\endcsname{19.4}
\expandafter\def\csname res@llmjp@time@las@16@law\endcsname{2.0}
\expandafter\def\csname res@llmjp@time@las@16@plan\endcsname{1.8}
\expandafter\def\csname res@llmjp@time@las@16@code\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@las@16@sel\endcsname{4.3}
\expandafter\def\csname res@llmjp@time@las@16@total\endcsname{23.7}
\expandafter\def\csname res@llmjp@time@las@16@recv\endcsname{24.5}
\expandafter\def\csname res@llmjp@time@las@16@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@las@16@topk\endcsname{0.6}
\expandafter\def\csname res@llmjp@time@las@16@fwdpertok\endcsname{1.34}
\expandafter\def\csname res@llmjp@time@native@64@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@native@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@64@plan\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@native@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@native@64@sel\endcsname{1.9}
\expandafter\def\csname res@llmjp@time@native@64@total\endcsname{16.3}
\expandafter\def\csname res@llmjp@time@native@64@recv\endcsname{15.5}
\expandafter\def\csname res@llmjp@time@native@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@native@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@basic@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@basic@64@plan\endcsname{0.8}
\expandafter\def\csname res@llmjp@time@basic@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@64@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@basic@64@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@basic@64@recv\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@basic@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@basic@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@64@filter\endcsname{0.3}
\expandafter\def\csname res@llmjp@time@mwis@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@mwis@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@64@plan\endcsname{0.8}
\expandafter\def\csname res@llmjp@time@mwis@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@64@sel\endcsname{2.2}
\expandafter\def\csname res@llmjp@time@mwis@64@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@mwis@64@recv\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@mwis@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@mwis@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@64@filter\endcsname{0.3}
\expandafter\def\csname res@llmjp@time@stepwise@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@stepwise@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@stepwise@64@plan\endcsname{6.7}
\expandafter\def\csname res@llmjp@time@stepwise@64@code\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@stepwise@64@sel\endcsname{8.1}
\expandafter\def\csname res@llmjp@time@stepwise@64@total\endcsname{22.7}
\expandafter\def\csname res@llmjp@time@stepwise@64@recv\endcsname{22.7}
\expandafter\def\csname res@llmjp@time@stepwise@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@stepwise@64@filter\endcsname{6.7}
\expandafter\def\csname res@llmjp@time@syncpool@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@syncpool@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@64@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@syncpool@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@64@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@syncpool@64@total\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@syncpool@64@recv\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@syncpool@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@syncpool@64@group\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@syncpool@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@coin@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@64@plan\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@coin@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@64@sel\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@coin@64@total\endcsname{16.7}
\expandafter\def\csname res@llmjp@time@coin@64@recv\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@coin@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@coin@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@64@prf\endcsname{0.0}
\expandafter\def\csname res@llmjp@time@coin@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@coin@64@proj\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@hubdrop@64@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@hubdrop@64@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@64@plan\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@hubdrop@64@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@64@sel\endcsname{2.3}
\expandafter\def\csname res@llmjp@time@hubdrop@64@total\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@hubdrop@64@recv\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@hubdrop@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@hubdrop@64@topk\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@64@group\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@hubdrop@64@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@las@64@fwd\endcsname{23.9}
\expandafter\def\csname res@llmjp@time@las@64@law\endcsname{2.4}
\expandafter\def\csname res@llmjp@time@las@64@plan\endcsname{2.7}
\expandafter\def\csname res@llmjp@time@las@64@code\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@las@64@sel\endcsname{5.8}
\expandafter\def\csname res@llmjp@time@las@64@total\endcsname{29.7}
\expandafter\def\csname res@llmjp@time@las@64@recv\endcsname{30.5}
\expandafter\def\csname res@llmjp@time@las@64@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@las@64@topk\endcsname{0.7}
\expandafter\def\csname res@llmjp@time@las@64@fwdpertok\endcsname{1.64}
\expandafter\def\csname res@llmjp@time@native@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@native@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@256@plan\endcsname{0.6}
\expandafter\def\csname res@llmjp@time@native@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@native@256@sel\endcsname{2.0}
\expandafter\def\csname res@llmjp@time@native@256@total\endcsname{16.5}
\expandafter\def\csname res@llmjp@time@native@256@recv\endcsname{16.5}
\expandafter\def\csname res@llmjp@time@native@256@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@native@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@basic@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@basic@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@basic@256@plan\endcsname{1.4}
\expandafter\def\csname res@llmjp@time@basic@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@256@sel\endcsname{2.8}
\expandafter\def\csname res@llmjp@time@basic@256@total\endcsname{17.4}
\expandafter\def\csname res@llmjp@time@basic@256@recv\endcsname{17.4}
\expandafter\def\csname res@llmjp@time@basic@256@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@basic@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@basic@256@filter\endcsname{0.8}
\expandafter\def\csname res@llmjp@time@mwis@256@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@mwis@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@256@plan\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@mwis@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@256@sel\endcsname{2.3}
\expandafter\def\csname res@llmjp@time@mwis@256@total\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@mwis@256@recv\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@mwis@256@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@mwis@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@mwis@256@filter\endcsname{0.3}
\expandafter\def\csname res@llmjp@time@stepwise@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@stepwise@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@stepwise@256@plan\endcsname{25.6}
\expandafter\def\csname res@llmjp@time@stepwise@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@stepwise@256@sel\endcsname{27.0}
\expandafter\def\csname res@llmjp@time@stepwise@256@total\endcsname{41.6}
\expandafter\def\csname res@llmjp@time@stepwise@256@recv\endcsname{41.3}
\expandafter\def\csname res@llmjp@time@stepwise@256@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@stepwise@256@filter\endcsname{25.6}
\expandafter\def\csname res@llmjp@time@syncpool@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@syncpool@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@256@plan\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@syncpool@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@256@sel\endcsname{2.3}
\expandafter\def\csname res@llmjp@time@syncpool@256@total\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@syncpool@256@recv\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@syncpool@256@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@syncpool@256@group\endcsname{0.3}
\expandafter\def\csname res@llmjp@time@syncpool@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@coin@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@coin@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@256@plan\endcsname{0.8}
\expandafter\def\csname res@llmjp@time@coin@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@256@sel\endcsname{2.2}
\expandafter\def\csname res@llmjp@time@coin@256@total\endcsname{16.8}
\expandafter\def\csname res@llmjp@time@coin@256@recv\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@coin@256@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@coin@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@coin@256@prf\endcsname{0.0}
\expandafter\def\csname res@llmjp@time@coin@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@coin@256@proj\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@hubdrop@256@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@hubdrop@256@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@256@plan\endcsname{1.2}
\expandafter\def\csname res@llmjp@time@hubdrop@256@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@256@sel\endcsname{2.6}
\expandafter\def\csname res@llmjp@time@hubdrop@256@total\endcsname{17.2}
\expandafter\def\csname res@llmjp@time@hubdrop@256@recv\endcsname{17.2}
\expandafter\def\csname res@llmjp@time@hubdrop@256@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@hubdrop@256@topk\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@hubdrop@256@group\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@hubdrop@256@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@las@256@fwd\endcsname{29.1}
\expandafter\def\csname res@llmjp@time@las@256@law\endcsname{3.2}
\expandafter\def\csname res@llmjp@time@las@256@plan\endcsname{4.9}
\expandafter\def\csname res@llmjp@time@las@256@code\endcsname{0.8}
\expandafter\def\csname res@llmjp@time@las@256@sel\endcsname{8.9}
\expandafter\def\csname res@llmjp@time@las@256@total\endcsname{38.0}
\expandafter\def\csname res@llmjp@time@las@256@recv\endcsname{39.1}
\expandafter\def\csname res@llmjp@time@las@256@prefill\endcsname{15.7}
\expandafter\def\csname res@llmjp@time@las@256@topk\endcsname{1.1}
\expandafter\def\csname res@llmjp@time@las@256@fwdpertok\endcsname{1.99}
\expandafter\def\csname res@llmjp@time@native@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@native@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@1k@plan\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@native@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@native@1k@sel\endcsname{2.3}
\expandafter\def\csname res@llmjp@time@native@1k@total\endcsname{16.9}
\expandafter\def\csname res@llmjp@time@native@1k@recv\endcsname{15.4}
\expandafter\def\csname res@llmjp@time@native@1k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@native@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@basic@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@basic@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@basic@1k@plan\endcsname{4.1}
\expandafter\def\csname res@llmjp@time@basic@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@basic@1k@sel\endcsname{5.5}
\expandafter\def\csname res@llmjp@time@basic@1k@total\endcsname{20.2}
\expandafter\def\csname res@llmjp@time@basic@1k@recv\endcsname{20.1}
\expandafter\def\csname res@llmjp@time@basic@1k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@basic@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@basic@1k@filter\endcsname{3.0}
\expandafter\def\csname res@llmjp@time@mwis@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@mwis@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@1k@plan\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@mwis@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@1k@sel\endcsname{3.0}
\expandafter\def\csname res@llmjp@time@mwis@1k@total\endcsname{17.6}
\expandafter\def\csname res@llmjp@time@mwis@1k@recv\endcsname{17.6}
\expandafter\def\csname res@llmjp@time@mwis@1k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@mwis@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@mwis@1k@filter\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@stepwise@1k@fwd\endcsname{14.7}
\expandafter\def\csname res@llmjp@time@stepwise@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@stepwise@1k@plan\endcsname{108.4}
\expandafter\def\csname res@llmjp@time@stepwise@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@stepwise@1k@sel\endcsname{109.8}
\expandafter\def\csname res@llmjp@time@stepwise@1k@total\endcsname{124.4}
\expandafter\def\csname res@llmjp@time@stepwise@1k@recv\endcsname{124.0}
\expandafter\def\csname res@llmjp@time@stepwise@1k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@stepwise@1k@filter\endcsname{108.4}
\expandafter\def\csname res@llmjp@time@syncpool@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@syncpool@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@1k@plan\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@syncpool@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@1k@sel\endcsname{3.0}
\expandafter\def\csname res@llmjp@time@syncpool@1k@total\endcsname{17.6}
\expandafter\def\csname res@llmjp@time@syncpool@1k@recv\endcsname{17.6}
\expandafter\def\csname res@llmjp@time@syncpool@1k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@syncpool@1k@group\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@syncpool@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@coin@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@coin@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@1k@plan\endcsname{1.3}
\expandafter\def\csname res@llmjp@time@coin@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@1k@sel\endcsname{2.7}
\expandafter\def\csname res@llmjp@time@coin@1k@total\endcsname{17.3}
\expandafter\def\csname res@llmjp@time@coin@1k@recv\endcsname{17.3}
\expandafter\def\csname res@llmjp@time@coin@1k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@coin@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@coin@1k@prf\endcsname{0.0}
\expandafter\def\csname res@llmjp@time@coin@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@coin@1k@proj\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@plan\endcsname{2.1}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@sel\endcsname{3.5}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@total\endcsname{18.1}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@recv\endcsname{18.1}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@topk\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@group\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@keylaw\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@las@1k@fwd\endcsname{43.6}
\expandafter\def\csname res@llmjp@time@las@1k@law\endcsname{5.7}
\expandafter\def\csname res@llmjp@time@las@1k@plan\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@las@1k@code\endcsname{1.3}
\expandafter\def\csname res@llmjp@time@las@1k@sel\endcsname{21.5}
\expandafter\def\csname res@llmjp@time@las@1k@total\endcsname{65.2}
\expandafter\def\csname res@llmjp@time@las@1k@recv\endcsname{66.9}
\expandafter\def\csname res@llmjp@time@las@1k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@las@1k@topk\endcsname{2.5}
\expandafter\def\csname res@llmjp@time@las@1k@fwdpertok\endcsname{2.98}
\expandafter\def\csname res@llmjp@time@native@4k@fwd\endcsname{14.5}
\expandafter\def\csname res@llmjp@time@native@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@4k@plan\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@native@4k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@native@4k@sel\endcsname{3.0}
\expandafter\def\csname res@llmjp@time@native@4k@total\endcsname{17.5}
\expandafter\def\csname res@llmjp@time@native@4k@recv\endcsname{17.5}
\expandafter\def\csname res@llmjp@time@native@4k@prefill\endcsname{16.0}
\expandafter\def\csname res@llmjp@time@native@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llmjp@time@basic@4k@fwd\endcsname{14.7}
\expandafter\def\csname res@llmjp@time@basic@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@basic@4k@plan\endcsname{22.3}
\expandafter\def\csname res@llmjp@time@basic@4k@code\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@basic@4k@sel\endcsname{23.8}
\expandafter\def\csname res@llmjp@time@basic@4k@total\endcsname{38.5}
\expandafter\def\csname res@llmjp@time@basic@4k@recv\endcsname{38.4}
\expandafter\def\csname res@llmjp@time@basic@4k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@basic@4k@topk\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@basic@4k@filter\endcsname{19.8}
\expandafter\def\csname res@llmjp@time@mwis@4k@fwd\endcsname{14.7}
\expandafter\def\csname res@llmjp@time@mwis@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@4k@plan\endcsname{3.4}
\expandafter\def\csname res@llmjp@time@mwis@4k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@mwis@4k@sel\endcsname{4.8}
\expandafter\def\csname res@llmjp@time@mwis@4k@total\endcsname{19.5}
\expandafter\def\csname res@llmjp@time@mwis@4k@recv\endcsname{19.3}
\expandafter\def\csname res@llmjp@time@mwis@4k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@mwis@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llmjp@time@mwis@4k@filter\endcsname{1.3}
\expandafter\def\csname res@llmjp@time@stepwise@4k@fwd\endcsname{14.9}
\expandafter\def\csname res@llmjp@time@stepwise@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@stepwise@4k@plan\endcsname{432.1}
\expandafter\def\csname res@llmjp@time@stepwise@4k@code\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@stepwise@4k@sel\endcsname{433.5}
\expandafter\def\csname res@llmjp@time@stepwise@4k@total\endcsname{448.4}
\expandafter\def\csname res@llmjp@time@stepwise@4k@recv\endcsname{447.6}
\expandafter\def\csname res@llmjp@time@stepwise@4k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@stepwise@4k@filter\endcsname{432.0}
\expandafter\def\csname res@llmjp@time@syncpool@4k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@syncpool@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@4k@plan\endcsname{3.5}
\expandafter\def\csname res@llmjp@time@syncpool@4k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@4k@sel\endcsname{4.9}
\expandafter\def\csname res@llmjp@time@syncpool@4k@total\endcsname{19.6}
\expandafter\def\csname res@llmjp@time@syncpool@4k@recv\endcsname{19.5}
\expandafter\def\csname res@llmjp@time@syncpool@4k@prefill\endcsname{16.2}
\expandafter\def\csname res@llmjp@time@syncpool@4k@group\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@syncpool@4k@topk\endcsname{1.6}
\expandafter\def\csname res@llmjp@time@coin@4k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@coin@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@4k@plan\endcsname{2.3}
\expandafter\def\csname res@llmjp@time@coin@4k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@coin@4k@sel\endcsname{3.8}
\expandafter\def\csname res@llmjp@time@coin@4k@total\endcsname{18.4}
\expandafter\def\csname res@llmjp@time@coin@4k@recv\endcsname{18.4}
\expandafter\def\csname res@llmjp@time@coin@4k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@coin@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llmjp@time@coin@4k@prf\endcsname{0.1}
\expandafter\def\csname res@llmjp@time@coin@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@coin@4k@proj\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@plan\endcsname{5.1}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@sel\endcsname{6.6}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@total\endcsname{21.1}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@recv\endcsname{21.1}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@topk\endcsname{1.5}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@group\endcsname{1.4}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@keylaw\endcsname{0.2}
\expandafter\def\csname res@llmjp@time@las@4k@fwd\endcsname{54.0}
\expandafter\def\csname res@llmjp@time@las@4k@law\endcsname{9.7}
\expandafter\def\csname res@llmjp@time@las@4k@plan\endcsname{44.1}
\expandafter\def\csname res@llmjp@time@las@4k@code\endcsname{1.7}
\expandafter\def\csname res@llmjp@time@las@4k@sel\endcsname{55.4}
\expandafter\def\csname res@llmjp@time@las@4k@total\endcsname{109.4}
\expandafter\def\csname res@llmjp@time@las@4k@recv\endcsname{112.4}
\expandafter\def\csname res@llmjp@time@las@4k@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@las@4k@topk\endcsname{5.6}
\expandafter\def\csname res@llmjp@time@las@4k@fwdpertok\endcsname{3.67}
\expandafter\def\csname res@llmjp@time@native@Full@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@native@Full@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@native@Full@plan\endcsname{6.0}
\expandafter\def\csname res@llmjp@time@native@Full@code\endcsname{0.6}
\expandafter\def\csname res@llmjp@time@native@Full@sel\endcsname{7.6}
\expandafter\def\csname res@llmjp@time@native@Full@total\endcsname{22.2}
\expandafter\def\csname res@llmjp@time@native@Full@recv\endcsname{22.4}
\expandafter\def\csname res@llmjp@time@native@Full@prefill\endcsname{16.0}
\expandafter\def\csname res@llmjp@time@native@Full@topk\endcsname{6.0}
\expandafter\def\csname res@llmjp@time@mwis@Full@fwd\endcsname{14.7}
\expandafter\def\csname res@llmjp@time@mwis@Full@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@mwis@Full@plan\endcsname{43.7}
\expandafter\def\csname res@llmjp@time@mwis@Full@code\endcsname{0.6}
\expandafter\def\csname res@llmjp@time@mwis@Full@sel\endcsname{45.3}
\expandafter\def\csname res@llmjp@time@mwis@Full@total\endcsname{59.9}
\expandafter\def\csname res@llmjp@time@mwis@Full@recv\endcsname{59.7}
\expandafter\def\csname res@llmjp@time@mwis@Full@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@mwis@Full@topk\endcsname{6.0}
\expandafter\def\csname res@llmjp@time@mwis@Full@filter\endcsname{27.8}
\expandafter\def\csname res@llmjp@time@syncpool@Full@fwd\endcsname{14.6}
\expandafter\def\csname res@llmjp@time@syncpool@Full@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@syncpool@Full@plan\endcsname{51.2}
\expandafter\def\csname res@llmjp@time@syncpool@Full@code\endcsname{0.4}
\expandafter\def\csname res@llmjp@time@syncpool@Full@sel\endcsname{52.6}
\expandafter\def\csname res@llmjp@time@syncpool@Full@total\endcsname{67.3}
\expandafter\def\csname res@llmjp@time@syncpool@Full@recv\endcsname{67.1}
\expandafter\def\csname res@llmjp@time@syncpool@Full@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@syncpool@Full@group\endcsname{40.8}
\expandafter\def\csname res@llmjp@time@syncpool@Full@topk\endcsname{6.0}
\expandafter\def\csname res@llmjp@time@coin@Full@fwd\endcsname{14.9}
\expandafter\def\csname res@llmjp@time@coin@Full@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@coin@Full@plan\endcsname{13.8}
\expandafter\def\csname res@llmjp@time@coin@Full@code\endcsname{0.6}
\expandafter\def\csname res@llmjp@time@coin@Full@sel\endcsname{15.3}
\expandafter\def\csname res@llmjp@time@coin@Full@total\endcsname{30.3}
\expandafter\def\csname res@llmjp@time@coin@Full@recv\endcsname{30.2}
\expandafter\def\csname res@llmjp@time@coin@Full@prefill\endcsname{15.9}
\expandafter\def\csname res@llmjp@time@coin@Full@topk\endcsname{5.9}
\expandafter\def\csname res@llmjp@time@coin@Full@prf\endcsname{0.3}
\expandafter\def\csname res@llmjp@time@coin@Full@keylaw\endcsname{0.9}
\expandafter\def\csname res@llmjp@time@coin@Full@proj\endcsname{6.6}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@fwd\endcsname{14.7}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@law\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@plan\endcsname{87.1}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@code\endcsname{0.5}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@sel\endcsname{88.6}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@total\endcsname{103.3}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@recv\endcsname{103.3}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@prefill\endcsname{15.8}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@topk\endcsname{6.0}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@group\endcsname{39.9}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@keylaw\endcsname{1.0}
\expandafter\def\csname res@llmjp@time@las@Full@fwd\endcsname{65.1}
\expandafter\def\csname res@llmjp@time@las@Full@law\endcsname{32.3}
\expandafter\def\csname res@llmjp@time@las@Full@plan\endcsname{17.7}
\expandafter\def\csname res@llmjp@time@las@Full@code\endcsname{2.0}
\expandafter\def\csname res@llmjp@time@las@Full@sel\endcsname{52.1}
\expandafter\def\csname res@llmjp@time@las@Full@total\endcsname{117.2}
\expandafter\def\csname res@llmjp@time@las@Full@recv\endcsname{120.2}
\expandafter\def\csname res@llmjp@time@las@Full@prefill\endcsname{16.0}
\expandafter\def\csname res@llmjp@time@las@Full@topk\endcsname{26.1}
\expandafter\def\csname res@llmjp@time@las@Full@fwdpertok\endcsname{4.40}
\expandafter\def\csname res@llmjp@time@lascoin@Full@ratio\endcsname{3.9}
\expandafter\def\csname res@llmjp@time@basic@16@relnative\endcsname{1.01}
\expandafter\def\csname res@llmjp@time@mwis@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@stepwise@16@relnative\endcsname{1.10}
\expandafter\def\csname res@llmjp@time@syncpool@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@coin@16@relnative\endcsname{1.01}
\expandafter\def\csname res@llmjp@time@hubdrop@16@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@las@16@relnative\endcsname{1.45}
\expandafter\def\csname res@llmjp@time@basic@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@mwis@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@stepwise@64@relnative\endcsname{1.39}
\expandafter\def\csname res@llmjp@time@syncpool@64@relnative\endcsname{1.03}
\expandafter\def\csname res@llmjp@time@coin@64@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@hubdrop@64@relnative\endcsname{1.03}
\expandafter\def\csname res@llmjp@time@las@64@relnative\endcsname{1.82}
\expandafter\def\csname res@llmjp@time@basic@256@relnative\endcsname{1.06}
\expandafter\def\csname res@llmjp@time@mwis@256@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@stepwise@256@relnative\endcsname{2.52}
\expandafter\def\csname res@llmjp@time@syncpool@256@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@coin@256@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@hubdrop@256@relnative\endcsname{1.04}
\expandafter\def\csname res@llmjp@time@las@256@relnative\endcsname{2.30}
\expandafter\def\csname res@llmjp@time@basic@1k@relnative\endcsname{1.19}
\expandafter\def\csname res@llmjp@time@mwis@1k@relnative\endcsname{1.04}
\expandafter\def\csname res@llmjp@time@stepwise@1k@relnative\endcsname{7.35}
\expandafter\def\csname res@llmjp@time@syncpool@1k@relnative\endcsname{1.04}
\expandafter\def\csname res@llmjp@time@coin@1k@relnative\endcsname{1.02}
\expandafter\def\csname res@llmjp@time@hubdrop@1k@relnative\endcsname{1.07}
\expandafter\def\csname res@llmjp@time@las@1k@relnative\endcsname{3.85}
\expandafter\def\csname res@llmjp@time@basic@4k@relnative\endcsname{2.19}
\expandafter\def\csname res@llmjp@time@mwis@4k@relnative\endcsname{1.11}
\expandafter\def\csname res@llmjp@time@stepwise@4k@relnative\endcsname{25.56}
\expandafter\def\csname res@llmjp@time@syncpool@4k@relnative\endcsname{1.12}
\expandafter\def\csname res@llmjp@time@coin@4k@relnative\endcsname{1.05}
\expandafter\def\csname res@llmjp@time@hubdrop@4k@relnative\endcsname{1.20}
\expandafter\def\csname res@llmjp@time@las@4k@relnative\endcsname{6.24}
\expandafter\def\csname res@llmjp@time@mwis@Full@relnative\endcsname{2.70}
\expandafter\def\csname res@llmjp@time@syncpool@Full@relnative\endcsname{3.03}
\expandafter\def\csname res@llmjp@time@coin@Full@relnative\endcsname{1.36}
\expandafter\def\csname res@llmjp@time@hubdrop@Full@relnative\endcsname{4.66}
\expandafter\def\csname res@llmjp@time@las@Full@relnative\endcsname{5.29}
\expandafter\def\csname res@llmjp@time@any@gpu\endcsname{GeForce RTX 5090}
\expandafter\def\csname res@all@time@basic@relmin\endcsname{1.00}
\expandafter\def\csname res@all@time@basic@relmax\endcsname{2.34}
\expandafter\def\csname res@all@time@mwis@relmin\endcsname{1.01}
\expandafter\def\csname res@all@time@mwis@relmax\endcsname{3.69}
\expandafter\def\csname res@all@time@stepwise@relmin\endcsname{1.07}
\expandafter\def\csname res@all@time@stepwise@relmax\endcsname{29.43}
\expandafter\def\csname res@all@time@syncpool@relmin\endcsname{1.00}
\expandafter\def\csname res@all@time@syncpool@relmax\endcsname{3.65}
\expandafter\def\csname res@all@time@coin@relmin\endcsname{1.01}
\expandafter\def\csname res@all@time@coin@relmax\endcsname{1.57}
\expandafter\def\csname res@all@time@hubdrop@relmin\endcsname{1.01}
\expandafter\def\csname res@all@time@hubdrop@relmax\endcsname{5.68}
\expandafter\def\csname res@all@time@las@relmin\endcsname{1.36}
\expandafter\def\csname res@all@time@las@relmax\endcsname{6.24}
\expandafter\def\csname res@all@time@lascoin@Full@min\endcsname{3.4}
\expandafter\def\csname res@all@time@lascoin@Full@max\endcsname{3.9}
\expandafter\def\csname res@all@las@Full@utilgapmin\endcsname{6.0}
\expandafter\def\csname res@all@las@Full@utilgapmax\endcsname{7.0}
\expandafter\def\csname res@llama@tb@native@16@auto\endcsname{0.78}
\expandafter\def\csname res@llama@tb@basic@16@auto\endcsname{0.94}
\expandafter\def\csname res@llama@tb@basic@16@dense\endcsname{1.68}
\expandafter\def\csname res@llama@tb@basic@16@sparse\endcsname{0.95}
\expandafter\def\csname res@llama@tb@mwis@16@auto\endcsname{1.01}
\expandafter\def\csname res@llama@tb@mwis@16@dense\endcsname{2.49}
\expandafter\def\csname res@llama@tb@mwis@16@sparse\endcsname{1.00}
\expandafter\def\csname res@llama@tb@stepwise@16@auto\endcsname{1.65}
\expandafter\def\csname res@llama@tb@syncpool@16@auto\endcsname{1.01}
\expandafter\def\csname res@llama@tb@syncpool@16@dense\endcsname{1.75}
\expandafter\def\csname res@llama@tb@syncpool@16@sparse\endcsname{0.99}
\expandafter\def\csname res@llama@tb@coin@16@auto\endcsname{1.07}
\expandafter\def\csname res@llama@tb@coin@16@dense\endcsname{2.58}
\expandafter\def\csname res@llama@tb@coin@16@sparse\endcsname{0.97}
\expandafter\def\csname res@llama@tb@hubdrop@16@auto\endcsname{1.07}
\expandafter\def\csname res@llama@tb@native@64@auto\endcsname{0.81}
\expandafter\def\csname res@llama@tb@basic@64@auto\endcsname{1.04}
\expandafter\def\csname res@llama@tb@basic@64@dense\endcsname{1.80}
\expandafter\def\csname res@llama@tb@basic@64@sparse\endcsname{1.06}
\expandafter\def\csname res@llama@tb@mwis@64@auto\endcsname{1.07}
\expandafter\def\csname res@llama@tb@mwis@64@dense\endcsname{2.56}
\expandafter\def\csname res@llama@tb@mwis@64@sparse\endcsname{1.06}
\expandafter\def\csname res@llama@tb@stepwise@64@auto\endcsname{3.63}
\expandafter\def\csname res@llama@tb@syncpool@64@auto\endcsname{1.06}
\expandafter\def\csname res@llama@tb@syncpool@64@dense\endcsname{1.80}
\expandafter\def\csname res@llama@tb@syncpool@64@sparse\endcsname{1.03}
\expandafter\def\csname res@llama@tb@coin@64@auto\endcsname{1.10}
\expandafter\def\csname res@llama@tb@coin@64@dense\endcsname{2.63}
\expandafter\def\csname res@llama@tb@coin@64@sparse\endcsname{1.02}
\expandafter\def\csname res@llama@tb@hubdrop@64@auto\endcsname{1.14}
\expandafter\def\csname res@llama@tb@native@256@auto\endcsname{0.89}
\expandafter\def\csname res@llama@tb@basic@256@auto\endcsname{1.51}
\expandafter\def\csname res@llama@tb@basic@256@dense\endcsname{2.27}
\expandafter\def\csname res@llama@tb@basic@256@sparse\endcsname{1.54}
\expandafter\def\csname res@llama@tb@mwis@256@auto\endcsname{1.27}
\expandafter\def\csname res@llama@tb@mwis@256@dense\endcsname{2.72}
\expandafter\def\csname res@llama@tb@mwis@256@sparse\endcsname{1.26}
\expandafter\def\csname res@llama@tb@stepwise@256@auto\endcsname{11.39}
\expandafter\def\csname res@llama@tb@syncpool@256@auto\endcsname{1.21}
\expandafter\def\csname res@llama@tb@syncpool@256@dense\endcsname{1.96}
\expandafter\def\csname res@llama@tb@syncpool@256@sparse\endcsname{1.21}
\expandafter\def\csname res@llama@tb@coin@256@auto\endcsname{1.24}
\expandafter\def\csname res@llama@tb@coin@256@dense\endcsname{2.75}
\expandafter\def\csname res@llama@tb@coin@256@sparse\endcsname{1.16}
\expandafter\def\csname res@llama@tb@hubdrop@256@auto\endcsname{1.38}
\expandafter\def\csname res@llama@tb@native@1k@auto\endcsname{1.16}
\expandafter\def\csname res@llama@tb@basic@1k@auto\endcsname{3.76}
\expandafter\def\csname res@llama@tb@basic@1k@dense\endcsname{4.55}
\expandafter\def\csname res@llama@tb@basic@1k@sparse\endcsname{3.76}
\expandafter\def\csname res@llama@tb@mwis@1k@auto\endcsname{1.88}
\expandafter\def\csname res@llama@tb@mwis@1k@dense\endcsname{3.39}
\expandafter\def\csname res@llama@tb@mwis@1k@sparse\endcsname{1.92}
\expandafter\def\csname res@llama@tb@stepwise@1k@auto\endcsname{43.73}
\expandafter\def\csname res@llama@tb@syncpool@1k@auto\endcsname{1.77}
\expandafter\def\csname res@llama@tb@syncpool@1k@dense\endcsname{2.53}
\expandafter\def\csname res@llama@tb@syncpool@1k@sparse\endcsname{1.78}
\expandafter\def\csname res@llama@tb@coin@1k@auto\endcsname{1.66}
\expandafter\def\csname res@llama@tb@coin@1k@dense\endcsname{3.16}
\expandafter\def\csname res@llama@tb@coin@1k@sparse\endcsname{1.59}
\expandafter\def\csname res@llama@tb@hubdrop@1k@auto\endcsname{2.17}
\expandafter\def\csname res@llama@tb@native@4k@auto\endcsname{1.98}
\expandafter\def\csname res@llama@tb@mwis@4k@auto\endcsname{4.14}
\expandafter\def\csname res@llama@tb@mwis@4k@dense\endcsname{5.78}
\expandafter\def\csname res@llama@tb@mwis@4k@sparse\endcsname{4.16}
\expandafter\def\csname res@llama@tb@stepwise@4k@auto\endcsname{172.93}
\expandafter\def\csname res@llama@tb@syncpool@4k@auto\endcsname{3.78}
\expandafter\def\csname res@llama@tb@syncpool@4k@dense\endcsname{4.59}
\expandafter\def\csname res@llama@tb@syncpool@4k@sparse\endcsname{3.82}
\expandafter\def\csname res@llama@tb@coin@4k@auto\endcsname{3.04}
\expandafter\def\csname res@llama@tb@coin@4k@dense\endcsname{4.69}
\expandafter\def\csname res@llama@tb@coin@4k@sparse\endcsname{2.98}
\expandafter\def\csname res@llama@tb@hubdrop@4k@auto\endcsname{5.40}
\expandafter\def\csname res@llama@tb@native@Full@auto\endcsname{7.95}
\expandafter\def\csname res@llama@tb@mwis@Full@auto\endcsname{73.97}
\expandafter\def\csname res@llama@tb@mwis@Full@dense\endcsname{70.93}
\expandafter\def\csname res@llama@tb@mwis@Full@sparse\endcsname{74.68}
\expandafter\def\csname res@llama@tb@syncpool@Full@auto\endcsname{75.88}
\expandafter\def\csname res@llama@tb@syncpool@Full@dense\endcsname{74.98}
\expandafter\def\csname res@llama@tb@syncpool@Full@sparse\endcsname{79.34}
\expandafter\def\csname res@llama@tb@coin@Full@auto\endcsname{22.06}
\expandafter\def\csname res@llama@tb@coin@Full@dense\endcsname{21.38}
\expandafter\def\csname res@llama@tb@coin@Full@sparse\endcsname{29.11}
\expandafter\def\csname res@llama@tb@hubdrop@Full@auto\endcsname{122.50}
\expandafter\def\csname res@llama@tb@coin@any@speedupmax\endcsname{2.7}
\expandafter\def\csname res@llama@tb@syncpool@any@speedupmax\endcsname{1.8}
\expandafter\def\csname res@llama@tb@mwis@any@speedupmax\endcsname{2.5}
\expandafter\def\csname res@llama@tb@basic@any@speedupmax\endcsname{1.8}
\expandafter\def\csname res@llama@tb@cnt@16@keys\endcsname{16}
\expandafter\def\csname res@llama@tb@cnt@16@pairs\endcsname{1}
\expandafter\def\csname res@llama@tb@cnt@16@nodes\endcsname{1}
\expandafter\def\csname res@llama@tb@cnt@16@survivors\endcsname{14}
\expandafter\def\csname res@llama@tb@cnt@64@keys\endcsname{64}
\expandafter\def\csname res@llama@tb@cnt@64@pairs\endcsname{45}
\expandafter\def\csname res@llama@tb@cnt@64@nodes\endcsname{7}
\expandafter\def\csname res@llama@tb@cnt@64@survivors\endcsname{55}
\expandafter\def\csname res@llama@tb@cnt@256@keys\endcsname{256}
\expandafter\def\csname res@llama@tb@cnt@256@pairs\endcsname{355}
\expandafter\def\csname res@llama@tb@cnt@256@nodes\endcsname{44}
\expandafter\def\csname res@llama@tb@cnt@256@survivors\endcsname{195}
\expandafter\def\csname res@llama@tb@cnt@1k@keys\endcsname{1{,}024}
\expandafter\def\csname res@llama@tb@cnt@1k@pairs\endcsname{2{,}294}
\expandafter\def\csname res@llama@tb@cnt@1k@nodes\endcsname{234}
\expandafter\def\csname res@llama@tb@cnt@1k@survivors\endcsname{655}
\expandafter\def\csname res@llama@tb@cnt@4k@keys\endcsname{4{,}096}
\expandafter\def\csname res@llama@tb@cnt@4k@pairs\endcsname{12{,}413}
\expandafter\def\csname res@llama@tb@cnt@4k@nodes\endcsname{1{,}139}
\expandafter\def\csname res@llama@tb@cnt@4k@survivors\endcsname{2{,}336}
\expandafter\def\csname res@llama@tb@cnt@Full@keys\endcsname{128{,}000}
\expandafter\def\csname res@llama@tb@cnt@Full@pairs\endcsname{458{,}043}
\expandafter\def\csname res@llama@tb@cnt@Full@nodes\endcsname{41{,}302}
\expandafter\def\csname res@llama@tb@cnt@Full@survivors\endcsname{56{,}706}
\expandafter\def\csname res@qwen@tb@native@16@auto\endcsname{0.85}
\expandafter\def\csname res@qwen@tb@basic@16@auto\endcsname{1.00}
\expandafter\def\csname res@qwen@tb@basic@16@dense\endcsname{1.86}
\expandafter\def\csname res@qwen@tb@basic@16@sparse\endcsname{1.04}
\expandafter\def\csname res@qwen@tb@mwis@16@auto\endcsname{1.09}
\expandafter\def\csname res@qwen@tb@mwis@16@dense\endcsname{2.74}
\expandafter\def\csname res@qwen@tb@mwis@16@sparse\endcsname{1.09}
\expandafter\def\csname res@qwen@tb@stepwise@16@auto\endcsname{1.61}
\expandafter\def\csname res@qwen@tb@syncpool@16@auto\endcsname{1.08}
\expandafter\def\csname res@qwen@tb@syncpool@16@dense\endcsname{1.94}
\expandafter\def\csname res@qwen@tb@syncpool@16@sparse\endcsname{1.07}
\expandafter\def\csname res@qwen@tb@coin@16@auto\endcsname{1.14}
\expandafter\def\csname res@qwen@tb@coin@16@dense\endcsname{3.00}
\expandafter\def\csname res@qwen@tb@coin@16@sparse\endcsname{1.08}
\expandafter\def\csname res@qwen@tb@hubdrop@16@auto\endcsname{1.19}
\expandafter\def\csname res@qwen@tb@native@64@auto\endcsname{0.86}
\expandafter\def\csname res@qwen@tb@basic@64@auto\endcsname{1.09}
\expandafter\def\csname res@qwen@tb@basic@64@dense\endcsname{1.95}
\expandafter\def\csname res@qwen@tb@basic@64@sparse\endcsname{1.11}
\expandafter\def\csname res@qwen@tb@mwis@64@auto\endcsname{1.13}
\expandafter\def\csname res@qwen@tb@mwis@64@dense\endcsname{2.77}
\expandafter\def\csname res@qwen@tb@mwis@64@sparse\endcsname{1.12}
\expandafter\def\csname res@qwen@tb@stepwise@64@auto\endcsname{3.21}
\expandafter\def\csname res@qwen@tb@syncpool@64@auto\endcsname{1.12}
\expandafter\def\csname res@qwen@tb@syncpool@64@dense\endcsname{1.97}
\expandafter\def\csname res@qwen@tb@syncpool@64@sparse\endcsname{1.11}
\expandafter\def\csname res@qwen@tb@coin@64@auto\endcsname{1.18}
\expandafter\def\csname res@qwen@tb@coin@64@dense\endcsname{2.98}
\expandafter\def\csname res@qwen@tb@coin@64@sparse\endcsname{1.11}
\expandafter\def\csname res@qwen@tb@hubdrop@64@auto\endcsname{1.22}
\expandafter\def\csname res@qwen@tb@native@256@auto\endcsname{0.95}
\expandafter\def\csname res@qwen@tb@basic@256@auto\endcsname{1.46}
\expandafter\def\csname res@qwen@tb@basic@256@dense\endcsname{2.32}
\expandafter\def\csname res@qwen@tb@basic@256@sparse\endcsname{1.49}
\expandafter\def\csname res@qwen@tb@mwis@256@auto\endcsname{1.32}
\expandafter\def\csname res@qwen@tb@mwis@256@dense\endcsname{2.93}
\expandafter\def\csname res@qwen@tb@mwis@256@sparse\endcsname{1.31}
\expandafter\def\csname res@qwen@tb@stepwise@256@auto\endcsname{9.67}
\expandafter\def\csname res@qwen@tb@syncpool@256@auto\endcsname{1.31}
\expandafter\def\csname res@qwen@tb@syncpool@256@dense\endcsname{2.16}
\expandafter\def\csname res@qwen@tb@syncpool@256@sparse\endcsname{1.30}
\expandafter\def\csname res@qwen@tb@coin@256@auto\endcsname{1.30}
\expandafter\def\csname res@qwen@tb@coin@256@dense\endcsname{3.10}
\expandafter\def\csname res@qwen@tb@coin@256@sparse\endcsname{1.23}
\expandafter\def\csname res@qwen@tb@hubdrop@256@auto\endcsname{1.44}
\expandafter\def\csname res@qwen@tb@native@1k@auto\endcsname{1.30}
\expandafter\def\csname res@qwen@tb@basic@1k@auto\endcsname{3.07}
\expandafter\def\csname res@qwen@tb@basic@1k@dense\endcsname{3.95}
\expandafter\def\csname res@qwen@tb@basic@1k@sparse\endcsname{3.12}
\expandafter\def\csname res@qwen@tb@mwis@1k@auto\endcsname{1.90}
\expandafter\def\csname res@qwen@tb@mwis@1k@dense\endcsname{3.55}
\expandafter\def\csname res@qwen@tb@mwis@1k@sparse\endcsname{1.93}
\expandafter\def\csname res@qwen@tb@stepwise@1k@auto\endcsname{35.39}
\expandafter\def\csname res@qwen@tb@syncpool@1k@auto\endcsname{2.03}
\expandafter\def\csname res@qwen@tb@syncpool@1k@dense\endcsname{2.89}
\expandafter\def\csname res@qwen@tb@syncpool@1k@sparse\endcsname{2.05}
\expandafter\def\csname res@qwen@tb@coin@1k@auto\endcsname{1.73}
\expandafter\def\csname res@qwen@tb@coin@1k@dense\endcsname{3.53}
\expandafter\def\csname res@qwen@tb@coin@1k@sparse\endcsname{1.67}
\expandafter\def\csname res@qwen@tb@hubdrop@1k@auto\endcsname{2.24}
\expandafter\def\csname res@qwen@tb@native@4k@auto\endcsname{1.88}
\expandafter\def\csname res@qwen@tb@mwis@4k@auto\endcsname{3.46}
\expandafter\def\csname res@qwen@tb@mwis@4k@dense\endcsname{5.32}
\expandafter\def\csname res@qwen@tb@mwis@4k@sparse\endcsname{3.52}
\expandafter\def\csname res@qwen@tb@stepwise@4k@auto\endcsname{143.61}
\expandafter\def\csname res@qwen@tb@syncpool@4k@auto\endcsname{3.97}
\expandafter\def\csname res@qwen@tb@syncpool@4k@dense\endcsname{5.04}
\expandafter\def\csname res@qwen@tb@syncpool@4k@sparse\endcsname{4.00}
\expandafter\def\csname res@qwen@tb@coin@4k@auto\endcsname{2.74}
\expandafter\def\csname res@qwen@tb@coin@4k@dense\endcsname{4.75}
\expandafter\def\csname res@qwen@tb@coin@4k@sparse\endcsname{2.65}
\expandafter\def\csname res@qwen@tb@hubdrop@4k@auto\endcsname{4.77}
\expandafter\def\csname res@qwen@tb@native@Full@auto\endcsname{7.86}
\expandafter\def\csname res@qwen@tb@mwis@Full@auto\endcsname{83.63}
\expandafter\def\csname res@qwen@tb@mwis@Full@dense\endcsname{78.70}
\expandafter\def\csname res@qwen@tb@mwis@Full@sparse\endcsname{83.29}
\expandafter\def\csname res@qwen@tb@syncpool@Full@auto\endcsname{88.83}
\expandafter\def\csname res@qwen@tb@syncpool@Full@dense\endcsname{87.36}
\expandafter\def\csname res@qwen@tb@syncpool@Full@sparse\endcsname{92.72}
\expandafter\def\csname res@qwen@tb@coin@Full@auto\endcsname{23.47}
\expandafter\def\csname res@qwen@tb@coin@Full@dense\endcsname{22.75}
\expandafter\def\csname res@qwen@tb@coin@Full@sparse\endcsname{31.56}
\expandafter\def\csname res@qwen@tb@hubdrop@Full@auto\endcsname{129.86}
\expandafter\def\csname res@qwen@tb@coin@any@speedupmax\endcsname{2.8}
\expandafter\def\csname res@qwen@tb@syncpool@any@speedupmax\endcsname{1.8}
\expandafter\def\csname res@qwen@tb@mwis@any@speedupmax\endcsname{2.5}
\expandafter\def\csname res@qwen@tb@basic@any@speedupmax\endcsname{1.8}
\expandafter\def\csname res@qwen@tb@cnt@16@keys\endcsname{16}
\expandafter\def\csname res@qwen@tb@cnt@16@pairs\endcsname{1}
\expandafter\def\csname res@qwen@tb@cnt@16@nodes\endcsname{1}
\expandafter\def\csname res@qwen@tb@cnt@16@survivors\endcsname{15}
\expandafter\def\csname res@qwen@tb@cnt@64@keys\endcsname{64}
\expandafter\def\csname res@qwen@tb@cnt@64@pairs\endcsname{7}
\expandafter\def\csname res@qwen@tb@cnt@64@nodes\endcsname{6}
\expandafter\def\csname res@qwen@tb@cnt@64@survivors\endcsname{57}
\expandafter\def\csname res@qwen@tb@cnt@256@keys\endcsname{256}
\expandafter\def\csname res@qwen@tb@cnt@256@pairs\endcsname{60}
\expandafter\def\csname res@qwen@tb@cnt@256@nodes\endcsname{36}
\expandafter\def\csname res@qwen@tb@cnt@256@survivors\endcsname{209}
\expandafter\def\csname res@qwen@tb@cnt@1k@keys\endcsname{1{,}024}
\expandafter\def\csname res@qwen@tb@cnt@1k@pairs\endcsname{417}
\expandafter\def\csname res@qwen@tb@cnt@1k@nodes\endcsname{190}
\expandafter\def\csname res@qwen@tb@cnt@1k@survivors\endcsname{767}
\expandafter\def\csname res@qwen@tb@cnt@4k@keys\endcsname{4{,}096}
\expandafter\def\csname res@qwen@tb@cnt@4k@pairs\endcsname{3{,}340}
\expandafter\def\csname res@qwen@tb@cnt@4k@nodes\endcsname{890}
\expandafter\def\csname res@qwen@tb@cnt@4k@survivors\endcsname{2{,}579}
\expandafter\def\csname res@qwen@tb@cnt@Full@keys\endcsname{151{,}643}
\expandafter\def\csname res@qwen@tb@cnt@Full@pairs\endcsname{519{,}106}
\expandafter\def\csname res@qwen@tb@cnt@Full@nodes\endcsname{45{,}399}
\expandafter\def\csname res@qwen@tb@cnt@Full@survivors\endcsname{63{,}310}
\expandafter\def\csname res@llmjp@tb@native@16@auto\endcsname{0.71}
\expandafter\def\csname res@llmjp@tb@basic@16@auto\endcsname{0.87}
\expandafter\def\csname res@llmjp@tb@basic@16@dense\endcsname{1.24}
\expandafter\def\csname res@llmjp@tb@basic@16@sparse\endcsname{0.86}
\expandafter\def\csname res@llmjp@tb@mwis@16@auto\endcsname{0.92}
\expandafter\def\csname res@llmjp@tb@mwis@16@dense\endcsname{1.59}
\expandafter\def\csname res@llmjp@tb@mwis@16@sparse\endcsname{0.91}
\expandafter\def\csname res@llmjp@tb@stepwise@16@auto\endcsname{1.47}
\expandafter\def\csname res@llmjp@tb@syncpool@16@auto\endcsname{0.93}
\expandafter\def\csname res@llmjp@tb@syncpool@16@dense\endcsname{1.31}
\expandafter\def\csname res@llmjp@tb@syncpool@16@sparse\endcsname{0.90}
\expandafter\def\csname res@llmjp@tb@coin@16@auto\endcsname{0.99}
\expandafter\def\csname res@llmjp@tb@coin@16@dense\endcsname{1.94}
\expandafter\def\csname res@llmjp@tb@coin@16@sparse\endcsname{0.90}
\expandafter\def\csname res@llmjp@tb@hubdrop@16@auto\endcsname{1.02}
\expandafter\def\csname res@llmjp@tb@native@64@auto\endcsname{0.73}
\expandafter\def\csname res@llmjp@tb@basic@64@auto\endcsname{0.98}
\expandafter\def\csname res@llmjp@tb@basic@64@dense\endcsname{1.36}
\expandafter\def\csname res@llmjp@tb@basic@64@sparse\endcsname{0.97}
\expandafter\def\csname res@llmjp@tb@mwis@64@auto\endcsname{0.98}
\expandafter\def\csname res@llmjp@tb@mwis@64@dense\endcsname{1.65}
\expandafter\def\csname res@llmjp@tb@mwis@64@sparse\endcsname{0.97}
\expandafter\def\csname res@llmjp@tb@stepwise@64@auto\endcsname{3.08}
\expandafter\def\csname res@llmjp@tb@syncpool@64@auto\endcsname{0.99}
\expandafter\def\csname res@llmjp@tb@syncpool@64@dense\endcsname{1.36}
\expandafter\def\csname res@llmjp@tb@syncpool@64@sparse\endcsname{0.95}
\expandafter\def\csname res@llmjp@tb@coin@64@auto\endcsname{1.02}
\expandafter\def\csname res@llmjp@tb@coin@64@dense\endcsname{1.98}
\expandafter\def\csname res@llmjp@tb@coin@64@sparse\endcsname{0.94}
\expandafter\def\csname res@llmjp@tb@hubdrop@64@auto\endcsname{1.10}
\expandafter\def\csname res@llmjp@tb@native@256@auto\endcsname{0.83}
\expandafter\def\csname res@llmjp@tb@basic@256@auto\endcsname{1.40}
\expandafter\def\csname res@llmjp@tb@basic@256@dense\endcsname{1.78}
\expandafter\def\csname res@llmjp@tb@basic@256@sparse\endcsname{1.41}
\expandafter\def\csname res@llmjp@tb@mwis@256@auto\endcsname{1.17}
\expandafter\def\csname res@llmjp@tb@mwis@256@dense\endcsname{1.83}
\expandafter\def\csname res@llmjp@tb@mwis@256@sparse\endcsname{1.16}
\expandafter\def\csname res@llmjp@tb@stepwise@256@auto\endcsname{9.73}
\expandafter\def\csname res@llmjp@tb@syncpool@256@auto\endcsname{1.18}
\expandafter\def\csname res@llmjp@tb@syncpool@256@dense\endcsname{1.54}
\expandafter\def\csname res@llmjp@tb@syncpool@256@sparse\endcsname{1.14}
\expandafter\def\csname res@llmjp@tb@coin@256@auto\endcsname{1.16}
\expandafter\def\csname res@llmjp@tb@coin@256@dense\endcsname{2.10}
\expandafter\def\csname res@llmjp@tb@coin@256@sparse\endcsname{1.08}
\expandafter\def\csname res@llmjp@tb@hubdrop@256@auto\endcsname{1.41}
\expandafter\def\csname res@llmjp@tb@native@1k@auto\endcsname{1.22}
\expandafter\def\csname res@llmjp@tb@basic@1k@auto\endcsname{3.26}
\expandafter\def\csname res@llmjp@tb@basic@1k@dense\endcsname{3.63}
\expandafter\def\csname res@llmjp@tb@basic@1k@sparse\endcsname{3.26}
\expandafter\def\csname res@llmjp@tb@mwis@1k@auto\endcsname{1.82}
\expandafter\def\csname res@llmjp@tb@mwis@1k@dense\endcsname{2.47}
\expandafter\def\csname res@llmjp@tb@mwis@1k@sparse\endcsname{1.81}
\expandafter\def\csname res@llmjp@tb@stepwise@1k@auto\endcsname{36.55}
\expandafter\def\csname res@llmjp@tb@syncpool@1k@auto\endcsname{1.88}
\expandafter\def\csname res@llmjp@tb@syncpool@1k@dense\endcsname{2.26}
\expandafter\def\csname res@llmjp@tb@syncpool@1k@sparse\endcsname{1.86}
\expandafter\def\csname res@llmjp@tb@coin@1k@auto\endcsname{1.64}
\expandafter\def\csname res@llmjp@tb@coin@1k@dense\endcsname{2.58}
\expandafter\def\csname res@llmjp@tb@coin@1k@sparse\endcsname{1.56}
\expandafter\def\csname res@llmjp@tb@hubdrop@1k@auto\endcsname{2.39}
\expandafter\def\csname res@llmjp@tb@native@4k@auto\endcsname{1.85}
\expandafter\def\csname res@llmjp@tb@mwis@4k@auto\endcsname{3.51}
\expandafter\def\csname res@llmjp@tb@mwis@4k@dense\endcsname{4.21}
\expandafter\def\csname res@llmjp@tb@mwis@4k@sparse\endcsname{3.54}
\expandafter\def\csname res@llmjp@tb@stepwise@4k@auto\endcsname{148.21}
\expandafter\def\csname res@llmjp@tb@syncpool@4k@auto\endcsname{3.84}
\expandafter\def\csname res@llmjp@tb@syncpool@4k@dense\endcsname{4.28}
\expandafter\def\csname res@llmjp@tb@syncpool@4k@sparse\endcsname{3.84}
\expandafter\def\csname res@llmjp@tb@coin@4k@auto\endcsname{2.71}
\expandafter\def\csname res@llmjp@tb@coin@4k@dense\endcsname{3.71}
\expandafter\def\csname res@llmjp@tb@coin@4k@sparse\endcsname{2.63}
\expandafter\def\csname res@llmjp@tb@hubdrop@4k@auto\endcsname{5.44}
\expandafter\def\csname res@llmjp@tb@native@Full@auto\endcsname{6.62}
\expandafter\def\csname res@llmjp@tb@mwis@Full@auto\endcsname{43.70}
\expandafter\def\csname res@llmjp@tb@mwis@Full@dense\endcsname{43.19}
\expandafter\def\csname res@llmjp@tb@mwis@Full@sparse\endcsname{45.35}
\expandafter\def\csname res@llmjp@tb@syncpool@Full@auto\endcsname{59.36}
\expandafter\def\csname res@llmjp@tb@syncpool@Full@dense\endcsname{59.08}
\expandafter\def\csname res@llmjp@tb@syncpool@Full@sparse\endcsname{61.54}
\expandafter\def\csname res@llmjp@tb@coin@Full@auto\endcsname{14.54}
\expandafter\def\csname res@llmjp@tb@coin@Full@dense\endcsname{14.25}
\expandafter\def\csname res@llmjp@tb@coin@Full@sparse\endcsname{19.02}
\expandafter\def\csname res@llmjp@tb@hubdrop@Full@auto\endcsname{96.58}
\expandafter\def\csname res@llmjp@tb@coin@any@speedupmax\endcsname{2.2}
\expandafter\def\csname res@llmjp@tb@syncpool@any@speedupmax\endcsname{1.5}
\expandafter\def\csname res@llmjp@tb@mwis@any@speedupmax\endcsname{1.7}
\expandafter\def\csname res@llmjp@tb@basic@any@speedupmax\endcsname{1.4}
\expandafter\def\csname res@llmjp@tb@cnt@16@keys\endcsname{16}
\expandafter\def\csname res@llmjp@tb@cnt@16@pairs\endcsname{5}
\expandafter\def\csname res@llmjp@tb@cnt@16@nodes\endcsname{2}
\expandafter\def\csname res@llmjp@tb@cnt@16@survivors\endcsname{14}
\expandafter\def\csname res@llmjp@tb@cnt@64@keys\endcsname{64}
\expandafter\def\csname res@llmjp@tb@cnt@64@pairs\endcsname{38}
\expandafter\def\csname res@llmjp@tb@cnt@64@nodes\endcsname{10}
\expandafter\def\csname res@llmjp@tb@cnt@64@survivors\endcsname{51}
\expandafter\def\csname res@llmjp@tb@cnt@256@keys\endcsname{256}
\expandafter\def\csname res@llmjp@tb@cnt@256@pairs\endcsname{198}
\expandafter\def\csname res@llmjp@tb@cnt@256@nodes\endcsname{39}
\expandafter\def\csname res@llmjp@tb@cnt@256@survivors\endcsname{196}
\expandafter\def\csname res@llmjp@tb@cnt@1k@keys\endcsname{1{,}024}
\expandafter\def\csname res@llmjp@tb@cnt@1k@pairs\endcsname{1{,}077}
\expandafter\def\csname res@llmjp@tb@cnt@1k@nodes\endcsname{185}
\expandafter\def\csname res@llmjp@tb@cnt@1k@survivors\endcsname{738}
\expandafter\def\csname res@llmjp@tb@cnt@4k@keys\endcsname{4{,}096}
\expandafter\def\csname res@llmjp@tb@cnt@4k@pairs\endcsname{6{,}006}
\expandafter\def\csname res@llmjp@tb@cnt@4k@nodes\endcsname{871}
\expandafter\def\csname res@llmjp@tb@cnt@4k@survivors\endcsname{2{,}719}
\expandafter\def\csname res@llmjp@tb@cnt@Full@keys\endcsname{99{,}441}
\expandafter\def\csname res@llmjp@tb@cnt@Full@pairs\endcsname{245{,}534}
\expandafter\def\csname res@llmjp@tb@cnt@Full@nodes\endcsname{23{,}850}
\expandafter\def\csname res@llmjp@tb@cnt@Full@survivors\endcsname{58{,}954}
\expandafter\def\csname res@llama@long@Full@nativeutil\endcsname{.998}
\expandafter\def\csname res@llama@long@Full@nativebpt\endcsname{3.93}
\expandafter\def\csname res@llama@long@Full@nativeerr\endcsname{5}
\expandafter\def\csname res@llama@long@Full@syncpoolutil\endcsname{.139}
\expandafter\def\csname res@llama@long@Full@syncpoolbpt\endcsname{0.56}
\expandafter\def\csname res@llama@long@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@long@Full@coinutil\endcsname{.904}
\expandafter\def\csname res@llama@long@Full@coinbpt\endcsname{3.63}
\expandafter\def\csname res@llama@long@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@long@Full@gain\endcsname{6.49}
\expandafter\def\csname res@llama@long@Full@gainlo\endcsname{5.69}
\expandafter\def\csname res@llama@long@Full@gainhi\endcsname{7.37}
\expandafter\def\csname res@llama@long@Full@n\endcsname{30}
\expandafter\def\csname res@llama@temp@256@nativeutil\endcsname{.984}
\expandafter\def\csname res@llama@temp@256@nativebpt\endcsname{1.68}
\expandafter\def\csname res@llama@temp@256@nativeerr\endcsname{0}
\expandafter\def\csname res@llama@temp@256@stepwiseutil\endcsname{.992}
\expandafter\def\csname res@llama@temp@256@stepwisebpt\endcsname{1.72}
\expandafter\def\csname res@llama@temp@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llama@temp@256@syncpoolutil\endcsname{.290}
\expandafter\def\csname res@llama@temp@256@syncpoolbpt\endcsname{0.48}
\expandafter\def\csname res@llama@temp@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@temp@256@coinutil\endcsname{.870}
\expandafter\def\csname res@llama@temp@256@coinbpt\endcsname{1.50}
\expandafter\def\csname res@llama@temp@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@temp@256@gain\endcsname{3.00}
\expandafter\def\csname res@llama@temp@256@gainlo\endcsname{2.62}
\expandafter\def\csname res@llama@temp@256@gainhi\endcsname{3.42}
\expandafter\def\csname res@llama@temp@256@n\endcsname{50}
\expandafter\def\csname res@llama@temp@256@pred\endcsname{3.06}
\expandafter\def\csname res@llama@temp@256@stepwisekl\endcsname{.0016}
\expandafter\def\csname res@llama@temp@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llama@temp@256@gainsw\endcsname{0.88}
\expandafter\def\csname res@llama@temp@256@gainswlo\endcsname{0.84}
\expandafter\def\csname res@llama@temp@256@gainswhi\endcsname{0.92}
\expandafter\def\csname res@llama@temp@Full@nativeutil\endcsname{.987}
\expandafter\def\csname res@llama@temp@Full@nativebpt\endcsname{1.70}
\expandafter\def\csname res@llama@temp@Full@nativeerr\endcsname{0}
\expandafter\def\csname res@llama@temp@Full@syncpoolutil\endcsname{.102}
\expandafter\def\csname res@llama@temp@Full@syncpoolbpt\endcsname{0.18}
\expandafter\def\csname res@llama@temp@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@temp@Full@coinutil\endcsname{.918}
\expandafter\def\csname res@llama@temp@Full@coinbpt\endcsname{1.59}
\expandafter\def\csname res@llama@temp@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@temp@Full@gain\endcsname{9.00}
\expandafter\def\csname res@llama@temp@Full@gainlo\endcsname{6.87}
\expandafter\def\csname res@llama@temp@Full@gainhi\endcsname{11.94}
\expandafter\def\csname res@llama@temp@Full@n\endcsname{50}
\expandafter\def\csname res@llama@temp@Full@pred\endcsname{5.32}
\expandafter\def\csname res@llama@nucleus@256@nativeutil\endcsname{.959}
\expandafter\def\csname res@llama@nucleus@256@nativebpt\endcsname{2.86}
\expandafter\def\csname res@llama@nucleus@256@nativeerr\endcsname{1}
\expandafter\def\csname res@llama@nucleus@256@stepwiseutil\endcsname{.938}
\expandafter\def\csname res@llama@nucleus@256@stepwisebpt\endcsname{2.79}
\expandafter\def\csname res@llama@nucleus@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llama@nucleus@256@syncpoolutil\endcsname{.469}
\expandafter\def\csname res@llama@nucleus@256@syncpoolbpt\endcsname{1.43}
\expandafter\def\csname res@llama@nucleus@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@nucleus@256@coinutil\endcsname{.861}
\expandafter\def\csname res@llama@nucleus@256@coinbpt\endcsname{2.42}
\expandafter\def\csname res@llama@nucleus@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@nucleus@256@gain\endcsname{1.84}
\expandafter\def\csname res@llama@nucleus@256@gainlo\endcsname{1.71}
\expandafter\def\csname res@llama@nucleus@256@gainhi\endcsname{1.99}
\expandafter\def\csname res@llama@nucleus@256@n\endcsname{50}
\expandafter\def\csname res@llama@nucleus@256@pred\endcsname{1.97}
\expandafter\def\csname res@llama@nucleus@256@stepwisekl\endcsname{.00047}
\expandafter\def\csname res@llama@nucleus@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llama@nucleus@256@gainsw\endcsname{0.92}
\expandafter\def\csname res@llama@nucleus@256@gainswlo\endcsname{0.89}
\expandafter\def\csname res@llama@nucleus@256@gainswhi\endcsname{0.95}
\expandafter\def\csname res@llama@nucleus@Full@nativeutil\endcsname{.994}
\expandafter\def\csname res@llama@nucleus@Full@nativebpt\endcsname{3.11}
\expandafter\def\csname res@llama@nucleus@Full@nativeerr\endcsname{2}
\expandafter\def\csname res@llama@nucleus@Full@syncpoolutil\endcsname{.412}
\expandafter\def\csname res@llama@nucleus@Full@syncpoolbpt\endcsname{1.30}
\expandafter\def\csname res@llama@nucleus@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@nucleus@Full@coinutil\endcsname{.920}
\expandafter\def\csname res@llama@nucleus@Full@coinbpt\endcsname{2.76}
\expandafter\def\csname res@llama@nucleus@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@nucleus@Full@gain\endcsname{2.23}
\expandafter\def\csname res@llama@nucleus@Full@gainlo\endcsname{2.03}
\expandafter\def\csname res@llama@nucleus@Full@gainhi\endcsname{2.46}
\expandafter\def\csname res@llama@nucleus@Full@n\endcsname{50}
\expandafter\def\csname res@llama@nucleus@Full@pred\endcsname{2.16}
\expandafter\def\csname res@llama@prompt@256@nativeutil\endcsname{.906}
\expandafter\def\csname res@llama@prompt@256@nativebpt\endcsname{2.99}
\expandafter\def\csname res@llama@prompt@256@nativeerr\endcsname{1}
\expandafter\def\csname res@llama@prompt@256@stepwiseutil\endcsname{.904}
\expandafter\def\csname res@llama@prompt@256@stepwisebpt\endcsname{2.97}
\expandafter\def\csname res@llama@prompt@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@256@syncpoolutil\endcsname{.265}
\expandafter\def\csname res@llama@prompt@256@syncpoolbpt\endcsname{0.86}
\expandafter\def\csname res@llama@prompt@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@256@coinutil\endcsname{.834}
\expandafter\def\csname res@llama@prompt@256@coinbpt\endcsname{2.84}
\expandafter\def\csname res@llama@prompt@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@256@gain\endcsname{3.15}
\expandafter\def\csname res@llama@prompt@256@gainlo\endcsname{2.81}
\expandafter\def\csname res@llama@prompt@256@gainhi\endcsname{3.59}
\expandafter\def\csname res@llama@prompt@256@n\endcsname{50}
\expandafter\def\csname res@llama@prompt@256@pred\endcsname{3.16}
\expandafter\def\csname res@llama@prompt@256@stepwisekl\endcsname{.00042}
\expandafter\def\csname res@llama@prompt@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llama@prompt@256@gainsw\endcsname{0.92}
\expandafter\def\csname res@llama@prompt@256@gainswlo\endcsname{0.90}
\expandafter\def\csname res@llama@prompt@256@gainswhi\endcsname{0.95}
\expandafter\def\csname res@llama@prompt@Full@nativeutil\endcsname{.971}
\expandafter\def\csname res@llama@prompt@Full@nativebpt\endcsname{3.35}
\expandafter\def\csname res@llama@prompt@Full@nativeerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@Full@syncpoolutil\endcsname{.107}
\expandafter\def\csname res@llama@prompt@Full@syncpoolbpt\endcsname{0.37}
\expandafter\def\csname res@llama@prompt@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@Full@coinutil\endcsname{.897}
\expandafter\def\csname res@llama@prompt@Full@coinbpt\endcsname{2.98}
\expandafter\def\csname res@llama@prompt@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@prompt@Full@gain\endcsname{8.36}
\expandafter\def\csname res@llama@prompt@Full@gainlo\endcsname{7.40}
\expandafter\def\csname res@llama@prompt@Full@gainhi\endcsname{9.46}
\expandafter\def\csname res@llama@prompt@Full@n\endcsname{50}
\expandafter\def\csname res@llama@prompt@Full@pred\endcsname{7.17}
\expandafter\def\csname res@qwen@long@Full@nativeutil\endcsname{1.003}
\expandafter\def\csname res@qwen@long@Full@nativebpt\endcsname{4.39}
\expandafter\def\csname res@qwen@long@Full@nativeerr\endcsname{16}
\expandafter\def\csname res@qwen@long@Full@syncpoolutil\endcsname{.397}
\expandafter\def\csname res@qwen@long@Full@syncpoolbpt\endcsname{1.89}
\expandafter\def\csname res@qwen@long@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@long@Full@coinutil\endcsname{.922}
\expandafter\def\csname res@qwen@long@Full@coinbpt\endcsname{4.05}
\expandafter\def\csname res@qwen@long@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@long@Full@gain\endcsname{2.32}
\expandafter\def\csname res@qwen@long@Full@gainlo\endcsname{2.21}
\expandafter\def\csname res@qwen@long@Full@gainhi\endcsname{2.44}
\expandafter\def\csname res@qwen@long@Full@n\endcsname{30}
\expandafter\def\csname res@qwen@temp@256@nativeutil\endcsname{.935}
\expandafter\def\csname res@qwen@temp@256@nativebpt\endcsname{1.36}
\expandafter\def\csname res@qwen@temp@256@nativeerr\endcsname{4}
\expandafter\def\csname res@qwen@temp@256@stepwiseutil\endcsname{.956}
\expandafter\def\csname res@qwen@temp@256@stepwisebpt\endcsname{1.33}
\expandafter\def\csname res@qwen@temp@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@qwen@temp@256@syncpoolutil\endcsname{.823}
\expandafter\def\csname res@qwen@temp@256@syncpoolbpt\endcsname{1.22}
\expandafter\def\csname res@qwen@temp@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@temp@256@coinutil\endcsname{.856}
\expandafter\def\csname res@qwen@temp@256@coinbpt\endcsname{1.21}
\expandafter\def\csname res@qwen@temp@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@temp@256@gain\endcsname{1.04}
\expandafter\def\csname res@qwen@temp@256@gainlo\endcsname{1.00}
\expandafter\def\csname res@qwen@temp@256@gainhi\endcsname{1.09}
\expandafter\def\csname res@qwen@temp@256@n\endcsname{50}
\expandafter\def\csname res@qwen@temp@256@pred\endcsname{1.06}
\expandafter\def\csname res@qwen@temp@256@stepwisekl\endcsname{.043}
\expandafter\def\csname res@qwen@temp@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@qwen@temp@256@gainsw\endcsname{0.90}
\expandafter\def\csname res@qwen@temp@256@gainswlo\endcsname{0.85}
\expandafter\def\csname res@qwen@temp@256@gainswhi\endcsname{0.94}
\expandafter\def\csname res@qwen@temp@Full@nativeutil\endcsname{.968}
\expandafter\def\csname res@qwen@temp@Full@nativebpt\endcsname{1.50}
\expandafter\def\csname res@qwen@temp@Full@nativeerr\endcsname{2}
\expandafter\def\csname res@qwen@temp@Full@syncpoolutil\endcsname{.543}
\expandafter\def\csname res@qwen@temp@Full@syncpoolbpt\endcsname{0.85}
\expandafter\def\csname res@qwen@temp@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@temp@Full@coinutil\endcsname{.902}
\expandafter\def\csname res@qwen@temp@Full@coinbpt\endcsname{1.41}
\expandafter\def\csname res@qwen@temp@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@temp@Full@gain\endcsname{1.66}
\expandafter\def\csname res@qwen@temp@Full@gainlo\endcsname{1.56}
\expandafter\def\csname res@qwen@temp@Full@gainhi\endcsname{1.77}
\expandafter\def\csname res@qwen@temp@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@temp@Full@pred\endcsname{1.60}
\expandafter\def\csname res@qwen@nucleus@256@nativeutil\endcsname{.928}
\expandafter\def\csname res@qwen@nucleus@256@nativebpt\endcsname{2.76}
\expandafter\def\csname res@qwen@nucleus@256@nativeerr\endcsname{3}
\expandafter\def\csname res@qwen@nucleus@256@stepwiseutil\endcsname{.919}
\expandafter\def\csname res@qwen@nucleus@256@stepwisebpt\endcsname{2.62}
\expandafter\def\csname res@qwen@nucleus@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@qwen@nucleus@256@syncpoolutil\endcsname{.800}
\expandafter\def\csname res@qwen@nucleus@256@syncpoolbpt\endcsname{2.43}
\expandafter\def\csname res@qwen@nucleus@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@nucleus@256@coinutil\endcsname{.852}
\expandafter\def\csname res@qwen@nucleus@256@coinbpt\endcsname{2.42}
\expandafter\def\csname res@qwen@nucleus@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@nucleus@256@gain\endcsname{1.07}
\expandafter\def\csname res@qwen@nucleus@256@gainlo\endcsname{1.04}
\expandafter\def\csname res@qwen@nucleus@256@gainhi\endcsname{1.10}
\expandafter\def\csname res@qwen@nucleus@256@n\endcsname{50}
\expandafter\def\csname res@qwen@nucleus@256@pred\endcsname{1.08}
\expandafter\def\csname res@qwen@nucleus@256@stepwisekl\endcsname{$\infty$}
\expandafter\def\csname res@qwen@nucleus@256@stepwiseoutside\endcsname{5}
\expandafter\def\csname res@qwen@nucleus@256@gainsw\endcsname{0.93}
\expandafter\def\csname res@qwen@nucleus@256@gainswlo\endcsname{0.90}
\expandafter\def\csname res@qwen@nucleus@256@gainswhi\endcsname{0.95}
\expandafter\def\csname res@qwen@nucleus@Full@nativeutil\endcsname{.987}
\expandafter\def\csname res@qwen@nucleus@Full@nativebpt\endcsname{3.20}
\expandafter\def\csname res@qwen@nucleus@Full@nativeerr\endcsname{12}
\expandafter\def\csname res@qwen@nucleus@Full@syncpoolutil\endcsname{.803}
\expandafter\def\csname res@qwen@nucleus@Full@syncpoolbpt\endcsname{2.65}
\expandafter\def\csname res@qwen@nucleus@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@nucleus@Full@coinutil\endcsname{.920}
\expandafter\def\csname res@qwen@nucleus@Full@coinbpt\endcsname{2.93}
\expandafter\def\csname res@qwen@nucleus@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@nucleus@Full@gain\endcsname{1.15}
\expandafter\def\csname res@qwen@nucleus@Full@gainlo\endcsname{1.10}
\expandafter\def\csname res@qwen@nucleus@Full@gainhi\endcsname{1.20}
\expandafter\def\csname res@qwen@nucleus@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@nucleus@Full@pred\endcsname{1.11}
\expandafter\def\csname res@qwen@prompt@256@nativeutil\endcsname{.854}
\expandafter\def\csname res@qwen@prompt@256@nativebpt\endcsname{2.61}
\expandafter\def\csname res@qwen@prompt@256@nativeerr\endcsname{3}
\expandafter\def\csname res@qwen@prompt@256@stepwiseutil\endcsname{.855}
\expandafter\def\csname res@qwen@prompt@256@stepwisebpt\endcsname{3.05}
\expandafter\def\csname res@qwen@prompt@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@qwen@prompt@256@syncpoolutil\endcsname{.727}
\expandafter\def\csname res@qwen@prompt@256@syncpoolbpt\endcsname{2.42}
\expandafter\def\csname res@qwen@prompt@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@prompt@256@coinutil\endcsname{.780}
\expandafter\def\csname res@qwen@prompt@256@coinbpt\endcsname{2.51}
\expandafter\def\csname res@qwen@prompt@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@prompt@256@gain\endcsname{1.07}
\expandafter\def\csname res@qwen@prompt@256@gainlo\endcsname{1.03}
\expandafter\def\csname res@qwen@prompt@256@gainhi\endcsname{1.12}
\expandafter\def\csname res@qwen@prompt@256@n\endcsname{50}
\expandafter\def\csname res@qwen@prompt@256@pred\endcsname{1.09}
\expandafter\def\csname res@qwen@prompt@256@stepwisekl\endcsname{.030}
\expandafter\def\csname res@qwen@prompt@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@qwen@prompt@256@gainsw\endcsname{0.91}
\expandafter\def\csname res@qwen@prompt@256@gainswlo\endcsname{0.88}
\expandafter\def\csname res@qwen@prompt@256@gainswhi\endcsname{0.94}
\expandafter\def\csname res@qwen@prompt@Full@nativeutil\endcsname{1.003}
\expandafter\def\csname res@qwen@prompt@Full@nativebpt\endcsname{3.73}
\expandafter\def\csname res@qwen@prompt@Full@nativeerr\endcsname{8}
\expandafter\def\csname res@qwen@prompt@Full@syncpoolutil\endcsname{.419}
\expandafter\def\csname res@qwen@prompt@Full@syncpoolbpt\endcsname{1.68}
\expandafter\def\csname res@qwen@prompt@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@prompt@Full@coinutil\endcsname{.912}
\expandafter\def\csname res@qwen@prompt@Full@coinbpt\endcsname{3.68}
\expandafter\def\csname res@qwen@prompt@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@prompt@Full@gain\endcsname{2.18}
\expandafter\def\csname res@qwen@prompt@Full@gainlo\endcsname{2.07}
\expandafter\def\csname res@qwen@prompt@Full@gainhi\endcsname{2.28}
\expandafter\def\csname res@qwen@prompt@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@prompt@Full@pred\endcsname{2.11}
\expandafter\def\csname res@llmjp@long@Full@nativeutil\endcsname{.998}
\expandafter\def\csname res@llmjp@long@Full@nativebpt\endcsname{4.86}
\expandafter\def\csname res@llmjp@long@Full@nativeerr\endcsname{19}
\expandafter\def\csname res@llmjp@long@Full@syncpoolutil\endcsname{.321}
\expandafter\def\csname res@llmjp@long@Full@syncpoolbpt\endcsname{1.52}
\expandafter\def\csname res@llmjp@long@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@long@Full@coinutil\endcsname{.921}
\expandafter\def\csname res@llmjp@long@Full@coinbpt\endcsname{4.30}
\expandafter\def\csname res@llmjp@long@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@long@Full@gain\endcsname{2.87}
\expandafter\def\csname res@llmjp@long@Full@gainlo\endcsname{2.69}
\expandafter\def\csname res@llmjp@long@Full@gainhi\endcsname{3.09}
\expandafter\def\csname res@llmjp@long@Full@n\endcsname{30}
\expandafter\def\csname res@llmjp@temp@256@nativeutil\endcsname{.923}
\expandafter\def\csname res@llmjp@temp@256@nativebpt\endcsname{1.34}
\expandafter\def\csname res@llmjp@temp@256@nativeerr\endcsname{3}
\expandafter\def\csname res@llmjp@temp@256@stepwiseutil\endcsname{.942}
\expandafter\def\csname res@llmjp@temp@256@stepwisebpt\endcsname{1.44}
\expandafter\def\csname res@llmjp@temp@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llmjp@temp@256@syncpoolutil\endcsname{.724}
\expandafter\def\csname res@llmjp@temp@256@syncpoolbpt\endcsname{1.03}
\expandafter\def\csname res@llmjp@temp@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@temp@256@coinutil\endcsname{.882}
\expandafter\def\csname res@llmjp@temp@256@coinbpt\endcsname{1.33}
\expandafter\def\csname res@llmjp@temp@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@temp@256@gain\endcsname{1.22}
\expandafter\def\csname res@llmjp@temp@256@gainlo\endcsname{1.13}
\expandafter\def\csname res@llmjp@temp@256@gainhi\endcsname{1.33}
\expandafter\def\csname res@llmjp@temp@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@temp@256@pred\endcsname{1.23}
\expandafter\def\csname res@llmjp@temp@256@stepwisekl\endcsname{.0011}
\expandafter\def\csname res@llmjp@temp@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llmjp@temp@256@gainsw\endcsname{0.94}
\expandafter\def\csname res@llmjp@temp@256@gainswlo\endcsname{0.89}
\expandafter\def\csname res@llmjp@temp@256@gainswhi\endcsname{0.98}
\expandafter\def\csname res@llmjp@temp@Full@nativeutil\endcsname{.948}
\expandafter\def\csname res@llmjp@temp@Full@nativebpt\endcsname{1.31}
\expandafter\def\csname res@llmjp@temp@Full@nativeerr\endcsname{3}
\expandafter\def\csname res@llmjp@temp@Full@syncpoolutil\endcsname{.403}
\expandafter\def\csname res@llmjp@temp@Full@syncpoolbpt\endcsname{0.55}
\expandafter\def\csname res@llmjp@temp@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@temp@Full@coinutil\endcsname{.879}
\expandafter\def\csname res@llmjp@temp@Full@coinbpt\endcsname{1.41}
\expandafter\def\csname res@llmjp@temp@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@temp@Full@gain\endcsname{2.18}
\expandafter\def\csname res@llmjp@temp@Full@gainlo\endcsname{1.95}
\expandafter\def\csname res@llmjp@temp@Full@gainhi\endcsname{2.44}
\expandafter\def\csname res@llmjp@temp@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@temp@Full@pred\endcsname{2.11}
\expandafter\def\csname res@llmjp@nucleus@256@nativeutil\endcsname{.879}
\expandafter\def\csname res@llmjp@nucleus@256@nativebpt\endcsname{2.70}
\expandafter\def\csname res@llmjp@nucleus@256@nativeerr\endcsname{3}
\expandafter\def\csname res@llmjp@nucleus@256@stepwiseutil\endcsname{.914}
\expandafter\def\csname res@llmjp@nucleus@256@stepwisebpt\endcsname{2.71}
\expandafter\def\csname res@llmjp@nucleus@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@256@syncpoolutil\endcsname{.707}
\expandafter\def\csname res@llmjp@nucleus@256@syncpoolbpt\endcsname{2.08}
\expandafter\def\csname res@llmjp@nucleus@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@256@coinutil\endcsname{.819}
\expandafter\def\csname res@llmjp@nucleus@256@coinbpt\endcsname{2.51}
\expandafter\def\csname res@llmjp@nucleus@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@256@gain\endcsname{1.16}
\expandafter\def\csname res@llmjp@nucleus@256@gainlo\endcsname{1.11}
\expandafter\def\csname res@llmjp@nucleus@256@gainhi\endcsname{1.22}
\expandafter\def\csname res@llmjp@nucleus@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@nucleus@256@pred\endcsname{1.17}
\expandafter\def\csname res@llmjp@nucleus@256@stepwisekl\endcsname{.0024}
\expandafter\def\csname res@llmjp@nucleus@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@256@gainsw\endcsname{0.90}
\expandafter\def\csname res@llmjp@nucleus@256@gainswlo\endcsname{0.87}
\expandafter\def\csname res@llmjp@nucleus@256@gainswhi\endcsname{0.92}
\expandafter\def\csname res@llmjp@nucleus@Full@nativeutil\endcsname{.985}
\expandafter\def\csname res@llmjp@nucleus@Full@nativebpt\endcsname{3.14}
\expandafter\def\csname res@llmjp@nucleus@Full@nativeerr\endcsname{8}
\expandafter\def\csname res@llmjp@nucleus@Full@syncpoolutil\endcsname{.711}
\expandafter\def\csname res@llmjp@nucleus@Full@syncpoolbpt\endcsname{2.21}
\expandafter\def\csname res@llmjp@nucleus@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@Full@coinutil\endcsname{.911}
\expandafter\def\csname res@llmjp@nucleus@Full@coinbpt\endcsname{3.15}
\expandafter\def\csname res@llmjp@nucleus@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@nucleus@Full@gain\endcsname{1.28}
\expandafter\def\csname res@llmjp@nucleus@Full@gainlo\endcsname{1.21}
\expandafter\def\csname res@llmjp@nucleus@Full@gainhi\endcsname{1.37}
\expandafter\def\csname res@llmjp@nucleus@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@nucleus@Full@pred\endcsname{1.31}
\expandafter\def\csname res@llmjp@prompt@256@nativeutil\endcsname{.827}
\expandafter\def\csname res@llmjp@prompt@256@nativebpt\endcsname{3.01}
\expandafter\def\csname res@llmjp@prompt@256@nativeerr\endcsname{5}
\expandafter\def\csname res@llmjp@prompt@256@stepwiseutil\endcsname{.823}
\expandafter\def\csname res@llmjp@prompt@256@stepwisebpt\endcsname{3.01}
\expandafter\def\csname res@llmjp@prompt@256@stepwiseerr\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@256@syncpoolutil\endcsname{.648}
\expandafter\def\csname res@llmjp@prompt@256@syncpoolbpt\endcsname{2.37}
\expandafter\def\csname res@llmjp@prompt@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@256@coinutil\endcsname{.754}
\expandafter\def\csname res@llmjp@prompt@256@coinbpt\endcsname{2.68}
\expandafter\def\csname res@llmjp@prompt@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@256@gain\endcsname{1.16}
\expandafter\def\csname res@llmjp@prompt@256@gainlo\endcsname{1.12}
\expandafter\def\csname res@llmjp@prompt@256@gainhi\endcsname{1.22}
\expandafter\def\csname res@llmjp@prompt@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@prompt@256@pred\endcsname{1.15}
\expandafter\def\csname res@llmjp@prompt@256@stepwisekl\endcsname{.0023}
\expandafter\def\csname res@llmjp@prompt@256@stepwiseoutside\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@256@gainsw\endcsname{0.92}
\expandafter\def\csname res@llmjp@prompt@256@gainswlo\endcsname{0.89}
\expandafter\def\csname res@llmjp@prompt@256@gainswhi\endcsname{0.95}
\expandafter\def\csname res@llmjp@prompt@Full@nativeutil\endcsname{.981}
\expandafter\def\csname res@llmjp@prompt@Full@nativebpt\endcsname{4.26}
\expandafter\def\csname res@llmjp@prompt@Full@nativeerr\endcsname{13}
\expandafter\def\csname res@llmjp@prompt@Full@syncpoolutil\endcsname{.337}
\expandafter\def\csname res@llmjp@prompt@Full@syncpoolbpt\endcsname{1.44}
\expandafter\def\csname res@llmjp@prompt@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@Full@coinutil\endcsname{.898}
\expandafter\def\csname res@llmjp@prompt@Full@coinbpt\endcsname{3.80}
\expandafter\def\csname res@llmjp@prompt@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@prompt@Full@gain\endcsname{2.66}
\expandafter\def\csname res@llmjp@prompt@Full@gainlo\endcsname{2.51}
\expandafter\def\csname res@llmjp@prompt@Full@gainhi\endcsname{2.84}
\expandafter\def\csname res@llmjp@prompt@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@prompt@Full@pred\endcsname{2.54}
\expandafter\def\csname res@all@robust@gain@min\endcsname{1.04}
\expandafter\def\csname res@all@robust@ci@above\endcsname{2}
\expandafter\def\csname res@all@robust@ci@below\endcsname{0}
\expandafter\def\csname res@all@robust@ci@inside\endcsname{16}
\expandafter\def\csname res@all@robust@ci@n\endcsname{18}
\expandafter\def\csname res@all@robust@gain@max\endcsname{9.00}
\expandafter\def\csname res@all@robust@gainsw@min\endcsname{0.88}
\expandafter\def\csname res@all@robust@gainsw@max\endcsname{0.94}
\expandafter\def\csname res@all@robust@swout@texts\endcsname{5}
\expandafter\def\csname res@all@robust@swout@cells\endcsname{1}
\expandafter\def\csname res@llama@coder@rrc@256@nativeutil\endcsname{.892}
\expandafter\def\csname res@llama@coder@rrc@256@nativebpt\endcsname{3.15}
\expandafter\def\csname res@llama@coder@rrc@256@nativeerr\endcsname{2}
\expandafter\def\csname res@llama@coder@rrc@256@syncpoolutil\endcsname{.245}
\expandafter\def\csname res@llama@coder@rrc@256@syncpoolbpt\endcsname{0.85}
\expandafter\def\csname res@llama@coder@rrc@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@rrc@256@coinutil\endcsname{.812}
\expandafter\def\csname res@llama@coder@rrc@256@coinbpt\endcsname{2.90}
\expandafter\def\csname res@llama@coder@rrc@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@rrc@256@gain\endcsname{3.31}
\expandafter\def\csname res@llama@coder@rrc@256@gainlo\endcsname{2.98}
\expandafter\def\csname res@llama@coder@rrc@256@gainhi\endcsname{3.65}
\expandafter\def\csname res@llama@coder@rrc@256@n\endcsname{50}
\expandafter\def\csname res@llama@coder@discop@256@nativeutil\endcsname{.828}
\expandafter\def\csname res@llama@coder@discop@256@nativebpt\endcsname{2.76}
\expandafter\def\csname res@llama@coder@discop@256@nativeerr\endcsname{1}
\expandafter\def\csname res@llama@coder@discop@256@syncpoolutil\endcsname{.215}
\expandafter\def\csname res@llama@coder@discop@256@syncpoolbpt\endcsname{0.76}
\expandafter\def\csname res@llama@coder@discop@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@discop@256@coinutil\endcsname{.743}
\expandafter\def\csname res@llama@coder@discop@256@coinbpt\endcsname{2.62}
\expandafter\def\csname res@llama@coder@discop@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@discop@256@gain\endcsname{3.45}
\expandafter\def\csname res@llama@coder@discop@256@gainlo\endcsname{3.12}
\expandafter\def\csname res@llama@coder@discop@256@gainhi\endcsname{3.81}
\expandafter\def\csname res@llama@coder@discop@256@n\endcsname{50}
\expandafter\def\csname res@llama@coder@discop@256@coindev\endcsname{-8.5}
\expandafter\def\csname res@llama@coder@ac@256@nativeutil\endcsname{.870}
\expandafter\def\csname res@llama@coder@ac@256@nativebpt\endcsname{2.99}
\expandafter\def\csname res@llama@coder@ac@256@nativeerr\endcsname{2}
\expandafter\def\csname res@llama@coder@ac@256@syncpoolutil\endcsname{.252}
\expandafter\def\csname res@llama@coder@ac@256@syncpoolbpt\endcsname{0.89}
\expandafter\def\csname res@llama@coder@ac@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@ac@256@coinutil\endcsname{.818}
\expandafter\def\csname res@llama@coder@ac@256@coinbpt\endcsname{2.84}
\expandafter\def\csname res@llama@coder@ac@256@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@ac@256@gain\endcsname{3.24}
\expandafter\def\csname res@llama@coder@ac@256@gainlo\endcsname{2.88}
\expandafter\def\csname res@llama@coder@ac@256@gainhi\endcsname{3.63}
\expandafter\def\csname res@llama@coder@ac@256@n\endcsname{50}
\expandafter\def\csname res@llama@coder@ac@256@coindev\endcsname{+0.7}
\expandafter\def\csname res@llama@coder@rrc@Full@nativeutil\endcsname{.989}
\expandafter\def\csname res@llama@coder@rrc@Full@nativebpt\endcsname{3.82}
\expandafter\def\csname res@llama@coder@rrc@Full@nativeerr\endcsname{2}
\expandafter\def\csname res@llama@coder@rrc@Full@syncpoolutil\endcsname{.131}
\expandafter\def\csname res@llama@coder@rrc@Full@syncpoolbpt\endcsname{0.52}
\expandafter\def\csname res@llama@coder@rrc@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@rrc@Full@coinutil\endcsname{.912}
\expandafter\def\csname res@llama@coder@rrc@Full@coinbpt\endcsname{3.54}
\expandafter\def\csname res@llama@coder@rrc@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@rrc@Full@gain\endcsname{6.95}
\expandafter\def\csname res@llama@coder@rrc@Full@gainlo\endcsname{6.15}
\expandafter\def\csname res@llama@coder@rrc@Full@gainhi\endcsname{7.98}
\expandafter\def\csname res@llama@coder@rrc@Full@n\endcsname{50}
\expandafter\def\csname res@llama@coder@discop@Full@nativeutil\endcsname{.917}
\expandafter\def\csname res@llama@coder@discop@Full@nativebpt\endcsname{3.48}
\expandafter\def\csname res@llama@coder@discop@Full@nativeerr\endcsname{4}
\expandafter\def\csname res@llama@coder@discop@Full@syncpoolutil\endcsname{.109}
\expandafter\def\csname res@llama@coder@discop@Full@syncpoolbpt\endcsname{0.42}
\expandafter\def\csname res@llama@coder@discop@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@discop@Full@coinutil\endcsname{.835}
\expandafter\def\csname res@llama@coder@discop@Full@coinbpt\endcsname{3.31}
\expandafter\def\csname res@llama@coder@discop@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@discop@Full@gain\endcsname{7.66}
\expandafter\def\csname res@llama@coder@discop@Full@gainlo\endcsname{6.70}
\expandafter\def\csname res@llama@coder@discop@Full@gainhi\endcsname{8.76}
\expandafter\def\csname res@llama@coder@discop@Full@n\endcsname{50}
\expandafter\def\csname res@llama@coder@discop@Full@coindev\endcsname{-8.4}
\expandafter\def\csname res@llama@coder@ac@Full@nativeutil\endcsname{.978}
\expandafter\def\csname res@llama@coder@ac@Full@nativebpt\endcsname{3.86}
\expandafter\def\csname res@llama@coder@ac@Full@nativeerr\endcsname{4}
\expandafter\def\csname res@llama@coder@ac@Full@syncpoolutil\endcsname{.141}
\expandafter\def\csname res@llama@coder@ac@Full@syncpoolbpt\endcsname{0.54}
\expandafter\def\csname res@llama@coder@ac@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llama@coder@ac@Full@coinutil\endcsname{.906}
\expandafter\def\csname res@llama@coder@ac@Full@coinbpt\endcsname{3.37}
\expandafter\def\csname res@llama@coder@ac@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llama@coder@ac@Full@gain\endcsname{6.42}
\expandafter\def\csname res@llama@coder@ac@Full@gainlo\endcsname{5.80}
\expandafter\def\csname res@llama@coder@ac@Full@gainhi\endcsname{7.10}
\expandafter\def\csname res@llama@coder@ac@Full@n\endcsname{50}
\expandafter\def\csname res@llama@coder@ac@Full@coindev\endcsname{-0.6}
\expandafter\def\csname res@qwen@coder@rrc@256@nativeutil\endcsname{.853}
\expandafter\def\csname res@qwen@coder@rrc@256@nativebpt\endcsname{2.92}
\expandafter\def\csname res@qwen@coder@rrc@256@nativeerr\endcsname{6}
\expandafter\def\csname res@qwen@coder@rrc@256@syncpoolutil\endcsname{.734}
\expandafter\def\csname res@qwen@coder@rrc@256@syncpoolbpt\endcsname{2.68}
\expandafter\def\csname res@qwen@coder@rrc@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@rrc@256@coinutil\endcsname{.797}
\expandafter\def\csname res@qwen@coder@rrc@256@coinbpt\endcsname{2.74}
\expandafter\def\csname res@qwen@coder@rrc@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@rrc@256@gain\endcsname{1.09}
\expandafter\def\csname res@qwen@coder@rrc@256@gainlo\endcsname{1.05}
\expandafter\def\csname res@qwen@coder@rrc@256@gainhi\endcsname{1.13}
\expandafter\def\csname res@qwen@coder@rrc@256@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@discop@256@nativeutil\endcsname{.791}
\expandafter\def\csname res@qwen@coder@discop@256@nativebpt\endcsname{2.81}
\expandafter\def\csname res@qwen@coder@discop@256@nativeerr\endcsname{5}
\expandafter\def\csname res@qwen@coder@discop@256@syncpoolutil\endcsname{.680}
\expandafter\def\csname res@qwen@coder@discop@256@syncpoolbpt\endcsname{2.52}
\expandafter\def\csname res@qwen@coder@discop@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@discop@256@coinutil\endcsname{.724}
\expandafter\def\csname res@qwen@coder@discop@256@coinbpt\endcsname{2.29}
\expandafter\def\csname res@qwen@coder@discop@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@discop@256@gain\endcsname{1.07}
\expandafter\def\csname res@qwen@coder@discop@256@gainlo\endcsname{1.04}
\expandafter\def\csname res@qwen@coder@discop@256@gainhi\endcsname{1.10}
\expandafter\def\csname res@qwen@coder@discop@256@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@discop@256@coindev\endcsname{-9.1}
\expandafter\def\csname res@qwen@coder@ac@256@nativeutil\endcsname{.868}
\expandafter\def\csname res@qwen@coder@ac@256@nativebpt\endcsname{2.91}
\expandafter\def\csname res@qwen@coder@ac@256@nativeerr\endcsname{4}
\expandafter\def\csname res@qwen@coder@ac@256@syncpoolutil\endcsname{.755}
\expandafter\def\csname res@qwen@coder@ac@256@syncpoolbpt\endcsname{2.40}
\expandafter\def\csname res@qwen@coder@ac@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@ac@256@coinutil\endcsname{.791}
\expandafter\def\csname res@qwen@coder@ac@256@coinbpt\endcsname{2.76}
\expandafter\def\csname res@qwen@coder@ac@256@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@ac@256@gain\endcsname{1.05}
\expandafter\def\csname res@qwen@coder@ac@256@gainlo\endcsname{1.02}
\expandafter\def\csname res@qwen@coder@ac@256@gainhi\endcsname{1.08}
\expandafter\def\csname res@qwen@coder@ac@256@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@ac@256@coindev\endcsname{-0.7}
\expandafter\def\csname res@qwen@coder@rrc@Full@nativeutil\endcsname{.989}
\expandafter\def\csname res@qwen@coder@rrc@Full@nativebpt\endcsname{4.09}
\expandafter\def\csname res@qwen@coder@rrc@Full@nativeerr\endcsname{7}
\expandafter\def\csname res@qwen@coder@rrc@Full@syncpoolutil\endcsname{.417}
\expandafter\def\csname res@qwen@coder@rrc@Full@syncpoolbpt\endcsname{1.67}
\expandafter\def\csname res@qwen@coder@rrc@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@rrc@Full@coinutil\endcsname{.928}
\expandafter\def\csname res@qwen@coder@rrc@Full@coinbpt\endcsname{4.06}
\expandafter\def\csname res@qwen@coder@rrc@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@rrc@Full@gain\endcsname{2.23}
\expandafter\def\csname res@qwen@coder@rrc@Full@gainlo\endcsname{2.12}
\expandafter\def\csname res@qwen@coder@rrc@Full@gainhi\endcsname{2.32}
\expandafter\def\csname res@qwen@coder@rrc@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@discop@Full@nativeutil\endcsname{.931}
\expandafter\def\csname res@qwen@coder@discop@Full@nativebpt\endcsname{3.56}
\expandafter\def\csname res@qwen@coder@discop@Full@nativeerr\endcsname{3}
\expandafter\def\csname res@qwen@coder@discop@Full@syncpoolutil\endcsname{.367}
\expandafter\def\csname res@qwen@coder@discop@Full@syncpoolbpt\endcsname{1.51}
\expandafter\def\csname res@qwen@coder@discop@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@discop@Full@coinutil\endcsname{.856}
\expandafter\def\csname res@qwen@coder@discop@Full@coinbpt\endcsname{3.68}
\expandafter\def\csname res@qwen@coder@discop@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@discop@Full@gain\endcsname{2.33}
\expandafter\def\csname res@qwen@coder@discop@Full@gainlo\endcsname{2.25}
\expandafter\def\csname res@qwen@coder@discop@Full@gainhi\endcsname{2.42}
\expandafter\def\csname res@qwen@coder@discop@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@discop@Full@coindev\endcsname{-7.8}
\expandafter\def\csname res@qwen@coder@ac@Full@nativeutil\endcsname{.998}
\expandafter\def\csname res@qwen@coder@ac@Full@nativebpt\endcsname{4.05}
\expandafter\def\csname res@qwen@coder@ac@Full@nativeerr\endcsname{10}
\expandafter\def\csname res@qwen@coder@ac@Full@syncpoolutil\endcsname{.422}
\expandafter\def\csname res@qwen@coder@ac@Full@syncpoolbpt\endcsname{1.83}
\expandafter\def\csname res@qwen@coder@ac@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@ac@Full@coinutil\endcsname{.916}
\expandafter\def\csname res@qwen@coder@ac@Full@coinbpt\endcsname{3.78}
\expandafter\def\csname res@qwen@coder@ac@Full@coinerr\endcsname{0}
\expandafter\def\csname res@qwen@coder@ac@Full@gain\endcsname{2.17}
\expandafter\def\csname res@qwen@coder@ac@Full@gainlo\endcsname{2.05}
\expandafter\def\csname res@qwen@coder@ac@Full@gainhi\endcsname{2.28}
\expandafter\def\csname res@qwen@coder@ac@Full@n\endcsname{50}
\expandafter\def\csname res@qwen@coder@ac@Full@coindev\endcsname{-1.3}
\expandafter\def\csname res@llmjp@coder@rrc@256@nativeutil\endcsname{.821}
\expandafter\def\csname res@llmjp@coder@rrc@256@nativebpt\endcsname{2.83}
\expandafter\def\csname res@llmjp@coder@rrc@256@nativeerr\endcsname{8}
\expandafter\def\csname res@llmjp@coder@rrc@256@syncpoolutil\endcsname{.648}
\expandafter\def\csname res@llmjp@coder@rrc@256@syncpoolbpt\endcsname{2.20}
\expandafter\def\csname res@llmjp@coder@rrc@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@rrc@256@coinutil\endcsname{.775}
\expandafter\def\csname res@llmjp@coder@rrc@256@coinbpt\endcsname{2.87}
\expandafter\def\csname res@llmjp@coder@rrc@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@rrc@256@gain\endcsname{1.20}
\expandafter\def\csname res@llmjp@coder@rrc@256@gainlo\endcsname{1.14}
\expandafter\def\csname res@llmjp@coder@rrc@256@gainhi\endcsname{1.27}
\expandafter\def\csname res@llmjp@coder@rrc@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@discop@256@nativeutil\endcsname{.762}
\expandafter\def\csname res@llmjp@coder@discop@256@nativebpt\endcsname{2.70}
\expandafter\def\csname res@llmjp@coder@discop@256@nativeerr\endcsname{5}
\expandafter\def\csname res@llmjp@coder@discop@256@syncpoolutil\endcsname{.568}
\expandafter\def\csname res@llmjp@coder@discop@256@syncpoolbpt\endcsname{2.03}
\expandafter\def\csname res@llmjp@coder@discop@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@discop@256@coinutil\endcsname{.709}
\expandafter\def\csname res@llmjp@coder@discop@256@coinbpt\endcsname{2.33}
\expandafter\def\csname res@llmjp@coder@discop@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@discop@256@gain\endcsname{1.25}
\expandafter\def\csname res@llmjp@coder@discop@256@gainlo\endcsname{1.18}
\expandafter\def\csname res@llmjp@coder@discop@256@gainhi\endcsname{1.34}
\expandafter\def\csname res@llmjp@coder@discop@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@discop@256@coindev\endcsname{-8.6}
\expandafter\def\csname res@llmjp@coder@ac@256@nativeutil\endcsname{.823}
\expandafter\def\csname res@llmjp@coder@ac@256@nativebpt\endcsname{2.98}
\expandafter\def\csname res@llmjp@coder@ac@256@nativeerr\endcsname{6}
\expandafter\def\csname res@llmjp@coder@ac@256@syncpoolutil\endcsname{.637}
\expandafter\def\csname res@llmjp@coder@ac@256@syncpoolbpt\endcsname{2.31}
\expandafter\def\csname res@llmjp@coder@ac@256@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@ac@256@coinutil\endcsname{.771}
\expandafter\def\csname res@llmjp@coder@ac@256@coinbpt\endcsname{2.80}
\expandafter\def\csname res@llmjp@coder@ac@256@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@ac@256@gain\endcsname{1.21}
\expandafter\def\csname res@llmjp@coder@ac@256@gainlo\endcsname{1.15}
\expandafter\def\csname res@llmjp@coder@ac@256@gainhi\endcsname{1.27}
\expandafter\def\csname res@llmjp@coder@ac@256@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@ac@256@coindev\endcsname{-0.5}
\expandafter\def\csname res@llmjp@coder@rrc@Full@nativeutil\endcsname{.980}
\expandafter\def\csname res@llmjp@coder@rrc@Full@nativebpt\endcsname{4.03}
\expandafter\def\csname res@llmjp@coder@rrc@Full@nativeerr\endcsname{7}
\expandafter\def\csname res@llmjp@coder@rrc@Full@syncpoolutil\endcsname{.332}
\expandafter\def\csname res@llmjp@coder@rrc@Full@syncpoolbpt\endcsname{1.45}
\expandafter\def\csname res@llmjp@coder@rrc@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@rrc@Full@coinutil\endcsname{.918}
\expandafter\def\csname res@llmjp@coder@rrc@Full@coinbpt\endcsname{4.03}
\expandafter\def\csname res@llmjp@coder@rrc@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@rrc@Full@gain\endcsname{2.76}
\expandafter\def\csname res@llmjp@coder@rrc@Full@gainlo\endcsname{2.54}
\expandafter\def\csname res@llmjp@coder@rrc@Full@gainhi\endcsname{3.03}
\expandafter\def\csname res@llmjp@coder@rrc@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@discop@Full@nativeutil\endcsname{.924}
\expandafter\def\csname res@llmjp@coder@discop@Full@nativebpt\endcsname{3.85}
\expandafter\def\csname res@llmjp@coder@discop@Full@nativeerr\endcsname{9}
\expandafter\def\csname res@llmjp@coder@discop@Full@syncpoolutil\endcsname{.282}
\expandafter\def\csname res@llmjp@coder@discop@Full@syncpoolbpt\endcsname{1.22}
\expandafter\def\csname res@llmjp@coder@discop@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@discop@Full@coinutil\endcsname{.850}
\expandafter\def\csname res@llmjp@coder@discop@Full@coinbpt\endcsname{3.45}
\expandafter\def\csname res@llmjp@coder@discop@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@discop@Full@gain\endcsname{3.01}
\expandafter\def\csname res@llmjp@coder@discop@Full@gainlo\endcsname{2.81}
\expandafter\def\csname res@llmjp@coder@discop@Full@gainhi\endcsname{3.23}
\expandafter\def\csname res@llmjp@coder@discop@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@discop@Full@coindev\endcsname{-7.4}
\expandafter\def\csname res@llmjp@coder@ac@Full@nativeutil\endcsname{1.004}
\expandafter\def\csname res@llmjp@coder@ac@Full@nativebpt\endcsname{4.35}
\expandafter\def\csname res@llmjp@coder@ac@Full@nativeerr\endcsname{11}
\expandafter\def\csname res@llmjp@coder@ac@Full@syncpoolutil\endcsname{.334}
\expandafter\def\csname res@llmjp@coder@ac@Full@syncpoolbpt\endcsname{1.34}
\expandafter\def\csname res@llmjp@coder@ac@Full@syncpoolerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@ac@Full@coinutil\endcsname{.929}
\expandafter\def\csname res@llmjp@coder@ac@Full@coinbpt\endcsname{3.97}
\expandafter\def\csname res@llmjp@coder@ac@Full@coinerr\endcsname{0}
\expandafter\def\csname res@llmjp@coder@ac@Full@gain\endcsname{2.79}
\expandafter\def\csname res@llmjp@coder@ac@Full@gainlo\endcsname{2.59}
\expandafter\def\csname res@llmjp@coder@ac@Full@gainhi\endcsname{3.00}
\expandafter\def\csname res@llmjp@coder@ac@Full@n\endcsname{50}
\expandafter\def\csname res@llmjp@coder@ac@Full@coindev\endcsname{+1.3}
\expandafter\def\csname res@all@coder@256@gainmin\endcsname{1.05}
\expandafter\def\csname res@all@coder@256@gainmax\endcsname{3.45}
\expandafter\def\csname res@all@coder@Full@gainmin\endcsname{2.17}
\expandafter\def\csname res@all@coder@Full@gainmax\endcsname{7.66}
\expandafter\def\csname res@all@coder@any@coindevmax\endcsname{9.1}
\expandafter\def\csname res@all@coder@discop@native@devmin\endcsname{-7.4}
\expandafter\def\csname res@all@coder@discop@native@devmax\endcsname{-5.7}
\expandafter\def\csname res@all@coder@discop@native@devabs\endcsname{7.4}
\expandafter\def\csname res@all@coder@discop@syncpool@devmin\endcsname{-16.9}
\expandafter\def\csname res@all@coder@discop@syncpool@devmax\endcsname{-7.4}
\expandafter\def\csname res@all@coder@discop@syncpool@devabs\endcsname{16.9}
\expandafter\def\csname res@all@coder@discop@coin@devmin\endcsname{-9.1}
\expandafter\def\csname res@all@coder@discop@coin@devmax\endcsname{-7.4}
\expandafter\def\csname res@all@coder@discop@coin@devabs\endcsname{9.1}
\expandafter\def\csname res@all@coder@ac@native@devmin\endcsname{-2.4}
\expandafter\def\csname res@all@coder@ac@native@devmax\endcsname{2.5}
\expandafter\def\csname res@all@coder@ac@native@devabs\endcsname{2.5}
\expandafter\def\csname res@all@coder@ac@syncpool@devmin\endcsname{-1.7}
\expandafter\def\csname res@all@coder@ac@syncpool@devmax\endcsname{7.6}
\expandafter\def\csname res@all@coder@ac@syncpool@devabs\endcsname{7.6}
\expandafter\def\csname res@all@coder@ac@coin@devmin\endcsname{-1.3}
\expandafter\def\csname res@all@coder@ac@coin@devmax\endcsname{1.3}
\expandafter\def\csname res@all@coder@ac@coin@devabs\endcsname{1.3}
\expandafter\def\csname res@all@coder@any@exacterr\endcsname{0}
\expandafter\def\csname res@all@coder@any@n\endcsname{50}
\expandafter\def\csname res@llama@gof@basic@16@rej\endcsname{14}
\expandafter\def\csname res@llama@gof@basic@16@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@basic@16@fisher\endcsname{0}
\expandafter\def\csname res@llama@gof@basic@256@rej\endcsname{18}
\expandafter\def\csname res@llama@gof@basic@256@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@basic@256@fisher\endcsname{0}
\expandafter\def\csname res@llama@gof@coin@16@rej\endcsname{0}
\expandafter\def\csname res@llama@gof@coin@16@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@coin@16@fisher\endcsname{0.96}
\expandafter\def\csname res@llama@gof@coin@256@rej\endcsname{1}
\expandafter\def\csname res@llama@gof@coin@256@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@coin@256@fisher\endcsname{0.47}
\expandafter\def\csname res@llama@gof@coin@Full@rej\endcsname{0}
\expandafter\def\csname res@llama@gof@coin@Full@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@coin@Full@fisher\endcsname{0.55}
\expandafter\def\csname res@llama@gof@mwis@16@rej\endcsname{13}
\expandafter\def\csname res@llama@gof@mwis@16@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@mwis@16@fisher\endcsname{0}
\expandafter\def\csname res@llama@gof@mwis@256@rej\endcsname{16}
\expandafter\def\csname res@llama@gof@mwis@256@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@mwis@256@fisher\endcsname{0}
\expandafter\def\csname res@llama@gof@mwis@Full@rej\endcsname{15}
\expandafter\def\csname res@llama@gof@mwis@Full@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@mwis@Full@fisher\endcsname{0}
\expandafter\def\csname res@llama@gof@native@16@rej\endcsname{3}
\expandafter\def\csname res@llama@gof@native@16@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@native@16@fisher\endcsname{0.24}
\expandafter\def\csname res@llama@gof@native@256@rej\endcsname{0}
\expandafter\def\csname res@llama@gof@native@256@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@native@256@fisher\endcsname{0.57}
\expandafter\def\csname res@llama@gof@native@Full@rej\endcsname{1}
\expandafter\def\csname res@llama@gof@native@Full@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@native@Full@fisher\endcsname{0.6}
\expandafter\def\csname res@llama@gof@syncpool@16@rej\endcsname{1}
\expandafter\def\csname res@llama@gof@syncpool@16@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@syncpool@16@fisher\endcsname{0.45}
\expandafter\def\csname res@llama@gof@syncpool@256@rej\endcsname{1}
\expandafter\def\csname res@llama@gof@syncpool@256@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@syncpool@256@fisher\endcsname{0.78}
\expandafter\def\csname res@llama@gof@syncpool@Full@rej\endcsname{0}
\expandafter\def\csname res@llama@gof@syncpool@Full@ctx\endcsname{20}
\expandafter\def\csname res@llama@gof@syncpool@Full@fisher\endcsname{1}
\expandafter\def\csname res@qwen@gof@basic@16@rej\endcsname{17}
\expandafter\def\csname res@qwen@gof@basic@16@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@basic@16@fisher\endcsname{0}
\expandafter\def\csname res@qwen@gof@basic@256@rej\endcsname{19}
\expandafter\def\csname res@qwen@gof@basic@256@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@basic@256@fisher\endcsname{0}
\expandafter\def\csname res@qwen@gof@coin@16@rej\endcsname{0}
\expandafter\def\csname res@qwen@gof@coin@16@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@coin@16@fisher\endcsname{0.49}
\expandafter\def\csname res@qwen@gof@coin@256@rej\endcsname{0}
\expandafter\def\csname res@qwen@gof@coin@256@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@coin@256@fisher\endcsname{0.89}
\expandafter\def\csname res@qwen@gof@coin@Full@rej\endcsname{0}
\expandafter\def\csname res@qwen@gof@coin@Full@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@coin@Full@fisher\endcsname{0.79}
\expandafter\def\csname res@qwen@gof@mwis@16@rej\endcsname{15}
\expandafter\def\csname res@qwen@gof@mwis@16@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@mwis@16@fisher\endcsname{0}
\expandafter\def\csname res@qwen@gof@mwis@256@rej\endcsname{19}
\expandafter\def\csname res@qwen@gof@mwis@256@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@mwis@256@fisher\endcsname{0}
\expandafter\def\csname res@qwen@gof@mwis@Full@rej\endcsname{20}
\expandafter\def\csname res@qwen@gof@mwis@Full@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@mwis@Full@fisher\endcsname{0}
\expandafter\def\csname res@qwen@gof@native@16@rej\endcsname{1}
\expandafter\def\csname res@qwen@gof@native@16@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@native@16@fisher\endcsname{0.14}
\expandafter\def\csname res@qwen@gof@native@256@rej\endcsname{2}
\expandafter\def\csname res@qwen@gof@native@256@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@native@256@fisher\endcsname{0.28}
\expandafter\def\csname res@qwen@gof@native@Full@rej\endcsname{1}
\expandafter\def\csname res@qwen@gof@native@Full@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@native@Full@fisher\endcsname{0.7}
\expandafter\def\csname res@qwen@gof@syncpool@16@rej\endcsname{2}
\expandafter\def\csname res@qwen@gof@syncpool@16@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@syncpool@16@fisher\endcsname{0.14}
\expandafter\def\csname res@qwen@gof@syncpool@256@rej\endcsname{1}
\expandafter\def\csname res@qwen@gof@syncpool@256@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@syncpool@256@fisher\endcsname{0.43}
\expandafter\def\csname res@qwen@gof@syncpool@Full@rej\endcsname{0}
\expandafter\def\csname res@qwen@gof@syncpool@Full@ctx\endcsname{20}
\expandafter\def\csname res@qwen@gof@syncpool@Full@fisher\endcsname{0.84}
\expandafter\def\csname res@llmjp@gof@basic@16@rej\endcsname{15}
\expandafter\def\csname res@llmjp@gof@basic@16@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@basic@16@fisher\endcsname{0}
\expandafter\def\csname res@llmjp@gof@basic@256@rej\endcsname{18}
\expandafter\def\csname res@llmjp@gof@basic@256@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@basic@256@fisher\endcsname{0}
\expandafter\def\csname res@llmjp@gof@coin@16@rej\endcsname{0}
\expandafter\def\csname res@llmjp@gof@coin@16@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@coin@16@fisher\endcsname{0.97}
\expandafter\def\csname res@llmjp@gof@coin@256@rej\endcsname{1}
\expandafter\def\csname res@llmjp@gof@coin@256@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@coin@256@fisher\endcsname{0.27}
\expandafter\def\csname res@llmjp@gof@coin@Full@rej\endcsname{1}
\expandafter\def\csname res@llmjp@gof@coin@Full@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@coin@Full@fisher\endcsname{0.036}
\expandafter\def\csname res@llmjp@gof@mwis@16@rej\endcsname{15}
\expandafter\def\csname res@llmjp@gof@mwis@16@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@mwis@16@fisher\endcsname{0}
\expandafter\def\csname res@llmjp@gof@mwis@256@rej\endcsname{16}
\expandafter\def\csname res@llmjp@gof@mwis@256@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@mwis@256@fisher\endcsname{0}
\expandafter\def\csname res@llmjp@gof@mwis@Full@rej\endcsname{16}
\expandafter\def\csname res@llmjp@gof@mwis@Full@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@mwis@Full@fisher\endcsname{0}
\expandafter\def\csname res@llmjp@gof@native@16@rej\endcsname{3}
\expandafter\def\csname res@llmjp@gof@native@16@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@native@16@fisher\endcsname{0.11}
\expandafter\def\csname res@llmjp@gof@native@256@rej\endcsname{2}
\expandafter\def\csname res@llmjp@gof@native@256@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@native@256@fisher\endcsname{0.056}
\expandafter\def\csname res@llmjp@gof@native@Full@rej\endcsname{2}
\expandafter\def\csname res@llmjp@gof@native@Full@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@native@Full@fisher\endcsname{0.34}
\expandafter\def\csname res@llmjp@gof@syncpool@16@rej\endcsname{1}
\expandafter\def\csname res@llmjp@gof@syncpool@16@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@syncpool@16@fisher\endcsname{0.82}
\expandafter\def\csname res@llmjp@gof@syncpool@256@rej\endcsname{1}
\expandafter\def\csname res@llmjp@gof@syncpool@256@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@syncpool@256@fisher\endcsname{0.55}
\expandafter\def\csname res@llmjp@gof@syncpool@Full@rej\endcsname{3}
\expandafter\def\csname res@llmjp@gof@syncpool@Full@ctx\endcsname{20}
\expandafter\def\csname res@llmjp@gof@syncpool@Full@fisher\endcsname{0.11}
\expandafter\def\csname res@all@gof@ctrl@rejmin\endcsname{13}
\expandafter\def\csname res@all@gof@ctrl@fishermax\endcsname{0}
\expandafter\def\csname res@all@gof@exact@rejmax\endcsname{3}
\expandafter\def\csname res@all@gof@exact@rejtot\endcsname{28}
\expandafter\def\csname res@all@gof@exact@ctxtot\endcsname{540}
\expandafter\def\csname res@all@gof@exact@fishermin\endcsname{0.036}
\expandafter\def\csname res@llama@e2b@native@64@ppl\endcsname{6.77}
\expandafter\def\csname res@llama@e2b@stepwise@64@ppl\endcsname{7.58}
\expandafter\def\csname res@llama@e2b@syncpool@64@ppl\endcsname{7.55}
\expandafter\def\csname res@llama@e2b@syncpool@64@effpct\endcsname{96}
\expandafter\def\csname res@llama@e2b@coin@64@ppl\endcsname{6.81}
\expandafter\def\csname res@llama@e2b@coin@64@effpct\endcsname{99}
\expandafter\def\csname res@llama@e2b@native@1k@ppl\endcsname{11.90}
\expandafter\def\csname res@llama@e2b@stepwise@1k@ppl\endcsname{12.15}
\expandafter\def\csname res@llama@e2b@syncpool@1k@ppl\endcsname{12.91}
\expandafter\def\csname res@llama@e2b@syncpool@1k@effpct\endcsname{96}
\expandafter\def\csname res@llama@e2b@coin@1k@ppl\endcsname{10.59}
\expandafter\def\csname res@llama@e2b@coin@1k@effpct\endcsname{98}
\expandafter\def\csname res@llama@e2b@native@4k@ppl\endcsname{11.57}
\expandafter\def\csname res@llama@e2b@stepwise@4k@ppl\endcsname{10.98}
\expandafter\def\csname res@llama@e2b@syncpool@4k@ppl\endcsname{10.77}
\expandafter\def\csname res@llama@e2b@syncpool@4k@effpct\endcsname{86}
\expandafter\def\csname res@llama@e2b@coin@4k@ppl\endcsname{11.91}
\expandafter\def\csname res@llama@e2b@coin@4k@effpct\endcsname{100}
\expandafter\def\csname res@llama@e2b@native@Full@ppl\endcsname{13.26}
\expandafter\def\csname res@llama@e2b@syncpool@Full@ppl\endcsname{17.04}
\expandafter\def\csname res@llama@e2b@syncpool@Full@effpct\endcsname{92}
\expandafter\def\csname res@llama@e2b@coin@Full@ppl\endcsname{14.99}
\expandafter\def\csname res@llama@e2b@coin@Full@effpct\endcsname{100}
\expandafter\def\csname res@qwen@e2b@native@64@ppl\endcsname{6.52}
\expandafter\def\csname res@qwen@e2b@stepwise@64@ppl\endcsname{6.86}
\expandafter\def\csname res@qwen@e2b@syncpool@64@ppl\endcsname{4.84}
\expandafter\def\csname res@qwen@e2b@syncpool@64@effpct\endcsname{95}
\expandafter\def\csname res@qwen@e2b@coin@64@ppl\endcsname{6.34}
\expandafter\def\csname res@qwen@e2b@coin@64@effpct\endcsname{97}
\expandafter\def\csname res@qwen@e2b@native@1k@ppl\endcsname{9.53}
\expandafter\def\csname res@qwen@e2b@stepwise@1k@ppl\endcsname{13.59}
\expandafter\def\csname res@qwen@e2b@syncpool@1k@ppl\endcsname{14.76}
\expandafter\def\csname res@qwen@e2b@syncpool@1k@effpct\endcsname{102}
\expandafter\def\csname res@qwen@e2b@coin@1k@ppl\endcsname{12.07}
\expandafter\def\csname res@qwen@e2b@coin@1k@effpct\endcsname{101}
\expandafter\def\csname res@qwen@e2b@native@4k@ppl\endcsname{11.79}
\expandafter\def\csname res@qwen@e2b@stepwise@4k@ppl\endcsname{19.09}
\expandafter\def\csname res@qwen@e2b@syncpool@4k@ppl\endcsname{18.31}
\expandafter\def\csname res@qwen@e2b@syncpool@4k@effpct\endcsname{101}
\expandafter\def\csname res@qwen@e2b@coin@4k@ppl\endcsname{14.34}
\expandafter\def\csname res@qwen@e2b@coin@4k@effpct\endcsname{101}
\expandafter\def\csname res@qwen@e2b@native@Full@ppl\endcsname{14.93}
\expandafter\def\csname res@qwen@e2b@syncpool@Full@ppl\endcsname{22.49}
\expandafter\def\csname res@qwen@e2b@syncpool@Full@effpct\endcsname{97}
\expandafter\def\csname res@qwen@e2b@coin@Full@ppl\endcsname{31.02}
\expandafter\def\csname res@qwen@e2b@coin@Full@effpct\endcsname{102}
\expandafter\def\csname res@llmjp@e2b@native@64@ppl\endcsname{5.42}
\expandafter\def\csname res@llmjp@e2b@stepwise@64@ppl\endcsname{4.62}
\expandafter\def\csname res@llmjp@e2b@syncpool@64@ppl\endcsname{5.95}
\expandafter\def\csname res@llmjp@e2b@syncpool@64@effpct\endcsname{100}
\expandafter\def\csname res@llmjp@e2b@coin@64@ppl\endcsname{5.21}
\expandafter\def\csname res@llmjp@e2b@coin@64@effpct\endcsname{98}
\expandafter\def\csname res@llmjp@e2b@native@1k@ppl\endcsname{9.30}
\expandafter\def\csname res@llmjp@e2b@stepwise@1k@ppl\endcsname{12.82}
\expandafter\def\csname res@llmjp@e2b@syncpool@1k@ppl\endcsname{13.47}
\expandafter\def\csname res@llmjp@e2b@syncpool@1k@effpct\endcsname{101}
\expandafter\def\csname res@llmjp@e2b@coin@1k@ppl\endcsname{9.69}
\expandafter\def\csname res@llmjp@e2b@coin@1k@effpct\endcsname{99}
\expandafter\def\csname res@llmjp@e2b@native@4k@ppl\endcsname{13.97}
\expandafter\def\csname res@llmjp@e2b@stepwise@4k@ppl\endcsname{11.93}
\expandafter\def\csname res@llmjp@e2b@syncpool@4k@ppl\endcsname{12.93}
\expandafter\def\csname res@llmjp@e2b@syncpool@4k@effpct\endcsname{93}
\expandafter\def\csname res@llmjp@e2b@coin@4k@ppl\endcsname{17.07}
\expandafter\def\csname res@llmjp@e2b@coin@4k@effpct\endcsname{99}
\expandafter\def\csname res@llmjp@e2b@native@Full@ppl\endcsname{14.31}
\expandafter\def\csname res@llmjp@e2b@syncpool@Full@ppl\endcsname{16.75}
\expandafter\def\csname res@llmjp@e2b@syncpool@Full@effpct\endcsname{97}
\expandafter\def\csname res@llmjp@e2b@coin@Full@ppl\endcsname{17.80}
\expandafter\def\csname res@llmjp@e2b@coin@Full@effpct\endcsname{100}
\expandafter\def\csname res@all@e2b@syncpool@effmin\endcsname{86}
\expandafter\def\csname res@all@e2b@syncpool@effmax\endcsname{102}
\expandafter\def\csname res@all@e2b@coin@effmin\endcsname{97}
\expandafter\def\csname res@all@e2b@coin@effmax\endcsname{102}
\expandafter\def\csname res@llama@tok@any@spaceshare\endcsname{45}
\expandafter\def\csname res@llama@tok@any@partial\endcsname{1,068}
\expandafter\def\csname res@llama@tok@any@levels\endcsname{85}
\expandafter\def\csname res@llama@tok@any@nodes\endcsname{41,302}
\expandafter\def\csname res@llama@tok@any@multi\endcsname{2,105}
\expandafter\def\csname res@llama@tok@any@multipref\endcsname{2,098}
\expandafter\def\csname res@llama@tok@any@space\endcsname{57,874}
\expandafter\def\csname res@llama@tok@any@leadbyte\endcsname{0xE0}
\expandafter\def\csname res@llama@tok@any@leadext\endcsname{1,940}
\expandafter\def\csname res@llama@tok@any@leadshare\endcsname{1.5}
\expandafter\def\csname res@llama@tok@any@merges\endcsname{280,147}
\expandafter\def\csname res@qwen@tok@any@spaceshare\endcsname{35}
\expandafter\def\csname res@qwen@tok@any@partial\endcsname{1,255}
\expandafter\def\csname res@qwen@tok@any@levels\endcsname{85}
\expandafter\def\csname res@qwen@tok@any@nodes\endcsname{45,399}
\expandafter\def\csname res@qwen@tok@any@multi\endcsname{18,246}
\expandafter\def\csname res@qwen@tok@any@multipref\endcsname{18,246}
\expandafter\def\csname res@qwen@tok@any@space\endcsname{53,020}
\expandafter\def\csname res@qwen@tok@any@leadbyte\endcsname{0xE5}
\expandafter\def\csname res@qwen@tok@any@leadext\endcsname{7,012}
\expandafter\def\csname res@qwen@tok@any@leadshare\endcsname{4.6}
\expandafter\def\csname res@qwen@tok@any@merges\endcsname{151,387}
\expandafter\def\csname res@llmjp@tok@any@spaceshare\endcsname{44}
\expandafter\def\csname res@llmjp@tok@any@partial\endcsname{51}
\expandafter\def\csname res@llmjp@tok@any@levels\endcsname{15}
\expandafter\def\csname res@llmjp@tok@any@nodes\endcsname{23,850}
\expandafter\def\csname res@llmjp@tok@any@multi\endcsname{24,701}
\expandafter\def\csname res@llmjp@tok@any@multipref\endcsname{24,700}
\expandafter\def\csname res@llmjp@tok@any@space\endcsname{43,266}
\expandafter\def\csname res@llmjp@tok@any@leadbyte\endcsname{0xE3}
\expandafter\def\csname res@llmjp@tok@any@leadext\endcsname{12,433}
\expandafter\def\csname res@llmjp@tok@any@leadshare\endcsname{12.5}
\expandafter\def\csname res@qwen@swdiag@any@partialmin\endcsname{1.3}
\expandafter\def\csname res@qwen@swdiag@any@partialmax\endcsname{1.8}
\expandafter\def\csname res@qwen@swdiag@any@sharemin\endcsname{77}
\expandafter\def\csname res@qwen@swdiag@any@sharemax\endcsname{89}
\expandafter\def\csname res@qwen@swdiag@any@predmin\endcsname{.017}
\expandafter\def\csname res@qwen@swdiag@any@predmax\endcsname{.021}
\expandafter\def\csname res@qwen@swdiag@any@measmin\endcsname{.021}
\expandafter\def\csname res@qwen@swdiag@any@measmax\endcsname{.029}
\expandafter\def\csname res@qwen@swdiag@any@explmin\endcsname{63}
\expandafter\def\csname res@qwen@swdiag@any@explmax\endcsname{103}
\expandafter\def\csname res@all@swdiag@enja@partialmax\endcsname{0.3}
\expandafter\def\csname res@all@swdiag@enja@predmax\endcsname{.003}
\expandafter\def\csname res@all@swdiag@enja@measmax\endcsname{.004}
\expandafter\def\csname res@llama@amb@all@per1k\endcsname{1.2}
\expandafter\def\csname res@llama@amb@all@tokens\endcsname{230{,}401}
\expandafter\def\csname res@llama@native@all@affected\endcsname{27}
\expandafter\def\csname res@llama@native@all@affectedok\endcsname{4}
\expandafter\def\csname res@llama@native@all@canonwrong\endcsname{0}
\expandafter\def\csname res@llama@rej@128@pct\endcsname{3.8}
\expandafter\def\csname res@llama@rej@128@kl\endcsname{0.04}
\expandafter\def\csname res@qwen@amb@all@per1k\endcsname{4.2}
\expandafter\def\csname res@qwen@amb@all@tokens\endcsname{230{,}424}
\expandafter\def\csname res@qwen@native@all@affected\endcsname{67}
\expandafter\def\csname res@qwen@native@all@affectedok\endcsname{0}
\expandafter\def\csname res@qwen@native@all@canonwrong\endcsname{0}
\expandafter\def\csname res@qwen@rej@128@pct\endcsname{11.2}
\expandafter\def\csname res@qwen@rej@128@kl\endcsname{0.12}
\expandafter\def\csname res@llmjp@amb@all@per1k\endcsname{6.2}
\expandafter\def\csname res@llmjp@amb@all@tokens\endcsname{230{,}411}
\expandafter\def\csname res@llmjp@native@all@affected\endcsname{73}
\expandafter\def\csname res@llmjp@native@all@affectedok\endcsname{1}
\expandafter\def\csname res@llmjp@native@all@canonwrong\endcsname{0}
\expandafter\def\csname res@llmjp@rej@128@pct\endcsname{12.0}
\expandafter\def\csname res@llmjp@rej@128@kl\endcsname{0.13}
\expandafter\def\csname res@all@rej@128@min\endcsname{4}
\expandafter\def\csname res@all@rej@128@max\endcsname{12}
\expandafter\def\csname res@all@rej@128@range\endcsname{4--12}
\expandafter\def\csname res@all@rej@128@klmax\endcsname{0.13}
\expandafter\def\csname res@all@amb@any@max\endcsname{8}
\expandafter\def\csname res@all@amb@any@min\endcsname{1}
\expandafter\def\csname res@all@amb@any@cells\endcsname{18}
\expandafter\def\csname res@all@native@all@affectedok\endcsname{5}
\expandafter\def\csname res@all@native@all@canonwrong\endcsname{0}
\expandafter\def\csname res@all@e0@any@coinmin\endcsname{91}
\expandafter\def\csname res@all@e0@any@coinmax\endcsname{93}
\expandafter\def\csname res@all@e0@any@stopmin\endcsname{7.0}
\expandafter\def\csname res@all@e0@any@stopmax\endcsname{9.0}
\expandafter\def\csname res@all@e0@any@noncanonmax\endcsname{10}
\expandafter\def\csname res@all@e0@any@models\endcsname{3}
\makeatother
\providecommand{\res}[4]{\ifcsname res@#1@#2@#3@#4\endcsname\csname res@#1@#2@#3@#4\endcsname\else\textcolor{red}{??}\GenericWarning{}{LaTeX Warning: res undefined: #1@#2@#3@#4}\fi}


==> gen/numbers_extra.tex <==
% generated by plots/make_extra.py -- do not edit
\makeatletter
\expandafter\def\csname res@all@xlang@any@stopmin\endcsname{4.2}
\expandafter\def\csname res@all@xlang@any@stopmax\endcsname{9.5}
\expandafter\def\csname res@all@xlang@cross@stopmin\endcsname{4.2}
\expandafter\def\csname res@all@xlang@cross@stopmax\endcsname{9.5}
\expandafter\def\csname res@all@xlang@any@cells\endcsname{9}
\expandafter\def\csname res@llama@xlang@en16@root\endcsname{80.5}
\expandafter\def\csname res@llama@xlang@en16@branch\endcsname{11.6}
\expandafter\def\csname res@llama@xlang@en16@stop\endcsname{8.0}
\expandafter\def\csname res@llama@xlang@en64@root\endcsname{54.8}
\expandafter\def\csname res@llama@xlang@en64@branch\endcsname{37.2}
\expandafter\def\csname res@llama@xlang@en64@stop\endcsname{8.0}
\expandafter\def\csname res@llama@xlang@en256@root\endcsname{29.0}
\expandafter\def\csname res@llama@xlang@en256@branch\endcsname{62.7}
\expandafter\def\csname res@llama@xlang@en256@stop\endcsname{8.3}
\expandafter\def\csname res@llama@xlang@en1k@root\endcsname{14.2}
\expandafter\def\csname res@llama@xlang@en1k@branch\endcsname{77.2}
\expandafter\def\csname res@llama@xlang@en1k@stop\endcsname{8.6}
\expandafter\def\csname res@llama@xlang@en4k@root\endcsname{14.7}
\expandafter\def\csname res@llama@xlang@en4k@branch\endcsname{76.6}
\expandafter\def\csname res@llama@xlang@en4k@stop\endcsname{8.7}
\expandafter\def\csname res@llama@xlang@enFull@root\endcsname{14.2}
\expandafter\def\csname res@llama@xlang@enFull@branch\endcsname{77.0}
\expandafter\def\csname res@llama@xlang@enFull@stop\endcsname{8.7}
\expandafter\def\csname res@llama@xlang@zh16@root\endcsname{85.9}
\expandafter\def\csname res@llama@xlang@zh16@branch\endcsname{7.2}
\expandafter\def\csname res@llama@xlang@zh16@stop\endcsname{6.9}
\expandafter\def\csname res@llama@xlang@zh64@root\endcsname{79.0}
\expandafter\def\csname res@llama@xlang@zh64@branch\endcsname{14.7}
\expandafter\def\csname res@llama@xlang@zh64@stop\endcsname{6.3}
\expandafter\def\csname res@llama@xlang@zh256@root\endcsname{66.2}
\expandafter\def\csname res@llama@xlang@zh256@branch\endcsname{26.7}
\expandafter\def\csname res@llama@xlang@zh256@stop\endcsname{7.0}
\expandafter\def\csname res@llama@xlang@zh1k@root\endcsname{64.4}
\expandafter\def\csname res@llama@xlang@zh1k@branch\endcsname{28.7}
\expandafter\def\csname res@llama@xlang@zh1k@stop\endcsname{6.9}
\expandafter\def\csname res@llama@xlang@zh4k@root\endcsname{44.8}
\expandafter\def\csname res@llama@xlang@zh4k@branch\endcsname{47.9}
\expandafter\def\csname res@llama@xlang@zh4k@stop\endcsname{7.3}
\expandafter\def\csname res@llama@xlang@zhFull@root\endcsname{36.6}
\expandafter\def\csname res@llama@xlang@zhFull@branch\endcsname{55.7}
\expandafter\def\csname res@llama@xlang@zhFull@stop\endcsname{7.7}
\expandafter\def\csname res@llama@xlang@ja16@root\endcsname{80.4}
\expandafter\def\csname res@llama@xlang@ja16@branch\endcsname{10.7}
\expandafter\def\csname res@llama@xlang@ja16@stop\endcsname{8.9}
\expandafter\def\csname res@llama@xlang@ja64@root\endcsname{69.3}
\expandafter\def\csname res@llama@xlang@ja64@branch\endcsname{21.5}
\expandafter\def\csname res@llama@xlang@ja64@stop\endcsname{9.2}
\expandafter\def\csname res@llama@xlang@ja256@root\endcsname{59.7}
\expandafter\def\csname res@llama@xlang@ja256@branch\endcsname{32.1}
\expandafter\def\csname res@llama@xlang@ja256@stop\endcsname{8.2}
\expandafter\def\csname res@llama@xlang@ja1k@root\endcsname{49.2}
\expandafter\def\csname res@llama@xlang@ja1k@branch\endcsname{42.2}
\expandafter\def\csname res@llama@xlang@ja1k@stop\endcsname{8.6}
\expandafter\def\csname res@llama@xlang@ja4k@root\endcsname{36.2}
\expandafter\def\csname res@llama@xlang@ja4k@branch\endcsname{54.7}
\expandafter\def\csname res@llama@xlang@ja4k@stop\endcsname{9.0}
\expandafter\def\csname res@llama@xlang@jaFull@root\endcsname{31.6}
\expandafter\def\csname res@llama@xlang@jaFull@branch\endcsname{59.2}
\expandafter\def\csname res@llama@xlang@jaFull@stop\endcsname{9.2}
\expandafter\def\csname res@qwen@xlang@en16@root\endcsname{81.6}
\expandafter\def\csname res@qwen@xlang@en16@branch\endcsname{10.9}
\expandafter\def\csname res@qwen@xlang@en16@stop\endcsname{7.5}
\expandafter\def\csname res@qwen@xlang@en64@root\endcsname{57.2}
\expandafter\def\csname res@qwen@xlang@en64@branch\endcsname{35.0}
\expandafter\def\csname res@qwen@xlang@en64@stop\endcsname{7.7}
\expandafter\def\csname res@qwen@xlang@en256@root\endcsname{32.1}
\expandafter\def\csname res@qwen@xlang@en256@branch\endcsname{59.8}
\expandafter\def\csname res@qwen@xlang@en256@stop\endcsname{8.1}
\expandafter\def\csname res@qwen@xlang@en1k@root\endcsname{20.8}
\expandafter\def\csname res@qwen@xlang@en1k@branch\endcsname{70.8}
\expandafter\def\csname res@qwen@xlang@en1k@stop\endcsname{8.4}
\expandafter\def\csname res@qwen@xlang@en4k@root\endcsname{17.6}
\expandafter\def\csname res@qwen@xlang@en4k@branch\endcsname{73.6}
\expandafter\def\csname res@qwen@xlang@en4k@stop\endcsname{8.8}
\expandafter\def\csname res@qwen@xlang@enFull@root\endcsname{15.4}
\expandafter\def\csname res@qwen@xlang@enFull@branch\endcsname{76.0}
\expandafter\def\csname res@qwen@xlang@enFull@stop\endcsname{8.6}
\expandafter\def\csname res@qwen@xlang@zh16@root\endcsname{87.0}
\expandafter\def\csname res@qwen@xlang@zh16@branch\endcsname{3.9}
\expandafter\def\csname res@qwen@xlang@zh16@stop\endcsname{9.0}
\expandafter\def\csname res@qwen@xlang@zh64@root\endcsname{85.4}
\expandafter\def\csname res@qwen@xlang@zh64@branch\endcsname{6.1}
\expandafter\def\csname res@qwen@xlang@zh64@stop\endcsname{8.5}
\expandafter\def\csname res@qwen@xlang@zh256@root\endcsname{85.1}
\expandafter\def\csname res@qwen@xlang@zh256@branch\endcsname{6.7}
\expandafter\def\csname res@qwen@xlang@zh256@stop\endcsname{8.3}
\expandafter\def\csname res@qwen@xlang@zh1k@root\endcsname{82.8}
\expandafter\def\csname res@qwen@xlang@zh1k@branch\endcsname{9.3}
\expandafter\def\csname res@qwen@xlang@zh1k@stop\endcsname{7.8}
\expandafter\def\csname res@qwen@xlang@zh4k@root\endcsname{79.0}
\expandafter\def\csname res@qwen@xlang@zh4k@branch\endcsname{13.0}
\expandafter\def\csname res@qwen@xlang@zh4k@stop\endcsname{8.0}
\expandafter\def\csname res@qwen@xlang@zhFull@root\endcsname{43.0}
\expandafter\def\csname res@qwen@xlang@zhFull@branch\endcsname{49.1}
\expandafter\def\csname res@qwen@xlang@zhFull@stop\endcsname{7.9}
\expandafter\def\csname res@qwen@xlang@ja16@root\endcsname{85.9}
\expandafter\def\csname res@qwen@xlang@ja16@branch\endcsname{5.4}
\expandafter\def\csname res@qwen@xlang@ja16@stop\endcsname{8.7}
\expandafter\def\csname res@qwen@xlang@ja64@root\endcsname{82.1}
\expandafter\def\csname res@qwen@xlang@ja64@branch\endcsname{9.4}
\expandafter\def\csname res@qwen@xlang@ja64@stop\endcsname{8.5}
\expandafter\def\csname res@qwen@xlang@ja256@root\endcsname{79.0}
\expandafter\def\csname res@qwen@xlang@ja256@branch\endcsname{12.1}
\expandafter\def\csname res@qwen@xlang@ja256@stop\endcsname{8.8}
\expandafter\def\csname res@qwen@xlang@ja1k@root\endcsname{74.3}
\expandafter\def\csname res@qwen@xlang@ja1k@branch\endcsname{17.0}
\expandafter\def\csname res@qwen@xlang@ja1k@stop\endcsname{8.7}
\expandafter\def\csname res@qwen@xlang@ja4k@root\endcsname{61.3}
\expandafter\def\csname res@qwen@xlang@ja4k@branch\endcsname{29.3}
\expandafter\def\csname res@qwen@xlang@ja4k@stop\endcsname{9.4}
\expandafter\def\csname res@qwen@xlang@jaFull@root\endcsname{34.7}
\expandafter\def\csname res@qwen@xlang@jaFull@branch\endcsname{55.8}
\expandafter\def\csname res@qwen@xlang@jaFull@stop\endcsname{9.5}
\expandafter\def\csname res@llmjp@xlang@en16@root\endcsname{90.0}
\expandafter\def\csname res@llmjp@xlang@en16@branch\endcsname{4.2}
\expandafter\def\csname res@llmjp@xlang@en16@stop\endcsname{5.7}
\expandafter\def\csname res@llmjp@xlang@en64@root\endcsname{77.2}
\expandafter\def\csname res@llmjp@xlang@en64@branch\endcsname{16.4}
\expandafter\def\csname res@llmjp@xlang@en64@stop\endcsname{6.5}
\expandafter\def\csname res@llmjp@xlang@en256@root\endcsname{42.8}
\expandafter\def\csname res@llmjp@xlang@en256@branch\endcsname{50.4}
\expandafter\def\csname res@llmjp@xlang@en256@stop\endcsname{6.8}
\expandafter\def\csname res@llmjp@xlang@en1k@root\endcsname{17.5}
\expandafter\def\csname res@llmjp@xlang@en1k@branch\endcsname{75.1}
\expandafter\def\csname res@llmjp@xlang@en1k@stop\endcsname{7.4}
\expandafter\def\csname res@llmjp@xlang@en4k@root\endcsname{17.4}
\expandafter\def\csname res@llmjp@xlang@en4k@branch\endcsname{75.1}
\expandafter\def\csname res@llmjp@xlang@en4k@stop\endcsname{7.5}
\expandafter\def\csname res@llmjp@xlang@enFull@root\endcsname{15.8}
\expandafter\def\csname res@llmjp@xlang@enFull@branch\endcsname{76.5}
\expandafter\def\csname res@llmjp@xlang@enFull@stop\endcsname{7.8}
\expandafter\def\csname res@llmjp@xlang@zh16@root\endcsname{92.2}
\expandafter\def\csname res@llmjp@xlang@zh16@branch\endcsname{2.9}
\expandafter\def\csname res@llmjp@xlang@zh16@stop\endcsname{4.9}
\expandafter\def\csname res@llmjp@xlang@zh64@root\endcsname{86.7}
\expandafter\def\csname res@llmjp@xlang@zh64@branch\endcsname{8.5}
\expandafter\def\csname res@llmjp@xlang@zh64@stop\endcsname{4.9}
\expandafter\def\csname res@llmjp@xlang@zh256@root\endcsname{83.3}
\expandafter\def\csname res@llmjp@xlang@zh256@branch\endcsname{12.5}
\expandafter\def\csname res@llmjp@xlang@zh256@stop\endcsname{4.2}
\expandafter\def\csname res@llmjp@xlang@zh1k@root\endcsname{76.8}
\expandafter\def\csname res@llmjp@xlang@zh1k@branch\endcsname{18.9}
\expandafter\def\csname res@llmjp@xlang@zh1k@stop\endcsname{4.2}
\expandafter\def\csname res@llmjp@xlang@zh4k@root\endcsname{54.0}
\expandafter\def\csname res@llmjp@xlang@zh4k@branch\endcsname{40.8}
\expandafter\def\csname res@llmjp@xlang@zh4k@stop\endcsname{5.2}
\expandafter\def\csname res@llmjp@xlang@zhFull@root\endcsname{39.8}
\expandafter\def\csname res@llmjp@xlang@zhFull@branch\endcsname{54.5}
\expandafter\def\csname res@llmjp@xlang@zhFull@stop\endcsname{5.7}
\expandafter\def\csname res@llmjp@xlang@ja16@root\endcsname{87.7}
\expandafter\def\csname res@llmjp@xlang@ja16@branch\endcsname{5.3}
\expandafter\def\csname res@llmjp@xlang@ja16@stop\endcsname{7.0}
\expandafter\def\csname res@llmjp@xlang@ja64@root\endcsname{81.2}
\expandafter\def\csname res@llmjp@xlang@ja64@branch\endcsname{11.3}
\expandafter\def\csname res@llmjp@xlang@ja64@stop\endcsname{7.5}
\expandafter\def\csname res@llmjp@xlang@ja256@root\endcsname{74.0}
\expandafter\def\csname res@llmjp@xlang@ja256@branch\endcsname{17.9}
\expandafter\def\csname res@llmjp@xlang@ja256@stop\endcsname{8.1}
\expandafter\def\csname res@llmjp@xlang@ja1k@root\endcsname{70.7}
\expandafter\def\csname res@llmjp@xlang@ja1k@branch\endcsname{21.9}
\expandafter\def\csname res@llmjp@xlang@ja1k@stop\endcsname{7.4}
\expandafter\def\csname res@llmjp@xlang@ja4k@root\endcsname{57.7}
\expandafter\def\csname res@llmjp@xlang@ja4k@branch\endcsname{34.5}
\expandafter\def\csname res@llmjp@xlang@ja4k@stop\endcsname{7.8}
\expandafter\def\csname res@llmjp@xlang@jaFull@root\endcsname{36.4}
\expandafter\def\csname res@llmjp@xlang@jaFull@branch\endcsname{55.8}
\expandafter\def\csname res@llmjp@xlang@jaFull@stop\endcsname{7.8}
\expandafter\def\csname res@all@recvall@syncpool@decoded\endcsname{1,800}
\expandafter\def\csname res@all@recvall@syncpool@wrong\endcsname{0}
\expandafter\def\csname res@all@recvall@syncpool@cellmin\endcsname{100}
\expandafter\def\csname res@all@recvall@syncpool@cells\endcsname{18}
\expandafter\def\csname res@all@recvall@coin@decoded\endcsname{1,800}
\expandafter\def\csname res@all@recvall@coin@wrong\endcsname{0}
\expandafter\def\csname res@all@recvall@coin@cellmin\endcsname{100}
\expandafter\def\csname res@all@recvall@coin@cells\endcsname{18}
\makeatother


==> gen/numbers_rts.tex <==
% generated by plots/make_rts.py -- do not edit
\makeatletter
\expandafter\def\csname res@llama@rts@256@util\endcsname{.802}
\expandafter\def\csname res@llama@rts@256@ber\endcsname{0.11}
\expandafter\def\csname res@llama@rts@256@texterr\endcsname{4}
\expandafter\def\csname res@llama@rts@256@resets\endcsname{17.2}
\expandafter\def\csname res@llama@rts@256@reuse\endcsname{17.19}
\expandafter\def\csname res@llama@rts@256@kl\endcsname{.068}
\expandafter\def\csname res@llama@rts@256@klinf\endcsname{4.1}
\expandafter\def\csname res@llama@rts@256@corr\endcsname{0.66}
\expandafter\def\csname res@llama@rts@256@extratok\endcsname{1.2}
\expandafter\def\csname res@llama@rts@256@nativefail\endcsname{2}
\expandafter\def\csname res@llama@rts@256@coinratio\endcsname{0.91}
\expandafter\def\csname res@llama@rts@256@rtsnative\endcsname{99}
\expandafter\def\csname res@llama@rts@Full@util\endcsname{.884}
\expandafter\def\csname res@llama@rts@Full@ber\endcsname{0.10}
\expandafter\def\csname res@llama@rts@Full@texterr\endcsname{6}
\expandafter\def\csname res@llama@rts@Full@resets\endcsname{4.4}
\expandafter\def\csname res@llama@rts@Full@reuse\endcsname{3.91}
\expandafter\def\csname res@llama@rts@Full@kl\endcsname{.046}
\expandafter\def\csname res@llama@rts@Full@klinf\endcsname{0.0}
\expandafter\def\csname res@llama@rts@Full@corr\endcsname{0.53}
\expandafter\def\csname res@llama@rts@Full@extratok\endcsname{1.2}
\expandafter\def\csname res@llama@rts@Full@nativefail\endcsname{8}
\expandafter\def\csname res@llama@rts@Full@coinratio\endcsname{0.91}
\expandafter\def\csname res@llama@rts@Full@rtsnative\endcsname{99}
\expandafter\def\csname res@qwen@rts@256@util\endcsname{.788}
\expandafter\def\csname res@qwen@rts@256@ber\endcsname{0.22}
\expandafter\def\csname res@qwen@rts@256@texterr\endcsname{16}
\expandafter\def\csname res@qwen@rts@256@resets\endcsname{5.5}
\expandafter\def\csname res@qwen@rts@256@reuse\endcsname{5.00}
\expandafter\def\csname res@qwen@rts@256@kl\endcsname{.076}
\expandafter\def\csname res@qwen@rts@256@klinf\endcsname{11.5}
\expandafter\def\csname res@qwen@rts@256@corr\endcsname{1.37}
\expandafter\def\csname res@qwen@rts@256@extratok\endcsname{1.9}
\expandafter\def\csname res@qwen@rts@256@nativefail\endcsname{10}
\expandafter\def\csname res@qwen@rts@256@coinratio\endcsname{0.92}
\expandafter\def\csname res@qwen@rts@256@rtsnative\endcsname{100}
\expandafter\def\csname res@qwen@rts@Full@util\endcsname{.921}
\expandafter\def\csname res@qwen@rts@Full@ber\endcsname{0.14}
\expandafter\def\csname res@qwen@rts@Full@texterr\endcsname{14}
\expandafter\def\csname res@qwen@rts@Full@resets\endcsname{2.7}
\expandafter\def\csname res@qwen@rts@Full@reuse\endcsname{2.34}
\expandafter\def\csname res@qwen@rts@Full@kl\endcsname{.027}
\expandafter\def\csname res@qwen@rts@Full@klinf\endcsname{0.0}
\expandafter\def\csname res@qwen@rts@Full@corr\endcsname{0.85}
\expandafter\def\csname res@qwen@rts@Full@extratok\endcsname{1.5}
\expandafter\def\csname res@qwen@rts@Full@nativefail\endcsname{6}
\expandafter\def\csname res@qwen@rts@Full@coinratio\endcsname{0.91}
\expandafter\def\csname res@qwen@rts@Full@rtsnative\endcsname{100}
\expandafter\def\csname res@llmjp@rts@256@util\endcsname{.757}
\expandafter\def\csname res@llmjp@rts@256@ber\endcsname{0.04}
\expandafter\def\csname res@llmjp@rts@256@texterr\endcsname{6}
\expandafter\def\csname res@llmjp@rts@256@resets\endcsname{1.4}
\expandafter\def\csname res@llmjp@rts@256@reuse\endcsname{1.41}
\expandafter\def\csname res@llmjp@rts@256@kl\endcsname{.0053}
\expandafter\def\csname res@llmjp@rts@256@klinf\endcsname{9.2}
\expandafter\def\csname res@llmjp@rts@256@corr\endcsname{0.52}
\expandafter\def\csname res@llmjp@rts@256@extratok\endcsname{0.7}
\expandafter\def\csname res@llmjp@rts@256@nativefail\endcsname{10}
\expandafter\def\csname res@llmjp@rts@256@coinratio\endcsname{0.92}
\expandafter\def\csname res@llmjp@rts@256@rtsnative\endcsname{99}
\expandafter\def\csname res@llmjp@rts@Full@util\endcsname{.921}
\expandafter\def\csname res@llmjp@rts@Full@ber\endcsname{0.14}
\expandafter\def\csname res@llmjp@rts@Full@texterr\endcsname{16}
\expandafter\def\csname res@llmjp@rts@Full@resets\endcsname{1.9}
\expandafter\def\csname res@llmjp@rts@Full@reuse\endcsname{1.09}
\expandafter\def\csname res@llmjp@rts@Full@kl\endcsname{.0025}
\expandafter\def\csname res@llmjp@rts@Full@klinf\endcsname{0.0}
\expandafter\def\csname res@llmjp@rts@Full@corr\endcsname{0.84}
\expandafter\def\csname res@llmjp@rts@Full@extratok\endcsname{1.7}
\expandafter\def\csname res@llmjp@rts@Full@nativefail\endcsname{18}
\expandafter\def\csname res@llmjp@rts@Full@coinratio\endcsname{0.90}
\expandafter\def\csname res@llmjp@rts@Full@rtsnative\endcsname{100}
\expandafter\def\csname res@all@rts@any@bermin\endcsname{0.04}
\expandafter\def\csname res@all@rts@any@bermax\endcsname{0.22}
\expandafter\def\csname res@all@rts@any@texterrmin\endcsname{4}
\expandafter\def\csname res@all@rts@any@texterrmax\endcsname{16}
\expandafter\def\csname res@all@rts@any@resetsmin\endcsname{1.4}
\expandafter\def\csname res@all@rts@any@resetsmax\endcsname{17.2}
\expandafter\def\csname res@all@rts@any@reusemin\endcsname{1.09}
\expandafter\def\csname res@all@rts@any@reusemax\endcsname{17.19}
\expandafter\def\csname res@all@rts@any@klmin\endcsname{.0025}
\expandafter\def\csname res@all@rts@any@klmax\endcsname{.076}
\expandafter\def\csname res@all@rts@any@klinfsharemin\endcsname{0.0}
\expandafter\def\csname res@all@rts@any@klinfsharemax\endcsname{11.5}
\expandafter\def\csname res@all@rts@any@corrratiomin\endcsname{0.52}
\expandafter\def\csname res@all@rts@any@corrratiomax\endcsname{1.37}
\expandafter\def\csname res@all@rts@any@extratokmin\endcsname{0.7}
\expandafter\def\csname res@all@rts@any@extratokmax\endcsname{1.9}
\expandafter\def\csname res@all@rts@any@nativefailmin\endcsname{2}
\expandafter\def\csname res@all@rts@any@nativefailmax\endcsname{18}
\expandafter\def\csname res@all@rts@any@e2evscoinmin\endcsname{0.91}
\expandafter\def\csname res@all@rts@any@e2evscoinmax\endcsname{0.93}
\expandafter\def\csname res@all@rts@any@rtsnativemin\endcsname{99}
\expandafter\def\csname res@all@rts@any@rtsnativemax\endcsname{100}
\expandafter\def\csname res@all@rts@any@rtscoinmin\endcsname{1.09}
\expandafter\def\csname res@all@rts@any@rtscoinmax\endcsname{1.11}
\expandafter\def\csname res@all@rts@any@rtscoine2emin\endcsname{1.07}
\expandafter\def\csname res@all@rts@any@rtscoine2emax\endcsname{1.09}
\expandafter\def\csname res@all@rts@any@nativenmin\endcsname{50}
\expandafter\def\csname res@all@rts@any@nativenmax\endcsname{50}
\expandafter\def\csname res@all@rts@any@callsmin\endcsname{1.003}
\expandafter\def\csname res@all@rts@any@callsmax\endcsname{1.034}
\expandafter\def\csname res@all@rts@any@ratiocoinmin\endcsname{0.90}
\expandafter\def\csname res@all@rts@any@ratiocoinmax\endcsname{0.92}
\expandafter\def\csname res@all@rts@256@bermin\endcsname{0.04}
\expandafter\def\csname res@all@rts@256@bermax\endcsname{0.22}
\expandafter\def\csname res@all@rts@256@texterrmin\endcsname{4}
\expandafter\def\csname res@all@rts@256@texterrmax\endcsname{16}
\expandafter\def\csname res@all@rts@256@resetsmin\endcsname{1.4}
\expandafter\def\csname res@all@rts@256@resetsmax\endcsname{17.2}
\expandafter\def\csname res@all@rts@256@reusemin\endcsname{1.41}
\expandafter\def\csname res@all@rts@256@reusemax\endcsname{17.19}
\expandafter\def\csname res@all@rts@256@klmin\endcsname{.0053}
\expandafter\def\csname res@all@rts@256@klmax\endcsname{.076}
\expandafter\def\csname res@all@rts@256@klinfsharemin\endcsname{4.1}
\expandafter\def\csname res@all@rts@256@klinfsharemax\endcsname{11.5}
\expandafter\def\csname res@all@rts@256@corrratiomin\endcsname{0.52}
\expandafter\def\csname res@all@rts@256@corrratiomax\endcsname{1.37}
\expandafter\def\csname res@all@rts@256@extratokmin\endcsname{0.7}
\expandafter\def\csname res@all@rts@256@extratokmax\endcsname{1.9}
\expandafter\def\csname res@all@rts@256@nativefailmin\endcsname{2}
\expandafter\def\csname res@all@rts@256@nativefailmax\endcsname{10}
\expandafter\def\csname res@all@rts@256@e2evscoinmin\endcsname{0.92}
\expandafter\def\csname res@all@rts@256@e2evscoinmax\endcsname{0.93}
\expandafter\def\csname res@all@rts@256@rtsnativemin\endcsname{99}
\expandafter\def\csname res@all@rts@256@rtsnativemax\endcsname{100}
\expandafter\def\csname res@all@rts@256@rtscoinmin\endcsname{1.09}
\expandafter\def\csname res@all@rts@256@rtscoinmax\endcsname{1.10}
\expandafter\def\csname res@all@rts@256@rtscoine2emin\endcsname{1.07}
\expandafter\def\csname res@all@rts@256@rtscoine2emax\endcsname{1.08}
\expandafter\def\csname res@all@rts@256@nativenmin\endcsname{50}
\expandafter\def\csname res@all@rts@256@nativenmax\endcsname{50}
\expandafter\def\csname res@all@rts@256@callsmin\endcsname{1.003}
\expandafter\def\csname res@all@rts@256@callsmax\endcsname{1.034}
\expandafter\def\csname res@all@rts@256@ratiocoinmin\endcsname{0.91}
\expandafter\def\csname res@all@rts@256@ratiocoinmax\endcsname{0.92}
\expandafter\def\csname res@all@rts@Full@bermin\endcsname{0.10}
\expandafter\def\csname res@all@rts@Full@bermax\endcsname{0.14}
\expandafter\def\csname res@all@rts@Full@texterrmin\endcsname{6}
\expandafter\def\csname res@all@rts@Full@texterrmax\endcsname{16}
\expandafter\def\csname res@all@rts@Full@resetsmin\endcsname{1.9}
\expandafter\def\csname res@all@rts@Full@resetsmax\endcsname{4.4}
\expandafter\def\csname res@all@rts@Full@reusemin\endcsname{1.09}
\expandafter\def\csname res@all@rts@Full@reusemax\endcsname{3.91}
\expandafter\def\csname res@all@rts@Full@klmin\endcsname{.0025}
\expandafter\def\csname res@all@rts@Full@klmax\endcsname{.046}
\expandafter\def\csname res@all@rts@Full@klinfsharemin\endcsname{0.0}
\expandafter\def\csname res@all@rts@Full@klinfsharemax\endcsname{0.0}
\expandafter\def\csname res@all@rts@Full@corrratiomin\endcsname{0.53}
\expandafter\def\csname res@all@rts@Full@corrratiomax\endcsname{0.85}
\expandafter\def\csname res@all@rts@Full@extratokmin\endcsname{1.2}
\expandafter\def\csname res@all@rts@Full@extratokmax\endcsname{1.7}
\expandafter\def\csname res@all@rts@Full@nativefailmin\endcsname{6}
\expandafter\def\csname res@all@rts@Full@nativefailmax\endcsname{18}
\expandafter\def\csname res@all@rts@Full@e2evscoinmin\endcsname{0.91}
\expandafter\def\csname res@all@rts@Full@e2evscoinmax\endcsname{0.93}
\expandafter\def\csname res@all@rts@Full@rtsnativemin\endcsname{99}
\expandafter\def\csname res@all@rts@Full@rtsnativemax\endcsname{100}
\expandafter\def\csname res@all@rts@Full@rtscoinmin\endcsname{1.09}
\expandafter\def\csname res@all@rts@Full@rtscoinmax\endcsname{1.11}
\expandafter\def\csname res@all@rts@Full@rtscoine2emin\endcsname{1.08}
\expandafter\def\csname res@all@rts@Full@rtscoine2emax\endcsname{1.09}
\expandafter\def\csname res@all@rts@Full@nativenmin\endcsname{50}
\expandafter\def\csname res@all@rts@Full@nativenmax\endcsname{50}
\expandafter\def\csname res@all@rts@Full@callsmin\endcsname{1.003}
\expandafter\def\csname res@all@rts@Full@callsmax\endcsname{1.008}
\expandafter\def\csname res@all@rts@Full@ratiocoinmin\endcsname{0.90}
\expandafter\def\csname res@all@rts@Full@ratiocoinmax\endcsname{0.91}
\expandafter\def\csname res@all@rts@any@n\endcsname{50}
\makeatother

